Espresso: Robust Concept Filtering in Text-to-Image Models

Diffusion based text-to-image models are trained on large datasets scraped from the Internet, potentially containing unacceptable concepts (e.g., copyright-infringing or unsafe). We need concept removal techniques (CRTs) which are i) effective in preventing the generation of images with unacceptable concepts, ii) utility-preserving on acceptable concepts, and, iii) robust against evasion with adversarial prompts. No prior CRT satisfies all these requirements simultaneously. We introduce Espresso, the first robust concept filter based on Contrastive Language-Image Pre-Training (CLIP). We identify unacceptable concepts by using the distance between the embedding of a generated image to the text embeddings of both unacceptable and acceptable concepts. This lets us fine-tune for robustness by separating the text embeddings of unacceptable and acceptable concepts while preserving utility. We present a pipeline to evaluate various CRTs to show that Espresso is more effective and robust than prior CRTs, while retaining utility.

==> figures/fig_architecture.tex <==
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\tikzstyle{defense} = [rectangle,  minimum width=1.4cm, minimum height=0.5cm, text centered, draw=black, fill=mynicered!30]
\tikzstyle{risk} = [rectangle,  minimum width=1.4cm, minimum height=0.5cm, text centered, draw=black]
\tikzstyle{entity} = [rectangle, minimum width=1.4cm, minimum height=0.5cm, text centered, draw=black]
\tikzstyle{databl} = [rectangle,  minimum width=1cm, minimum height=0.5cm, text centered, draw=black, fill=green!30]


\begin{figure*}[!htb]
\centering
\begin{tikzpicture}


\node (clip) [risk, align=center] {\footnotesize \textbf{CLIP Encoder}\\ (\textbf{\te})};
\node (diffmod) [risk, right of=clip, xshift=1.5cm, align=center] {\footnotesize \textbf{Diffusion Model}\\ (\textbf{\dm})};

\draw[->, ultra thick] (clip.east) -- (diffmod.west);

\begin{scope}[on background layer]
    \node (model) [fit=(clip) (diffmod), rounded corners, draw=black, dashed, inner sep=.2cm, label={above:\textbf{Text-to-Image (\tti) model ($\target$)}}] {};
\end{scope}

\node [left of = clip,align=center, rectangle, rounded corners, draw=black, xshift=-1.5cm, yshift=0.5cm] (prompt) {\footnotesize \textbf{Textual}\\\footnotesize \textbf{Prompts} \textbf{\prompt}};
\draw[->, ultra thick] (prompt.east) -- (model.west);

\node [right of = diffmod,align=center, rectangle, rounded corners, draw=black, xshift=1.5cm] (imageclean) {\footnotesize \textbf{Image \imgclean}\\ \footnotesize (\imgacc or \imgunacc)};

\node (filter) [entity, align=center, right of=model, xshift=4.75cm] {\footnotesize \textbf{Filter \filter}};
\draw[->, ultra thick] (imageclean.east) -- (filter.west);
\draw[->, ultra thick] (model.east) -- (imageclean.west);

\node [right of = filter,align=center, yshift=-0.75cm, xshift=1.5cm, minimum width=1cm] (safe) {\footnotesize \textbf{Acceptable}};
\node [right of = filter,align=center, yshift=0.75cm, xshift=1.5cm] (notsafe) {\footnotesize \textbf{Unacceptable}};
\draw[->, ultra thick] (filter.east) -- ([xshift=-0.7cm]notsafe.south);
\draw[->, ultra thick] (filter.east) -- ([xshift=-0.7cm]safe.north);


\node [below of = prompt,align=center, rectangle, rounded corners, draw=black, fill=mynicered!30] (advprompt) {\footnotesize \textbf{Adversarial}\\\footnotesize \textbf{Prompts} \textbf{$\advprompt$}};
\node (inv) [defense, left of =advprompt, align=center, xshift=-1cm] {\footnotesize \textbf{\adv}};
% \node (hand) [defense, below of=diffmod, align=center, yshift=-0.5cm, xshift=-0.2cm] {\footnotesize \textbf{Handcrafted}\\ \footnotesize\textbf{Attack}};
% \begin{scope}[on background layer]
%     \node (attacks) [fit=(inv) (hand), fill= red!15, rounded corners, draw=black, dashed, inner sep=.2cm, label={below:\textbf{Circumvention Techniques}}] {};
% \end{scope}
\draw[->, ultra thick, mynicered, solid] (inv.east) -- (advprompt.west);

% \node [below of = imageclean,align=center, draw=black, fill=red!30] (imgadv) {\footnotesize \textbf{Adv. Image}\\ \footnotesize \textbf{\imgunacc'}};
\draw[->, ultra thick, mynicered] (advprompt.east) -- ([yshift=-0.1cm]model.west);
% \draw[->, ultra thick, mynicered] (model.east) -- (imgadv.west);
% \draw[->, ultra thick, mynicered] (imgadv.east) -- node [below, align=center, xshift=0.5cm] {} ([yshift=-0.1cm]filter.west);

\draw[->, ultra thick, mynicered] (filter.south) |- ++(0, -1cm) -| (inv.south) node[midway,above, xshift=6cm] {\footnotesize Filter's Loss for Attack};

\end{tikzpicture}
% }
\caption{\underline{Overview of Filtering based \crt{s}:} $\target$ generates \imgclean from \prompt which is passed to Filter which classifies \imgclean as acceptable (if \imgacc) or not (if \imgacc). \adv generate an adversarial prompt $\advprompt$ to force Filter to misclassify generated image \imgunacc' as acceptable. Rectangles with rounded corners indicate data component, while sharp corners indicate software component (also includes \adv). \textcolor{mynicered}{Red} indicates information flow and components for the attacks.}
\label{fig:overview}
\end{figure*}

==> figures/fig_images.tex <==
\begin{figure}[!htb]
    \centering
    \begin{minipage}[b]{1\linewidth}
    \centering
    \subfigure[False Positive (Group-1)]{
    \includegraphics[width=0.40\linewidth]{figures/adversarial_images/nudity_yes.png}
    }%
    \hspace{0.75cm}
    \subfigure[True Positive (Group-1)]{\includegraphics[width=0.40\linewidth]{figures/adversarial_images/nudity_no.png}}
    \end{minipage}\\
    \begin{minipage}[b]{1\linewidth}
    \centering
    \subfigure[False Positive (Group-2)]{
    \includegraphics[width=0.40\linewidth]{figures/adversarial_images/grumpy_yes.png}
    }%
    \hspace{0.75cm}
    \subfigure[True Positive (Group-2)]{\includegraphics[width=0.40\linewidth]{figures/adversarial_images/grumpy_no.png}}
    \end{minipage}\\
    \begin{minipage}[b]{1\linewidth}
    \centering
    \subfigure[False Positive (Group-3)]{
    \includegraphics[width=0.40\linewidth]{figures/adversarial_images/swift_yes.png}
    }%
    \hspace{0.75cm}
    \subfigure[True Positive (Group-3)]{\includegraphics[width=0.40\linewidth]{figures/adversarial_images/swift_no.png}}
    \end{minipage}
    \caption{Examples of $\imgadv$ where images on the left include $\cunacc$ but can be successfully detected by \method while $\imgadv$ on the right can evade \method but does not include $\cunacc$.}
    \label{fig:images}
\end{figure}


==> figures/fig_robustness_diagram.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1.5\columnwidth]{figures/espresso_robustness_diagram_cropped.pdf}
    \caption{The perturbation required to evade \method (right) is greater than that required for the SD filter (left) due to the use of both unacceptable and acceptable concepts for the threshold. Generated images lose their unacceptable quality at large perturbations.}
    \label{fig:espresso_robustness_diagram}
\end{figure}

==> generative-concept-removal/00acks.tex <==
\section*{Acknowledgments}
This work is supported in part by the Government of Ontario. 
Vasisht is supported by IBM PhD Fellowship, David R. Cheriton Scholarship, and Cybersecurity and Privacy Excellence Graduate Scholarship. Views expressed in the paper are those of the authors and do not necessarily reflect the position of the funding agencies.

==> generative-concept-removal/00macros.tex <==
\usepackage{tikz}
\usetikzlibrary{shapes,arrows}
\usetikzlibrary{backgrounds, positioning, fit}
\usepackage{dblfloatfix}
\usepackage[inline]{enumitem}
\usepackage{graphics}
\usepackage[T1]{fontenc}
\usepackage{soul}
% \usepackage[labelfont=normalfont,textfont=normalfont]{caption}
\usepackage{xspace}
\usepackage{multirow}
\usepackage[table]{colortbl}
\usepackage{versions}
% \usepackage{wasysym}
\usepackage{pifont}
% \usepackage{subfigure}
\usepackage{subcaption}
\usepackage[normalem]{ulem}

\usepackage{amsmath,amsthm}
\usepackage{booktabs}
% \usepackage{cite}
\newtheorem{theorem}{Theorem}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand{\dm}{$\epsilon_\theta$\xspace}
\newcommand{\adv}{\protect{$\mathcal{A}dv$}\xspace}
\newcommand{\tti}{T2I\xspace}
\newcommand{\crt}{CRT\xspace}
\newcommand{\te}{$\phi$\xspace}
\newcommand{\prompt}{\texttt{p}\xspace}
\newcommand{\promptacc}{\texttt{p}^{a}\xspace}
\newcommand{\promptuacc}{\texttt{p}^{u}\xspace}
\newcommand{\advprompt}{\texttt{p}^{adv}\xspace}
\newcommand{\filter}{\texttt{F}\xspace}
\newcommand{\target}{\emph{f}\xspace}
\newcommand{\surrogate}{\bar{f}\xspace}


\newcommand{\imgclean}{\texttt{$x$}\xspace}
\newcommand{\imgadv}{\texttt{$x$}^{adv}\xspace}
\newcommand{\concept}{c\xspace}
\newcommand{\cacc}{c^{a}\xspace}
\newcommand{\caccc}{\hat{c}^{a}\xspace}
\newcommand{\cunacc}{c^{u}\xspace}
\newcommand{\cunaccc}{\hat{c}^{u}\xspace}
\newcommand{\imgunacc}{\texttt{$x^{u}$}\xspace}
\newcommand{\imgacc}{\texttt{$x^{a}$}\xspace}
\newcommand{\dtrain}{\mathcal{D}_{tr}\xspace}
\newcommand{\dtestadv}{\mathcal{D}_{adv}^{u}\xspace}
\newcommand{\dtestacc}{\mathcal{D}_{te}^{a}\xspace}
\newcommand{\dtestunacc}{\mathcal{D}_{te}^{u}\xspace}
\newcommand{\dvalacc}
{\mathcal{D}_{val}^{a}\xspace}
\newcommand{\dvalunacc}
{\mathcal{D}_{val}^{u}\xspace}

\newcommand{\method}{\textsc{Espresso}\xspace}
\newcommand{\methodFT}{\textsc{Sieve-FT}\xspace}
\newcommand{\esd}{\texttt{ESD}\xspace}
\newcommand{\sdd}{\texttt{SDD}\xspace}
\newcommand{\unifiedCE}{\texttt{UCE}\xspace}
\newcommand{\unsafediff}{\texttt{UD}\xspace}
\newcommand{\sa}{\texttt{SA}\xspace}
\newcommand{\forgetNot}{\texttt{FMN}\xspace}
\newcommand{\sld}{\texttt{SLD}\xspace}
\newcommand{\ca}{\texttt{CA}\xspace}
\newcommand{\moderator}{\texttt{Mod}\xspace}


\newcommand{\cce}{\texttt{CCE}\xspace}
\newcommand{\pez}{\texttt{PEZ}\xspace}
\newcommand{\ringbell}{\texttt{RingBell}\xspace}
\newcommand{\typo}{\texttt{Typo}\xspace}
\newcommand{\sneaky}{\texttt{SneakyPrompt}\xspace}

\newcommand\todo[1]{{\color{red}\textbf{TODO: #1}\xspace}}
\newcommand\topics[1]{{\color{blue}\textbf{#1\\}\xspace}}
\newcommand\change[1]{{\color{purple}{#1}\xspace}}
\newcommand{\smark}{$\LEFTcircle$\xspace}
\newcommand{\xmark}{$\Circle$\xspace}
\newcommand{\cmark}{$\CIRCLE$\xspace}

\usepackage{xcolor}
\definecolor{mynicegreen}{RGB}{171,195,47}
\definecolor{mynicered}{RGB}{255,154,154}
\definecolor{myniceblue}{RGB}{153,153,255}

%% Set up section label for \autoref
\def\Snospace~{\S{}}
% \renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{\Snospace}
\def\subsectionautorefname{\Snospace}
\def\subsubsectionautorefname{\Snospace}
\def\chapterautorefname{\Snospace}


==> generative-concept-removal/01abstract.tex <==
Diffusion based text-to-image models are trained on large datasets scraped from the Internet, potentially containing \textit{unacceptable concepts} (e.g., copyright-infringing or unsafe). 
We need concept removal techniques (\crt{s}) which are
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \textit{effective} in preventing the generation of images with unacceptable concepts
\item \textit{utility-preserving} on acceptable concepts, and 
\item \textit{robust} against evasion with adversarial prompts.
\end{enumerate*}
No prior \crt satisfies all these requirements simultaneously. 
We introduce \method, the first \emph{\textbf{robust \underline{co}ncept \underline{fi}lter}} based on Contrastive Language-Image Pre-Training (CLIP). 
We identify unacceptable concepts by using the distance between the embedding of a generated image to the text embeddings of \emph{both} unacceptable and acceptable concepts.
This lets us fine-tune for robustness by separating the text embeddings of unacceptable and acceptable concepts while preserving utility.
We present a pipeline to evaluate various \crt{s} to show that \method is \textbf{more effective and robust} than prior \crt{s}, while \textbf{retaining utility}.
\begin{arxiv}\footnote{ACM Conference on Data and Application Security and Privacy (CODASPY), 2025.}\end{arxiv}
\begin{submission}

\end{submission}
% Code will be publicly available upon publication.
%(CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) 

%(CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) 

%(normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]). 
% Finally, we present theoretical bounds for certified robustness of \method against adversarial prompts, and an empirical analysis.


==> generative-concept-removal/1introduction.tex <==
\section{Introduction}\label{sec:introduction}


Diffusion-based text-to-image (\tti) models have demonstrated a remarkable ability to generate high quality images from textual prompts~\cite{stable-diffusion,Rombach_2022_CVPR,ramesh2021dalle}.
They are trained on large datasets of unfiltered content from the Internet~\cite{radford2021learning,schuhmann2022laion}. 
Due to their large capacity, \tti models memorize specific \emph{concepts}, as seen in the generated images~\cite{Korn_2023,somepalli2022diffusion,carlini2023extracting}. 
Some of these concepts, may be \emph{unacceptable} for various reasons, such as copyright infringement (e.g., a movie character or celebrity), or inappropriateness (e.g., ``nudity'' or ``violence'')~\cite{gandikota2023erasing,schramowski2022safe,heng2023selective}. 
% Retraining \tti models after filtering out unacceptable concepts is inefficient, only partially effective~\cite{li2024safegen, huggingfaceStabilityaistablediffusion21Hugging}, and compromises utility~\cite{gandikota2023erasing}.
We need \emph{concept removal techniques} (\crt{s}) to minimize unacceptable concepts in  generated images.


Ideally, \crt{s} should be \emph{effective} in reducing generation of unacceptable concepts while preserving \emph{utility} on all others, and \emph{robust} to evasion with adversarial prompts.  
No existing \crt \emph{simultaneously} satisfies these requirements (\autoref{sec:evaluation}):
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \emph{fine-tuning \crt{s}} which modify \tti models, trade-off effectiveness for utility~\cite{gandikota2023erasing,kumari2023ablating,heng2023selective,schramowski2022safe}, and  lack robustness~\cite{Tsai2023RingABellHR, wen2023hard, pham2023circumventing, yang2023sneakyprompt}
\item \emph{filtering \crt{s}}, which detect unacceptable concepts, lack robustness~(\cite{rando2022redteaming} and \autoref{sec:filterEval}).
\end{enumerate*}
%Moreover, none of these \crt{s} are robust against adversarial prompts, i.e., adversarially modified prompts which force \tti{s} to generate unacceptable concepts.
Our goal is to design a \crt that can simultaneously meet all the requirements.

We opt to use a filter as it will not alter the \tti model, thus minimizing impact on utility. We construct our filter using a Contrastive Language-Image Pre-Training (CLIP) model~\cite{radford2021learning}, an essential component of \tti models. 
% CLIP co-locates the embeddings of textual prompts and their corresponding images within a unified embedding space where similar concepts are closer.
CLIP is pre-trained on a vast dataset encompassing a broad spectrum of concepts~\cite{radford2021learning}, making it a versatile choice for a filter, unlike specialized classifiers (e.g.,~\cite{unsafeDiff}).
However, a naive CLIP-based filter is susceptible to evasion~\cite{rando2022redteaming}. 
%by solely measuring the distance between the embeddings of a generated image, and an unacceptable concept,
\begin{arxiv}
Subsequently, prior works have identified the design of a robust filtering-based \crt as an open problem~\cite{rando2022redteaming,li2024safegen}.
\end{arxiv}

% \input{figures/fig_robustness_diagram}
% \change{Robustness diagram: figures/fig\_robustness\_diagram}

We present a \textbf{robust \underline{co}ntent \underline{fi}lter}, \method, by configuring CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts. 
% We present a \textbf{robust} \textbf{co}ntent \textbf{fi}lter, \method, that identifies unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both acceptable and unacceptable concepts}. 
% \change{This simple change in configuration translates to projecting} the image embedding onto the vector connecting the text embeddings of acceptable and unacceptable concepts. 
% This simple change makes it harder to generate effective adversarial prompts: the adversary is restricted to adding noise in the direction of the acceptable concept. 
%adversarial prompts must generate images far enough from unacceptable concepts to evade detection yet close enough to retain the unacceptable concepts.
This allows fine-tuning to improve robustness by increasing the separation between the text embeddings of unacceptable and acceptable concepts, while preserving utility by maintaining the closeness between embeddings of prompts and their images. %by maintaining their pairing with their corresponding image embeddings.
% We liken this to adversarial training in classifiers, thus, improving the robustness of \method.
% This fine-tuning approach is further supported by fine-tuning \crt{s} which show that such an optimization leads to better utility~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}.
Our contributions are presenting 
\begin{enumerate}[leftmargin=*]
\item \method\footnote{Code: \url{https://github.com/ssg-research/concept-filtering}.}
\begin{submission}
\footnote{Full paper: \url{https://arxiv.org/abs/2404.19227}}
\end{submission}, the \textbf{first robust \underline{co}ntent \underline{fi}lter} (\autoref{sec:approach}), which identifies unacceptable concepts in generated images by measuring the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts
\item a \textbf{complete pipeline} for comparative evaluation of \crt{s} and attacks, %which includes generating datasets and various metrics, %state-of-the-art \crt{s} and attacks
(\autoref{sec:setup}), and
\item a comprehensive evaluation of \method against seven fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective and robust} while \textbf{retaining utility} (\autoref{sec:evaluation}).
\end{enumerate}
In \autoref{sec:discussions} and \begin{arxiv}Appendix~\ref{sec:bound}\end{arxiv}\begin{submission}Appendix in our paper's full version~\cite{das2024espresso}\end{submission}, we present the first approach for certifiable robustness of \crt{s}, exploring theoretical robustness bounds of \method against a hypothetically strong adversary.
We analyze these bounds to show that \method is more robust in practice.
% \begin{enumerate}[leftmargin=*,wide,  labelindent=0pt]
% \item \method\footnote{We will open-source the code upon publication.}, the \textbf{first robust} (CLIP-based) \underline{co}ntent \underline{fi}lter (Section~\ref{sec:approach}) 
%which identifies unacceptable concepts in generated images by measuring the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts ,
% \item a comprehensive comparative evaluation of \method with six state-of-the-art fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective} and \textbf{more robust} while \textbf{retaining utility}. (Section~\ref{sec:setup})
% (CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) and \textbf{more robust} (CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) than prior \crt{s}, while \textbf{retaining utility} (normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]).
%showing that \method is \textbf{effective} ($\sim$5\% CLIP accuracy  on unacceptable concepts), \textbf{utility-preserving} ($\sim$93\% 
% normalized CLIP score on acceptable concepts), and \textbf{robust} ($\sim$4\% CLIP accuracy of  on adversarial prompts) %of unacceptable concepts) 
% (Section~\ref{sec:evaluation}), and
% \item %the \textbf{first} approach towards \textbf{certifiable robustness of \crt{s}} by exploring 
% theoretical bounds for \textbf{certifying the robustness} of \method, assuming a hypothetically strong adversary, empirical analysis of these bounds, and making the case that \method is likely to be more robust in practice. (Section~\ref{sec:bound}). 
% \end{enumerate}

==> generative-concept-removal/2background.tex <==
\section{Background}\label{sec:background}

% We describe \tti models (\autoref{back-diffusion}), different \crt{s} (\autoref{back-conceptrem}), and attacks against them (\autoref{back-attacks}).

\subsection{Diffusion based \tti Models}\label{back-diffusion}

A diffusion based \tti model is a function $\target: \prompt \rightarrow \imgclean$ which generates an image $\imgclean$ for a given a textual prompt $\prompt$. It comprises two key components: an encoder (\te) which is used to incorporate the textual prompt in the image generation process, and a diffusion model (\dm) which is responsible for the generation of the image.

A popular encoder is CLIP, trained on a large dataset of image-text pairs, to map the embeddings of images and their corresponding text closer together in a joint text-image embedding space~\cite{radford2021learning}.
Given $N$ images $\{\imgclean_j\}_{j=1}^N$ and their corresponding text prompts $\{\prompt_j\}_{j=1}^{N}$, the training data is $\mathcal{D} = \{(\imgclean_j, \prompt_j)\}_{j=1}^N$. 

CLIP is trained to maximize the cosine similarity between the embeddings of a prompt $\prompt_j$ and its corresponding image $\imgclean_j$ while minimizing the similarity between $\prompt_j$ and any other $\imgclean_k$ for a $k \ne j$.
We denote the cosine similarity as \text{cos}($\phi_p(\prompt_j), \phi_x(\imgclean_j))$, where $\phi_x(\imgclean_j)$ is the CLIP image embedding of the image $\imgclean_j$, and $\phi_p(\prompt_j)$ is the CLIP text embedding of the prompt $\prompt_j$.
To achieve this, CLIP is trained using a contrastive loss function~\cite{yang2023robust,oord2019representation}: \[\mathcal{L}_{\text{Con}}(\mathcal{D}) = - \frac{1}{N} \sum_{j=1}^{N} \log \frac{\exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_j))/ \tau)}{\sum_{k=1}^{N} \exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_k))/ \tau)}\] where $\tau$ is the temperature parameter to scale predictions~\cite{radford2021learning, ModalityGap}. 
 


Given access to a pre-trained encoder \te, the actual images in \tti models are generated by a diffusion model, \dm, parameterized by $\theta$.
During training of \dm, Gaussian noise is added to an initial image $x_0$ for $T$ time steps to produce $x_T$, in a process known as the \emph{forward diffusion process}. The noise is then iteratively removed to approximate the initial image $\tilde{x_0}$ in the \emph{reverse diffusion process}.
During inference, the reverse diffusion process generates an image from noise.
Further, \dm can be conditioned with a textual prompt \prompt to guide the generation of $\tilde{x_0}$ to match the description in \prompt. After generating $\phi_p(\prompt)$, %from \te, 
\dm is trained by minimizing the following loss function: $\mathcal{L} = \mathbb{E}_{\epsilon, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(\imgclean_t,\phi_p(\prompt),t)||_2^2]$ for each time step $t$, and random Gaussian noise $\epsilon \sim \mathcal{N}(0,1)$.

Several prominent \tti models (e.g., Stable Diffusion v1.4 (SDv1.4)) improve the efficiency of the diffusion process by computing in the embedding space of a variational autoencoder (VAE), rather than on images~\cite{stable-diffusion}. For a VAE decoder $\mathit{D}$, VAE encoder $\mathcal{E}$, and $z_t \in \mathcal{E}(\imgclean)$ as the latent representation of $\imgclean$ in the VAE's latent space, \dm is trained by minimizing the following objective: \\
$\mathcal{L} = \mathbb{E}_{\epsilon, z_t, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(z_t,\phi_p(\prompt),t)||_2^2]$ where $\epsilon \sim \mathcal{N}(0,1)$. \\
The final image is generated from the approximation, $\tilde{z_0}$, by passing it through $\mathit{D}$: $\tilde{x_0} = \mathit{D}(\tilde{z_0})$.  
We summarize notations in Table~\ref{tab:notations}.

\input{tables/tab_notations}
 




\subsection{Concept Removal Techniques}\label{back-conceptrem}

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance?--- We use the same approach for selecting acceptable concepts as Kumari et. al.~\cite{kumari2023ablating}for group 2 and group 3 concepts. For these groups, the acceptable concept is a superset of the unacceptable concept. For example, the sex of a celebrity is the acceptable concept for a celebrity. For group 1, there is no clear definition of a superset (eg. the superset of \emph{nude} is unclear). Logically, the acceptable concept is the opposite of the unacceptable concept in this case since it is clearly defined. - SHOULD MOVE THIS EXPLANATION ELSEWHERE}

The textual phrase for an acceptable concept is $\cacc$, and for an unacceptable concept is $\cunacc$. 
For a given $\cunacc$, $\cacc$ is either the opposite (e.g., $\cunacc$ = \emph{violence} vs. $\cacc$ = \emph{peaceful}) or a general category of a specific character/object/person (e.g., $\cunacc$ = \emph{R2D2} vs. $\cacc$ = \emph{robot}). We discuss the selection of $\cacc$ for a given $\cunacc$ in \autoref{sec:pipeline}.
An image $\imgclean$ generated from a \tti model may either contain an unacceptable concept (referred to as $\imgunacc$) or an acceptable one (referred to as $\imgacc$). Similarly, a text prompt $\prompt$ may contain a phrase for an acceptable concept ($\promptacc$) or an unacceptable concept ($\promptuacc$). An example of an unacceptable prompt $\promptuacc$ containing an unacceptable concept $\cunacc$ = \emph{Captain Marvel}, is ``\emph{Captain Marvel} soaring through the sky''. \crt{s} thwart the generation of $\imgunacc$ by either fine-tuning the \tti model to suppress $\imgunacc$, or using a classifier as a filter to detect $\imgunacc$, and serve a replacement image instead. 
%

\subsubsection{Fine-tuning \crt{s}:} We first present six state-of-the-art fine-tuning \crt{s}:

\noindent\textbf{Concept Ablation (\ca)~\cite{kumari2023ablating}} fine-tunes the \tti model to minimize the KL divergence between the model's output for $\promptuacc$ and $\promptacc$ to force the generation of \imgacc instead of \imgunacc. Formally, they optimize the following objective function: 
 % \text{argmin}_\theta 
\[\begin{split}
\footnotesize
   \mathcal{L}_{\ca} =  \mathbb{E}_{\epsilon, z_t, \cunacc, \cacc, t}[w_t||\epsilon_\theta(z_t,\phi_p(\promptacc),t).sg()
    - \epsilon_\theta(z_t,\phi_p(\promptuacc),t)||_2^2]
\end{split}\]
where $\epsilon \sim \mathcal{N}(0,1)$, $z_t \in \mathcal{E}$, and $w_t$ is a time-dependent weight, and $.sg()$ is the stop-gradient operation.

\noindent\textbf{Forget-Me-Not (\forgetNot)~\cite{zhang2023forgetmenot}} minimizes the activation maps for $\cunacc$ by modifying \dm's cross-attention layers. Further, fine-tuning \dm, instead of just the cross-attention layers, results in degraded utility. 
% That is, given $a_i \in \mathcal{A}_i$, the $i$-th attention map in \dm of \tti, their loss is 
% \[\mathcal{L} = \sum_{a_i \in \mathcal{A}_i}||a_i||\]


\noindent\textbf{Selective Amnesia (\sa)~\cite{heng2023selective}} fine-tunes \tti models by adapting continuous learning techniques (elastic weight consolidation and generative replay) for \tti models to forget a concept. They optimize $\mathbb{P}(\imgclean|\theta^*,\cunacc)$, the probability of generating $\imgclean$ given $\theta^*$ and $\cunacc$, where $\theta^*$ are the frozen parameters of the original \tti model: 
\[
\begin{split}
\footnotesize
    \mathcal{L}_{\sa} = -\mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_f(\cunacc)}[\text{log}\mathbb{P}(\imgclean|\theta^*,\cunacc)] -\lambda\sum_i\frac{M_i}{2}(\theta_i^*-\theta_i)^2\\
     + \mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_r(\cacc)}[\text{log}\mathbb{P}(\imgclean|\theta,\cacc)]
\end{split}
\]
where $M$ is the Fisher information matrix over $\cacc$ and $\cunacc$, $\mathbb{P}_r$ and $\mathbb{P}_f$ are probabilities taken over the distributions of $\cacc$ and $\cunacc$ respectively, and $\lambda$ is a regularization parameter. 



\noindent\textbf{Erased Stable Diffusion (\esd)~\cite{gandikota2023erasing}} fine-tunes the \tti model by modifying the reverse diffusion process to reduce the probability of generating \imgunacc:
\[\begin{split}
\epsilon_\theta(\imgclean_t,\phi_p(\cunacc),t) = \epsilon_{\theta^*}(\imgclean_t, t)
+ \eta(\epsilon_{\theta^*}(\imgclean_t,\phi_p(\cunacc),t)-\epsilon_{\theta^*}(\imgclean_t,t))
\end{split}\]
where $\eta > 0$ encourages the noise conditioned on $\cunacc$ to match the unconditioned noise.


\noindent\textbf{Unified Concept Editing (\unifiedCE)~\cite{gandikota2023unified}} fine-tunes the \tti model's cross-attention layers to minimize the influence of $\cunacc$, while keeping the remaining concepts unchanged. Their optimization is:
% \text{min}_W
\[\begin{split}
    \mathcal{L}_{\unifiedCE} = \sum_{\cunacc \in \mathcal{C}^{u}, \cacc \in \mathcal{C}^{a}}||W\times\cunacc-W^*\times\cacc||_2^2 \\ 
    +  \sum_{c \in S}||W\times c - W^*\times c||_2^2
\end{split}\]
where $W$, $W^*$ are the parameters of the fine-tuned and original \emph{cross-attention layers in \dm}, $\mathcal{C}^{u}$ and $\mathcal{C}^{a}$ are the space of pre-defined unacceptable and acceptable concepts, and $S$ is a set of concepts for which to preserve utility. 

\noindent\textbf{Safe diffusion (\sdd)~\cite{kim2023towards}}
fine-tunes the \tti model by encouraging the diffusion model noise conditioned on $\cunacc$ to match the unconditioned noise, while minimizing the utility drop using the following objective function:
\[\begin{split}
    % \text{argmin}_\theta
    \mathcal{L}_{\sdd} = \mathbb{E}_{\epsilon, z_t, \cunacc, t}[||\epsilon_\theta(z_t,\phi_p(\cunacc),t) 
 - \epsilon_\theta(z_t,t).sg()
    ||_2^2]
\end{split}\]
where $\epsilon \sim \mathcal{N}(0,1)$ and $z_t \in \mathcal{E}(x)$.


\noindent\textbf{Moderator (\moderator)~\cite{wang2024moderator}} uses task vectors~\cite{ilharco2023editing} to remove the parameters responsible for generating $\imgunacc$ while maintaining the parameters for acceptable concepts. \moderator computes the task vector for the unacceptable parameters ($T_u$) and removes them from $\theta$: $\theta_{new} = \theta - scale \times T_u$ where $\theta_{new}$ are the new parameters. 


\subsubsection{Filtering \crt{s}:} We now describe two filtering \crt{s}:

\noindent\textbf{Stable Diffusion Filter (SD-Filter)~\cite{radford2021learning}} is black-box and the design of the filter is not publicly available. However, Rando et. al.~\cite{rando2022redteaming} hypothesize that it involves computing the cosine similarity between the embeddings of a generated image, $\imgclean$, and a pre-defined set of $\cunacc$. If the cosine similarity is greater than some threshold ($\Gamma$), then $\imgclean$ has $\cunacc$. Formally, their filter $\filter_{SD}$ can be described as
\[ \filter_{SD}(\imgclean) = \begin{cases} 
      1 & \text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) > \Gamma \\
      0 & \text{otherwise}
   \end{cases}
\]
where $\text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) = \overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\cunacc)}$, and $\overline{\cdot}$ denotes normalization. Here $\filter_{SD}(\imgclean) = 0$ indicates \imgacc and $\filter_{SD}(\imgclean) = 1$ indicates \imgunacc. Note that $\Gamma$ varies with $\cunacc$. 


\noindent\textbf{Unsafe Diffusion (\unsafediff)~\cite{unsafeDiff}} is the current state-of-the-art filtering \crt and outperforms SD-Filter~\cite{unsafeDiff}. \unsafediff trains a multi-headed neural network classifier on top of CLIP to identify $\imgunacc$ where each head classifies different $\cunacc$: \emph{nudity, violence, disturbing, hateful}, and \emph{political}. Their objective is given as $\filter_{\unsafediff}(\imgclean) = \text{MLP}(\phi_x(\imgclean))$ where MLP is a multi-layer perceptron, and $\filter_{\unsafediff} \in \{0,1\}$.


\subsection{Evading Concept Removal Techniques}\label{back-attacks} 

An adversary (\adv) may construct adversarial prompts ($\advprompt$) to evade \crt{s} and force a \tti model \target to generate unacceptable images. We denote a dataset containing adversarial prompts and their corresponding images ($\imgadv$) as $\dtestadv = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$ where ideally $\imgadv$ will contain $\cunacc$.
By default, we assume \adv is aware of \target using a \crt.
% account for the target \tti model \target, using a \crt. 
Otherwise we label \adv as \emph{na\"{i}ve}~\footnote{Some prior works refer to adversaries that take defenses into account as ``adaptive''. In line with standard practice in security research, we assume that adversaries are aware of defenses by default. We use the term ``na\"{i}ve,'' for adversaries who are not.}. 

\adv's objective is to construct $\advprompt$ which can force a \tti model to output images with $\cunacc$ while being semantically closer to acceptable prompts so that $\imgadv$ is incorrectly identified as acceptable while triggering the generation of unacceptable images.
The existing attacks construct $\advprompt$ as an optimization problem using some reference $\imgunacc$ (or the difference between $\promptacc$ and $\promptuacc$) as the ground truth. Different attacks vary in ways to solve this optimization. We present four state-of-the-art attacks below:

\noindent\textbf{PEZ~\cite{wen2023hard}} constructs $\advprompt$ by identifying text tokens by minimizing: $\mathcal{L}_{PEZ}= 1-\text{cos}(\phi_p(\advprompt),\phi_x(\imgunacc))$. 



\noindent\textbf{RingBell~\cite{Tsai2023RingABellHR}} identifies tokens for $\advprompt$ by first computing the average difference between the embedding vectors of $\promptuacc$ and $\promptacc$: $\phi_p(\hat{\prompt}) = \frac{1}{N}\sum_{i=1}^N\{\phi_p(\promptuacc_i) - \phi_p(\promptacc_i)\}$ from a set of $N$ prompts. Then, $\advprompt$ is computed by minimizing the distance of its text embedding to ($\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))$, formulated as: $\text{min}_{\advprompt} ||\phi_p(\advprompt) - (\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))||^2$ where $\prompt^{init}$ is an initial unacceptable prompt censored by a \crt, and solved using a genetic algorithm. 
%Further, the optimization relies on a fitness function using mean-squared error: $\mathcal{L}_{RingBell} = \mathcal{L}_{MSE}(\phi_p(\cunacc),\phi_p(\advprompt))$ where $\cunacc$ is a prompt that generates $\imgunacc$ in a \tti model.


\noindent\textbf{SneakyPrompt~\cite{yang2023sneakyprompt}} uses reinforcement learning to construct $\advprompt$ specifically against filtering \crt{s}. 
It searches for tokens to update an initial prompt $\prompt^{init}$ to form $\advprompt$. The reward function is the cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\advprompt)$. SneakyPrompt uses $\promptuacc$ as $\prompt^{init}$ for better effectiveness and faster convergence.

\noindent\textbf{CCE~\cite{pham2023circumventing}} uses textual-inversion to construct $\advprompt$~\cite{gal2022textualinversionimage}. \adv updates CLIP's vocabulary to include a new token ``<s>'' which, when included in $\advprompt$, generates \adv's desired image. To optimize <s>, we find $v$, an embedding for <s>, corresponding to least mean-squared-error loss $\mathcal{L}_{CCE}=\mathcal{L}_{MSE}(\epsilon, \epsilon_\theta(z_t,v,t))$, where $\epsilon\sim\mathcal{N}(0,1)$.


All of these attacks are na\"{i}ve except for CCE and SneakyPrompt, which account for different fine-tuning \crt{s}. 
In \autoref{sec:baseline}, we describe how we modify these na\"{i}ve attacks to account for \crt{s}.

==> generative-concept-removal/3problem.tex <==
\section{Problem Statement}\label{sec:problem}


 
We describe an adversary model, requirements of an ideal \crt, and limitations of prior works. 


\noindent\textbf{Adversary Model.} We consider a deployed target \tti model ($\target$) to which a client has blackbox access to send an input ($\prompt$) and obtain a generated image ($\imgclean$). Further, $\target$ uses some \crt. The goal of the adversary (\adv) is to force $\target$ to generate $\imgunacc$ despite the presence of a \crt.
We give an advantage to \adv by allowing whitebox access to a local identical copy of $\target$ with the \crt for use in designing attacks. This is reasonable as \dm and CLIP are publicly available. For filtering \crt{s}, we assume that \adv has whitebox access to the filter to use its loss function in designing the attacks. \adv aims to evade the entire \tti pipeline, including the \crt, but a real-world adversary can only directly control the text prompt, not the generated image. Testing a \crt{'s} robustness in isolation shows that the entire pipeline remains robust against such a hypothetical adversary, and hence also against the weaker real-world adversary.

\noindent\textbf{Requirements} An ideal \crt should be:
\begin{enumerate*}[label=\textbf{R\arabic*},leftmargin=*]
\item\label{effective} \textit{Effective} in minimizing the generation of $\imgunacc$;
\item\label{utility} \textit{Utility-preserving}, maintaining the quality of acceptable images (for fine-tuning \crt{s}) or not blocking them (for filtering \crt{s}); and
\item\label{robust} \textit{Robust} against evasion with $\advprompt$.
\end{enumerate*}



\noindent\textbf{Limitations of Prior Works.} 
%We now briefly discuss the limitations of different types of prior \crt{s} \emph{vis-a-vis} the requirements above. 
We summarize the limitations of prior works which are empirically evaluated later in \autoref{sec:evaluation}.
\textit{Fine-tuning \crt{s}} modify $\target$ thereby explicitly creating a trade-off between \ref{effective} and \ref{utility}~\cite{gandikota2023erasing,kumari2023ablating,zhang2023forgetmenot,heng2023selective,heng2023selective,gandikota2023unified,kim2023towards}.
Further, most of these \crt{s} do not consider \ref{robust} in their design and are susceptible to evasion by \adv with $\advprompt$.
\textit{Filtering \crt{s}}~\cite{radford2021learning,unsafeDiff} detect unacceptable concepts either in $\prompt$ (aka prompt filter) or in $\imgclean$ and block them (a.k.a image filter). Since, they do not modify $\target$, they can maintain \ref{utility} without impacting \ref{effective}. Prior filtering approaches may not be accurate in detecting unacceptable concepts (poor \ref{effective})~\cite{li2024safegen} and can be easily evaded (poor \ref{robust}) (\cite{rando2022redteaming} and \autoref{sec:filterEval}). The state-of-the-art filter, \unsafediff, trains specialized classifiers for each concept on large datasets, limiting its generalization to new concepts.


==> generative-concept-removal/4approach.tex <==
\section{\method: Robust Filtering CRT}\label{sec:approach}

We present \method, a robust \underline{co}ncept \underline{fi}ltering \crt.
\method uses a classifier \filter to detect unacceptable concepts in generated images. Following SDv1.4~\cite{stable-diffusion}, on detecting an unacceptable concept, \method outputs a replacement image~\cite{radford2021learning, rando2022redteaming}.
We identify CLIP as the natural choice for \filter as it is
\begin{enumerate*}[leftmargin=*,label=(\alph*)]
\item pre-trained on a large dataset covering a wide range of concepts, and
\item used in many \tti models, and encodes similar information as seen in them.
\end{enumerate*}
Hence, CLIP is a better choice for a filter than training specialized classifiers for each concept (e.g.,~\cite{unsafeDiff}).

 However, simply using CLIP as \filter is not sufficient as seen in SDv1.4's filter ($\filter_{SD}$)~\cite{radford2021learning}. 
Recall from \autoref{back-conceptrem} (Filtering \crt{s}), $\filter_{SD}$ thresholds the cosine similarity between the embeddings of $\imgclean$ and each pre-defined unacceptable concept to identify $\imgunacc$. 
Rando et al.~\cite{rando2022redteaming} evade $\filter_{SD}$ by constructing adversarial prompts.
Since $\filter_{SD}$ uses only the cosine similarity to $\cunacc$, \adv is free to modify the prompt embeddings in \emph{any direction}, while constructing $\advprompt$.
%
We address this in \method by configuring CLIP's classification objective to allow for fine-tuning to improve robustness. 

\noindent\textbf{Configuring CLIP's Classification Objective.} Instead of using the cosine similarity to only $\cunacc$ as in $\filter_{SD}$, we configure the objective function of \method to use the cosine similarity to \emph{both} $\cunacc$ and $\cacc$. 
% \change{This makes \adv's goal more difficult as they are forced to optimize $\advprompt$ such that the resulting image embedding is far from $\phi_p(\cunacc)$, \emph{and} close to $\phi_p(\cacc)$, which is an additional stipulation arising from the design of \method.}
Further, jointly optimizing for two embeddings yields better utility as observed in prior fine-tuning \crt{s}~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}. 
%
Given $\imgclean$, \method checks the cosine similarity of $\phi_x(\imgclean)$ to $\phi_p(\cunacc)$ and $\phi_p(\cacc)$. Formally, we define \method as
\begin{equation}\label{eq:att}
 \filter(x, \cunacc, \cacc) = \text{argmax}_{i, i\in{a,u}} \left\{\frac{\text{exp}{(\text{cos}(\phi_x(x),\phi_p(\concept_i)) / \tau)}}{\sum_{j \in \{a,u\}}\text{exp}(\text{cos}(\phi_x(x),\phi_p(\concept_j)) / \tau)}\right\}
\end{equation} 
where $\tau=\frac{1}{100}$ is the default temperature parameter used in CLIP. 
%Further, the cosine similarity is equivalent to the scaled Euclidean distance between the embeddings~\cite{ModalityGap}: 
%\[(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) = 2-2\overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\concept)}\]
%\[\implies \text{cos}(\imgclean, \concept) = -\frac{1}{2}(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) + 1\]
%Hence, by using CLIP as a filter, we \change{are effectively projecting} the image embeddings onto the vector between $\cunacc$ and $\cacc$ and classifying it based on its distance to both.  
%
% This simple configuration change in CLIP's classification objective restricts \adv to adding noise only along the low-dimensional vector joining $\cunacc$ and $\cacc$: $\phi_p(\cunacc) - \phi_p(\cacc)$ in the direction of $\cacc$.
% This is more challenging for \adv to evade than $\filter_{SD}$, as projecting to a lower-dimensional representation can improve robustness~\cite{pca1,pca2}.
% Hence, we conjecture that this can help satisfy \ref{effective} and \ref{robust} (as shown later in \autoref{sec:evaluation}).
% This change in objective function is required to apply fine-tuning.

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance? - ANSWERED}


% \change{Rationale for fine-tuning?}
\noindent\textbf{Fine-tuning.} The above configuration change lets us use fine-tuning to push acceptable and unacceptable concepts away from each other while maintaining their pairing with their corresponding image embeddings (for utility).
Our fine-tuning objectives, inspired by adversarial training, aim to increase the distance between training data and the decision boundary to reduce the impact of adversarial examples~\cite{zhang2019theoretically}. 
% may impact the utility on some concepts due to the close proximity of some $\cunacc$ and $\cacc$.
% To restore any drop in utility, we use fine-tuning. 
We use two different fine-tuning variants depending on the group of concepts.


For concepts that have a strong correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$ (for example, where $\cacc$ is a broader category that includes $\cunacc$; $\cunacc$ = \emph{R2D2} and $\cacc$ = \emph{robot}), we fine-tune \filter to increase the difference between $\phi_p(\promptuacc)$ and $\phi_p(\promptacc)$. We minimize:
\begin{equation}\label{eq:ft1}
L_{\method} = -||\overline{\phi_p(\promptuacc) - \phi_p(\promptacc)}||_2
\end{equation}
where $\overline{\cdot}$ denotes normalization. 
% The prompts used for the \tti model are not known before-hand, but we can define the concepts to be filtered. 
% Since the prompt includes these concepts, filtering the images generated from the prompts is sufficient.
For the case where $\cunacc$ and $\cacc$ are opposites (e.g., $\cunacc$ = \emph{violence} and $\cacc$ = \emph{peaceful}), the above objective function might have a low correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$, leading to poor utility. In this case, we use following objective function:
\begin{equation}\label{eq:ft2}
    \begin{split}
        \mathcal{L}_{\method} = \alpha_{\text{aa}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{aa}) 
        -\alpha_{\text{ua}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{ua}) \\
        + \alpha_{\text{uu}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{uu})  
        -\alpha_{\text{au}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{au}) \\
        -\alpha_{\text{uu-t}}\mathcal{L}_{MSE}(\phi_p(\mathcal{P}^{u}), \phi_p(\mathcal{P}^{a})) \\
    \end{split}
\end{equation}
where $\mathcal{D}_{aa} = \{(\imgacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{au} = \{(\imgacc_j, \promptuacc_j)\}_{j=1}^N$, \\$\mathcal{D}_{ua} = \{(\imgunacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{uu} = \{(\imgunacc_j, \promptuacc_j)\}_{j=1}^N$, $\mathcal{P}^u = \{\promptuacc_j\}$, and $\mathcal{P}^a = \{\promptacc_j\}$, and $\alpha_{(\cdot)}$ are regularization hyperparameters. We assign equal weight to the loss terms, thus choosing $\alpha_{(.)}= 1$, following prior work~\cite{lee2021soundguided}. This balances: (a) bringing similar concepts together (utility), and (b) pushing unrelated concepts away from the target concept (effectiveness).
\begin{submission}
We present additional experiments on the choice of $\alpha_{(\cdot)}$ in the Appendix of our full paper~\cite{das2024espresso}.
\end{submission}
\begin{arxiv}
We include additional experiments comparing different values of $\alpha_{(\cdot)}$ in Appendix~\ref{sec:alpha}.
\end{arxiv}
The above objective function encourages the CLIP embeddings of $\imgunacc$ and $\promptuacc$, and $\imgacc$ and $\promptacc$, to be closer together while increasing the distance between $\imgunacc$ and $\promptacc$, and $\imgacc$ and $\promptuacc$, respectively. 
When $\cacc$ is a generalization of $\cunacc$, the images corresponding to each are visually similar. Thus, separating prompt embeddings with \autoref{eq:ft1} is sufficient, whereas adding image embeddings with \autoref{eq:ft2} causes an over-correction and reduces utility. In contrast, when the concepts are opposites, we require a loss function that incorporates both text and image embeddings (\autoref{eq:ft2}).

We use prompts ($\promptuacc$ and $\promptacc$) for fine-tuning in Equations~\ref{eq:ft1} and~\ref{eq:ft2} instead of only concepts ($\cunacc$ and $\cacc$): 
$\promptuacc$ and $\promptacc$ already contain $\cunacc$ and $\cacc$, and provide more context. 
During fine-tuning, there is a trade-off between \ref{effective} and \ref{utility} which is inherent to all other fine-tuning \crt{s}. We subject our fine-tuning to the constraint that achieved the highest effectiveness for the least drop in utility.
In \autoref{sec:finetuningEval}, we discuss which fine-tuning objectives (Equation~\ref{eq:ft1} or~\ref{eq:ft2}) apply to each concept, and demonstrate the benefit of fine-tuning.

==> generative-concept-removal/5setup.tex <==
\section{Experimental Setup}\label{sec:setup}

% \input{figures/fig_trainvaltest}
We describe the attack baselines against \crt{s} (\autoref{sec:baseline}), metrics (\autoref{sec:metrics}), and present a pipeline for evaluating \crt{s} (\autoref{sec:pipeline}). 
We use SDv1.4~\cite{stable-diffusion} and its default configuration as \target following prior work~\cite{gandikota2023erasing, kumari2023ablating, zhang2023forgetmenot, heng2023selective, gandikota2023unified, kim2023towards}.
We compare \method with the seven fine-tuning and one filtering \crt{s} from \autoref{back-conceptrem} (we leave out SD-Filter as \unsafediff outperforms it).

\subsection{Revisiting Attack Baselines}\label{sec:baseline}

%\change{We compare \method with prior state-of-the-art \crt{s} across \ref{effective}, \ref{utility}, and \ref{robust}. 
%We use seven fine-tuning \crt{s} (\ca, \forgetNot, \sa, \esd, \unifiedCE, \sdd, and \moderator) and one filtering \crt (\unsafediff) which are described in \autoref{back-conceptrem}. For filtering \crt, we do not compare with SD-Filter as \unsafediff outperforms it.}
% To evaluate \ref{robust}, 
% We consider different state-of-art attacks from literature (\autoref{back-attacks}).
%
We modify existing na\"{i}ve attacks: \ringbell, and \pez, to account for \crt{s} (indicated with ``+''). 
All \crt{s} use some variant of the following optimization: detach $\cunacc$ from $\prompt$ such that the generated image is far from $\cunacc$ and closer to some $\cacc$. 
On the other hand, attacks against \tti models design $\advprompt$ such that $\imgadv$ is closer to $\cunacc$ and far from $\cacc$. 
Hence, to design an effective attack which accounts for such \crt{s}, in addition to the attacks' original objectives, we minimize the loss between $\phi_p(\advprompt)$ and $\phi_p(\cacc)$ while increasing the loss between $\phi_p(\advprompt)$ and $\phi_p(\cunacc)$.
We modify the attacks using the following loss: 
\begin{equation}\label{eq:attack}
    \begin{split}
\mathcal{L}_{att+} = \mathcal{L}_{att} - \alpha_u \mathcal{L}_{MSE}(\phi_p(\cunacc), \phi_p(\advprompt)) + \\
\alpha_a \mathcal{L}_{MSE}(\phi_p(\cacc), \phi_p(\advprompt))
    \end{split}
\end{equation}
where $att \in$ \{\ringbell, \pez\} when \crt$\in $\{\ca, \forgetNot, \sa, \esd, \unifiedCE, \sdd, \unsafediff, \method\}, and $\mathcal{L}_{att}$ is the attack's original objective.
We assign equal weight to all loss terms and use $\alpha_u = \alpha_a = 1.$
% Further, To design attacks against \unsafediff and \method, .
Recall from \autoref{back-attacks} that \cce already accounts for different fine-tuning \crt{s}. For filtering \crt{s} (\unsafediff and \method), we modify \cce using Equation~\ref{eq:attack} and call it \cce+. 
%
Finally, typographic attack~\cite{noever2021typographicattck} against CLIP superimposes text characters onto an (unrelated) image to fool CLIP by forcing it to focus on the text instead of the image. We turn this into an attack against \crt{s} by superimposing $\cacc$ at the bottom of $\imgunacc$. Using the resulting adversarial images, we use \pez+ to find their corresponding $\advprompt$. We call this attack \typo+.
%\footnote{Some prior works refer to adversaries that take defenses into account as ''adaptive''. In line with standard practice in security research, we assume that adversaries are typically aware of defenses. We use the term ``na\"{i}ve,'' for adversaries who are not.}.

\input{figures/fig_pipeline}

\subsection{Metrics}\label{sec:metrics}

We now describe the metrics to evaluate each of the requirements. 
\noindent We use a \emph{reference CLIP} (SDv1.4), separate from \target with the \crt{s}, following prior work~\cite{kumari2023ablating, gandikota2023erasing,gandikota2023unified,kim2023towards}.

\noindent\textbf{\underline{\ref{effective} (Effectiveness).}}
\begin{itemize}[leftmargin=*]
\item For fine-tuning \crt{s}, we use \textbf{CLIP accuracy}~\cite{hessel-etal-2021-clipscore,kumari2023ablating} which is the cosine similarity between the embeddings of the generated image $\imgclean$ with the embeddings of $\cunacc$ and $\cacc$ from the reference CLIP. This gives the likelihood of predicting $\cunacc$. Hence, CLIP accuracy should be low (ideally zero) for effective concept removal. Formally, it is:
\[\frac{\text{exp}{(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc)))}}{\text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc))) + \text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cacc)))}\]
where $\tilde{\phi_p}$ and $\tilde{\phi_x}$ are embeddings from the reference CLIP.
For \method, if $\imgunacc$ is detected, a replacement image is generated. Here, we calculate the CLIP accuracy on the final set of images after filtering. 
Since the metrics compare with the reference CLIP, we use the same default replacement image as in the SD v1.4.

\item For filtering \crt{s}, we use \textbf{false negative rates (FNR)~\cite{unsafeDiff,rando2022redteaming}} which is the fraction of images with $\cunacc$ which are not blocked. 
It should be low (ideally zero).
\end{itemize}


\noindent\textbf{\underline{\ref{utility} (Utility).}}
\begin{itemize}[leftmargin=*]
\item For fine-tuning \crt{s}, we use \textbf{normalized CLIP score} which is the ratio of cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$ from \target, to that from a reference CLIP as a baseline. Here, the baseline from a reference CLIP is assumed to have the maximum achievable CLIP score. Formally, we can write normalized CLIP score as $\frac{\text{cos}(\phi_x(\imgclean),\phi_p(\prompt))}{\text{cos}(\tilde\phi_x({\imgclean}), \tilde\phi_p(\prompt))}$. 
It should be high (ideally one) for high utility. 
% \change{For the normalized CLIP score to be greater than one, the fine-tuned \tti model should generate images that match their prompts more closely than the original \tti model. This is unlikely to occur in practice as seen in our evaluation} (c.f. Table~\ref{tab:utility}).
This metric is different from standard CLIP scores from prior work~\cite{hessel-etal-2021-clipscore,kumari2023ablating, kim2023towards,gandikota2023unified} which only measures the cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$. 
We did this to scale the CLIP score between zero and one while comparing \target to the reference CLIP.
%We modified it to compare the utility of the \tti model with the \crt to that of the \tti model without the \crt.
%Hence, a perfect match will give a score of one.

\item For filtering \crt{s}, we use \textbf{False Positive Rates (FPR)~\cite{unsafeDiff,rando2022redteaming}} which is the fraction of images without $\cunacc$ which are blocked.
It should be low (ideally zero).
\end{itemize} 


\noindent\textbf{\underline{\ref{robust} (Robustness).}} We use the same metrics as \ref{effective}, but in the presence of \adv.


\subsection{Pipeline for Evaluating \crt{s}}\label{sec:pipeline}

We now describe~\autoref{fig:pipeline} which includes identifying acceptable concepts (step 1), generation of datasets (step 2), training filters or fine-tuning \tti models with \crt{s} (step 3), validating acceptable concepts (step 4), and evaluating different \crt{s} (step 5). 
% We present an overview of the pipeline in Figure~\ref{fig:pipeline} and describe each of the steps below.



\noindent\textbf{Concept Types.}
We use the same $\cunacc$ as prior work~\cite{kumari2023ablating, pham2023circumventing, kim2023towards}, categorizing them into three groups:
\begin{itemize}[leftmargin=*]
\item Group-1 covers inappropriate concepts: \emph{nudity}, (e.g., genitalia), 
\emph{violence}, (e.g., bloody scenes), 
\emph{disturbing} (e.g., human flesh), 
 \emph{hateful} (e.g. harmful stereotypes).
\item Group-2 covers copyright-infringing concepts: \emph{Grumpy Cat, Nemo, Captain Marvel, Snoopy}, and \emph{R2D2}.
\item Group-3 covers unauthorized use of images: \emph{Taylor Swift, Angelina Jolie, Brad Pitt}, and \emph{Elon Musk}.
\end{itemize}


\noindent\textbf{\underline{Step 1: Identifying Acceptable Concepts}}
A good choice of $\cacc$ is one which effectively steers a \tti model away from generating $\imgunacc$ while maintaining utility on other concepts. Hence, the choice of $\cacc$ can impact \ref{effective} and \ref{utility}. 
We select $\cacc$ for a given $\cunacc$ such that it is either opposite to $\cunacc$ (Group-1) or is a semantic generalization of $\cunacc$ so as to avoid infringing copyrights (Groups-2,3).
For $\cunacc$ in Group-1, we consider multiple alternative synonyms for $\cacc$, from which we choose the best possible candidate by measuring effectiveness and utility on a validation dataset (see Step 4).
For $\cunacc$ in Groups-2,3, we use $\cacc$ from prior work for a fair comparison~\cite{kumari2023ablating,heng2023selective}.
We indicate them in the format ``$\cunacc$ $\rightarrow$ $\cacc$'':
\begin{itemize}[leftmargin=*]
\item For \textbf{Group-1}, $\cacc$ is the opposite of $\cunacc$ and we consider the following choices of $\cacc$: \emph{nudity} $\rightarrow$ \{\emph{clothed} and \emph{clean}\}; \emph{violence} $\rightarrow$ \{\emph{peaceful}, \emph{nonviolent}, and \emph{gentle}\}; \emph{disturbing} $\rightarrow$ \{\emph{pleasing}, \emph{calming}, and \emph{soothing}\}; \emph{hateful} $\rightarrow$ \{\emph{loving}, \emph{compassionate}, and \emph{kind}\}.
\item For \textbf{Group-2}: $\cacc$ is the broader category of $\cunacc$, following prior works~\cite{kumari2023ablating,heng2023selective,gandikota2023erasing}: \emph{Grumpy Cat} $\rightarrow$ \emph{cat}, \emph{Nemo} $\rightarrow$ \emph{fish}, \emph{Captain Marvel} $\rightarrow$ \emph{female superhero, Snoopy} $\rightarrow$ \emph{dog}, and \emph{R2D2} $\rightarrow$ \emph{robot}. 
\item For \textbf{Group-3}, $\cacc$ is the sex of $\cunacc$, following prior works~\cite{heng2023selective, zhang2023forgetmenot, kim2023towards}: \{\emph{Taylor Swift, Angelina Jolie}\} $\rightarrow$ \emph{woman} and \{\emph{Brad Pitt, Elon Musk}\} $\rightarrow$ \emph{man}.
\end{itemize}
We compare \method with each \crt category separately using concepts they were originally evaluated on: Group-1 for filtering \crt{s}~\cite{unsafeDiff}; all groups for fine-tuning \crt{s}~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards}.


% \subsection{Dataset and Model Configurations}\label{sec:datasets}

\noindent\textbf{\underline{Step 2: Generate and Split Datasets}}
We describe the generation of train, validation, and test datasets.

\noindent\textbf{Train Datasets.}
We summarize the different training/fine-tuning dataset configurations across \crt{s} in Table~\ref{tab:trconfig}. 
\input{tables/tab_trconfig}
For \emph{fine-tuning \crt{s}}, we use the exact same configuration as described in their original works. 
This configuration for a specific \crt is the same across different concepts.
\ca uses acceptable prompts which are generated from ChatGPT such that they contain $\cacc$, and 1 image per prompt. \esd and \sdd both use only $\cunacc$, and \sdd additionally uses 10 images corresponding to $\cunacc$. All images are generated using SD v1.4. 
\forgetNot uses unacceptable prompts of the form ``An image of \{$\cunacc$\}'', and 1 image per prompt.
\moderator uses $\cunacc$ and 120 corresponding images.
For all of them, we use their code for consistency with their original papers~\cite{githubGitHubNupurkmr9conceptablation,githubGitHubRohitgandikotaerasing,githubGitHubSHILabsForgetMeNot,githubGitHubRohitgandikotaunifiedconceptediting,githubGitHubClearnusselectiveamnesia,githubGitHubNannullnasafediffusion,githubGitHubYitingQuunsafediffusion,githubGitHubWangModerator}.



\noindent For \emph{filtering \crt{s},} we train $\filter_{\unsafediff}$ using the original dataset configuration and code~\cite{unsafeDiff}. 
For \method, we follow \ca~\cite{kumari2023ablating} to generate 10 unacceptable and acceptable prompts using ChatGPT, with one image per prompt from SDv1.4.
For Group-2, we randomly select 10 ChatGPT-generated prompts from \ca~\cite{kumari2023ablating}.
We use a small amount of training data following prior works which show little data is enough to modify CLIP~\cite{yang2023robust,carlini2022poisoning}. This is validated by our results (\autoref{sec:evaluation}).



\noindent\textbf{Validation Datasets.}
For validation datasets ($\mathcal{D}_{val}$), we denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalunacc$; and the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalacc$.
For \ref{effective}, we use $\dvalunacc$ by generating 10 unacceptable prompts using ChatGPT, and generate 5 images per prompt using SD v1.4. 
For \ref{utility}, we use $\dvalacc$ by randomly choosing 100 acceptable prompts from the COCO 2014 dataset~\cite{coco}, and 1 image per prompt, from SD v1.4.
We summarize them in Table~\ref{tab:valconfig}. 

\input{tables/tab_valconfig}

\noindent\textbf{Test Datasets.} We now present test dataset ($\mathcal{D}_{te}$) for evaluating different \crt{s}. 
We denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dtestacc$; and with unacceptable prompts ($\promptuacc$) and corresponding images ($\imgunacc$) as $\dtestunacc$.



\noindent For evaluating effectiveness (\ref{effective}), we use $\dtestunacc$ generated as follows:
\begin{itemize}[leftmargin=*]
\item For Group-1 concepts (\emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing}), we use Inappropriate Image Prompts (I2P), containing prompts which are likely to generate unsafe images~\cite{schramowski2022safe}.
We process I2P dataset following prior work~\cite{gandikota2023erasing, gandikota2023unified} to obtain 300 unacceptable prompts:
For \emph{nudity}, I2P includes a ``nudity percentage'' attribute. We choose all unacceptable prompts with a nudity percentage $>10$, resulting in a total of 300 unacceptable prompts, in accordance with prior works~\cite{gandikota2023erasing, gandikota2023unified}.
\unsafediff~\cite{unsafeDiff} also used \emph{political} as a concept, which is excluded from our evaluation since it is not a part of I2P. 
% Note that I2P prompts do not explicitly contain $\cunacc$, \emph{i.e., the words \emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing} are not explicitly included in the prompts}.
\item For concepts in Group-2, 3, there are no standard benchmark datasets. Hence, we use the dataset from prior works~\cite{kumari2023ablating, gandikota2023erasing} with 200 unacceptable images generated from SDv1.4 from 10 unacceptable prompts generated from ChatGPT.
For \ref{utility}, we use the COCO 2014 test dataset as $\dtestacc$, consistent with prior work, with 200 randomly chosen acceptable prompts, non-overlapping with $\dvalacc$.
For \ref{robust}, we use $\dtestadv$ by applying different attacks on $\dtestunacc$ to generate adversarial prompts.
\end{itemize}
We summarize the datasets in Table~\ref{tab:teconfig}. 

\input{tables/tab_teconfig}

\noindent\textbf{\underline{Step 3: Fine-tuning with \crt{s}/training filter.}}
We train each baseline \crt in \autoref{back-attacks} using $\dtrain$.
We train \unsafediff's classifier on their dataset and we fine-tune \method on $\dtrain$ using Equation~\ref{eq:ft1} for Groups-2,3 concepts and Equation~\ref{eq:ft2} for Group-1 concepts. 
We use the CLIP L-patch-14~\cite{vit} due to its popularity, which is also the default encoder with SDv1.4. However, other variants of CLIP are also applicable.

\noindent\textbf{\underline{Step 4: Select best $\cacc$ using $\mathcal{D}_{val}$}.}
For Group-1 concepts, we evaluate \ref{effective} and \ref{utility} for different candidates of $\cacc$ on $\dvalunacc$ and $\dvalacc$ respectively. 
We found the concepts with the best results: \emph{nudity} $\rightarrow$ \emph{clean}, \emph{violence} $\rightarrow$ \emph{peaceful}, \emph{disturbing} $\rightarrow$ \emph{pleasing}, and \emph{hateful} $\rightarrow$ \emph{loving}.
For \emph{nudity}, we eliminated \emph{clothed} as it blocked images with minimal exposed skin despite being acceptable~\cite{unsafeDiff,schramowski2022safe}.
%
%
% We use concepts in Group-1 following prior work~\cite{unsafeDiff} to evaluate filtering \crt{s}. 
% We use \emph{nudity} and \emph{violence} from Group-1, and all the concepts from Group-2 and Group-3 following prior works~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards} to evaluate fine-tuning \crt{s}. 

% We summarize the final concepts for evaluation in Table~\ref{tab:concepts}.



\noindent\textbf{\underline{Step 5: Evaluation}.} 
We evaluate \ref{effective} on $\dtestunacc$, \ref{utility} on $\dtestacc$, and \ref{robust} on $\dtestadv$, which is generated by running different attacks on $\dtestunacc$ to get $\advprompt$. We pass the prompts from the datasets to the \tti model and compute different metrics.



==> generative-concept-removal/6evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

% We demonstrate the impact of fine-tuning (\autoref{sec:finetuningEval}), and compare \method with fine-tuning \crt{s} (\autoref{sec:finetuneEval}) and filtering \crt{s} (\autoref{sec:filterEval}).

\subsection{Impact of Fine-Tuning}\label{sec:finetuningEval}

We first empirically show how fine-tuning can improve \method's robustness similar to adversarial training in classifiers. 
Adversarial training~\cite{zhang2019theoretically} explicitly pushes the decision boundary away from training data records. 
Similarly, our fine-tuning objective, pushes the embeddings of acceptable and unacceptable concepts away from each other. 
This results in correctly classifying $\imgadv$ by \method. 



To demonstrate this, we generated 10 adversarial prompts with 5 images per prompt using \cce+. We evaluate with \cce+ because, being a white-box attack, it is the more effective than others (see \autoref{back-conceptrem}).
For each image, $\imgadv$, we compute the cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\cunacc)$, as well as between $\phi_x(\imgadv)$ and $\phi_p(\cacc)$. 
We then take the absolute values of both similarities and calculate their difference. We report the mean difference in \autoref{tab:advsims}.
We use Equation~\ref{eq:ft1} for fine-tuning in Group-2 and 3, where $\cacc$ is a broader category that includes $\cunacc$. We use Equation~\ref{eq:ft2} for Group-1 concepts as $\cunacc$ and $\cacc$ are opposites.

%We report the mean absolute difference between the cosine similarity of all the $\phi_x(\imgadv)$ and $\phi_p(\cunacc)$ and $\phi_p(\cacc)$ in Table~\ref{tab:advsims}. 


\input{tables/tab_adv_sims}
\input{tables/tab_effectiveness}
\input{tables/tab_utility}
\input{tables/tab_robustness}

Across all concepts, using fine-tuning (w/ FT) makes $\phi_x(\imgadv)$ closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$, compared to the baseline without fine-tuning (w/o FT). Hence, fine-tuning is likely to correctly identify $\imgadv$ as $\imgunacc$.
%
Furthermore, we evaluate the impact of fine-tuning on \ref{effective} and \ref{utility}. For \ref{effective}, CLIP accuracy for several concepts is better after fine-tuning: \emph{Angelina Jolie} (0.03 $\pm$ 0.00 from 0.12 $\pm$ 0.02), \emph{Brad Pitt} (0.00 $\pm$ 0.00 from 0.02 $\pm$ 0.01), \emph{Elon Musk} (0.03 $\pm$ 0.00 from 0.07 $\pm$ 0.01). For \ref{utility}, CLIP scores are better for some concepts after fine-tuning: \emph{nudity} (0.94 $\pm$ 0.08 from 0.83 $\pm$ 0.07); \emph{grumpy cat} (0.98 $\pm$ 0.04 from 0.88 $\pm$ 0.03), \emph{Nemo} (0.37 $\pm$ 0.02 from 0.24 $\pm$ 0.05), \emph{R2D2} (0.66 $\pm$ 0.02 from 0.52 $\pm$ 0.03), and \emph{Elon musk} (0.97 $\pm$ 0.01 from 0.92 $\pm$ 0.02).
The metrics for other concepts remains similar.




\subsection{Comparison with Fine-tuning \crt{s}}\label{sec:finetuneEval}


\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report CLIP accuracy on $\dtestunacc$ in Table~\ref{tab:effectiveness}. 
We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.
All \crt{s} exhibit poor accuracy on \emph{nudity} and \emph{violence}, likely due to fine-tuning \crt{s} being sensitive to input prompts~\cite{pham2024robust, ma2024jailbreaking}. Specifically, other \crt{s} depend on the $\cunacc$ being included in prompts, which is absent for \emph{nudity} and \emph{violence} prompts in the I2P dataset.
\method consistently maintains high accuracy on the I2P benchmark dataset as it classifies the generated images.
\unifiedCE, \sdd, and \moderator have better accuracy compared to the other four fine-tuning \crt{s}. 
For \sdd, this could be attributed to its optimization which includes fine-tuning \dm, conditioned on $\cunacc$, to match the unconditioned \dm to reduce the influence of $\cunacc$ on the output.
For \unifiedCE and \moderator, we attribute their higher effectiveness to directly removing the influence of $\cunacc$ from the parameters. \textbf{\textit{Overall, \method is more effective than other fine-tuning \crt{s}.}}



\noindent\textbf{\underline{\ref{utility} Utility.}} We report normalized CLIP scores in Table~\ref{tab:utility} on $\dtestacc$.
We use \colorbox{mynicered}{red} if score is between 50-70, \colorbox{myniceblue}{blue} if between 70-90; \colorbox{mynicegreen}{green} if $>$90.
All the fine-tuning \crt{s} perform well across all concepts (either \colorbox{myniceblue}{blue} or \colorbox{mynicegreen}{green}) since the explicitly account for \ref{utility}. We observe that \ca with KL-Divergence-based optimization for cross-attention layers, and \unifiedCE with a precise closed-form solution to model updates, preserve \ref{utility} better than others. 
%
\method has high utility for all concepts except for \emph{violence}, and Group-2 concepts (\emph{Nemo}, \emph{Captain Marvel}, \emph{Snoopy}, and \emph{R2D2}).
For \textit{violence}, we attribute this to the trade-off between \ref{effective} and \ref{utility} during fine-tuning: we observed an early decrease in utility during the very first epoch resulting in poor trade-off.
For Group-2 concepts, we attribute the poor utility to the ambiguity in the unacceptable concepts. For instance, \emph{Nemo} is both a fish and a ship captain~\cite{VERNE_2024}, and \emph{Captain Marvel} represents both a male and a female superhero~\cite{Friedwald_2019_marvel}. 
To verify this, we precisely specify the unacceptable concepts to reduce ambiguity: as \emph{Nemo}$\rightarrow$ \emph{Nemo fish}, \emph{Captain Marvel}$\rightarrow$ \emph{Captain Marvel female superhero}, \emph{Snoopy}$\rightarrow$ \emph{Snoopy dog}, and \emph{R2D2}$\rightarrow$ \emph{R2D2 robot}. We evaluate \method on $\dvalacc$, and
compared to the results in Table~\ref{tab:utility}, the normalized CLIP score for this new configuration is: 0.97 $\pm$ 0.00 (\emph{Nemo fish}), 0.90 $\pm$ 0.02 (\emph{Captain Marvel female superhero}), 0.98 $\pm$ 0.03 (\emph{Snoopy dog}), 0.92 $\pm$ 0.02 (\emph{R2D2 robot}), which are now labeled as \colorbox{mynicegreen}{green}.
We also report the CLIP accuracy on $\dvalunacc$ to evaluate \ref{effective} with this new configuration: 0.02 $\pm$ 0.00 (\emph{Nemo fish}), 0.00 $\pm$ 0.00 (\emph{Captain Marvel female superhero}), 0.02 $\pm$ 0.01 (\emph{Snoopy dog}), 0.00 $\pm$ 0.00 (\emph{R2D2 robot}), which are effective, same as before. Hence, precisely specifying $\cunacc$ is important for \method and can satisfy \ref{utility} without sacrificing \ref{effective}. 
\textbf{\textit{Overall, \method suffers from a small drop in utility (\ref{utility}) while performing significantly better in effectiveness (\ref{effective}).}}


\noindent\textbf{\underline{\ref{robust} Robustness.}} We report CLIP accuracy on $\dtestadv$ in Table~\ref{tab:robust}. 
% \change{We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.}
We evaluate different \crt{s} against \typo+, \pez+, \cce/\cce+, and \ringbell+. We use the same color coding as in \ref{effective}. 
%
\cce/\cce+, being a white-box attack that uses the parameters of the entire \tti model, is the most powerful attack and renders all fine-tuning \crt{s} ineffective. However, \method is robust against \cce/\cce+ and outperforms all fine-tuning \crt{s}. While \moderator outperforms \method for \textit{Snoopy}, \textit{Grumpy Cat}, and \textit{Brad Pitt} for \pez+ and \typo+, \method outperforms on the remaining concepts and attacks.
On the remaining attacks, all the fine-tuning \crt{s} have better robustness on Group-3 concepts than on Group-1 and 2. We attribute this to the difficulty of \tti models in generating high quality celebrity faces while also evading detection, as also observed in prior work~\cite{Matthias_2023}.
As expected, we note that all \crt{s} perform poorly on \emph{nudity} and \emph{violence} across all the attacks as they do not satisfy \ref{effective}.
Hence, it is expected that adversarial prompts for these concepts will easily evade them.
\textbf{\emph{Overall, \method is more robust than all prior work across all the concepts and attacks.}}
% We discuss the possibility of future attacks against \method in \autoref{sec:future}.



\noindent\textbf{\underline{Summary.}} 
We depict the trade-offs among \ref{effective}, \ref{utility}, and \ref{robust} in Figure~\ref{fig:radarsFT}. We use (1-CLIP accuracy) for \ref{effective} on $\dtestunacc$, normalized CLIP score on $\dtestacc$ for \ref{utility}, and (1-CLIP accuracy) for \ref{robust} on $\dtestadv$ using \cce/\cce+. 
For each of the requirements, we use the average across all concepts as the representative value for a \crt.
\emph{Overall, although \method suffers a small drop in utility \ref{utility}, it provides a better trade-off across the three requirements compared to other \crt{s}.}

\input{figures/fig_radar_ft}

































\subsection{Comparison with Filtering \crt}\label{sec:filterEval}

We now compare with \unsafediff~\cite{unsafeDiff}, the state-of-the-art filtering \crt, across the three requirements and summarize the results. 
To compare with \unsafediff~\cite{unsafeDiff}, we use FNR to evaluate effectiveness on $\dtestunacc$, FPR for utility on $\dtestacc$, and FNR for robustness on $\dtestadv$.


\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report FNR across four concepts (\emph{nudity}, \emph{violence}, \emph{disturbing}, and \emph{hateful}) in Table~\ref{tab:FilterEffective}.
We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FNR is $<$0.25.
\method has better FNR for three of the four concepts: \emph{nudity}, \emph{violence} (in \colorbox{mynicegreen}{green}), and \emph{hateful} (\colorbox{myniceblue}{blue} for \method and \colorbox{mynicered}{red} for \unsafediff). However, both \method and \unsafediff perform poorly on \emph{disturbing}. 
We attribute this poor effectiveness on Group-1 concepts to the subjective description of $\cunacc$. Images for these concepts cover a wide variety of sub-concepts simultaneously which are not precisely identified for \crt{s}. 
\emph{\textbf{Overall, \method is more effective than \unsafediff on most concepts.}}

\input{tables/tab_filter_effective}



\noindent\textbf{\underline{\ref{utility} Utility.}} We present FPR in Table~\ref{tab:FilterUtility} and use \colorbox{mynicered}{red} if FPR is $>$0.50, \colorbox{myniceblue}{blue} if FPR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FPR is $<$0.25. As expected, we observe that both \emph{\textbf{\method and \unsafediff have comparable utility as they demonstrate a low FPR}}. \unsafediff explicitly includes images containing $\cacc$ while training the multi-headed classifier.

\input{tables/tab_filter_utility}

\noindent\textbf{\underline{\ref{robust} Robustness.}} We report FNR on the dataset for adversarial prompts and corresponding images in Table~\ref{tab:FilterRobust}. 
We use the same color-coding as \ref{effective}.
% \change{We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; and \colorbox{mynicegreen}{green} if FNR is $<$0.25.}
In addition to the four attacks from Table~\ref{tab:robust}, recall that \sneaky~\cite{yang2023sneakyprompt} is specifically designed to attack filtering \crt{s}. Hence, we also evaluate against \sneaky. 
Also, since \cce is not adaptive against filtering \crt's, we evaluate \unsafediff and \method against \cce+. We are the first to evaluate different attacks against \unsafediff.
%
\input{tables/tab_filter_robust}
%
We observe that \method is effective against \pez+ while \unsafediff can be evaded.
On all the remaining attacks, we show that \method is robust on more concepts than \unsafediff.
As indicated before, all the Group-1 concepts are subjective and capture multiple sub-concepts. This ambiguity could be the reason for poor \ref{robust}.
\emph{\textbf{Overall, \method is more robust than \unsafediff on a majority of the concepts across various attacks.}}





\noindent\textbf{\underline{Summary.}} 
We present the trade-offs in the form of radar plots in Figure~\ref{fig:radarsFilt}. 
We use (1- FNR) on $\dtestunacc$ for \ref{effective}, (1- FPR) on $\dtestacc$ for \ref{utility}, and (1- FNR) on $\dtestadv$ using CCE+ for \ref{robust}. Hence, a higher value indicates better performance.
\method has comparable utility to \unsafediff but outperforms in effectiveness and robustness.
\emph{Overall, \method covers a larger area, and hence provides a better trade-off than \unsafediff.}

\input{figures/fig_radar_filter}



==> generative-concept-removal/9discussion.tex <==
\section{Discussion and Future Work}\label{sec:discussions}

%We revisit our discussion on robustness, applicability/extensions of \method, and a summary of this work.



\subsection{Certifying Robustness of \method}
% \section{Certifying Robustness of \method}\label{sec:bound}
% We empirically showed that \method is robust against several state-of-the-art attacks (\autoref{sec:evaluation}).
Inspired by the literature on certified robustness against adversarial examples~\cite{cohen2019certified}, it is natural to ask whether a similar notion of certified robustness is possible for \crt{s}.
None of the existing \crt{s} have considered certified robustness.
We are the first to explore its feasibility for \method.
%
We first present a theoretical bound on the worst-case input modification by \adv under which we can guarantee \method's accuracy. 

% \input{figures/fig_adversarial}

% \subsection{Theoretical Bound}\label{sec:theoretical} 

\noindent\emph{Theoretical Bound.} Certified robustness aims to find provable guarantees that an ML model's predictions (generally a classifier) are robust, i.e., the predictions do not change on adding noise to the input~\cite{carlini2023certified}. 
Our goal is to have a similar robustness bound for a \tti model with \method. 
We want to find the maximum input noise which \method can tolerate.

We give advantage to \adv by assuming they can directly add adversarial noise to \method's embeddings. This is a strong assumption as in practice, \adv can only send prompts to the \tti model. \begin{arxiv}
We revisit this assumption later in Appendix~\autoref{sec:implications}.    
\end{arxiv}
\begin{submission}
We discuss this assumption in the Appendix of our full version of our paper~\cite{das2024espresso}.
\end{submission}

Formally, given an unacceptable image $\imgunacc$, \adv adds noise $\delta$ to its embeddings, $\phi_x(\imgunacc)$, such that $\filter(\phi_x(\imgunacc) + \delta)$ is misclassified as acceptable.
Using this assumption, we specify the maximum noise $\delta$ added to the embeddings, $\phi_x(\imgunacc)$, that \method can tolerate in Theorem~\ref{thm.1}.


\begin{theorem}~\label{thm.1}
    Let $\hat{x} = \phi_x(x), \hat{c}^i = \phi_p(c^i), i\in\{a,u\}$. 
    % For $F(x)$ defined in equation~\ref{eq:att}, 
    Define 
    \[g_i(\hat{x}):=\frac{exp(s(\hat{x},\hat{c}^i))}{exp(s(\hat{x},\caccc))+exp(s(\hat{x},\cunaccc))},\] 
    where $s(\hat{x},\hat{c}^i) = \tau \text{cos}(\hat{x},\hat{c}^i))$, then $g_i$ is the confidence of $\hat{x}$ being classified as $\concept^i$. $F(x)$ can be defined as $F(\hat{x})=argmax_i g_i(\hat{x})$, and $F(\hat{x})$ classifies $\hat{x}$ as unacceptable if $g_u(\hat{x})>\Gamma$, where $\Gamma$ is the decision threshold.
     For a given image embedding $\hat{x}$, if $g(\hat{x}):=g_u(\hat{x})>\Gamma$, then $g$ is robust against noise $\delta$ where 
     \[||\delta||\leq\left(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|}\right)||\hat{x}||,\]
     % on the image embedding, 
     and $\Gamma$ is the decision threshold i.e. 
    \begin{equation}\label{eq:bound}
            F(\hat{x}) = F(\hat{x}+\delta), \forall ||\delta||\leq \left(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|}\right)||\hat{x}||.
    \end{equation}
\end{theorem}

\begin{proof}
    For an unacceptable image embedding $\hat{x} = \phi_x(\imgunacc)$,
    % We assume that $F(\hat{x})=1$ and 
    $g(\hat{x}):=g_u(\hat{x})$, then $g(\hat{x})-\Gamma>0$, and $\Gamma$ is the decision threshold for classification.
    Let $s_1=\tau\text{cos}(\hat{x},\cunaccc)$, $s_2=\tau\text{cos}(\hat{x},\caccc)$, $\textbf{s}=[s_1,s_2]^T$, 
    then
    $$g(\hat{x})=S(s_1) = \frac{exp(s_1)}{exp(s_1)+exp(s_2)},$$
    where $S(s_1)$ is the first item of Softmax function with respect to $\textbf{s}$.
    Then, we have $\frac{\partial}{\partial s_1} S = S(s_1)(1-S(s_1))\leq0.25, \frac{\partial}{\partial s_2} S = -S(s_1)S(s_2)\leq0.25$.

    Note that $||\hat{x}||>0$ and $||\caccc||>0$,
    we have 
    \begin{equation*}
    \begin{aligned}
        ||\frac{\partial}{\partial \hat{x}} s(\hat{x},\caccc)|| = ||\frac{\tau||\caccc||(I-xx^T)\caccc}{||\hat{x}||||\caccc||^2}||=\frac{\tau sin(\hat{x},\caccc)}{||\hat{x}||}\leq\frac{\tau}{||\hat{x}||}
    \end{aligned}
    \end{equation*}
    where $||\frac{\partial}{\partial\hat{x}} s(\hat{x}, \cunaccc)||\leq\frac{\tau}{||\hat{x}||}$. 

    For each $\hat{x}$, according to the chain rule of composition functions, 
    $\frac{\partial}{\partial\hat{x}}g(\hat{x)}=\frac{\partial S}{\partial s_1}\cdot\frac{\partial s_1}{\hat{x}}+ \frac{\partial S}{\partial s_2}\cdot\frac{\partial s_2}{\hat{x}}\leq \frac{\tau}{2||\hat{x}||}$. Therefore, the Lipschitz constant of $g(\hat{x})$ with respect to $\hat{x}$ is $\frac{\tau}{2||\hat{x}||}$, and
    \begin{equation*}
    \begin{aligned}
            ||g(\hat{x}+\delta)-g(\hat{x})||&\leq\frac{1}{2}\frac{\tau }{\min\{||u|||u\in U(\hat{x},\delta)\}} ||\delta||\\&\leq\frac{1}{2}\frac{\tau }{|||\hat{x}||-||\delta|||}||\delta||,
    \end{aligned}
    \end{equation*}
    where $U(\hat{x},\delta)$ is a $l_2$-ball of $\hat{x}$ with radius $\delta$.   
    
    When
    $||\delta||\leq(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|})||\hat{x}||<||\hat{x}||$, we have
    \begin{equation*}
    \begin{aligned}
        |g(\hat{x}+\delta)-g(\hat{x})|&=||g(\hat{x}+\delta)-g(\hat{x})||\\& \leq\frac{\tau }{2\left(\frac{||\hat{x}||}{||\delta||}-1\right)}\\
        &\leq\frac{\tau }{2\left(\frac{\tau +2|g(\hat{x})-\Gamma|}{2|g(\hat{x})-\Gamma|}-1\right)}\\
        &\leq|g(\hat{x})-\Gamma|=g(\hat{x})-\Gamma.
    \end{aligned}
    \end{equation*}
    Then,
    \begin{equation*}
    \begin{aligned}
        g(\hat{x}+\delta)\geq|g(\hat{x})|-|g(\hat{x}+\delta)-g(\hat{x})|
        \geq g(\hat{x})- |g(\hat{x})-\Gamma|\geq \Gamma,
    \end{aligned}
    \end{equation*}
    which concludes the proof.
\end{proof}

% \noindent\textit{Proof Sketch.} 
% We prove the above theorem by applying Lipschitz continuity over $g(\hat{x})$. \filter($\cdot$) is the composition of the softmax function and the scaled cosine similarity over the embeddings, where both functions are Lipschitz continuous when $||\hat{x}||>0$. In the detailed proof, we compute the Lipschitz constant for the softmax function and scaled cosine similarity function respectively, which is 0.25 and $\frac{\tau}{||\hat{x}||}$. Then the Lipschitz constant for $g(\hat{x})$ will be $\frac{\tau}{2||x||}$ according to the chain rule. Finally, using the triangle inequality on $|g(\hat{x})-g(\hat{x}+\delta)|$, and plugging the bound in to the inequality, we get $g(\hat{x}+\delta)\geq \Gamma$.
% We present the full proof, empirically evaluate this bound on different concepts, and discuss its practical implications in \autoref{sec:bound}.
The proof says that when the noise does not exceed a certain bound, which is a fraction of $x$, \method is able to predict the noisy samples the same as the original samples. 
We then empirically evaluate this bound on different concepts, and discuss its practical implications in \begin{submission}
Appendix in our full version~\cite{das2024espresso}.    
\end{submission}
\begin{arxiv}  
\autoref{sec:bound}.
\end{arxiv}
We discuss that \method is likely more robust in practice as our certified robustness bound is loose. We leave improving the bound as future work.

% We discuss extending the bound to prompt space in \autoref{sec:future}.

\subsection{Other Discussions}

\noindent\textbf{Addressing Future Attacks.} Recall that \method, fine-tuned using Equation~\ref{eq:ft1} and~\ref{eq:ft2}, maintains high robustness across all evaluated concepts. 
The design of new attacks which can preserve unacceptable concepts while evading \method is an open problem. For additional robustness against new attacks, in addition to Equation~\ref{eq:ft1} and~\ref{eq:ft2}, we can use the objective function for adversarial training:
\[\mathcal{L}_{\text{adv}}(\dtestadv)= - \frac{1}{N} \sum_{j = 1}^N \log \frac{\exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(\cunacc))/ \tau)}{\sum_{k \in \{a,u\}} \exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(c_k))/ \tau)}\]
where $\mathcal{D}_{adv} = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$. Assuming $\imgadv$ evades \method, we optimize $\phi_p$ and $\phi_x$, such that $\phi_p(\imgadv_j)$ is closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$. 
% This loss would be added to Equation~\ref{eq:ft1} and~\ref{eq:ft2}. 
Empirical evaluation of adversarially-trained \method is left as future work.


% \noindent\textbf{Extending the Theoretical Bound to Prompts.} 
% % Although \adv cannot modify text embeddings in practice, analyzing robustness in the CLIP embedding space is valuable as recent works have shown that small changes in the text embeddings of prompts, allow for fine-grained control over their generated images~\cite{yu2024uncovering, kawar2023imagic}. 
% To extend our theoretical bounds in Theorem~\ref{thm.1} to the prompt space,
% we assume Lipschitz continuity, commonly used in ML~\cite{bousquet2002stability}, certified robustness~\cite{li2023sok}, and more recently in the context of \tti models~\cite{chen2024your}.
% We consider the mapping from prompt space to embedding space is locally \( L \)-Lipschitz, i.e., the function \( \phi_x(f(\text{\prompt})) \) satisfies the following condition:

% For each prompt \(\text{\prompt}\), there exists a \(\delta_{\text{\prompt}} > 0\) such that
% $
% ||\phi_x(f(\text{\prompt})) - \phi_x(f(\text{\prompt} + \delta_{\text{\prompt}}))|| \leq L ||\delta_{\text{\prompt}}||.
% $

% Then, the inequality in Equation~\ref{eq:bound} can be related to the prompt space by a scalar factor \(\frac{1}{L}\). 
% Therefore, when \(\|\delta_{\text{\prompt}}\| \leq \frac{1}{L} \|\delta\|\), where \(\|\delta\|\) satisfies inequality in Equation~\ref{eq:bound}, the difference in embedding space will be bounded by \(\|\delta\|\), and CLIP remains robust.


% \subsection{Applications and Extensions to \method}\label{sec:extensions}
\noindent\textbf{Systematic Generation of Acceptable Concepts.} Given a $\cunacc$, candidates for $\cacc$ can be generated using a thesaurus API~\footnote{https://dictionaryapi.com/}. For Group-1 concepts, antonyms of $\cunacc$ are used, while synonyms are considered for others. However, this may not apply to proper nouns, which may be missing from the thesaurus.

\noindent\textbf{Classification of Acceptable Images closer to Decision Boundary.} Acceptable images close to the decision boundary of a filtering \crt{s} can mistakenly be blocked, causing a false positive. However, we argue that this is different than \ref{utility}, which is meant to measure the effect of \method on the \emph{typical} query distributions that a \tti model is likely to encounter in practice (e.g., COCO dataset used in our evaluation).
Evaluation of such acceptable images is missing in the literature and left for future work.

\noindent\textbf{Generalization to Other Concepts.} Our evaluation across 11 concepts aimed to assess \method's performance on different concept types (Group 1 vs. 2 vs. 3). Initial results suggested updating the \method objective for Group 1 concepts (\autoref{eq:ft2}) compared to Groups 2 and 3 (\autoref{eq:ft1}). We expect new concepts within the same group to behave similarly. Understanding the properties of concepts resulting in different behaviors is left as future work.

\noindent\textbf{Filtering Multiple Concepts.} UCE~\cite{gandikota2023unified} and Moderator~\cite{wang2024moderator} remove multiple concepts simultaneously.
\method can be extended by including multiple concepts simultaneously as well. Specifically, for \method in Equation~\ref{eq:att}, instead of specifying $\cunacc$ and $\cacc$ for a single concept, we can include $\cunacc$ and $\cacc$ for multiple concepts as a list. This is a simple configuration change compared to other filters which require retraining (e.g.,~\cite{unsafeDiff}). 
% Since none of the prior filtering \crt{s} evaluate multiple $\cunacc$, 
We leave this as future work.
% \change{Tried to add comment; didn't work so here it is: we said that none of prior crts evaluate against multiple concepts but cite gandikota as 1 crt that does, should we say "no other" prior crts?}. 

% \noindent\textbf{Filtering Artistic Styles.} 
% None of the prior filtering \crt{s} consider any copyrighted content and focus on only \emph{inapproriate Group-1 concepts}. 
% \method is the first filtering \crt which is applicable to concepts which are copyright-infringing (Group-2) or involve unauthorized use of personalized images (Group-3).
% Prior fine-tuning \crt{s} have considered removing artistic styles (e.g., painting in the style of Monet or Van Gogh) as copyrighted content~\cite{kumari2023ablating,gandikota2023erasing}.
% However, we observed that \method does not differentiate between images with and without artistic styles very well. Specifically, \emph{Monet painting} as $\cunacc$ and \emph{painting} as $\cacc$, are very similar for \method, thus reducing its effectiveness. We leave the optimization of \method to account for artistic styles as future work.

\noindent\textbf{Applicability to other \tti Models.} Fine-tuning \crt{s} are specific to particular stable diffusion models due to their tailored optimizations for \tti models. In contrast, filtering \crt{s} offer versatility as they can be applicable to any \tti model. 
Filters analyze only the generated image and the list of concepts, independent of the \tti model. 
And fine-tuning the filter using data from \tti model, as we do for \method, can satisfy \ref{effective} and \ref{utility}. 
This allows us to have a filter that will work with \tti models in different domains (e.g., anime images).
Explicit evaluation of \method for different \tti models is deferred to future work.


\noindent\textbf{Efficiency of \crt{s}.}
We report the execution time for fine-tuning or training the \crt{s} (average across ten runs) on a single NVIDIA A100 GPU (Table~\ref{tab:efficiency}). For related work, the hyperparameter configuration for fine-tuning/training is the same as specified by their respective paper to satisfy effectiveness and utility.

\input{tables/tab_efficiency}

We see that \method is reasonably fast to train.
For fine-tuning \crt{s}, inference time is identical to using the baseline SD v1.4 because they do not add any additional components to the \tti generation process. The inference time for filtering \crt{s} is marginally higher (+0.01\%) than the baseline (of only the image generation time taken by the \tti model). % as it includes the inference time from both the \tti model and the filter.

\begin{arxiv}
\subsection{Summary}
    
% \noindent\textbf{Summary.} 
Removing unacceptable concepts from \tti models is crucial, but no prior \crt{s} simultaneously meet all three requirements: preventing unacceptable concepts, preserving utility on other concepts, and ensuring robustness against evasion. We propose \method, the \emph{first} robust \underline{co}ncept \underline{fi}ltering \crt which provides a better trade-off among the three requirements compared to prior state-of-the-art \crt{s}.
\end{arxiv}

==> generative-concept-removal/figures/fig_adversarial.tex <==
\begin{table}[htb]
\caption{(Column 1) Adversarial image ($\imgadv$) using PGD~\cite{MadryPgd} against \method, (Column 2) adversarial prompt ($\advprompt$) generated from $\imgadv$ using PEZ~\cite{wen2023hard}, and (Column 3) image generated by SDv1.4 \tti model using $\advprompt$ as input.}
\label{tab:framework}
% \begin{center}
\centering
\footnotesize
\begin{tabular}{|l|p{2cm}|p{2cm}|p{2cm}|}
\hline 
{\bf Concept} & {\bf Adversarial Image ($\imgadv$)} & {\bf Adversarial Prompt ($\advprompt$)} & {\bf Image Generated from $\advprompt$} \\
\hline     

\textbf{Nudity} 
&
\includegraphics[width=0.20\columnwidth]{figures/adversarial_images/nudity_yes.png}
& \vspace{-1.5cm}``artsy wbo venus moc bday oilandgoddess thru cropped endurindiefilm cropped r underetal <copyright sign>'' & 
\includegraphics[width=0.20\columnwidth]{figures/adversarial_images/nudity_no.png}
\\
\hline

\textbf{Nemo}
&
\includegraphics[width=0.20\columnwidth]{figures/adversarial_images/nemo_yes.png}
& \vspace{-1.5cm}``moma fishy pet <heart emoji> constrafrm orange optimistic soaking …… vacancy trippy troubles groovy averages \~!'' & 
\includegraphics[width=0.20\columnwidth]{figures/adversarial_images/nemo_no.png}
\\
\hline


\textbf{Elon Musk}
&
\includegraphics[width=0.20\columnwidth]{figures/adversarial_images/musk_yes.png}
& \vspace{-1.5cm}``poet moderstare rested wakeupamerica (" blurred vaportide driverless <smiley emoji> broker celebrated mandelclap'' & 
\includegraphics[width=0.20\columnwidth]{figures/adversarial_images/musk_no.png}
\\
\hline
\end{tabular}
% \end{center}
\label{fig:adversarial_images}
\end{table}

==> generative-concept-removal/figures/fig_architecture.tex <==
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\tikzstyle{defense} = [rectangle,  minimum width=1.4cm, minimum height=0.5cm, text centered, draw=black, fill=mynicered!30]
\tikzstyle{risk} = [rectangle,  minimum width=1.4cm, minimum height=0.5cm, text centered, draw=black]
\tikzstyle{entity} = [rectangle, minimum width=1.4cm, minimum height=0.5cm, text centered, draw=black]
\tikzstyle{databl} = [rectangle,  minimum width=1cm, minimum height=0.5cm, text centered, draw=black, fill=green!30]


\begin{figure*}[!htb]
\centering
\begin{tikzpicture}


\node (clip) [risk, align=center] {\footnotesize \textbf{CLIP Encoder}\\ (\textbf{\te})};
\node (diffmod) [risk, right of=clip, xshift=1.5cm, align=center] {\footnotesize \textbf{Diffusion Model}\\ (\textbf{\dm})};

\draw[->, ultra thick] (clip.east) -- (diffmod.west);

\begin{scope}[on background layer]
    \node (model) [fit=(clip) (diffmod), rounded corners, draw=black, dashed, inner sep=.2cm, label={above:\textbf{Text-to-Image (\tti) model ($\target$)}}] {};
\end{scope}

\node [left of = clip,align=center, rectangle, rounded corners, draw=black, xshift=-1.5cm, yshift=0.5cm] (prompt) {\footnotesize \textbf{Textual}\\\footnotesize \textbf{Prompts} \textbf{\prompt}};
\draw[->, ultra thick] (prompt.east) -- (model.west);

\node [right of = diffmod,align=center, rectangle, rounded corners, draw=black, xshift=1.5cm] (imageclean) {\footnotesize \textbf{Image \imgclean}\\ \footnotesize (\imgacc or \imgunacc)};

\node (filter) [entity, align=center, right of=model, xshift=4.75cm] {\footnotesize \textbf{Filter \filter}};
\draw[->, ultra thick] (imageclean.east) -- (filter.west);
\draw[->, ultra thick] (model.east) -- (imageclean.west);

\node [right of = filter,align=center, yshift=-0.75cm, xshift=1.5cm, minimum width=1cm] (safe) {\footnotesize \textbf{Acceptable}};
\node [right of = filter,align=center, yshift=0.75cm, xshift=1.5cm] (notsafe) {\footnotesize \textbf{Unacceptable}};
\draw[->, ultra thick] (filter.east) -- ([xshift=-0.7cm]notsafe.south);
\draw[->, ultra thick] (filter.east) -- ([xshift=-0.7cm]safe.north);


\node [below of = prompt,align=center, rectangle, rounded corners, draw=black, fill=mynicered!30] (advprompt) {\footnotesize \textbf{Adversarial}\\\footnotesize \textbf{Prompts} \textbf{$\advprompt$}};
\node (inv) [defense, left of =advprompt, align=center, xshift=-1cm] {\footnotesize \textbf{\adv}};
% \node (hand) [defense, below of=diffmod, align=center, yshift=-0.5cm, xshift=-0.2cm] {\footnotesize \textbf{Handcrafted}\\ \footnotesize\textbf{Attack}};
% \begin{scope}[on background layer]
%     \node (attacks) [fit=(inv) (hand), fill= red!15, rounded corners, draw=black, dashed, inner sep=.2cm, label={below:\textbf{Circumvention Techniques}}] {};
% \end{scope}
\draw[->, ultra thick, mynicered, solid] (inv.east) -- (advprompt.west);

% \node [below of = imageclean,align=center, draw=black, fill=red!30] (imgadv) {\footnotesize \textbf{Adv. Image}\\ \footnotesize \textbf{\imgunacc'}};
\draw[->, ultra thick, mynicered] (advprompt.east) -- ([yshift=-0.1cm]model.west);
% \draw[->, ultra thick, mynicered] (model.east) -- (imgadv.west);
% \draw[->, ultra thick, mynicered] (imgadv.east) -- node [below, align=center, xshift=0.5cm] {} ([yshift=-0.1cm]filter.west);

\draw[->, ultra thick, mynicered] (filter.south) |- ++(0, -1cm) -| (inv.south) node[midway,above, xshift=6cm] {\footnotesize Filter's Loss for Attack};

\end{tikzpicture}
% }
\caption{\underline{Overview of Filtering based \crt{s}:} $\target$ generates \imgclean from \prompt which is passed to Filter which classifies \imgclean as acceptable (if \imgacc) or not (if \imgacc). \adv generate an adversarial prompt $\advprompt$ to force Filter to misclassify generated image \imgunacc' as acceptable. Rectangles with rounded corners indicate data component, while sharp corners indicate software component (also includes \adv). \textcolor{mynicered}{Red} indicates information flow and components for the attacks.}
\label{fig:overview}
\end{figure*}

==> generative-concept-removal/figures/fig_certified.tex <==
\begin{figure}[htb]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/group_1.pdf}
        \caption{Group-1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/group_2.pdf}
        \caption{Group-2}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/group_3.pdf}
        \caption{Group-3}
    \end{subfigure}
    \caption{Certified accuracy of \method{} vs. adversarial noise $\delta$, for a strong \adv{} with access to embeddings of generated images.}
    \label{fig:certified}
\end{figure}


==> generative-concept-removal/figures/fig_images.tex <==
\begin{figure}[!htb]
    \centering
    \begin{minipage}[b]{1\linewidth}
    \centering
    \subfigure[False Positive (Group-1)]{
    \includegraphics[width=0.40\linewidth]{figures/adversarial_images/nudity_yes.png}
    }%
    \hspace{0.75cm}
    \subfigure[True Positive (Group-1)]{\includegraphics[width=0.40\linewidth]{figures/adversarial_images/nudity_no.png}}
    \end{minipage}\\
    \begin{minipage}[b]{1\linewidth}
    \centering
    \subfigure[False Positive (Group-2)]{
    \includegraphics[width=0.40\linewidth]{figures/adversarial_images/grumpy_yes.png}
    }%
    \hspace{0.75cm}
    \subfigure[True Positive (Group-2)]{\includegraphics[width=0.40\linewidth]{figures/adversarial_images/grumpy_no.png}}
    \end{minipage}\\
    \begin{minipage}[b]{1\linewidth}
    \centering
    \subfigure[False Positive (Group-3)]{
    \includegraphics[width=0.40\linewidth]{figures/adversarial_images/swift_yes.png}
    }%
    \hspace{0.75cm}
    \subfigure[True Positive (Group-3)]{\includegraphics[width=0.40\linewidth]{figures/adversarial_images/swift_no.png}}
    \end{minipage}
    \caption{Examples of $\imgadv$ where images on the left include $\cunacc$ but can be successfully detected by \method while $\imgadv$ on the right can evade \method but does not include $\cunacc$.}
    \label{fig:images}
\end{figure}


==> generative-concept-removal/figures/fig_pipeline.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/espresso_gen_pipeline.pdf}
    % \underline{\textbf{Step 1}} $\rightarrow$ Identify some possible $\cacc$ for each $\cunacc$. 
    % \underline{\textbf{Step 2}} $\rightarrow$ Generate datasets containing prompts and corresponding images for both $\cacc$ and $\cunacc$ for train ($\dtrain$), test ($\mathcal{D}_{te}$), and validation ($\mathcal{D}_{val}$). 
    % \underline{\textbf{Step 3}} $\rightarrow$ Use $\dtrain$ to fine-tune \tti model with \crt{s} and train the filtering classifier. 
    % \underline{\textbf{Step 4}} $\rightarrow$ Evaluate effectiveness and utility on $\mathcal{D}_{val}$ and choose the best candidate for $\cacc$.
    % \underline{\textbf{Step 5}} $\rightarrow$ Evaluate using $\mathcal{D}_{te}$: for effectiveness (\ref{effective}), use CLIP accuracy or FNR on unacceptable prompts ($\dtestunacc$), utility (\ref{utility}) on acceptable prompts ($\dtestacc$), and robustness (\ref{robust}) using CLIP score or FPR on $\dtestadv$ which includes $\advprompt$ constructed using attacks on $\dtestunacc$. 
    \caption{\textbf{Overview of pipeline for evaluating \crt{s}.} Prompts, images and arrows for unacceptable (acceptable) in \colorbox{red!20}{red} (\colorbox{green!20}{green}).}
    \label{fig:pipeline}
\end{figure*}

==> generative-concept-removal/figures/fig_radar_filter.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/radar_filter.pdf}
    \caption{\method has a better trade-off than \unsafediff filter.}
    \label{fig:radarsFilt}
\end{figure}


==> generative-concept-removal/figures/fig_radar_ft.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/radar_ft.pdf}
    \caption{\method is better than other fine-tuning \crt{s}.}
    \label{fig:radarsFT}
\end{figure}



==> generative-concept-removal/figures/fig_robustness_diagram.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1.5\columnwidth]{figures/espresso_robustness_diagram_cropped.pdf}
    \caption{The perturbation required to evade \method (right) is greater than that required for the SD filter (left) due to the use of both unacceptable and acceptable concepts for the threshold. Generated images lose their unacceptable quality at large perturbations.}
    \label{fig:espresso_robustness_diagram}
\end{figure}

==> generative-concept-removal/old_versions/01abstract.tex <==
Diffusion based text-to-image (\tti) models generate high fidelity images for given textual prompts. They are trained on large datasets scraped from the Internet, potentially containing \textit{unacceptable concepts} (e.g., copyright infringing or unsafe). Retraining \tti models after filtering out unacceptable concepts in the training data is inefficient and degrades utility. Hence, we need concept removal techniques (\crt{s}) which are
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \textit{effective} in preventing the generation of images with unacceptable concepts
\item \textit{utility-preserving} on acceptable concepts, and 
\item \textit{robust} against evasion with adversarial prompts.
\end{enumerate*}
None of the prior \crt{s} satisfy all these requirements simultaneously. 

We introduce \method, the first \emph{\textbf{robust} \underline{co}ncept \underline{fi}lter} based on Contrastive Language-Image Pre-Training (CLIP). 
We configure CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts.
This simple change significantly improves robustness by restricting the adversary to add noise \emph{only} along the vector connecting the embeddings of unacceptable and acceptable concepts.
Further, fine-tuning \method to separate embeddings of unacceptable and acceptable concepts, while preserving their pairing with image embeddings, improves utility. 
We evaluate \method on eleven concepts to show that it is more \emph{effective} (CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) and more \emph{robust} (CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) than prior \crt{s}, while retaining \emph{utility} (normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]). 
Finally, we present theoretical bounds for certified robustness of \method against adversarial prompts, and an empirical analysis.


==> generative-concept-removal/old_versions/1introduction.tex <==
\section{Introduction}\label{sec:introduction}


Diffusion based text-to-image (\tti) models have demonstrated a remarkable ability to generate high quality images from textual prompts~\cite{stable-diffusion,Rombach_2022_CVPR,ramesh2021dalle}.
These models are trained on large datasets of unfiltered content from the Internet~\cite{radford2021learning,schuhmann2022laion}. 
Due to their large capacity, \tti models memorize specific \emph{concepts}, as seen in the generated images~\cite{Korn_2023,somepalli2022diffusion,carlini2023extracting}. 
Some of these concepts, may be \emph{unacceptable} for various reasons, such as copyright infringement (e.g., a movie character or celebrity), or inappropriateness (e.g., ``nudity'' or ``violence'')~\cite{gandikota2023erasing,schramowski2022safe,heng2023selective}. 
Retraining \tti models after filtering out unacceptable concepts is inefficient, only partially effective~\cite{li2024safegen, huggingfaceStabilityaistablediffusion21Hugging}, and compromises utility~\cite{gandikota2023erasing}.
Hence, there is a need for \emph{concept removal techniques} (\crt{s}) to minimize unacceptable concepts in  generated images.


Ideally, \crt{s} should be \emph{effective} in reducing the generation of unacceptable concepts while preserving the \emph{utility} on all others, and \emph{robust} to evasion with adversarial prompts.  
As we show in Section~\ref{sec:evaluation}, none of the existing \crt{s} \emph{simultaneously} satisfy these requirements:
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \emph{filtering \crt{s}}, which detect unacceptable concepts, lack robustness~(\cite{rando2022redteaming} and Section~\ref{sec:filterEval})
\item \emph{fine-tuning \crt{s}} which modify \tti models, trade-off effectiveness and utility~\cite{gandikota2023erasing,kumari2023ablating,heng2023selective,schramowski2022safe}, and may lack robustness~\cite{Tsai2023RingABellHR, wen2023hard, pham2023circumventing, yang2023sneakyprompt}.
\end{enumerate*}
%Moreover, none of these \crt{s} are robust against adversarial prompts, i.e., adversarially modified prompts which force \tti{s} to generate unacceptable concepts.
Designing a \crt meeting all the requirements is an open problem. Our goal is to design such a \crt.

We opt to use a filter as it will not alter the \tti model, thus reducing its impact on utility. We construct our filter using the Contrastive Language-Image Pre-Training (CLIP)~\cite{radford2021learning}, an essential component of \tti models. CLIP co-locates the embeddings of textual prompts and their corresponding images within a unified embedding space where similar concepts are closer.
CLIP is pre-trained on a vast dataset which encodes a broad spectrum of concepts~\cite{radford2021learning}, making it a versatile choice for a filter, unlike specialized classifiers (e.g.,~\cite{unsafeDiff}).
However, relying on CLIP to identify unacceptable images by solely measuring the distance between the embeddings of a generated image, and an unacceptable concept, was shown not to be robust (~\cite{rando2022redteaming}). Subsequently, several prior works have identified filtering as a viable direction which needs further exploration~\cite{rando2022redteaming,li2024safegen}.

% \input{figures/fig_robustness_diagram}
% \change{Robustness diagram: figures/fig\_robustness\_diagram}

We present a \textbf{robust} (CLIP-based) \underline{co}ntent \underline{fi}lter, \method, by configuring CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts. 
% We present a \textbf{robust} \textbf{co}ntent \textbf{fi}lter, \method, that identifies unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both acceptable and unacceptable concepts}. 
% \change{This simple change in configuration translates to projecting} the image embedding onto the vector connecting the text embeddings of acceptable and unacceptable concepts. 
This simple change makes it harder to generate effective adversarial prompts: the adversary is restricted to adding noise in the direction of the acceptable concept. 
%adversarial prompts must generate images far enough from unacceptable concepts to evade detection yet close enough to retain the unacceptable concepts.
To restore any drop in utility stemming from this change, we fine-tune \method to increase the separation between the text embeddings of unacceptable and acceptable concepts, while maintaining their pairing with their corresponding image embeddings. 
This fine-tuning approach is further supported by fine-tuning \crt{s} which show that such an optimization leads to better utility~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}.
We claim the following main contributions: we present
\begin{enumerate}[leftmargin=*,wide,  labelindent=0pt]
\item \method\footnote{We will open-source the code upon publication.}, the \textbf{first robust} (CLIP-based) \underline{co}ntent \underline{fi}lter which identifies unacceptable concepts in generated images by measuring the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts (Section~\ref{sec:approach}),
\item a comprehensive comparative evaluation (Section~\ref{sec:setup}) of the fine-tuned variant of \method with six state-of-the-art fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective} (CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) and \textbf{more robust} (CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) than prior \crt{s}, while \textbf{retaining utility} (normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]).
%showing that \method is \textbf{effective} ($\sim$5\% CLIP accuracy  on unacceptable concepts), \textbf{utility-preserving} ($\sim$93\% 
% normalized CLIP score on acceptable concepts), and \textbf{robust} ($\sim$4\% CLIP accuracy of  on adversarial prompts) %of unacceptable concepts) 
(Section~\ref{sec:evaluation}), and
\item %the \textbf{first} approach towards \textbf{certifiable robustness of \crt{s}} by exploring 
theoretical bounds for \textbf{certifying the robustness} of \method, assuming a hypothetically strong adversary, empirical analysis of these bounds, and making the case that \method is likely to be more robust in practice. (Section~\ref{sec:bound}). 
\end{enumerate}

==> generative-concept-removal/old_versions/2background.tex <==
\section{Background}\label{sec:background}

We describe \tti models (Section~\ref{back-diffusion}), different \crt{s} (Section~\ref{back-conceptrem}), and attacks against them (Section~\ref{back-attacks}).

\subsection{Diffusion based \tti Models}\label{back-diffusion}

A diffusion based \tti model is a function $\target: \prompt \rightarrow \imgclean$ which generates an image $\imgclean$ for a given a textual prompt $\prompt$. It comprises two key components: an encoder (\te) which is used to incorporate the textual prompt in the image generation process, and a diffusion model (\dm) which is responsible for the generation of the image.

A popular encoder is CLIP, trained on a large dataset of image-text pairs, to map the embeddings of images and their corresponding text closer together in a joint text-image embedding space~\cite{radford2021learning}.
Given $N$ images $\{\imgclean_j\}_{j=1}^N$ and their corresponding text prompts $\{\prompt_j\}_{j=1}^{N}$, the training data is $\mathcal{D} = \{(\imgclean_j, \prompt_j)\}_{j=1}^N$. 

CLIP is trained to maximize the cosine similarity between the embeddings of a prompt $\prompt_j$ and its corresponding image $\imgclean_j$ while minimizing the similarity between $\prompt_j$ and any other $\imgclean_k$ for a $k \ne j$.
We denote the cosine similarity as \text{cos}($\phi_p(\prompt_j), \phi_x(\imgclean_j))$, where $\phi_x(\imgclean_j)$ is the CLIP image embedding of the image $\imgclean_j$, and $\phi_p(\prompt_j)$ is the CLIP text embedding of the prompt $\prompt_j$.
To achieve this, CLIP is trained using a contrastive loss function~\cite{yang2023robust,oord2019representation,lee2021soundguided}: \[\mathcal{L}_{\text{Con}}(\mathcal{D}) = - \frac{1}{N} \sum_{j=1}^{N} \log \frac{\exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_j))/ \tau)}{\sum_{k=1}^{N} \exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_k))/ \tau)}\] where $\tau$ is the temperature parameter for scaling the predictions~\cite{radford2021learning, ModalityGap}. 
 


Given access to a pre-trained encoder \te, the actual images in \tti models are generated by a diffusion model, \dm, parameterized by $\theta$.
During training of \dm, Gaussian noise is added to an initial image $x_0$ for $T$ time steps to produce $x_T$, in a process known as the \emph{forward diffusion process}. The noise is then iteratively removed to approximate the initial image $\tilde{x_0}$ in the \emph{reverse diffusion process}.
During inference, the reverse diffusion process generates an image from noise.
Further, \dm can be conditioned with a textual prompt \prompt to guide the generation of $\tilde{x_0}$ to match the description in \prompt. After generating $\phi_p(\prompt)$, %from \te, 
\dm is trained by minimizing the following loss function: $\mathcal{L} = \mathbb{E}_{\epsilon, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(\imgclean_t,\phi_p(\prompt),t)||_2^2]$ for each time step $t$, and random Gaussian noise $\epsilon \sim \mathcal{N}(0,1)$.

Several prominent \tti models (e.g., Stable Diffusion v1.4 (SDv1.4)) improve the efficiency of the diffusion process by conducting it in the embedding space of a variational autoencoder (VAE), rather than on images \cite{stable-diffusion}. For a VAE decoder $\mathit{D}$, VAE encoder $\mathcal{E}$, and $z_t \in \mathcal{E}(\imgclean)$ as the latent representation of $\imgclean$ in the VAE's latent space, \dm is trained by minimizing the following objective: \\
$\mathcal{L} = \mathbb{E}_{\epsilon, z_t, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(z_t,\phi_p(\prompt),t)||_2^2]$ where $\epsilon \sim \mathcal{N}(0,1)$. The final image is generated from the approximation, $\tilde{z_0}$, by passing it through $\mathit{D}$: $\tilde{x_0} = \mathit{D}(\tilde{z_0})$.  Table~\ref{tab:notations} in Appendix~\ref{app:notations} summarizes frequently used notations.

 




\subsection{Concept Removal Techniques}\label{back-conceptrem}

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance?--- We use the same approach for selecting acceptable concepts as Kumari et. al.~\cite{kumari2023ablating}for group 2 and group 3 concepts. For these groups, the acceptable concept is a superset of the unacceptable concept. For example, the sex of a celebrity is the acceptable concept for a celebrity. For group 1, there is no clear definition of a superset (eg. the superset of \emph{nude} is unclear). Logically, the acceptable concept is the opposite of the unacceptable concept in this case since it is clearly defined. - SHOULD MOVE THIS EXPLANATION ELSEWHERE}

The textual phrase for an acceptable concept is $\cacc$, and for an unacceptable concept is $\cunacc$. 
For a given $\cunacc$, $\cacc$ is either the opposite (e.g., $\cunacc$ = \emph{violence} vs. $\cacc$ = \emph{peaceful}) or a general category of a specific character/object/person (e.g., $\cunacc$ = \emph{R2D2} vs. $\cacc$ = \emph{robot}). We discuss the selection of $\cacc$ for a given $\cunacc$ in Section~\ref{sec:concepts}.
An image $\imgclean$ generated from a \tti model may either contain an unacceptable concept (referred to as $\imgunacc$) or an acceptable one (referred to as $\imgacc$). Similarly, a text prompt $\prompt$ may contain a phrase for an acceptable concept ($\promptacc$) or an unacceptable concept ($\promptuacc$). An example of an unacceptable prompt $\promptuacc$ containing an unacceptable concept $\cunacc$ = \emph{Captain Marvel}, is ``\emph{Captain Marvel} soaring through the sky''. \crt{s} seek to thwart the generation of $\imgunacc$ by either fine-tuning the \tti model to suppress $\imgunacc$, or using a classifier as a filter to detect $\imgunacc$, and serve a replacement image instead. 
%
We first present six state-of-the-art fine-tuning \crt{s}:

\noindent\textbf{Concept Ablation (\ca)~\cite{kumari2023ablating}} fine-tunes the \tti model to minimize the KL divergence between the model's output for $\promptuacc$ and $\promptacc$ to force the generation of \imgacc instead of \imgunacc. Formally, they optimize the following objective function: 
 % \text{argmin}_\theta 
\[\begin{split}
\footnotesize
   \mathcal{L}_{\ca} =  \mathbb{E}_{\epsilon, z_t, \cunacc, \cacc, t}[w_t||\epsilon_\theta(z_t,\phi_p(\promptacc),t).sg() \\
    - \epsilon_\theta(z_t,\phi_p(\promptuacc),t)||_2^2]
\end{split}\]
where $\epsilon \sim \mathcal{N}(0,1)$, $z_t \in \mathcal{E}$, and $w_t$ is a time-dependent weight, and $.sg()$ is the stop-gradient operation.

\noindent\textbf{Forget-Me-Not (\forgetNot)~\cite{zhang2023forgetmenot}} minimizes the activation maps for $\cunacc$ by modifying \dm's cross-attention layers. Further, fine-tuning \dm, instead of just the cross-attention layers, results in degraded utility. 
% That is, given $a_i \in \mathcal{A}_i$, the $i$-th attention map in \dm of \tti, their loss is 
% \[\mathcal{L} = \sum_{a_i \in \mathcal{A}_i}||a_i||\]


\noindent\textbf{Selective Amnesia (\sa)~\cite{heng2023selective}} fine-tunes \tti models by adapting continuous learning techniques (elastic weight consolidation and generative replay) for \tti models to forget a concept. They optimize $\mathbb{P}(\imgclean|\theta^*,\cunacc)$, the probability of generating $\imgclean$ given $\theta^*$ and $\cunacc$, where $\theta^*$ are the frozen parameters of the original \tti model: 
\[
\begin{split}
\footnotesize
    \mathcal{L}_{\sa} = -\mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_f(\cunacc)}[\text{log}\mathbb{P}(\imgclean|\theta^*,\cunacc)] -\lambda\sum_i\frac{M_i}{2}(\theta_i^*-\theta_i)^2\\
     + \mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_r(\cacc)}[\text{log}\mathbb{P}(\imgclean|\theta,\cacc)]
\end{split}
\]
where $M$ is the Fisher information matrix over $\cacc$ and $\cunacc$, $\mathbb{P}_r$ and $\mathbb{P}_f$ are probabilities taken over the distributions of $\cacc$ and $\cunacc$ respectively, and $\lambda$ is a regularization parameter. 



\noindent\textbf{Erased Stable Diffusion (\esd)~\cite{gandikota2023erasing}} fine-tunes the \tti model by modifying the reverse diffusion process to reduce the probability of generating \imgunacc:
\[\begin{split}
\epsilon_\theta(\imgclean_t,\phi_p(\cunacc),t) = \epsilon_{\theta^*}(\imgclean_t, t)
+ \eta(\epsilon_{\theta^*}(\imgclean_t,\phi_p(\cunacc),t)\\-\epsilon_{\theta^*}(\imgclean_t,t))
\end{split}\]
where $\eta > 0$ encourages the noise conditioned on $\cunacc$ to match the unconditioned noise.


\noindent\textbf{Unified Concept Editing (\unifiedCE)~\cite{gandikota2023unified}} fine-tunes the \tti model's cross-attention layers with a language model to minimize the influence of $\cunacc$, while keeping the influence of remaining concepts unchanged. Their optimization is:
% \text{min}_W
\[\begin{split}
    \mathcal{L}_{\unifiedCE} = \sum_{\cunacc \in \mathcal{C}^{u}, \cacc \in \mathcal{C}^{a}}||W\times\cunacc-W^*\times\cacc||_2^2 \\ 
    +  \sum_{c \in S}||W\times c - W^*\times c||_2^2
\end{split}\]
where $W$, $W^*$ are the parameters of the fine-tuned and original \emph{cross-attention layers in \dm}, $\mathcal{C}^{u}$ and $\mathcal{C}^{a}$ are the space of pre-defined unacceptable and acceptable concepts, and $S$ is a set of concepts for which to preserve utility. 

\noindent\textbf{Safe diffusion (\sdd)~\cite{kim2023towards}}
fine-tunes the \tti model by encouraging the diffusion model noise conditioned on $\cunacc$ to match the unconditioned noise, while minimizing the utility drop using the following objective function:
\[\begin{split}
    % \text{argmin}_\theta
    \mathcal{L}_{\sdd} = \mathbb{E}_{\epsilon, z_t, \cunacc, t}[||\epsilon_\theta(z_t,\phi_p(\cunacc),t) 
 - \epsilon_\theta(z_t,t).sg()
    ||_2^2]
\end{split}\]
where $\epsilon \sim \mathcal{N}(0,1)$ and $z_t \in \mathcal{E}(x)$.

\noindent We now describe two filtering \crt{s}:

\noindent\textbf{Stable Diffusion Filter (SD-Filter)~\cite{radford2021learning}} is black-box and the design of the filter is not publicly available. However, Rando et. al.~\cite{rando2022redteaming} hypothesize that it involves computing the cosine similarity between the embeddings of a generated image, $\imgclean$, and a pre-defined set of $\cunacc$. If the cosine similarity is greater than some threshold ($\Gamma$), then $\imgclean$ has $\cunacc$. Formally, their filter $\filter_{SD}$ can be described as
\[ \filter_{SD}(\imgclean) = \begin{cases} 
      1 & \text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) > \Gamma \\
      0 & \text{otherwise}
   \end{cases}
\]
where $\text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) = \overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\cunacc)}$, and $\overline{\cdot}$ denotes normalization. Here $\filter_{SD}(\imgclean) = 0$ indicates \imgacc and $\filter_{SD}(\imgclean) = 1$ indicates \imgunacc. Note that $\Gamma$ varies with $\cunacc$. 


\noindent\textbf{Unsafe Diffusion (\unsafediff)~\cite{unsafeDiff}} is the current state-of-the-art filtering \crt and outperforms SD-Filter~\cite{unsafeDiff}. \unsafediff trains a multi-headed neural network classifier on top of CLIP to identify $\imgunacc$ where each head classifies different $\cunacc$: \emph{nudity, violence, disturbing, hateful}, and \emph{political}. Their objective is given as $\filter_{\unsafediff}(\imgclean) = \text{MLP}(\phi_x(\imgclean))$ where MLP is a multi-layer perceptron, and $\filter_{\unsafediff} \in \{0,1\}$.


\subsection{Evading Concept Removal Techniques}\label{back-attacks} 

An adversary (\adv) may construct adversarial prompts ($\advprompt$) to evade \crt{s} and force the \tti model to generate unacceptable images. We denote a dataset containing adversarial prompts and their corresponding images ($\imgadv$) as $\dtestadv = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$ where ideally $\imgadv$ will contain $\cunacc$.
\adv is assumed to account for the target \tti model \target, using a \crt. A dumb \adv who does not account for this is \emph{na\"{i}ve}. 

\adv's objective is to construct $\advprompt$ which can force a \tti model to output images with $\cunacc$ while being semantically closer to acceptable prompts so that $\imgadv$ is incorrectly identified as acceptable while triggering the generation of unacceptable images.
The existing attacks formulate the construction of $\advprompt$ as an optimization problem using some reference $\imgunacc$ (or the difference between $\promptacc$ and $\promptuacc$) as the ground truth. Different attacks vary in ways to solve this optimization. We present four state-of-the-art attacks below:

\noindent\textbf{PEZ~\cite{wen2023hard}} constructs $\advprompt$ by identifying text tokens by minimizing: $\mathcal{L}_{PEZ}= 1-\text{cos}(\phi_p(\advprompt),\phi_x(\imgunacc))$. 



\noindent\textbf{RingBell~\cite{Tsai2023RingABellHR}} identifies tokens for $\advprompt$ by first calculating the average difference between the embedding vectors of $\promptuacc$ and $\promptacc$: $\phi_p(\hat{\prompt}) = \frac{1}{N}\sum_{i=1}^N\{\phi_p(\promptuacc_i) - \phi_p(\promptacc_i)\}$ from a set of $N$ prompts. Then, RingBell computes $\advprompt$ by minimizing the distance of its text embedding to ($\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))$, formulated as: $\text{min}_{\advprompt} ||\phi_p(\advprompt) - (\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))||^2$ where $\prompt^{init}$ is an initial unacceptable prompt which is censored by a \crt. They solve this using a genetic algorithm. 
%Further, the optimization relies on a fitness function using mean-squared error: $\mathcal{L}_{RingBell} = \mathcal{L}_{MSE}(\phi_p(\cunacc),\phi_p(\advprompt))$ where $\cunacc$ is a prompt that generates $\imgunacc$ in a \tti model.


\noindent\textbf{SneakyPrompt~\cite{yang2023sneakyprompt}} uses reinforcement learning to construct $\advprompt$ specifically against filtering \crt{s}. Given an initial prompt $\prompt^{init}$, the attack searches for tokens to update $\prompt^{init}$ to form $\advprompt$. The reward function is the cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\advprompt)$. Typically, they use $\promptuacc$ as $\prompt^{init}$ for better effectiveness and faster convergence.

\noindent\textbf{CCE~\cite{pham2023circumventing}} uses textual-inversion to construct $\advprompt$~\cite{gal2022textualinversionimage}. \adv updates CLIP's vocabulary to include a new token ``<s>'' which, when included in $\advprompt$, generates \adv's desired image. To optimize <s>, we find $v$, an embedding for <s>, corresponding to least loss $\mathcal{L}_{CCE}=\mathcal{L}_{MSE}(\epsilon, \epsilon_\theta(z_t,v,t))$, where $\epsilon\sim\mathcal{N}(0,1)$, and $\mathcal{L}_{MSE}$ is the mean-squared-error. 


All of these attacks are na\"{i}ve except for CCE and SneakyPrompt, which account for different fine-tuning \crt{s}. 
In Section~\ref{sec:baseline}, we describe how we modify these na\"{i}ve attacks to account for \crt{s}.

==> generative-concept-removal/old_versions/3problem.tex <==
\section{Problem Statement}\label{sec:problem}


Our goal is to design a \crt which can effectively detect unacceptable concepts in images generated from \tti models. We describe an adversary model, requirements of an ideal \crt, and limitations of prior works according to the requirements.


\noindent\textbf{Adversary Model.} We assume (blackbox) access to a deployed target \tti model ($\target$) to which a client can send an input ($\prompt$) to generate an image ($\imgclean$). Further, $\target$ uses some \crt. The goal of the adversary (\adv) is to force $\target$ to generate $\imgunacc$ despite the presence of a \crt to suppress it.
We give an advantage to \adv by allowing whitebox access to a local identical copy of $\target$ with the \crt for use in designing attacks. This is reasonable as \dm and CLIP are publicly available. For filtering \crt{s}, we assume that \adv has whitebox access to the filter to use its loss function in designing the attacks.

\noindent\textbf{Requirements} An ideal \crt should be:
\begin{enumerate*}[label=\textbf{R\arabic*},leftmargin=*]
\item\label{effective} \textit{Effective} in minimizing the generation of $\imgunacc$;
\item\label{utility} \textit{Utility-preserving}, maintaining the quality of acceptable images (for fine-tuning \crt{s}) or not blocking them (for filtering \crt{s}); and
\item\label{robust} \textit{Robust} to resist evasion with adversarial prompts ($\advprompt$).
\end{enumerate*}



\noindent\textbf{Limitations of Prior Works.} 
%We now briefly discuss the limitations of different types of prior \crt{s} \emph{vis-a-vis} the requirements above. 
In Section~\ref{sec:evaluation}, we empirically show the limitations of prior works by evaluating \ref{effective}, \ref{utility}, and \ref{robust} of different \crt{s}. We provide a brief summary here.
\textit{Fine-tuning \crt{s}} modify $\target$ thereby explicitly creating a trade-off between effectiveness (\ref{effective}) and utility (\ref{utility})~\cite{gandikota2023erasing,kumari2023ablating,zhang2023forgetmenot,heng2023selective,heng2023selective,gandikota2023unified,kim2023towards}.
Further, these \crt{s} do not consider robustness (\ref{robust}) in their design and are susceptible to evasion by \adv with $\advprompt$. 
\textit{Filtering \crt{s}}~\cite{radford2021learning,unsafeDiff} detect unacceptable concepts either in $\prompt$ (aka prompt filter) or in $\imgclean$ and block them (a.k.a image filter). Since, they do not modify $\target$, they can maintain utility without impacting effectiveness. Prior filtering approaches may not be accurate in detecting unacceptable concepts (impacts \ref{effective})~\cite{li2024safegen}.
They can also be easily evaded (harms \ref{robust}) (\cite{rando2022redteaming} and Section~\ref{sec:filterEval}). Further, the current state-of-the-art filter, \unsafediff~\cite{unsafeDiff}, trains specialized classifiers for each concept on substantial data, which limits their generalization to new concepts.


==> generative-concept-removal/old_versions/4approach.tex <==
\section{\method: Robust Filtering CRT}\label{sec:approach}

We present \method, a robust \underline{co}ncept \underline{fi}ltering \crt which aims to satisfy the requirements from Section~\ref{sec:problem} and achieve a better trade-off than prior \crt{s}. 
\method uses a classifier \filter to detect images and filter unacceptable concepts in generated images. Following SDv1.4, on detecting an unacceptable concept, \method generates a replacement image~\cite{radford2021learning, rando2022redteaming}.
We identify CLIP as the natural choice for such a classifier as it is
\begin{enumerate*}[leftmargin=*]
\item pre-trained on a large dataset covering a wide range of concepts, and
\item used across many \tti models, and encodes similar information as seen in them.
\end{enumerate*}
Hence, CLIP is a better choice for a filter than training specialized classifiers for each concept (e.g.,~\cite{unsafeDiff}).

 However, simply using CLIP for \method is not sufficient as seen in Stable Diffusion's filter ($\filter_{SD}$)~\cite{radford2021learning}. 
$\filter_{SD}$ thresholds the cosine similarity between the embeddings of $\imgclean$ and each pre-defined unacceptable concept to identify $\imgunacc$. 
Rando et al.~\cite{rando2022redteaming} design adversarial prompts ($\advprompt$) to evade $\filter_{SD}$. 
Since $\filter_{SD}$ uses only the cosine similarity to $\cunacc$, it gives \adv the freedom to modify the prompt embeddings in \emph{any direction}, while constructing $\advprompt$, to force a misclassification.
%
We address this in \method by (a) configuring CLIP's classification objective for effectiveness and robustness, and (b) fine-tuning to further improve utility. 

\noindent\textbf{Configuring CLIP's Classification Objective.} Instead of using the cosine similarity to only $\cunacc$ as in $\filter_{SD}$, we configure the objective function of \method for filtering $\imgunacc$ by using the cosine similarity to \emph{both} $\cunacc$ and $\cacc$. 
% \change{This makes \adv's goal more difficult as they are forced to optimize $\advprompt$ such that the resulting image embedding is far from $\phi_p(\cunacc)$, \emph{and} close to $\phi_p(\cacc)$, which is an additional stipulation arising from the design of \method.}
Further, jointly optimizing for two embeddings yields better utility as observed in prior fine-tuning \crt{s}~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}. 

Given $\imgclean$, \method checks the cosine similarity of $\phi_x(\imgclean)$ to $\phi_p(\cunacc)$ and $\phi_p(\cacc)$. Formally, we define \method as $\filter(x, \cunacc, \cacc)$
\begin{equation}\label{eq:att}
 = \text{argmax}_{i, i\in{a,u}} \left\{\frac{\text{exp}{(\text{cos}(\phi_x(x),\phi_p(\concept_i)) / \tau)}}{\sum_{j \in \{a,u\}}\text{exp}(\text{cos}(\phi_x(x),\phi_p(\concept_j)) / \tau)}\right\}
\end{equation} 
where $\tau=\frac{1}{100}$ is the default temperature parameter used in CLIP. 
Further, the cosine similarity is equivalent to the scaled Euclidean distance between the embeddings~\cite{ModalityGap}: 
\[(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) = 2-2\overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\concept)}\]
\[\implies \text{cos}(\imgclean, \concept) = -\frac{1}{2}(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) + 1\]
Hence, by using CLIP as a filter, we project the image embeddings onto the vector between $\cunacc$ and $\cacc$ and classify it based on its distance to both.  
%
This simple configuration change in CLIP's classification objective restricts \adv to adding noise only along the low-dimensional vector joining $\cunacc$ and $\cacc$: $\phi_p(\cunacc) - \phi_p(\cacc)$ in the direction of $\cacc$.
This is more challenging for \adv to evade than $\filter_{SD}$, as projecting to a lower-dimensional representation can improve robustness~\cite{pca1,pca2}.
Hence, we conjecture that this can help satisfy \ref{effective} and \ref{robust} (as shown later in Section~\ref{sec:evaluation}).

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance? - ANSWERED}


% \change{Rationale for fine-tuning?}
\noindent\textbf{Fine-tuning.} The above configuration change may impact the utility on some concepts due to the close proximity of some $\cunacc$ and $\cacc$.
To restore any drop in utility, we use fine-tuning. 
We use two different fine-tuning variants depending on the group of concepts.


For the case where $\cunacc$ and $\cacc$ are opposites (e.g., Group-1 concepts where $\cunacc$ = \emph{violence} and $\cacc$ = \emph{peaceful}), the above objective function might have a low correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$. This might result in poor utility. We use following objective function:

\begin{equation}\label{eq:ft2}
    \begin{split}
        \mathcal{L}_{\method} = \alpha_{\text{aa}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{aa}) 
        -\alpha_{\text{ua}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{ua}) \\
        + \alpha_{\text{uu}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{uu})  
        -\alpha_{\text{au}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{au}) \\
        +\alpha_{\text{uu-t}}\mathcal{L}_{MSE}(\phi_p(\mathcal{P}^{u}), \phi_p(\mathcal{P}^{a})) \\
    \end{split}
\end{equation}
where $\mathcal{D}_{aa} = \{(\imgacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{au} = \{(\imgacc_j, \promptuacc_j)\}_{j=1}^N$, \\$\mathcal{D}_{ua} = \{(\imgunacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{uu} = \{(\imgunacc_j, \promptuacc_j)\}_{j=1}^N$, $\mathcal{P}^u = \{\promptuacc_j\}$, and $\mathcal{P}^a = \{\promptacc_j\}$, and $\alpha_\cdot$ are regularization hyperparameters. We assign equal weight to each of the loss terms, thus choosing $\alpha_{(.)}= 1$. 
The above objective function encourages the CLIP embeddings of $\imgunacc$ and $\promptuacc$, and $\imgacc$ and $\promptacc$, to be closer together while increasing the distance between $\imgunacc$ and $\promptacc$, and $\imgacc$ and $\promptuacc$, respectively. 
% \change{We were required two different fine-tuning methods because in the case where the unacceptable and acceptable prompts were opposites, simply optimizing the distance between their prompt embeddings without considering the image embeddings resulted in the CLIP model forgetting the mapping between the prompts and their corresponding images, resulting in poor filtering performance. Conversely, when Equation~\ref{eq:ft2} was used to optimize unacceptable/acceptable pairs where the acceptable concept was a general category, the performance was poor. We attribute this to overfitting, since images depicting characters/objects/celebrities are less varied than those depicting violence and nudity.}

In contrast, for concepts in Group-2 and 3, we fine-tune \filter to maximize the distance between $\phi_p(\promptuacc)$ and $\phi_p(\promptacc)$, and hence, minimize the following loss:
\begin{equation}\label{eq:ft1}
L_{\method} = -||\overline{\phi_p(\promptuacc) - \phi_p(\promptacc)}||_2
\end{equation}
We use prompts ($\promptuacc$ and $\promptacc$) for fine-tuning in Equation~\ref{eq:ft1} and Equation~\ref{eq:ft2} instead of only concepts ($\cunacc$ and $\cacc$): 
$\promptuacc$ and $\promptacc$ already contain $\cunacc$ and $\cacc$, and provide more context. 
% The prompts used for the \tti model are not known before-hand, but we can define the concepts to be filtered. 
% Since the prompt includes these concepts, filtering the images generated from the prompts is sufficient.

During fine-tuning of \method, there is a trade-off between effectiveness and utility which is inherent to all other fine-tuning \crt{s} as well. We subject our fine-tuning to the constraint that achieved the highest effectiveness for the least drop in utility.
We empirically show the benefit of fine-tuning in Appendix~\ref{app:FTEspresso}: Table~\ref{tab:FTImpact}).


% \change{Sec. 4 - A clear step-by-step overview of the Espresso generation pipeline is missing. Please consider adding a diagram.}




% \noindent\textbf{Replacement of Blocked Images.} 
% Following SDv1.4, on detecting $\imgunacc$, \method generates a replacement image~\cite{radford2021learning, rando2022redteaming}.
% As with other filters, on detecting $\imgunacc$, \method generates a replacement image as in SDv1.4~\cite{radford2021learning}.

% \input{tables/tab_nofinetune_effective}

==> generative-concept-removal/old_versions/5setup.tex <==
\section{Experimental Setup}\label{sec:setup}

% \input{figures/fig_trainvaltest}
We use Stable Diffusion v1.4~\cite{stable-diffusion} and its default configuration as the target \tti model following prior \crt{s}~\cite{gandikota2023erasing, kumari2023ablating, zhang2023forgetmenot, heng2023selective, gandikota2023unified, kim2023towards}.
We describe the attack baselines against \crt{s} (Section~\ref{sec:baseline}), metrics (Section~\ref{sec:metrics}), different concepts used for evaluation (Section~\ref{sec:concepts}), and pipeline used for evaluating \crt{s} (Section~\ref{sec:pipeline}).
% dataset and model configuration (Section~\ref{sec:datasets}).

\subsection{Revisiting Attack Baselines}\label{sec:baseline}

% We compare \method with prior state-of-the-art \crt{s} across \ref{effective}, \ref{utility}, and \ref{robust}. 
% We use six fine-tuning \crt{s} (\ca, \forgetNot, \sa, \esd, \unifiedCE, and \sdd) and one filtering \crt (\unsafediff) which are described in Section~\ref{back-conceptrem}. For filtering \crt, we do not compare with SD-Filter as \unsafediff outperforms it.
% To evaluate \ref{robust}, 
We consider different state-of-art attacks from literature (Section~\ref{back-attacks}).
We modify existing na\"{i}ve attacks (indicated with ``+''), Ring-a-Bell, and PEZ, to account for \crt{s}. 
All \crt{s} use some variant of the following optimization: detach $\cunacc$ from $\prompt$ such that the generated image is far from $\cunacc$ and closer to some $\cacc$. 
On the other hand, attacks against \tti models described in Section~\ref{back-attacks}, design $\advprompt$ such that $\imgadv$ is closer to $\cunacc$ and far from $\cacc$. 
Hence, to design an effective attack which accounts for such \crt{s}, in addition to the attacks' original objectives, we minimize the loss between the embeddings of $\advprompt$ and $\cacc$ while increasing the loss with the embeddings of $\cunacc$.
% Hence, an effective attack which accounts for such \crt{s} must find $\advprompt$ such that its generated image is unacceptable (via the attacks' original objective) in spite of the \crt. To do this, in addition to the attacks' original objectives, we minimize the loss between $\advprompt$ and $\cacc$ while increasing its loss with $\cunacc$.
% Hence, to design an effective attack which accounts for such \crt{s}, 
This, in turn, will move $\phi_p(\advprompt)$ closer to $\phi_p(\cacc)$ and farther from $\phi_p(\cunacc)$.
% \change{Since the attack objective is opposite to that of \crt{s}, the attack finds $\advprompt$ which counters the expected benefits of \crt{s}.}
% \change{This allows the generated image from $\advprompt$ to be incorrectly identified as acceptable while preserving the ability to generate $\imgunacc$.}
%
We modify the attacks to construct $\advprompt$ using following loss: 
\begin{equation}\label{eq:attack}
    \begin{split}
\mathcal{L}_{att+} = \mathcal{L}_{att} - \alpha_u \mathcal{L}_{MSE}(\phi_p(\cunacc), \phi_p(\advprompt)) + \\
\alpha_a \mathcal{L}_{MSE}(\phi_p(\cacc), \phi_p(\advprompt))
    \end{split}
\end{equation}
where $att \in \{RingBell, PEZ\}$ when $\crt \in \{$\ca, \forgetNot, \sa, \esd, \unifiedCE, \sdd, \unsafediff, \method$\}$, and $\mathcal{L}_{att}$ is from Section~\ref{back-conceptrem}.
We assign equal weight to all loss terms and use $\alpha_u = \alpha_a = 1.$
% Further, To design attacks against \unsafediff and \method, .
Recall from Section~\ref{back-attacks} that CCE already accounts for different fine-tuning \crt{s}. For filtering \crt{s} (\unsafediff and \method), we modify CCE using Equation~\ref{eq:attack} and call this attack CCE+. 


Finally, typographic attack~\cite{noever2021typographicattck} against CLIP is where text characters are superimposed onto an (unrelated) image to fool CLIP by forcing it to focus on this text instead of the image. We turn this into an attack against \crt{s} by superimposing $\cacc$ at the bottom of $\imgunacc$. Using the resulting adversarial images, we use PEZ+ to find their corresponding $\advprompt$. We call this attack \emph{Typo+}.



\subsection{Metrics}\label{sec:metrics}

We now describe the metrics to evaluate each of the requirements. We assume access to a \emph{reference CLIP}, separate from \target with the \crt{s}. The reference CLIP is a Stable Diffusion v1.4 model, a standard assumption in prior work~\cite{kumari2023ablating, gandikota2023erasing,gandikota2023unified,kim2023towards}.

\noindent\textbf{\underline{\ref{effective} (Effectiveness).}} Depending on the \crt, we use:
\begin{itemize}[leftmargin=*,wide,labelindent=0pt]
\item \textbf{CLIP accuracy}~\cite{hessel-etal-2021-clipscore,kumari2023ablating} for fine-tuning \crt{s}. This is the cosine similarity (divided by temperature parameter $\tau'=\frac{1}{100}$ of the reference CLIP) between the embeddings of the generated image $\imgclean$ with the embeddings of $\cunacc$ and $\cacc$ from the reference CLIP. This outputs the likelihood of predicting $\cunacc$. Hence, CLIP accuracy should be low (ideally zero) for effective concept removal. Formally, it is:
\[\frac{\text{exp}{(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc) / \tau'))}}{\text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc) / \tau')) + \text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cacc) / \tau'))}\]
where $\tilde{\phi_p}$ and $\tilde{\phi_x}$ are embeddings from the reference CLIP.
For filtering \crt, if $\imgunacc$ is detected, a replacement image is generated. Here, we calculate the CLIP accuracy on the final set of images after filtering. 
% Since the metrics compare with baseline reference CLIP, we use the same default replacement image as in the SD v1.4 filter.

\item \textbf{False Negative Rates (FNR)~\cite{unsafeDiff,rando2022redteaming}} for filtering \crt{s} is the fraction of images with $\cunacc$ which are not blocked. 
It should be low (ideally zero).
\end{itemize}


\noindent\textbf{\underline{\ref{utility} (Utility).}} Depending on the \crt, we use: 
\begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\item \textbf{Normalized CLIP score} for fine-tuning \crt{s} is is the ratio of cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$ from \target, compared to that from a reference CLIP as a baseline which is assumed to have the maximum achievable CLIP score. Formally, $\frac{\text{cos}(\phi_x(\imgclean),\phi_p(\prompt))}{\text{cos}(\tilde\phi_x({\imgclean}), \tilde\phi_p(\prompt))}$. 
Normalized CLIP score should be high (ideally one) for high utility. 
For the normalized CLIP score to be greater than one, the fine-tuned \tti model should generate images that match their prompts more closely than the original \tti model. This is unlikely to occur in practice as seen in our evaluation (c.f. Table~\ref{tab:utility}).
This metric is different from standard CLIP score from prior work~\cite{hessel-etal-2021-clipscore,kumari2023ablating, kim2023towards, gandikota2023unified} which measures the cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$ from \target. 
%We did this to scale the original CLIP score between zero and one while comparing \target to the reference CLIP.
We did this to compare the utility of the \tti with the \crt to that of the \tti without the \crt.
Hence, a perfect match between them will give a normalized CLIP score of one.

\item \textbf{False Positive Rates (FPR)~\cite{unsafeDiff,rando2022redteaming}} for filtering \crt{s} is the fraction of images without $\cunacc$ which are blocked.
It should be low (ideally zero).
\end{itemize} 


\noindent\textbf{\underline{\ref{robust} (Robustness).}} We use the same metrics as effectiveness: CLIP accuracy to evaluate fine-tuning \crt{s} and compare \method with them, and FNR for filtering \crt{s}. 




\subsection{Concept Types}\label{sec:concepts}

% \noindent\textbf{Concept Types.} 
We use the same set of unacceptable concepts as in prior work~\cite{kumari2023ablating, pham2023circumventing, kim2023towards}, categorizing them into three groups:
\begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\item Group-1 covers inappropriate concepts such as \emph{nudity} (e.g., female breasts or male/female genitalia), \emph{violence} (e.g., bloody scenes, fighting, burning, hanging, weapons, and wars), \emph{disturbing} (e.g., distorted faces, bodies, human flesh, or bodily fluids), and \emph{hateful} (e.g., defamatory racial depiction, harmful stereotypes, or Holocaust scenes).
\item Group-2 covers copyright-infringing concepts such as \emph{Grumpy Cat, Nemo, Captain Marvel, Snoopy}, and \emph{R2D2}.
\item Group-3 covers (unauthorized) use of personal images for celebrities such as \emph{Taylor Swift, Angelina Jolie, Brad Pitt}, and \emph{Elon Musk}.
\end{itemize}



\subsection{Pipeline for Evaluating \crt{s}}\label{sec:pipeline}

We now describe the pipeline which includes identifying acceptable concepts (step 1), generation of datasets (step 2), training filters or fine-tuning \tti models with \crt{s} (step 3), and validating acceptable concepts (step 4), and evaluating different \crt{s} (step 5). We present an overview of the pipeline in Figure~\ref{fig:pipeline} and describe each of the steps below.

\input{figures/fig_pipeline}



\subsubsection*{\underline{Step 1: Identifying Acceptable Concepts}}
A good choice of $\cacc$ is one which effectively steers a \tti model away from generating $\imgunacc$ while maintaining utility on other concepts. Hence, the choice of $\cacc$ can impact the overall effectiveness and utility of \crt{s}. 
We select $\cacc$ for a given $\cunacc$ such that it is either opposite to $\cunacc$ (Group-1) or is a semantic generalization of $\cunacc$ so as to avoid infringing copyrights (Group-2,3).
For $\cunacc$ in Group-1, we consider multiple alternative synonyms for $\cacc$ from which we choose the best possible candidate by measuring effectiveness and utility on a validation dataset (c.f. Step 4).
For $\cunacc$ in Group-2,3, we use $\cacc$ chosen by prior works~\cite{kumari2023ablating,heng2023selective} for a fair comparison.
% by evaluating the effectiveness and utility of using different synonyms on a validation dataset  and choosing the best possible candidate.
% We specify a matching $\cacc$ for every $\cunacc$ so that \crt{s} can steer away a \tti model from generating $\cunacc$ concepts and instead focus on $\cacc$. 
% For Group-1, we present the possible alternatives for $\cacc$, and for Group-2,3 we present the $\cacc$ taken from prior work. 
We indicate them in the format ``$\cunacc$ $\rightarrow$ $\cacc$'':
\begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\item \textbf{Group-1}: $\cacc$ is the opposite of $\cunacc$. We consider the following choices of $\cacc$: \emph{nudity} $\rightarrow$ \{\emph{clothed} and \emph{clean}\}; \emph{violence} $\rightarrow$ \{\emph{peaceful}, \emph{nonviolent}, and \emph{gentle}\}; \emph{disturbing} $\rightarrow$ \{\emph{pleasing}, \emph{calming}, and \emph{soothing}\}; \emph{hateful} $\rightarrow$ \{\emph{loving}, \emph{compassionate}, and \emph{kind}\}.
% For instance, \emph{violence} $\rightarrow$ \emph{peaceful}, \emph{disturbing} $\rightarrow$ \emph{pleasing}, and \emph{hateful} $\rightarrow$ \emph{loving}. For \emph{nudity}, we chose \emph{clean}.
% compared \emph{clothed} with \emph{clean} on a separate validation dataset (c.f. Section~\ref{sec:datasets} and Table~\ref{tab:valconfig}), and eliminated \emph{clothed} because it blocked images with minimal exposed skin despite being acceptable~\cite{unsafeDiff,schramowski2022safe}.
% Similarly, we evaluated and eliminated alternatives of $\cacc$ for \emph{violence} (\emph{nonviolent}, and \emph{gentle}), \emph{disturbing} (\emph{calming}, and \emph{soothing}), and \emph{hateful} (\emph{compassionate}, and \emph{kind}). 
\item \textbf{Group-2}: $\cacc$ is the type of $\cunacc$, following prior works~\cite{kumari2023ablating,heng2023selective,gandikota2023erasing}. For instance, \emph{Grumpy Cat} $\rightarrow$ \emph{cat}, \emph{Nemo} $\rightarrow$ \emph{fish}, \emph{Captain Marvel} $\rightarrow$ \emph{female superhero, Snoopy} $\rightarrow$ \emph{dog}, and \emph{R2D2} $\rightarrow$ \emph{robot}. 
\item \textbf{Group-3}: $\cacc$ is the sex of $\cunacc$, following prior works~\cite{heng2023selective, zhang2023forgetmenot, kim2023towards}: \{\emph{Taylor Swift, Angelina Jolie}\} $\rightarrow$ \emph{woman} and \{\emph{Brad Pitt, Elon Musk}\} $\rightarrow$ \emph{man}.
\end{itemize}



% \subsection{Dataset and Model Configurations}\label{sec:datasets}

\subsubsection*{\underline{Step 2: Generate and Split Datasets}}

We describe the generation of train, validation, and test datasets.

\noindent\textbf{Train Datasets.}
We summarize the different training/fine-tuning dataset configurations across \crt{s} in Table~\ref{tab:trconfig}. 

\input{tables/tab_trconfig}

\noindent\emph{Fine-tuning \crt{s}.} Different fine-tuning \crt{s} use different dataset configurations to ensure that \ref{effective} and \ref{utility} are met. We use the exact same configuration as described in each of the prior works to ensure that they satisfy the requirements claimed in their papers. While the configuration across different \crt{s} vary, the configuration for a specific \crt across different concepts is the same, in accordance with the instructions in the respective works. We briefly summarize them in Table~\ref{tab:trconfig}. \ca uses acceptable prompts which are generated from ChatGPT such that they contain $\cacc$, and 1 image per prompt. \esd and \sdd both use an unacceptable concept, and \sdd additionally uses 10 images corresponding to $\cunacc$. All images are generated using SD v1.4. 
\forgetNot uses unacceptable prompts of the form ``An image of \{$\cunacc$\}'', and 1 image per prompt.
For all the fine-tuning \crt{s}, we use their publicly available code for training to ensure the configuration is same as reported in their papers~\cite{githubGitHubNupurkmr9conceptablation,githubGitHubRohitgandikotaerasing,githubGitHubSHILabsForgetMeNot,githubGitHubRohitgandikotaunifiedconceptediting,githubGitHubClearnusselectiveamnesia,githubGitHubNannullnasafediffusion,githubGitHubYitingQuunsafediffusion}.



\noindent\emph{Filtering \crt{s}.} We train $\filter_{\unsafediff}$ using its exact dataset configuration (Table~\ref{tab:trconfig}) and code~\cite{unsafeDiff}. 
For \method, we follow the template by Kumari et al.~\cite{kumari2023ablating} to generate 10 unacceptable and acceptable prompts using ChatGPT, with one image per prompt from SDv1.4.
For Group-2 concepts, we randomly select 10 ChatGPT-generated prompts from the datasets provided by Kumari et al.~\cite{kumari2023ablating}.
Our choice for having a small amount of training data is inspired from prior works on poisoning attacks which show that little data is required to modify CLIP~\cite{yang2023robust, carlini2022poisoning}. Our results also show that using such little data is indeed sufficient to meet \ref{effective}, \ref{utility}, and \ref{robust} (c.f. Section~\ref{sec:evaluation}).



\noindent\textbf{Validation Datasets.}
We consider the following validation datasets ($\mathcal{D}_{val}$): we denote dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalunacc$; and dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalacc$.
For \ref{effective}, we use $\dvalunacc$ by generating 10 unacceptable prompts using ChatGPT, and generate 5 images per prompt using SD v1.4. 
For \ref{utility}, we use $\dvalacc$ by randomly choosing 100 non-overlapping acceptable prompts from the COCO 2014 dataset~\cite{coco}, and 1 image per prompt, generated from SD v1.4.
We summarize them in Table~\ref{tab:valconfig}. 

\input{tables/tab_valconfig}

\noindent\textbf{Test Datasets.} %We now present datasets for evaluating different \crt{s}. 
We consider test datasets ($\mathcal{D}_{te}$): we denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dtestacc$; and with unacceptable prompts ($\promptuacc$) and corresponding images ($\imgunacc$) as $\dtestunacc$.

\input{tables/tab_teconfig}

For evaluating effectiveness (\ref{effective}) and robustness (\ref{robust}), we use $\dtestunacc$ which is generated as follows:
For Group-1, we use an independent benchmark dataset, Inappropriate Image Prompts (I2P), containing prompts  likely to generate unsafe images~\cite{schramowski2022safe}. It covers all four Group-1 concepts. 
For \emph{nudity}, I2P includes a ``nudity percentage'' attribute. We choose all unacceptable prompts with a nudity percentage $>10$, resulting in a total of 300 unacceptable prompts, in accordance with prior works~\cite{gandikota2023erasing, gandikota2023unified}.
\unsafediff~\cite{unsafeDiff} also used \emph{political} as a concept, which is excluded from our evaluation since it is not a part of I2P. Note that I2P prompts do not explicitly contain $\cunacc$, \emph{i.e., the words \emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing} are not explicitly included in the prompts}.
For Group-2 and Group-3 concepts, there are no standard benchmark datasets. Hence, we generate the dataset by following prior works~\cite{kumari2023ablating, gandikota2023erasing} to obtain 200 unacceptable images generated from SDv1.4 from 10 unacceptable prompts generated from ChatGPT. 
For \ref{utility}, we use $\dtestacc$ which includes the COCO 2014 test dataset with 200 randomly chosen acceptable prompts.
We summarize the datasets in Table~\ref{tab:teconfig}. 


\subsubsection*{\underline{Step 3: Fine-tune \tti model with \crt{s} or train filter}}

Using $\dtrain$, we fine-tune \tti models using different fine-tuning \crt{s} whose optimizations are described in Section~\ref{back-attacks}.
We use six fine-tuning \crt{s} (\ca, \forgetNot, \sa, \esd, \unifiedCE, and \sdd). 
For filtering \crt, we consider one baseline (\unsafediff) and do not compare with SD-Filter as \unsafediff outperforms it.
For \unsafediff, we train the filtering classifier on their dataset. 
We fine-tune \method on $\dtrain$ and use the CLIP L-patch-14~\cite{vit} due to its popularity, which is also the default text encoder with Stable Diffusion v1.4. However, other variants of CLIP are also applicable.


\subsubsection*{\underline{Step 4: Select best $\cacc$ using $\mathcal{D}_{val}$}}

\input{tables/tab_concepts}
 \input{tables/tab_effectiveness}
 \input{tables/tab_utility}

 
For concepts in Group-1, we evaluate the effectiveness (\ref{effective}) and utility (\ref{utility}) for different candidates of $\cacc$ on $\dvalunacc$ and $\dvalacc$ respectively. 
We found that the following concepts gave the best results: \emph{nudity} $\rightarrow$ \emph{clean}, \emph{violence} $\rightarrow$ \emph{peaceful}, \emph{disturbing} $\rightarrow$ \emph{pleasing}, and \emph{hateful} $\rightarrow$ \emph{loving}.
For \emph{nudity}, we eliminated \emph{clothed} as it blocked images with minimal exposed skin despite being acceptable~\cite{unsafeDiff,schramowski2022safe}.



We use concepts in Group-1 following prior work~\cite{unsafeDiff} to evaluate filtering \crt{s}. 
We use \emph{nudity} and \emph{violence} from Group-1, and all the concepts from Group-2 and Group-3 following prior works~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards} to evaluate fine-tuning \crt{s}. 
Hence, we compare \method with each \crt category separately using concepts they were evaluated on.
We summarize the final concepts for evaluation in Table~\ref{tab:concepts}.



\subsubsection*{\underline{Step 5: Evaluating \ref{effective}, \ref{utility}, and \ref{robust} on $\mathcal{D}_{te}$}}

We evaluate effectiveness (\ref{effective}) on $\dtestunacc$, utility (\ref{utility} on $\dtestacc$, and robustness (\ref{robust}) $\dtestadv$ which is generated by running different attacks $\dtestunacc$ to get $\advprompt$. In all cases, we only pass the prompts from the dataset to \tti models and compute different metrics described in Section~\ref{sec:metrics}.

==> generative-concept-removal/old_versions/6evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}


\input{tables/tab_robustness}

We evaluate \method with fine-tuning \crt{s} (Section~\ref{sec:finetuneEval}), and then filtering \crt (Section~\ref{sec:filterEval}). 


\subsection{Comparison with Fine-tuning \crt{s}}\label{sec:finetuneEval}


\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report CLIP accuracy in Table~\ref{tab:effectiveness} for all eleven concepts on $\dtestunacc$. 
%
All \crt{s} show poor accuracy on \emph{nudity} and \emph{violence}. We attribute this to fine-tuning \crt{s} being sensitive to the input prompts~\cite{pham2024robust, yang2024guardt2i, ma2024jailbreaking}. Hence, they perform poorly for \emph{nudity} and \emph{violence} which do not explicitly include $\cunacc$.
In comparison to other \crt{s}, \method consistently maintains high accuracy on the I2P benchmark dataset as it classifies the generated images and does not depend on the prompts. 
Further, \method satisfies \ref{effective} using only 20 prompts and corresponding images for training. This is consistent with results on CLIP poisoning where changing the performance of CLIP only required a small number of poison samples~\cite{carlini2022poisoning, yang2023robust}.

\esd, \unifiedCE, and \sdd have better accuracy compared to the other three fine-tuning \crt{s}. 
This could be attributed to the similar optimizations used by \esd and \sdd for fine-tuning the \tti model: both fine-tune \dm, conditioned on $\cunacc$, to match original \dm without any prompt to reduce the influence of $\cunacc$ on the output.  
For \unifiedCE, higher effectiveness can be attributed to directly removing the influence of $\cunacc$ from the \tti model parameters. \textit{Overall, \method is more effective than other fine-tuning \crt{s}.}



\noindent\textbf{\underline{\ref{utility} Utility.}} We report normalized CLIP scores in Table~\ref{tab:utility} on $\dtestacc$.
%
All the fine-tuning \crt{s} perform well across all concepts (either \colorbox{myniceblue}{blue} or \colorbox{mynicegreen}{green}). This could be attributed to explicitly fine-tuning for utility. We observe that \ca with KL-Divergence-based optimization targeted for cross-attention layers, and \unifiedCE with a precise closed-form solution to model updates, preserve utility better than others. 

\method has high utility for all concepts except for \emph{violence}, and some Group-2 concepts (\emph{Nemo}, \emph{Captain Marvel}, \emph{Snoopy}, and \emph{R2D2}).
During fine-tuning, effectiveness improves but at the cost of utility, which is inherent to all fine-tuning \crt{s}.
For \textit{violence}, in our experiments, we observed an early decrease in utility during the very first epoch resulting in poor trade-off between effectiveness and utility. 
We attribute the poor utility on Group-2 concepts to the ambiguity in the unacceptable concepts. For instance, \emph{Nemo} is both a fish and a ship captain~\cite{VERNE_2024}, and \emph{Captain Marvel} represents both a male and a female superhero~\cite{Friedwald_2019_marvel}. 
To verify this, we precisely specify the unacceptable concepts to reduce ambiguity: as \emph{Nemo}$\rightarrow$ \emph{Nemo fish}, \emph{Captain Marvel}$\rightarrow$ \emph{Captain Marvel female superhero}, \emph{Snoopy}$\rightarrow$ \emph{Snoopy dog}, and \emph{R2D2}$\rightarrow$ \emph{R2D2 robot}. We evaluate \method on $\dvalacc$ and then report the numbers for the evaluation dataset below:
compared to the results in Table~\ref{tab:utility}, the normalized CLIP score for this new configuration is: 0.97 $\pm$ 0.00 (\emph{Nemo fish}), 0.90 $\pm$ 0.02 (\emph{Captain Marvel female superhero}), 0.98 $\pm$ 0.03 (\emph{Snoopy dog}), 0.92 $\pm$ 0.02 (\emph{R2D2 robot}), which are now indicated in \colorbox{mynicegreen}{green}.
We also report the CLIP accuracy on $\dvalunacc$ to evaluate effectiveness with this new configuration: 0.02 $\pm$ 0.00 (\emph{Nemo fish}), 0.00 $\pm$ 0.00 (\emph{Captain Marvel female superhero}), 0.02 $\pm$ 0.01 (\emph{Snoopy dog}), 0.00 $\pm$ 0.00 (\emph{R2D2 robot}), which are effective, same as before. Hence, precisely specifying $\cunacc$ is important for \method and can improve utility without sacrificing effectiveness. 
\textit{Overall, \method preserves utility on most concepts, and poor utility on some concepts can be improved by removing ambiguity in $\cunacc$.}


\noindent\textbf{\underline{\ref{robust} Robustness.}} We report CLIP accuracy in Table~\ref{tab:robust} on $\dtestadv$. We evaluate different \crt{s} against four attacks: Typo+, PEZ+, CCE/CCE+, and RingBell+. We evaluate fine-tuning \crt's against CCE, and evaluate \method against CCE+ as CCE already accounts for fine-tuning \crt{s}. We use the same color coding as in Table~\ref{tab:effectiveness}. 

CCE/CCE+, being a white-box attack which uses the parameters of the entire \tti model, is the strongest attack and it makes all fine-tuning \crt{s} ineffective. However, \method is more robust against CCE/CCE+ and outperforms all fine-tuning \crt{s}.
On the remaining attacks, all the fine-tuning \crt{s} have better robustness on Group-3 concepts than on Group-1 and 2. We attribute this to the difficulty of \tti models in generating precise faces while also evading detection, as shown in prior works~\cite{Matthias_2023}.
Similar to results in Table~\ref{tab:effectiveness}, we note that all \crt{s} perform poorly on \emph{nudity} and \emph{violence} across all the attacks. This is expected as the \crt{s} have poor effectiveness on these concepts as seen in Table~\ref{tab:effectiveness}. Hence, adversarial prompts for these concepts are likely to easily evade them. 
\emph{Overall, \method is more robust than all prior fine-tuning \crt{s} on all the concepts across all the attacks.} 
We discuss the possibility of future attacks against \method in Section~\ref{sec:future}.



\noindent\textbf{\underline{Summary.}} 
We depict the trade-offs among \ref{effective}, \ref{utility}, and \ref{robust} in Figure~\ref{fig:radarsFT}. We use (1-CLIP accuracy) for \ref{effective} on $\dtestunacc$, normalized CLIP score on $\dtestacc$ for \ref{utility}, and (1-CLIP accuracy) for \ref{robust} on $\dtestadv$ using CCE/CCE+. 
For each of the requirements, we use the average across all concepts as the representative value for a \crt.
\emph{Overall, \method provides a better trade-off across the three requirements compared to all the fine-tuning \crt{s}.}

\input{figures/fig_radar_ft}

































\subsection{Comparison with Filtering \crt}\label{sec:filterEval}

We now compare with \unsafediff~\cite{unsafeDiff}, the state-of-the-art filtering \crt, across the three requirements and summarize the results. We use FNR to evaluate effectiveness on $\dtestunacc$, FPR for utility on $\dtestacc$, and FNR for robustness on $\dtestadv$.




\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report FNR across four concepts (\emph{nudity}, \emph{violence}, \emph{disturbing}, and \emph{hateful}).
\method has better FNR for three of the four concepts: \emph{nudity}, \emph{violence} (in \colorbox{mynicegreen}{green}), and \emph{hateful} (\colorbox{myniceblue}{blue} for \method and \colorbox{mynicered}{red} for \unsafediff). However, both \method and \unsafediff perform poorly on \emph{disturbing}. 
We attribute this poor effectiveness on Group-1 concepts to the subjective description of $\cunacc$. Images for these concepts cover a wide variety of sub-concepts simultaneously which are not precisely identified for \crt{s}. 
\emph{Overall, \method is more effective than \unsafediff on most concepts.}

\input{tables/tab_filter_effective}



\noindent\textbf{\underline{\ref{utility} Utility.}} We present FPR in Table~\ref{tab:FilterUtility} across the four  Group-1 concepts. As expected, we observe that both \method and \unsafediff have comparable utility they demonstrate a low FPR. This is expected since \unsafediff explicitly includes images containing $\cacc$ while training the multi-headed classifier.

\input{tables/tab_filter_utility}

\noindent\textbf{\underline{\ref{robust} Robustness.}} We report FNR on the dataset for adversarial prompts and corresponding images in Table~\ref{tab:FilterRobust}. In addition to the four attacks from Table~\ref{tab:robust}, recall that SneakyPrompt~\cite{yang2023sneakyprompt} is specifically designed to attack filtering \crt{s}. Hence, we also include the evaluation against SneakyPrompt. 
Also, since CCE is not adaptive against filtering \crt's, we evaluate \unsafediff and \method against CCE+. We are the first to evaluate different attacks against \unsafediff.
\input{tables/tab_filter_robust}

We observe that \method is effective in thwarting $\advprompt${s} from PEZ+ while \unsafediff can be evaded.
On all the remaining attacks, we show that \method is robust on more concepts than \unsafediff.
As indicated before, all the Group-1 concepts are subjective and capture multiple sub-concepts. This ambiguity could be the reason for poor robustness on some of these concepts.
\emph{Overall, \method is more robust than \unsafediff on majority of the concepts across different attacks.}

\input{figures/fig_radar_filter}

\noindent\textbf{\underline{Summary.}} 
We present the trade-offs in the form of radar plots in Figure~\ref{fig:radarsFilt}. 
We use (1- FNR) on $\dtestunacc$ for \ref{effective}, (1- FPR) on $\dtestacc$ for \ref{utility}, and (1- FNR) on $\dtestadv$ using CCE+ for \ref{robust}. Hence, a higher value indicates better performance.
\method has comparable utility to \unsafediff but outperforms in effectiveness and robustness.
\emph{Overall, \method covers a larger area, and hence provides a better trade-off than \unsafediff.}






==> generative-concept-removal/old_versions/7robustness.tex <==
\section{Certifying Robustness of \method}\label{sec:bound}

We empirically showed that \method is robust against several state-of-the-art attacks (Section~\ref{sec:evaluation}).
Inspired by the literature on certified robustness against adversarial examples~\cite{cohen2019certified}, it is natural to ask whether a similar notion of certified robustness is possible for \crt{s}.
None of the existing \crt{s} have considered certified robustness.
To this end, we are the first to explore its feasibility for \method.


We first present a theoretical bound on the worst-case modification by \adv under which we can guarantee \method's accuracy (Section~\ref{sec:theoretical}). We then empirically evaluate this bound on different concepts (Section~\ref{sec:empirical}) and finally discuss some implications of our results (Section~\ref{sec:implications}).


\subsection{Theoretical Bound}\label{sec:theoretical} 

Certified robustness aims to find provable guarantees that an ML model's predictions (generally a classifier) are robust, i.e., the predictions do not change on adding noise to the input~\cite{carlini2023certified}. 
Our goal is to have a similar provable robustness bound for a \tti model with \method. 
We want to find the maximum noise to an input which \method can tolerate.

We give advantage to \adv by assuming they can directly add adversarial noise to \method's embeddings. This is a strong assumption as in practice, \adv can only send prompts to the \tti model. We revisit this assumption later in Section~\ref{sec:implications}.
Formally, given an unacceptable image $\imgunacc$, \adv adds noise $\delta$ to its embeddings, $\phi_x(\imgunacc)$, such that $\filter(\phi_x(\imgunacc) + \delta)$ is misclassified as acceptable.
Using this assumption, we specify the maximum noise $\delta$ added to the embeddings, $\phi_x(\imgunacc)$, that \method can tolerate in Theorem~\ref{thm.1}.


\input{figures/fig_certified}


\begin{theorem}~\label{thm.1}
    Let $\hat{x} = \phi_x(x), \hat{c}^i = \phi_p(c^i), i\in\{a,u\}$. 
    % For $F(x)$ defined in equation~\ref{eq:att}, 
    Define 
    \[g_i(\hat{x}):=\frac{exp(s(\hat{x},\hat{c}^i))}{exp(s(\hat{x},\caccc))+exp(s(\hat{x},\cunaccc))},\] 
    where $s(\hat{x},\hat{c}^i) = \tau \text{cos}(\hat{x},\hat{c}^i))$, then $g_i$ is the confidence of $\hat{x}$ being classified as $\concept^i$. $F(x)$ in equation~\ref{eq:att} can be defined as $F(\hat{x})=argmax_i g_i(\hat{x})$, and $F(\hat{x})$ classifies $\hat{x}$ as unacceptable if $g_u(\hat{x})>\Gamma$, where $\Gamma$ is the decision threshold.
     For a given image embedding $\hat{x}$, if $g(\hat{x}):=g_u(\hat{x})>\Gamma$, then $g$ is robust against noise $\delta$ where 
     \[||\delta||\leq\left(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|}\right)||\hat{x}||,\]
     % on the image embedding, 
     and $\Gamma$ is the decision threshold i.e. 
    \begin{equation}\label{eq:bound}
            F(\hat{x}) = F(\hat{x}+\delta), \forall ||\delta||\leq \left(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|}\right)||\hat{x}||.
    \end{equation}
\end{theorem}

\noindent\textit{Proof Sketch.} We prove the above theorem by applying Lipschitz continuity over $g(\hat{x})$. \filter($\cdot$) is the composition of the softmax function and the scaled cosine similarity over the embeddings, where both functions are Lipschitz continuous when $||\hat{x}||>0$. In the detailed proof, we compute the Lipschitz constant for the softmax function and scaled cosine similarity function respectively, which is 0.25 and $\frac{\tau}{||\hat{x}||}$. Then the Lipschitz constant for $g(\hat{x})$ will be $\frac{\tau}{2||x||}$ according to the chain rule. Finally, using the triangle inequality on $|g(\hat{x})-g(\hat{x}+\delta)|$, and plugging the bound in to the inequality, we get $g(\hat{x}+\delta)\geq \Gamma$.
We present the full proof in Appendix~\ref{app:proof}.
We discuss extending the bound to prompt space in Section~\ref{sec:future}.




\subsection{Empirical Validation}\label{sec:empirical}

We now compute the maximum noise that \method can tolerate for each unacceptable image's embedding using Equation~\ref{eq:bound}. 
Following prior literature on certified robustness~\cite{cohen2019certified}, we compute the certified accuracy described in~\cite{cohen2019certified} to evaluate the robustness of \method.
Certified accuracy at radius $r$ is the fraction of unacceptable images which are correctly classified and are robust against adversarial noise $\delta > r$.
This shows the robustness of \method against attacks under some noise $r$. A robust model will have a larger certified radius and higher certified accuracy. 
Since we add noise directly to $\phi_x(\imgunacc)$, we compare our certified accuracy with the accuracy of clean unacceptable images (without adversarial noise) which we refer as ``clean accuracy''. 
Ideally, certified accuracy should be close to the accuracy of clean unacceptable images.

We present the results in Figure~\ref{fig:certified} for the three groups of concepts. 
Clean accuracy in Figure~\ref{fig:certified} is the certified accuracy at radius zero. 
\method is robust against $\delta<0.07$, incurring less than a $5\%$ drop in certified accuracy. 
When $\delta<0.15$, the certified accuracy remains higher than $50\%$ for all concepts. 
\method is particularly robust for some concepts in Group-2 (\emph{Grumpy Cat}, \emph{R2D2}, \emph{Captain Marvel}), and Group-3 (\emph{Taylor Swift}, \emph{Angelina Jolie}, and \emph{Elon Musk}). For these concepts, the certified accuracy remains the same for the clean unacceptable images until $\delta>0.15$.
Further, \method is more robust for concepts where the clean accuracy is $1.00$ (CLIP accuracy from Table~\ref{tab:effectiveness}). We find that the robustness is higher for concepts on which \method is more accurate. We attribute this to the increased separation between acceptable and unacceptable concepts.



\subsection{Practical Implications}\label{sec:implications} 

Having discussed the theoretical bound and empirically validated it on different concepts, we now revisit the practicality of this bound.
We discuss the usefulness of the certification and revisit our assumption about \adv's capability.


\noindent\textbf{Usefulness of Certified Bound.} 
In Figure~\ref{fig:certified}, we find that the certified bound is less than \(0.15\) across all the concepts. We found this to be smaller than the $l_2$-norms of realistic image embeddings, which had a mean of \(17\).
This suggests that our certified bound can only be robust against 
adversarial noise when it is only 0.8\% (=0.15/17) of the embeddings.

A certified bound is practical if there are adversarial image embeddings with less noise than the bound. Then, the bound is effective against these embeddings.
We use \method without fine-tuning with Equation~\ref{eq:ft1} to check the existence of such adversarial image embeddings. We can find embeddings that  \emph{potentially} evade \method (without fine-tuning) when the noise is as small as $0.028$.
Our certified bound is useful against such embeddings\footnote{Note that to find an actual attack against \method, \adv will have to (a) find a prompt that generates this perturbed embedding, and (b) ensure that the resulting image retains the unacceptable content.}.


However, the distance between acceptable and unacceptable images, which is at least \(7\), is much larger than the certified bound. This suggests that our certified bound is loose. We leave a tighter certified bound and the possibility of using adversarial training for improving robustness as future work (c.f. Section~\ref{sec:future}). 


\noindent\textbf{\adv's Capability.} To compute the certified bound, we assumed a strong \adv who can directly add adversarial noise to the \emph{embeddings}.
In practice, \adv can only modify the \emph{prompts} sent to the \tti model, and can only obtain the corresponding filtered outputs. Hence, in practice, \adv is much weaker and the robustness of \method is much higher than indicated in Figure~\ref{fig:certified}.

To illustrate this, we consider a concrete attack that \adv could adopt given its inability to directly add adversarial noise to embeddings:
\adv begins with unacceptable images and incorporate adversarial noise using standard evasion techniques (e.g., PGD~\cite{MadryPgd}) to find an adversarial example that evades the \method classifier. 
\adv then finds the corresponding adversarial prompt using one of the attacks (PEZ+) in Section~\ref{back-attacks}. 
We want to see if \target still generates an adversarial image which evades \method. 
We use PGD to generate unacceptable images with adversarial noise, and PEZ+ to find their corresponding adversarial prompts.
We find that \target fails to generate an adversarial image which evades \method using the adversarial prompt.
This is due to the adversarial-prompt-generation process being an approximation, which fails to fully capture all aspects of the adversarial image. 
Moreover, using the \tti model to generate the image from the adversarial prompt is unlikely to capture the adversarial noise due to the de-noising used in the diffusion model (Section~\ref{back-diffusion}). This claim is further supported by prior literature on the robustness of diffusion models~\cite{Kim_2022_CVPR,chen2024diffusion,zhang2023diffsmooth,xiao2022densepure}. 

 
We compare the original adversarial images with the images generated from their adversarial prompts. We present one concept from each group in Appendix~\ref{app:adv}: Table~\ref{fig:adversarial}. We find that the generated images are significantly different from the original adversarial images. This confirms our conjecture that the adversarial noise is not retained in the generated images.
A more thorough exploration of such an attack is left as future work. Based on the above preliminary exploration, we conjecture that \method is likely to be robust against such attacks by \adv with realistic capabilities.

==> generative-concept-removal/old_versions/8related.tex <==
\section{Related Work}\label{sec:related}


\noindent\textbf{Prompt Filters.} We focus on image filters to detect $\imgunacc$. Prior works have explored using prompt filters to identify unacceptable concepts before passing them to \tti models~\cite{yang2024guardt2i}.
Such filters are being used for DALLE-2 \cite{ramesh2021dalle}, and MidJourney~\cite{midjourney}. However, these prompt filters are not robust and easy to evade~\cite{ba2023surrogateprompt,ma2024jailbreaking}. Hence, prior works have identified image filters are a better alternative, with the possibility of making it effective and robust~\cite{li2024safegen}.

% \change{https://arxiv.org/abs/2404.03631 
% https://arxiv.org/pdf/2405.16341v1
% Water down the claim that none of the prior fine-tuning CRTs are robust in intro and abstract...}

\noindent\textbf{Additional \crt{s}.} We use state-of-the-art \crt{s} for evaluation. Hence, we omit the discussion about prior \crt{s} which have been outperformed by those considered in this work~\cite{schramowski2022safe, automatic1111_negative_prompt,radford2021learning}. We discuss recent fine-tuning \crt{s}.

Hong et al.~\cite{hong2023one} propose an approach to make minimal changes for concept removal. Instead of matching the entire distribution of features for $\cunacc$ to the distribution of $\cacc$, they selectively modify the features with highest density in $\cunacc$. 
Wu et al.~\cite{wu2024erasediff} propose concept removal as an unlearning problem which is solved as constraint optimization while preserving utility. 
Basu et al.~\cite{basu2023ldiffquickfix} present a closed-form solution to remove concepts from \te by identifying causal features for one concept and overriding it with another concept. 
Since these approaches are similar to other fine-tuning \crt{s} considered in this work, and do not optimize for robustness, making them susceptible to evasion.

Huang et al.~\cite{huang2024receler} modify the cross entropy layers of \dm to erase $\cunacc$ with adversarial training for better robustness against only two na\"{i}ve attacks: Prompting4Debugging~\cite{chin2023prompting4debugging} and RingBell~\cite{Tsai2023RingABellHR}. 
Li et al.~\cite{li2024safegen} modify the self-attention layers of \dm using triplets of $\imgunacc$, censored $\imgunacc$, and $\imgacc$. They evaluate robustness against SneakyPrompt. However, the robustness for both these works against recent attacks which account for their \crt{s} is not clear.

Pham et al.~\cite{pham2024robust} fine-tune \tti model to generate a specific concept and subtract the task vector for this concept from the model parameters of the original model, thereby erasing $\cunacc$.
They demonstrate robustness against CCE and RingBell but suffer from a trade-off between \ref{utility} and \ref{robust}.
Wu et al.~\cite{wu2023backdooring} insert backdoors to textual inversion embeddings such that a $\cunacc$ results in a pre-defined image instead of $\imgunacc$.
Despite accounting for robustness, these \crt{s} incur trade-offs between \ref{effective}, \ref{utility}, and \ref{robust}.

\noindent\textbf{Additional Attacks against \crt{s}.} Prompting4Debugging uses PEZ while matching the noise between a \tti model with a \crt, and one without a \crt, during the reverse diffusion process. In our setting, \tti model with and without \method are identical, hence Prompting4Debugging reduces to PEZ.
Rando et al.~\cite{rando2022redteaming} propose PromptDilution against filters. However, as SneakyPrompt outperformed PromptDilution~\cite{yang2023sneakyprompt}, we do not consider it for evaluation.

Ba et al.~\cite{ba2023surrogateprompt} generate  substitutes for $\cunacc$ in their input prompts to evade a black-box filter. They show effectiveness against the Q16 filter which is outperformed by \unsafediff. 
Ma et al.~\cite{ma2024jailbreaking} optimize for $\advprompt$ to match $\cunacc$ using TextGrad, a gradient based search over text, to identify the tokens. Their attack outperforms Prompting4Debugging, Prompt Dilution, and RingBell. 
Shahgir~\cite{shahgir2024asymmetric} replace an object in $\imgclean$ with a target object to create $\imgadv$, which can be inverted to get $\advprompt$.
Kou et al.~\cite{ijcai2023p109} use a character-level gradient attack that replaces specific characters to design $\advprompt$.




==> generative-concept-removal/old_versions/9discussion.tex <==
\section{Discussion and Future Work}\label{sec:discussions}

We revisit our discussion on robustness  (Section~\ref{sec:future}), applicability/extensions of \method (Section~\ref{sec:extensions}), and a summary of this work (Section~\ref{sec:summary}).




\subsection{Revisiting Robustness}\label{sec:future}

\noindent\textbf{Addressing Future Attacks.} Recall that our certified robustness bound is loose (Section~\ref{sec:bound}). We leave the improvement of the bound as future work.

\method maintains high robustness across all evaluated concepts. 
The design of new attacks which can preserve unacceptable concepts while evading \method is an open problem. Here, adversarial training for \method can be used to increase its robustness.
We can fine-tune CLIP with this objective: $\mathcal{L}_{\text{Con-adv}}(\dtestadv)=$
\[- \frac{1}{N} \sum_{j = 1}^N \log \frac{\exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(\cunacc))/ \tau)}{\sum_{k \in \{a,u\}} \exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(c_k))/ \tau)}\]
where $\mathcal{D}_{adv} = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$. Assuming $\imgadv$ evades the filter, we optimize $\phi_p$ and $\phi_x$, such that $\phi_p(\imgadv_j)$ is closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$. This loss would be added to Equation~\ref{eq:ft1} and~\ref{eq:ft2}. 
Empirical evaluation of adversarially-trained \method is left as future work.


\noindent\textbf{Extending the Theoretical Bound to Prompts.} 
% Although \adv cannot modify text embeddings in practice, analyzing robustness in the CLIP embedding space is valuable as recent works have shown that small changes in the text embeddings of prompts, allow for fine-grained control over their generated images~\cite{yu2024uncovering, kawar2023imagic}. 
To extend our theoretical bounds in Theorem~\ref{thm.1} to the prompt space,
we assume Lipschitz continuity, commonly used in ML~\cite{bousquet2002stability}, certified robustness~\cite{li2023sok}, and more recently in the context of \tti models~\cite{chen2024your}.
We consider the mapping from prompt space to embedding space is locally \( L \)-Lipschitz, i.e., the function \( \phi_x(f(\text{\prompt})) \) satisfies the following condition:

For each prompt \(\text{\prompt}\), there exists a \(\delta_{\text{\prompt}} > 0\) such that
$
||\phi_x(f(\text{\prompt})) - \phi_x(f(\text{\prompt} + \delta_{\text{\prompt}}))|| \leq L ||\delta_{\text{\prompt}}||.
$

Then, the inequality in Equation~\ref{eq:bound} can be related to the prompt space by a scalar factor \(\frac{1}{L}\). 
Therefore, when \(\|\delta_{\text{\prompt}}\| \leq \frac{1}{L} \|\delta\|\), where \(\|\delta\|\) satisfies inequality in Equation~\ref{eq:bound}, the difference in embedding space will be bounded by \(\|\delta\|\), and CLIP remains robust.


\subsection{Applications and Extensions to \method}\label{sec:extensions}


\noindent\textbf{Filtering Multiple Concepts.} Gandikota et. al.~\cite{gandikota2023unified} have considered removing multiple concepts simultaneously.
While we focus on filtering one concept at a time for comparison with other \crt{s}, \method can be extended by including multiple concepts simultaneously as well. Specifically, for $\filter(x, \cunacc, \cacc)$ in Equation~\ref{eq:att}, instead of only specifying $\cunacc$ and $\cacc$ for a single concept, we can include $\cunacc$ and $\cacc$ for multiple concepts as a list. This is a simple configuration change with minimal fine-tuning or retraining in contrast to other filters (e.g.,~\cite{unsafeDiff}) which require training with extensive datasets. Since none of the prior \crt{s} evaluate multiple $\cunacc$, we leave its evaluation as future work. 

\noindent\textbf{Filtering Artistic Styles.} 
None of the prior filtering \crt{s} consider any copyrighted content and focus on only \emph{inapproriate Group-1 concepts}. 
\method is the first filtering \crt which is applicable to concepts which are copyright-infringing (Group-2) or involve unauthorized use of personalized images (Group-3).
Prior fine-tuning \crt{s} have considered removing artistic styles (e.g., painting in the style of Monet or Van Gogh) as copyrighted content~\cite{kumari2023ablating,gandikota2023erasing}.
However, we observed that \method does not differentiate between images with and without artistic styles very well. Specifically, \emph{Monet painting} as $\cunacc$ and \emph{painting} as $\cacc$, are very similar for \method, thus reducing its effectiveness. We leave the optimization of \method to account for artistic styles as future work.

\noindent\textbf{Applicability to other \tti Models.} Fine-tuning \crt{s} are specific to particular stable diffusion models due to their tailored optimizations for \tti models. In contrast, filtering \crt{s} offer versatility, as they can be applicable to any \tti model. 
Filters analyze only the generated image and the list of concepts, independently of the \tti model. 
However, fine-tuning the filter using data from \tti model, as we do it for \method, can improve effectiveness and utility. 
This allows to use the filter we will have a filter that will work with \tti model in different domains (e.g., anime images).
Explicit evaluation of \method for different \tti models is deferred to future work.


\subsection{Summary}\label{sec:summary}

Removing unacceptable concepts from \tti models is an important problem. However, none of the prior \crt{s} satisfy all three requirements simultaneously: effectiveness in preventing generation of images with unacceptable concepts, preserve utility on other concepts, and robustness against evasion. We propose \method, the \emph{first} robust \underline{co}ncept \underline{fi}ltering \crt which provides a better trade-off among the three requirements compared to prior \crt{s}.

==> generative-concept-removal/old_versions/WACV/01abstract.tex <==
Diffusion based text-to-image models are trained on large datasets scraped from the Internet, potentially containing \textit{unacceptable concepts} (e.g., copyright infringing or unsafe). 
We need concept removal techniques (\crt{s}) which are
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \textit{effective} in preventing the generation of images with unacceptable concepts
\item \textit{utility-preserving} on acceptable concepts, and 
\item \textit{robust} against evasion with adversarial prompts.
\end{enumerate*}
None of the prior \crt{s} satisfy all these requirements simultaneously. 
We introduce \method, the first \emph{\textbf{robust \underline{co}ncept \underline{fi}lter} }based on Contrastive Language-Image Pre-Training (CLIP). 
We configure CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts.
This lets us fine-tune for robustness by separating the text embeddings of unacceptable and acceptable concepts while preserving their pairing with image embeddings for utility.
We present a pipeline to evaluate various \crt{s}, attacks against them, and show that \method, is \textbf{more effective and robust} than prior \crt{s}, while retaining \emph{utility}.
% Code will be publicly available upon publication.
%(CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) 

%(CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) 

%(normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]). 
% Finally, we present theoretical bounds for certified robustness of \method against adversarial prompts, and an empirical analysis.


==> generative-concept-removal/old_versions/WACV/1introduction.tex <==
\section{Introduction}\label{sec:introduction}


Diffusion-based text-to-image (\tti) models have demonstrated a remarkable ability to generate high quality images from textual prompts~\cite{stable-diffusion,Rombach_2022_CVPR,ramesh2021dalle}.
They are trained on large datasets of unfiltered content from the Internet~\cite{radford2021learning,schuhmann2022laion}. 
Due to their large capacity, \tti models memorize specific \emph{concepts}, as seen in the generated images~\cite{Korn_2023,somepalli2022diffusion,carlini2023extracting}. 
Some of these concepts, may be \emph{unacceptable} for various reasons, such as copyright infringement (e.g., a movie character or celebrity), or inappropriateness (e.g., ``nudity'' or ``violence'')~\cite{gandikota2023erasing,schramowski2022safe,heng2023selective}. 
% Retraining \tti models after filtering out unacceptable concepts is inefficient, only partially effective~\cite{li2024safegen, huggingfaceStabilityaistablediffusion21Hugging}, and compromises utility~\cite{gandikota2023erasing}.
We need \emph{concept removal techniques} (\crt{s}) to minimize unacceptable concepts in  generated images.


Ideally, \crt{s} should be \emph{effective} in reducing the generation of unacceptable concepts while preserving the \emph{utility} on all others, and \emph{robust} to evasion with adversarial prompts.  
As we show in Section~\ref{sec:evaluation}, no existing \crt \emph{simultaneously} satisfies these requirements:
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \emph{fine-tuning \crt{s}} which modify \tti models, trade-off effectiveness for utility~\cite{gandikota2023erasing,kumari2023ablating,heng2023selective,schramowski2022safe}, and  lack robustness~\cite{Tsai2023RingABellHR, wen2023hard, pham2023circumventing, yang2023sneakyprompt}
\item \emph{filtering \crt{s}}, which detect unacceptable concepts, lack robustness~(\cite{rando2022redteaming} and Section~\ref{sec:filterEval}).
\end{enumerate*}
%Moreover, none of these \crt{s} are robust against adversarial prompts, i.e., adversarially modified prompts which force \tti{s} to generate unacceptable concepts.
Our goal is to design a \crt that can simultaneously meet all the requirements.

We opt to use a filter as it will not alter the \tti model, thus minimizing impact on utility. We construct our filter using a Contrastive Language-Image Pre-Training (CLIP) model~\cite{radford2021learning}, an essential component of \tti models. 
% CLIP co-locates the embeddings of textual prompts and their corresponding images within a unified embedding space where similar concepts are closer.
CLIP is pre-trained on a vast dataset which encodes a broad spectrum of concepts~\cite{radford2021learning}, making it a versatile choice for a filter, unlike specialized classifiers (e.g.,~\cite{unsafeDiff}).
However, a naive CLIP-based filter is susceptible to evasion~\cite{rando2022redteaming}. 
%by solely measuring the distance between the embeddings of a generated image, and an unacceptable concept,
\begin{arxiv}
Subsequently, prior works have identified the design of a robust filtering-based \crt as an open problem~\cite{rando2022redteaming,li2024safegen}.
\end{arxiv}

% \input{figures/fig_robustness_diagram}
% \change{Robustness diagram: figures/fig\_robustness\_diagram}

We present a \textbf{robust \underline{co}ntent \underline{fi}lter}, \method, by configuring CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts. 
% We present a \textbf{robust} \textbf{co}ntent \textbf{fi}lter, \method, that identifies unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both acceptable and unacceptable concepts}. 
% \change{This simple change in configuration translates to projecting} the image embedding onto the vector connecting the text embeddings of acceptable and unacceptable concepts. 
% This simple change makes it harder to generate effective adversarial prompts: the adversary is restricted to adding noise in the direction of the acceptable concept. 
%adversarial prompts must generate images far enough from unacceptable concepts to evade detection yet close enough to retain the unacceptable concepts.
This allows fine-tuning for better robustness by increasing the separation between the text embeddings of unacceptable and acceptable concepts, while preserving utility by maintaining their pairing with their corresponding image embeddings. 
% We liken this to adversarial training in classifiers, thus, improving the robustness of \method.
% This fine-tuning approach is further supported by fine-tuning \crt{s} which show that such an optimization leads to better utility~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}.
Our contributions are presenting 
\begin{enumerate*}[label=\roman*)]
\item \method, the \textbf{first robust \underline{co}ntent \underline{fi}lter} (Section~\ref{sec:approach}), 
\item \emph{a pipeline} to evaluate state-of-the-art \crt{s} and attacks (Section~\ref{sec:setup}),
\item and a comprehensive evaluation of \method against six fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective} and \textbf{robust} while \textbf{retaining utility} (Section~\ref{sec:evaluation}).
\end{enumerate*}\begin{arxiv} In Appendix~\cite{sec:bound} \end{arxiv}\begin{submission} In the supplementary material, \end{submission}
we present the \emph{first} approach for \emph{certifiable robustness of \crt{s}} by exploring 
theoretical robustness bounds of \method with a hypothetically strong adversary. 
We empirically analyze these bounds to show that \method is likely to be more robust in practice.
% \begin{enumerate}[leftmargin=*,wide,  labelindent=0pt]
% \item \method\footnote{We will open-source the code upon publication.}, the \textbf{first robust} (CLIP-based) \underline{co}ntent \underline{fi}lter (Section~\ref{sec:approach}) 
%which identifies unacceptable concepts in generated images by measuring the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts ,
% \item a comprehensive comparative evaluation of \method with six state-of-the-art fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective} and \textbf{more robust} while \textbf{retaining utility}. (Section~\ref{sec:setup})
% (CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) and \textbf{more robust} (CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) than prior \crt{s}, while \textbf{retaining utility} (normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]).
%showing that \method is \textbf{effective} ($\sim$5\% CLIP accuracy  on unacceptable concepts), \textbf{utility-preserving} ($\sim$93\% 
% normalized CLIP score on acceptable concepts), and \textbf{robust} ($\sim$4\% CLIP accuracy of  on adversarial prompts) %of unacceptable concepts) 
% (Section~\ref{sec:evaluation}), and
% \item %the \textbf{first} approach towards \textbf{certifiable robustness of \crt{s}} by exploring 
% theoretical bounds for \textbf{certifying the robustness} of \method, assuming a hypothetically strong adversary, empirical analysis of these bounds, and making the case that \method is likely to be more robust in practice. (Section~\ref{sec:bound}). 
% \end{enumerate}

==> generative-concept-removal/old_versions/WACV/2background.tex <==
\section{Background and Related Work}\label{sec:background}

% We describe \tti models (Section~\ref{back-diffusion}), different \crt{s} (Section~\ref{back-conceptrem}), and attacks against them (Section~\ref{back-attacks}).

\subsection{Diffusion based \tti Models}\label{back-diffusion}

A diffusion based \tti model is a function $\target: \prompt \rightarrow \imgclean$ which generates an image $\imgclean$ for a given a textual prompt $\prompt$. It comprises two key components: a text and image encoder ($\phi$) which is used to incorporate the textual prompt in the image generation process, and a diffusion model (\dm) which is responsible for the generation of the image.

A popular encoder is CLIP, trained on a large dataset of image-text pairs, to map the embeddings of images and their corresponding text closer together in a joint text-image embedding space~\cite{radford2021learning}.
We denote the image embeddings as $\phi_x()$ and text embeddings as $\phi_p()$.
%Given $N$ images $\{\imgclean_j\}_{j=1}^N$ and their corresponding text prompts $\{\prompt_j\}_{j=1}^{N}$, the training data is $\mathcal{D} = \{(\imgclean_j, \prompt_j)\}_{j=1}^N$. 
CLIP is trained to maximize the cosine similarity (\text{cos}($\phi_p(\prompt_j), \phi_x(\imgclean_j))$) between the embedding of a prompt $\prompt_j$ ($\phi_p(\prompt_j)$) and the embedding of its corresponding image $\imgclean_j$ ($\phi_x(\imgclean_j)$) while minimizing the similarity between $\phi_p(\prompt_j)$ and any other $\phi_x(\imgclean_k)$ for $k \ne j$.
% We denote the cosine similarity as , where $\phi_x(\imgclean_j)$ is the CLIP image embedding of the image $\imgclean_j$, and $\phi_p(\prompt_j)$ is the CLIP text embedding of the prompt $\prompt_j$.
To achieve this, CLIP is trained using a contrastive loss function ($\mathcal{L}_{\text{Con}}$)~\cite{yang2023robust,oord2019representation,lee2021soundguided,radford2021learning}.
 % \[\mathcal{L}_{\text{Con}}(\mathcal{D}) = - \frac{1}{N} \sum_{j=1}^{N} \log \frac{\exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_j))/ \tau)}{\sum_{k=1}^{N} \exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_k))/ \tau)}\] where $\tau$ is the temperature parameter for scaling the predictions~\cite{radford2021learning, ModalityGap}. 
 


Given access to a pre-trained encoder, the actual images in \tti models are generated by a diffusion model, \dm, parameterized by $\theta$.
%During training of \dm, Gaussian noise is added to an initial image $x_0$ for $T$ time steps to produce $x_T$, in a process known as the \emph{forward diffusion process}. The noise is then iteratively removed to approximate the initial image $\tilde{x_0}$ in the \emph{reverse diffusion process}.
During inference, \dm generates an image from noise and can be conditioned with the embedding of a textual prompt $\phi_p(\prompt)$ to guide the generation of the image to match the description in \prompt. %After generating $\phi_p(\prompt)$, %from \te, 
%\dm is trained by minimizing the following loss function: $\mathcal{L} = \mathbb{E}_{\epsilon, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(\imgclean_t,\phi_p(\prompt),t)||_2^2]$ for each time step $t$, and random Gaussian noise $\epsilon \sim \mathcal{N}(0,1)$.

%Several prominent \tti models (e.g., Stable Diffusion v1.4 (SDv1.4)) improve the efficiency of the diffusion process by conducting it in the embedding space of a variational autoencoder (VAE), rather than on images \cite{stable-diffusion}. For a VAE decoder $\mathit{D}$, VAE encoder $\mathcal{E}$, and $z_t \in \mathcal{E}(\imgclean)$ as the latent representation of $\imgclean$ in the VAE's latent space, \dm is trained by minimizing the following objective: \\
%$\mathcal{L} = \mathbb{E}_{\epsilon, z_t, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(z_t,\phi_p(\prompt),t)||_2^2]$ where $\epsilon \sim \mathcal{N}(0,1)$. The final image is generated from the approximation, $\tilde{z_0}$, by passing it through $\mathit{D}$: $\tilde{x_0} = \mathit{D}(\tilde{z_0})$.  
% Table~\ref{tab:notations} in Appendix~\ref{app:notations} summarizes frequently used notations.

 




\subsection{Concept Removal Techniques}\label{back-conceptrem}

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance?--- We use the same approach for selecting acceptable concepts as Kumari et. al.~\cite{kumari2023ablating}for group 2 and group 3 concepts. For these groups, the acceptable concept is a superset of the unacceptable concept. For example, the sex of a celebrity is the acceptable concept for a celebrity. For group 1, there is no clear definition of a superset (eg. the superset of \emph{nude} is unclear). Logically, the acceptable concept is the opposite of the unacceptable concept in this case since it is clearly defined. - SHOULD MOVE THIS EXPLANATION ELSEWHERE}

The textual phrase for an acceptable concept is $\cacc$, and for an unacceptable concept is $\cunacc$. 
For a given $\cunacc$, we define $\cacc$ as either the opposite, e.g., $\cunacc$ = \emph{violence} vs. $\cacc$ = \emph{peaceful}, or a generalization of a specific instance, e.g., $\cunacc$ = \emph{R2D2} vs. $\cacc$ = \emph{robot} (discussed later in Section~\ref{sec:pipeline}).
% We discuss the selection of $\cacc$ for a given $\cunacc$ in .
A \tti model may generate an image containing an unacceptable concept (referred to as $\imgunacc$) or an acceptable one (referred to as $\imgacc$). Similarly, a text prompt $\prompt$ may contain a phrase for an acceptable concept ($\promptacc$) or an unacceptable concept ($\promptuacc$). An example of $\promptuacc$ containing an unacceptable concept $\cunacc$ = \emph{Captain Marvel}, is ``\emph{Captain Marvel} soaring through the sky''. \crt{s} seek to thwart the generation of $\imgunacc$ by either fine-tuning the \tti model to suppress $\imgunacc$, or using a classifier as a filter to detect and replace $\imgunacc$. 
%
We discuss six state-of-the-art fine-tuning \crt{s}:
\noindent\textsc{Concept Ablation} (\ca)~\cite{kumari2023ablating} minimizes the KL divergence between the model's output for $\promptuacc$ and $\promptacc$ to force the generation of \imgacc instead of \imgunacc; 
% Formally, they optimize the following objective function: 
 % \text{argmin}_\theta 
% \[\begin{split}
% \footnotesize
%    \mathcal{L}_{\ca} =  \mathbb{E}_{\epsilon, z_t, \cunacc, \cacc, t}[w_t||\epsilon_\theta(z_t,\phi_p(\promptacc),t).sg() \\
%     - \epsilon_\theta(z_t,\phi_p(\promptuacc),t)||_2^2]
% \end{split}\]
% where $\epsilon \sim \mathcal{N}(0,1)$, $z_t \in \mathcal{E}$, and $w_t$ is a time-dependent weight, and $.sg()$ is the stop-gradient operation.
\textsc{Forget-Me-Not} (\forgetNot)~\cite{zhang2023forgetmenot} minimizes the activation maps for $\cunacc$ by modifying \dm's cross-attention layers; %Further, fine-tuning \dm, instead of just the cross-attention layers, results in degraded utility. 
% That is, given $a_i \in \mathcal{A}_i$, the $i$-th attention map in \dm of \tti, their loss is 
% \[\mathcal{L} = \sum_{a_i \in \mathcal{A}_i}||a_i||\]
\textsc{Selective Amnesia} (\sa)~\cite{heng2023selective} adapts continuous learning techniques (elastic weight consolidation and generative replay) for \tti models to forget a concept; %They optimize $\mathbb{P}(\imgclean|\theta^*,\cunacc)$, the probability of generating $\imgclean$ given $\theta^*$ and $\cunacc$, where $\theta^*$ are the frozen parameters of the original \tti model.
% \[
% \begin{split}
% \footnotesize
%     \mathcal{L}_{\sa} = -\mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_f(\cunacc)}[\text{log}\mathbb{P}(\imgclean|\theta^*,\cunacc)] -\lambda\sum_i\frac{M_i}{2}(\theta_i^*-\theta_i)^2\\
%      + \mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_r(\cacc)}[\text{log}\mathbb{P}(\imgclean|\theta,\cacc)]
% \end{split}
% \]
% where $M$ is the Fisher information matrix over $\cacc$ and $\cunacc$, $\mathbb{P}_r$ and $\mathbb{P}_f$ are probabilities taken over the distributions of $\cacc$ and $\cunacc$ respectively, and $\lambda$ is a regularization parameter. 
\textsc{Erased Stable Diffusion} (\esd)~\cite{gandikota2023erasing} modifies the diffusion process to reduce the probability of generating \imgunacc;
% \[\begin{split}
% \epsilon_\theta(\imgclean_t,\phi_p(\cunacc),t) = \epsilon_{\theta^*}(\imgclean_t, t)
% + \eta(\epsilon_{\theta^*}(\imgclean_t,\phi_p(\cunacc),t)\\-\epsilon_{\theta^*}(\imgclean_t,t))
% \end{split}\]
% where $\eta > 0$ encourages the noise conditioned on $\cunacc$ to match the unconditioned noise.
\textsc{Unified Concept Editing} (\unifiedCE)~\cite{gandikota2023unified} fine-tunes the cross-attention layers to minimize the influence of $\cunacc$; 
% Their optimization is:
% % \text{min}_W
% \[\begin{split}
%     \mathcal{L}_{\unifiedCE} = \sum_{\cunacc \in \mathcal{C}^{u}, \cacc \in \mathcal{C}^{a}}||W\times\cunacc-W^*\times\cacc||_2^2 \\ 
%     +  \sum_{c \in S}||W\times c - W^*\times c||_2^2
% \end{split}\]
% where $W$, $W^*$ are the parameters of the fine-tuned and original \emph{cross-attention layers in \dm}, $\mathcal{C}^{u}$ and $\mathcal{C}^{a}$ are the space of pre-defined unacceptable and acceptable concepts, and $S$ is a set of concepts for which to preserve utility. 
\textsc{Safe diffusion} (\sdd)~\cite{kim2023towards}
encourages the diffusion model output conditioned on $\cunacc$ to match the unconditioned output.
% using the following objective function:
% \[\begin{split}
%     % \text{argmin}_\theta
%     \mathcal{L}_{\sdd} = \mathbb{E}_{\epsilon, z_t, \cunacc, t}[||\epsilon_\theta(z_t,\phi_p(\cunacc),t) 
%  - \epsilon_\theta(z_t,t).sg()
%     ||_2^2]
% \end{split}\]
% where $\epsilon \sim \mathcal{N}(0,1)$ and $z_t \in \mathcal{E}(x)$.
All current fine-tuning \crt{s} trade-off effectiveness for utility~\cite{gandikota2023erasing,kumari2023ablating,heng2023selective,schramowski2022safe} and are not robust (see Section~\ref{back-attacks}).


\noindent We also discuss two state-of-the-art filtering \crt{s}.
\textsc{Stable Diffusion Filter} (\texttt{SD-Filter})~\cite{radford2021learning} is black-box and the design of the filter is not publicly available, but Rando et. al.~\cite{rando2022redteaming} hypothesize that it involves computing the cosine similarity between the embeddings of a generated image, $\imgclean$, and a pre-defined set of $\cunacc$. If the cosine similarity is greater than some threshold, then $\imgclean$ has $\cunacc$. 
% Formally, their filter $\filter_{SD}$ can be described as
% \[ \filter_{SD}(\imgclean) = \begin{cases} 
%       1 & \text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) > \Gamma \\
%       0 & \text{otherwise}
%    \end{cases}
% \]
% where $\text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) = \overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\cunacc)}$, and $\overline{\cdot}$ denotes normalization. Here $\filter_{SD}(\imgclean) = 0$ indicates \imgacc and $\filter_{SD}(\imgclean) = 1$ indicates \imgunacc. Note that $\Gamma$ varies with $\cunacc$. 
\textsc{Unsafe Diffusion} (\unsafediff)~\cite{unsafeDiff} is the current state-of-the-art filtering \crt and outperforms the SD-Filter~\cite{unsafeDiff}. \unsafediff trains a multi-headed neural network classifier on top of CLIP to identify $\imgunacc$ where each head classifies different $\cunacc$: \emph{nudity, violence, disturbing, hateful}, and \emph{political}. %Their objective is given as $\filter_{\unsafediff}(\imgclean) = \text{MLP}(\phi_x(\imgclean))$ where MLP is a multi-layer perceptron, and $\filter_{\unsafediff} \in \{0,1\}$.
In Section~\ref{sec:filterEval}, we show that \unsafediff is not robust.

\subsection{Evading Concept Removal Techniques}\label{back-attacks} 

An adversary \adv may construct adversarial prompts ($\advprompt$) to evade \crt{s} and force the \tti model to generate $\imgunacc$. %while being semantically closer to acceptable prompts so that $\imgadv$ is incorrectly identified as acceptable while triggering the generation of unacceptable images. We denote a dataset containing adversarial prompts and their corresponding images ($\imgadv$) as $\dtestadv = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$ where ideally $\imgadv$ will contain $\cunacc$.
\adv is assumed to know and account for the target \tti model \target and its \crt. A dumb \adv who does not account for this is \emph{na\"{i}ve}. 
%
% \adv's objective is to construct $\advprompt$ which can force a \tti model to output images with $\cunacc$ 
Existing attacks formulate the construction of $\advprompt$ as an optimization problem using some reference $\imgunacc$ (or the difference between $\promptacc$ and $\promptuacc$) as the ground truth. 
% Different attacks vary in ways to solve this optimization. We present four state-of-the-art attacks:
%
\noindent\pez~\cite{wen2023hard} constructs $\advprompt$ by identifying text tokens which 
minimize the cosine similarity between $\phi_p(\advprompt)$ and $\phi_x(\imgunacc)$.
% : $\mathcal{L}_{\pez}= 1-\text{cos}(\phi_p(\advprompt),\phi_x(\imgunacc))$. 
%
\ringbell~\cite{Tsai2023RingABellHR} identifies tokens for $\advprompt$ by first calculating the average difference between the embedding vectors of $\promptuacc$ and $\promptacc$ and then minimizes the distance of $\advprompt$'s text embedding to $\promptuacc$'s embedding using a genetic algorithm.
%: $\phi_p(\hat{\prompt}) = \frac{1}{N}\sum_{i=1}^N\{\phi_p(\promptuacc_i) - \phi_p(\promptacc_i)\}$ from a set of $N$ prompts.
% Then, RingBell computes $\advprompt$ by minimizing the distance of its text embedding to an acceptable prompt embedding using a genetic algorithm.
% , formulated as: $\text{min}_{\advprompt} ||\phi_p(\advprompt) - (\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))||^2$ where $\prompt^{init}$ is an initial unacceptable prompt which is censored by a \crt. They solve this using a genetic algorithm. 
%Further, the optimization relies on a fitness function using mean-squared error: $\mathcal{L}_{RingBell} = \mathcal{L}_{MSE}(\phi_p(\cunacc),\phi_p(\advprompt))$ where $\cunacc$ is a prompt that generates $\imgunacc$ in a \tti model.
%
\sneaky~\cite{yang2023sneakyprompt} uses reinforcement learning to construct $\advprompt$ (starting from some initial $\promptuacc$) specifically against filtering \crt{s} using cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\advprompt)$ as the reward function. 
% Given an initial prompt $\prompt^{init}$, the attack searches for tokens to update $\prompt^{init}$ to form $\advprompt$ using cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\advprompt)$ as the reward function. 
% Typically, they use $\promptuacc$ as $\prompt^{init}$ for better effectiveness and faster convergence.
%
\cce~\cite{pham2023circumventing} uses textual-inversion~\cite{gal2022textualinversionimage} to construct $\advprompt$ by updating CLIP's vocabulary to include a new token ``<s>'' which generates \adv's desired image. 
%
All these attacks are effective against fine-tuning \crt{s} in Section~\ref{back-conceptrem}.
%However, for proper robustness evaluation, it is important to evaluate \crt{s} against attacks which account for \crt{s}.}
% To optimize <s>, we find $v$, an embedding for <s>, corresponding to least loss $\mathcal{L}_{CCE}=\mathcal{L}_{MSE}(\epsilon, \epsilon_\theta(z_t,v,t))$, where $\epsilon\sim\mathcal{N}(0,1)$, and $\mathcal{L}_{MSE}$ is the mean-squared-error. 
% CCE and SneakyPrompt account for different fine-tuning \crt{s}. 
%Among the described attacks, only \ringbell and \pez are na\"{i}ve and we later describe how we modify them to account for \crt{s} (Section~\ref{sec:baseline}).
In Section~\ref{sec:baseline}, we enhance two na\"{i}ve attacks, \ringbell and \pez, to defeat all these \crt{s}, including \unsafediff.
\begin{arxiv}

SurrogatePrompt~\cite{ba2023surrogateprompt} is a recent attack against a \crt in a commercial \tti systems that targets input filters, not output filters like \method. Therefore we omit it in our robustness evaluation.
\end{arxiv}

==> generative-concept-removal/old_versions/WACV/3problem.tex <==
\section{Problem Statement}\label{sec:problem}


Our goal is to design a \crt which can effectively detect $\imgunacc$ from \tti models. 
% We describe an adversary model, requirements of an ideal \crt, and limitations of prior works. 
% according to the requirements.


\noindent\textbf{Adversary Model.} We consider a deployed target \tti model ($\target$) to which a client has blackbox access to send an input ($\prompt$) and obtain a generated image ($\imgclean$). Further, $\target$ uses some \crt. The goal of the adversary (\adv) is to force $\target$ to generate $\imgunacc$ despite the presence of a \crt to suppress it.
We give an advantage to \adv by allowing whitebox access to a local identical copy of $\target$ with the \crt for use in designing attacks. This is reasonable as \dm and CLIP are publicly available. For filtering \crt{s}, we assume that \adv has whitebox access to the filter to use its loss function in designing the attacks.

\noindent\textbf{Requirements} An ideal \crt should be:
\begin{enumerate*}[label=\textbf{R\arabic*},leftmargin=*]
\item\label{effective} \textit{Effective} in minimizing the generation of $\imgunacc$;
\item\label{utility} \textit{Utility-preserving}, maintaining the quality of acceptable images (for fine-tuning \crt{s}) or not blocking them (for filtering \crt{s}); and
\item\label{robust} \textit{Robust} against evasion with $\advprompt$.
\end{enumerate*}



\noindent\textbf{Limitations of Prior Works.} 
%We now briefly discuss the limitations of different types of prior \crt{s} \emph{vis-a-vis} the requirements above. 
% , we empirically show 
We summarize the limitations of prior works which are empirically evaluated later in Section~\ref{sec:evaluation}.
\textit{Fine-tuning \crt{s}} modify $\target$ thereby explicitly creating a trade-off between \ref{effective} and \ref{utility}~\cite{gandikota2023erasing,kumari2023ablating,zhang2023forgetmenot,heng2023selective,heng2023selective,gandikota2023unified,kim2023towards}.
Further, most of these \crt{s} do not consider \ref{robust} in their design and are susceptible to evasion by \adv with $\advprompt$.
\textit{Filtering \crt{s}}~\cite{radford2021learning,unsafeDiff} detect unacceptable concepts either in $\prompt$ (aka prompt filter) or in $\imgclean$ and block them (a.k.a image filter). Since, they do not modify $\target$, they can maintain \ref{utility} without impacting \ref{effective}. Prior filtering approaches may not be accurate in detecting unacceptable concepts (poor \ref{effective})~\cite{li2024safegen} and can be easily evaded (poor \ref{robust}) (\cite{rando2022redteaming} and Section~\ref{sec:filterEval}). Further, the current state-of-the-art filter, \unsafediff~\cite{unsafeDiff}, trains specialized classifiers for each concept on substantial data, which limits their generalization to new concepts.


==> generative-concept-removal/old_versions/WACV/4approach.tex <==
\section{\method: Robust Filtering CRT}\label{sec:approach}

We present \method, a robust \underline{co}ncept \underline{fi}ltering \crt. 
\method uses a classifier \filter to detect images and filter unacceptable concepts in generated images. Following Stable Diffusion v1.4 (SDv1.4)~\cite{stable-diffusion}, on detecting an unacceptable concept, \method generates a replacement image~\cite{radford2021learning, rando2022redteaming}.
We identify CLIP as the natural choice for such a classifier as it is
\begin{enumerate*}[leftmargin=*,label=(\alph*)]
\item pre-trained on a large dataset covering a wide range of concepts, and
\item used across many \tti models, and encodes similar information as seen in them.
\end{enumerate*}
Hence, CLIP is a better choice for a filter than training specialized classifiers for each concept (e.g.,~\cite{unsafeDiff}).

 However, simply using CLIP for \method is not sufficient as seen in SDv1.4's filter ($\filter_{SD}$)~\cite{radford2021learning}. 
$\filter_{SD}$ thresholds the cosine similarity between the embeddings of $\imgclean$ and each pre-defined unacceptable concept to identify $\imgunacc$. 
Rando et al.~\cite{rando2022redteaming} design adversarial prompts ($\advprompt$) to evade $\filter_{SD}$ by constructing $\advprompt$ to force a misclassification.
% Since $\filter_{SD}$ uses only the cosine similarity to $\cunacc$, it gives \adv the freedom to modify the prompt embeddings in \emph{any direction}, while constructing $\advprompt$, to force a misclassification.
%
We address this in \method by configuring CLIP's classification objective for fine-tuning to further improve robustness. 

\noindent\textbf{Configuring CLIP's Classification Objective.} Instead of using the cosine similarity to only $\cunacc$ as in $\filter_{SD}$, we configure the objective function of \method for filtering $\imgunacc$ by using the cosine similarity to \emph{both} $\cunacc$ and $\cacc$. 
% \change{This makes \adv's goal more difficult as they are forced to optimize $\advprompt$ such that the resulting image embedding is far from $\phi_p(\cunacc)$, \emph{and} close to $\phi_p(\cacc)$, which is an additional stipulation arising from the design of \method.}
Further, jointly optimizing for two embeddings yields better utility as observed in prior fine-tuning \crt{s}~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}. 
%
Given $\imgclean$, \method checks the cosine similarity of $\phi_x(\imgclean)$ to $\phi_p(\cunacc)$ and $\phi_p(\cacc)$. Formally, we define \method as $\filter(x, \cunacc, \cacc)$
\begin{equation}\label{eq:att}
 = \text{argmax}_{i, i\in{a,u}} \left\{\frac{\text{exp}{(\text{cos}(\phi_x(x),\phi_p(\concept_i)) / \tau)}}{\sum_{j \in \{a,u\}}\text{exp}(\text{cos}(\phi_x(x),\phi_p(\concept_j)) / \tau)}\right\}
\end{equation} 
$\tau=\frac{1}{100}$ is the default temperature parameter used in CLIP. 
%Further, the cosine similarity is equivalent to the scaled Euclidean distance between the embeddings~\cite{ModalityGap}: 
%\[(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) = 2-2\overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\concept)}\]
%\[\implies \text{cos}(\imgclean, \concept) = -\frac{1}{2}(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) + 1\]
%Hence, by using CLIP as a filter, we \change{are effectively projecting} the image embeddings onto the vector between $\cunacc$ and $\cacc$ and classifying it based on its distance to both.  
%
% This simple configuration change in CLIP's classification objective restricts \adv to adding noise only along the low-dimensional vector joining $\cunacc$ and $\cacc$: $\phi_p(\cunacc) - \phi_p(\cacc)$ in the direction of $\cacc$.
% This is more challenging for \adv to evade than $\filter_{SD}$, as projecting to a lower-dimensional representation can improve robustness~\cite{pca1,pca2}.
% Hence, we conjecture that this can help satisfy \ref{effective} and \ref{robust} (as shown later in Section~\ref{sec:evaluation}).
% This change in objective function is required to apply fine-tuning.

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance? - ANSWERED}


% \change{Rationale for fine-tuning?}
\noindent\textbf{Fine-tuning.} The above configuration change lets us use fine-tuning to push acceptable and unacceptable concepts away from each other while maintaining their pairing with their corresponding image embeddings (for utility).
Our fine-tuning objectives are inspired by the adversarial training literature which increase the distance of the training data records to the decision boundary to minimize the effect of adversarial examples~\cite{zhang2019theoretically}. 
% may impact the utility on some concepts due to the close proximity of some $\cunacc$ and $\cacc$.
% To restore any drop in utility, we use fine-tuning. 
We use two different fine-tuning variants depending on the group of concepts.


For concepts that have a strong correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$ (for example, where $\cacc$ is a broader category that includes $\cunacc$; $\cunacc$ = \emph{R2D2} and $\cacc$ = \emph{robot}), we fine-tune \filter to increase the difference between $\phi_p(\promptuacc)$ and $\phi_p(\promptacc)$. We minimize the following:
\begin{equation}\label{eq:ft1}
L_{\method} = -||\overline{\phi_p(\promptuacc) - \phi_p(\promptacc)}||_2
\end{equation}
where $\overline{\cdot}$ denotes normalization. 
% The prompts used for the \tti model are not known before-hand, but we can define the concepts to be filtered. 
% Since the prompt includes these concepts, filtering the images generated from the prompts is sufficient.
For the case where $\cunacc$ and $\cacc$ are opposites (e.g., $\cunacc$ = \emph{violence} and $\cacc$ = \emph{peaceful}), the above objective function might have a low correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$. This might result in poor utility. In this case, we use following objective function:
\begin{equation}\label{eq:ft2}
    \begin{split}
        \mathcal{L}_{\method} = \alpha_{\text{aa}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{aa}) 
        -\alpha_{\text{ua}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{ua}) \\
        + \alpha_{\text{uu}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{uu})  
        -\alpha_{\text{au}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{au}) \\
        -\alpha_{\text{uu-t}}\mathcal{L}_{MSE}(\phi_p(\mathcal{P}^{u}), \phi_p(\mathcal{P}^{a})) \\
    \end{split}
\end{equation}
where $\mathcal{D}_{aa} = \{(\imgacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{au} = \{(\imgacc_j, \promptuacc_j)\}_{j=1}^N$, \\$\mathcal{D}_{ua} = \{(\imgunacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{uu} = \{(\imgunacc_j, \promptuacc_j)\}_{j=1}^N$, $\mathcal{P}^u = \{\promptuacc_j\}$, and $\mathcal{P}^a = \{\promptacc_j\}$, and $\alpha_{(\cdot)}$ are regularization hyperparameters. We assign equal weight to each of the loss terms, thus choosing $\alpha_{(.)}= 1$. 
The above objective function encourages the CLIP embeddings of $\imgunacc$ and $\promptuacc$, and $\imgacc$ and $\promptacc$, to be closer together while increasing the distance between $\imgunacc$ and $\promptacc$, and $\imgacc$ and $\promptuacc$, respectively. 

We use prompts ($\promptuacc$ and $\promptacc$) for fine-tuning in Equation~\ref{eq:ft1} and Equation~\ref{eq:ft2} instead of only concepts ($\cunacc$ and $\cacc$): 
$\promptuacc$ and $\promptacc$ already contain $\cunacc$ and $\cacc$, and provide more context. 
During fine-tuning of \method, there is a trade-off between \ref{effective} and \ref{utility} which is inherent to all other fine-tuning \crt{s}. We subject our fine-tuning to the constraint that achieved the highest effectiveness for the least drop in utility.
We show the benefit of fine-tuning in Section~\ref{sec:finetuningEval}.  

==> generative-concept-removal/old_versions/WACV/5setup.tex <==
\section{Experimental Setup}\label{sec:setup}

% \input{figures/fig_trainvaltest}
We use SDv1.4~\cite{stable-diffusion} and its default configuration as \target following prior work~\cite{gandikota2023erasing, kumari2023ablating, zhang2023forgetmenot, heng2023selective, gandikota2023unified, kim2023towards}.
% We describe the attack baselines against \crt{s} (Section~\ref{sec:baseline}), metrics (Section~\ref{sec:metrics}), and pipeline used for evaluating \crt{s} (Section~\ref{sec:pipeline}).
% dataset and model configuration (Section~\ref{sec:datasets}).

\subsection{Revisiting Attack Baselines}\label{sec:baseline}

% We compare \method with prior state-of-the-art \crt{s} across \ref{effective}, \ref{utility}, and \ref{robust}. 
% We use six fine-tuning \crt{s} (\ca, \forgetNot, \sa, \esd, \unifiedCE, and \sdd) and one filtering \crt (\unsafediff) which are described in Section~\ref{back-conceptrem}. For filtering \crt, we do not compare with SD-Filter as \unsafediff outperforms it.
% To evaluate \ref{robust}, 
We consider different state-of-art attacks from literature (Section~\ref{back-attacks}).
%
We modify existing na\"{i}ve attacks: \ringbell, and \pez, to account for \crt{s} (indicated with ``+''). 
All \crt{s} use some variant of the following optimization: detach $\cunacc$ from $\prompt$ such that the generated image is far from $\cunacc$ and closer to some $\cacc$. 
On the other hand, attacks against \tti models design $\advprompt$ such that $\imgadv$ is closer to $\cunacc$ and far from $\cacc$. 
Hence, to design an effective attack which accounts for such \crt{s}, in addition to the attacks' original objectives, we minimize the loss between $\phi_p(\advprompt)$ and $\phi_p(\cacc)$ while increasing the loss with $\phi_p(\cunacc)$.
% Hence, an effective attack which accounts for such \crt{s} must find $\advprompt$ such that its generated image is unacceptable (via the attacks' original objective) in spite of the \crt. To do this, in addition to the attacks' original objectives, we minimize the loss between $\advprompt$ and $\cacc$ while increasing its loss with $\cunacc$.
% Hence, to design an effective attack which accounts for such \crt{s}, 
% This, in turn, will move $\phi_p(\advprompt)$ closer to $\phi_p(\cacc)$ and farther from $\phi_p(\cunacc)$.
% \change{Since the attack objective is opposite to that of \crt{s}, the attack finds $\advprompt$ which counters the expected benefits of \crt{s}.}
% \change{This allows the generated image from $\advprompt$ to be incorrectly identified as acceptable while preserving the ability to generate $\imgunacc$.}
%
We modify the attacks to construct $\advprompt$ using following loss: 
\begin{equation}\label{eq:attack}
    \begin{split}
\mathcal{L}_{att+} = \mathcal{L}_{att} - \alpha_u \mathcal{L}_{MSE}(\phi_p(\cunacc), \phi_p(\advprompt)) + \\
\alpha_a \mathcal{L}_{MSE}(\phi_p(\cacc), \phi_p(\advprompt))
    \end{split}
\end{equation}
where $att \in$ \{\ringbell, \pez\} when \crt$\in $\{\ca, \forgetNot, \sa, \esd, \unifiedCE, \sdd, \unsafediff, \method\}, and $\mathcal{L}_{att}$ is the attack's original objective.
We assign equal weight to all loss terms and use $\alpha_u = \alpha_a = 1.$
% Further, To design attacks against \unsafediff and \method, .
Recall from Section~\ref{back-attacks} that \cce already accounts for different fine-tuning \crt{s}. For filtering \crt{s} (\unsafediff and \method), we modify \cce using Equation~\ref{eq:attack} and call it \cce+. 
%
Finally, typographic attack~\cite{noever2021typographicattck} against CLIP superimposes text characters onto an (unrelated) image to fool CLIP by forcing it to focus on the text instead of the image. We turn this into an attack against \crt{s} by superimposing $\cacc$ at the bottom of $\imgunacc$. Using the resulting adversarial images, we use \pez+ to find their corresponding $\advprompt$. We call this attack \typo+.

\input{figures/fig_pipeline}

\subsection{Metrics}\label{sec:metrics}

% We now describe the metrics to evaluate each of the requirements. 
\noindent We use a \emph{reference CLIP} (SDv1.4), separate from \target with the \crt{s}, following prior work~\cite{kumari2023ablating, gandikota2023erasing,gandikota2023unified,kim2023towards}.

\noindent\textbf{\underline{\ref{effective} (Effectiveness).}} For fine-tuning \crt{s}, we use
% \begin{itemize}[leftmargin=*,wide,labelindent=0pt]
\noindent\textbf{CLIP accuracy}~\cite{hessel-etal-2021-clipscore,kumari2023ablating} which is the cosine similarity between the embeddings of the generated image $\imgclean$ with the embeddings of $\cunacc$ and $\cacc$ from the reference CLIP. This outputs the likelihood of predicting $\cunacc$. Hence, CLIP accuracy should be low (ideally zero) for effective concept removal. Formally, it is:
$\frac{\text{exp}{(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc)))}}{\text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc))) + \text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cacc)))}$
where $\tilde{\phi_p}$ and $\tilde{\phi_x}$ are embeddings from the reference CLIP.
For \method, if $\imgunacc$ is detected, a replacement image is generated. Here, we calculate the CLIP accuracy on the final set of images after filtering. 
% Since the metrics compare with baseline reference CLIP, we use the same default replacement image as in the SD v1.4 filter.

\noindent For filtering \crt{s}, we use \textbf{false negative rates (FNR)~\cite{unsafeDiff,rando2022redteaming}} which is the fraction of images with $\cunacc$ which are not blocked. 
It should be low (ideally zero).
% \end{itemize}


\noindent\textbf{\underline{\ref{utility} (Utility).}}
% \begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\noindent For fine-tuning \crt{s}, we use \textbf{normalized CLIP score} which is the ratio of cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$ from \target, compared to that from a reference CLIP as a baseline which is assumed to have the maximum achievable CLIP score. Formally, $\frac{\text{cos}(\phi_x(\imgclean),\phi_p(\prompt))}{\text{cos}(\tilde\phi_x({\imgclean}), \tilde\phi_p(\prompt))}$. 
Normalized CLIP score should be high (ideally one) for high utility. 
% For the normalized CLIP score to be greater than one, the fine-tuned \tti model should generate images that match their prompts more closely than the original \tti model. This is unlikely to occur in practice as seen in our evaluation (c.f. Table~\ref{tab:utility}).
This metric is different from standard CLIP score from prior work~\cite{hessel-etal-2021-clipscore,kumari2023ablating, kim2023towards,gandikota2023unified} which only measures the cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$. 
%We did this to scale the original CLIP score between zero and one while comparing \target to the reference CLIP.
We modified it to compare the utility of the \tti with the \crt to that of the \tti without the \crt.
Hence, a perfect match will give a score of one.

For filtering \crt{s}, we use \textbf{False Positive Rates (FPR)~\cite{unsafeDiff,rando2022redteaming}} which is the fraction of images without $\cunacc$ which are blocked.
It should be low (ideally zero).
% \end{itemize} 


\noindent\textbf{\underline{\ref{robust} (Robustness).}} We use the same metrics as \ref{effective}: CLIP accuracy for fine-tuning \crt{s}, and FNR for filtering \crt{s}. 




% \subsection{Concept Types}\label{sec:concepts}




\subsection{Pipeline for Evaluating \crt{s}}\label{sec:pipeline}

We now describe the pipeline which includes identifying acceptable concepts (step 1), generation of datasets (step 2), training filters or fine-tuning \tti models with \crt{s} (step 3), validating acceptable concepts (step 4), and evaluating different \crt{s} (step 5). We present an overview of the pipeline in Figure~\ref{fig:pipeline} and describe each of the steps below.



\noindent\textbf{Concept Types.}
We use the same $\cunacc$ as prior work~\cite{kumari2023ablating, pham2023circumventing, kim2023towards}, categorizing them into three groups.
% \begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
Group-1 covers inappropriate concepts: \emph{nudity},
%(e.g., female breasts or male/female genitalia), 
\emph{violence}, 
%(e.g., bloody scenes, fighting, burning, hanging, weapons, and wars), 
\emph{disturbing}, 
%(e.g., distorted faces, bodies, human flesh, or bodily fluids), 
and \emph{hateful}.
%(e.g., defamatory racial depiction, harmful stereotypes, or Holocaust scenes).
Group-2 covers copyright-infringing concepts: \emph{Grumpy Cat, Nemo, Captain Marvel, Snoopy}, and \emph{R2D2}.
Group-3 covers unauthorized use of images: \emph{Taylor Swift, Angelina Jolie, Brad Pitt}, and \emph{Elon Musk}.
% \end{itemize}


\noindent\textbf{\underline{Step 1: Identifying Acceptable Concepts}}
A good choice of $\cacc$ is one which effectively steers a \tti model away from generating $\imgunacc$ while maintaining utility on other concepts. Hence, the choice of $\cacc$ can impact \ref{effective} and \ref{utility}. 
We select $\cacc$ for a given $\cunacc$ such that it is either opposite to $\cunacc$ (Group-1) or is a semantic generalization of $\cunacc$ so as to avoid infringing copyrights (Groups-2,3).
For $\cunacc$ in Group-1, we consider multiple alternative synonyms for $\cacc$, from which we choose the best possible candidate by measuring effectiveness and utility on a validation dataset (see Step 4).
For $\cunacc$ in Groups-2,3, we use $\cacc$ from prior work for a fair comparison~\cite{kumari2023ablating,heng2023selective}.
We indicate them in the format ``$\cunacc$ $\rightarrow$ $\cacc$''.
For \textbf{Group-1}, $\cacc$ is the opposite of $\cunacc$ and we consider the following choices of $\cacc$: \emph{nudity} $\rightarrow$ \{\emph{clothed} and \emph{clean}\}; \emph{violence} $\rightarrow$ \{\emph{peaceful}, \emph{nonviolent}, and \emph{gentle}\}; \emph{disturbing} $\rightarrow$ \{\emph{pleasing}, \emph{calming}, and \emph{soothing}\}; \emph{hateful} $\rightarrow$ \{\emph{loving}, \emph{compassionate}, and \emph{kind}\}.
For \textbf{Group-2}: $\cacc$ is the broader category of $\cunacc$, following prior works~\cite{kumari2023ablating,heng2023selective,gandikota2023erasing}: \emph{Grumpy Cat} $\rightarrow$ \emph{cat}, \emph{Nemo} $\rightarrow$ \emph{fish}, \emph{Captain Marvel} $\rightarrow$ \emph{female superhero, Snoopy} $\rightarrow$ \emph{dog}, and \emph{R2D2} $\rightarrow$ \emph{robot}. 
For \textbf{Group-3}, $\cacc$ is the sex of $\cunacc$, following prior works~\cite{heng2023selective, zhang2023forgetmenot, kim2023towards}: \{\emph{Taylor Swift, Angelina Jolie}\} $\rightarrow$ \emph{woman} and \{\emph{Brad Pitt, Elon Musk}\} $\rightarrow$ \emph{man}.
We compare \method with each \crt category separately using concepts they were originally evaluated on: Group-1 for filtering \crt{s}~\cite{unsafeDiff}; all groups for fine-tuning \crt{s}~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards}.
% \end{itemize}



% \subsection{Dataset and Model Configurations}\label{sec:datasets}

\noindent\textbf{\underline{Step 2: Generate and Split Datasets}}

% We describe the generation of train, validation, and test datasets.

\noindent\textbf{Train Datasets.}
% We summarize the different training/fine-tuning dataset configurations across \crt{s} in Table~\ref{tab:trconfig}. 
% \input{tables/tab_trconfig}
For \emph{fine-tuning \crt{s}}, 
% Different fine-tuning \crt{s} use different dataset configurations to ensure that \ref{effective} and \ref{utility} are met. 
we use the exact same configuration as described in their original works. 
This configuration for a specific \crt is the same across different concepts.
% While the configuration across different \crt{s} vary, the configuration for a specific \crt across different concepts is the same, in accordance with the instructions in the respective works. 
% We briefly summarize them in Table~\ref{tab:trconfig}. 
\ca uses acceptable prompts which are generated from ChatGPT such that they contain $\cacc$, and 1 image per prompt. \esd and \sdd both use only $\cunacc$, and \sdd additionally uses 10 images corresponding to $\cunacc$. All images are generated using SD v1.4. 
\forgetNot uses unacceptable prompts of the form ``An image of \{$\cunacc$\}'', and 1 image per prompt.
For all of them, we use their code for consistency with their original papers~\cite{githubGitHubNupurkmr9conceptablation,githubGitHubRohitgandikotaerasing,githubGitHubSHILabsForgetMeNot,githubGitHubRohitgandikotaunifiedconceptediting,githubGitHubClearnusselectiveamnesia,githubGitHubNannullnasafediffusion,githubGitHubYitingQuunsafediffusion}.



\noindent For \emph{filtering \crt{s},} we train $\filter_{\unsafediff}$ using the original dataset configuration and code~\cite{unsafeDiff}. 
For \method, we follow \ca~\cite{kumari2023ablating} to generate 10 unacceptable and acceptable prompts using ChatGPT, with one image per prompt from SDv1.4.
For Group-2, we randomly select 10 ChatGPT-generated prompts from \ca~\cite{kumari2023ablating}.
We use a small amount of training data following prior works which show little data is enough to modify CLIP~\cite{yang2023robust,carlini2022poisoning}. This is validated by our results (Section~\ref{sec:evaluation}).



\noindent\textbf{Validation Datasets.}
For validation datasets ($\mathcal{D}_{val}$), we denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalunacc$; and the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalacc$.
For \ref{effective}, we use $\dvalunacc$ by generating 10 unacceptable prompts using ChatGPT, and generate 5 images per prompt using SD v1.4. 
For \ref{utility}, we use $\dvalacc$ by randomly choosing 100 acceptable prompts from the COCO 2014 dataset~\cite{coco}, and 1 image per prompt, from SD v1.4.
% We summarize them in Table~\ref{tab:valconfig}. 

% \input{tables/tab_valconfig}

\noindent\textbf{Test Datasets.} %We now present datasets for evaluating different \crt{s}. 
For test dataset ($\mathcal{D}_{te}$), we denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dtestacc$; and with unacceptable prompts ($\promptuacc$) and corresponding images ($\imgunacc$) as $\dtestunacc$.

% \input{tables/tab_teconfig}

\noindent For evaluating effectiveness (\ref{effective}), we use $\dtestunacc$ which is generated as follows:
For Group-1 concepts (\emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing}), we use Inappropriate Image Prompts (I2P), containing prompts which are likely to generate unsafe images~\cite{schramowski2022safe}.
We process I2P dataset following prior work~\cite{gandikota2023erasing, gandikota2023unified} to obtain 300 unacceptable prompts.
% For \emph{nudity}, I2P includes a ``nudity percentage'' attribute. We choose all unacceptable prompts with a nudity percentage $>10$, resulting in a total of 300 unacceptable prompts, in accordance with prior works~\cite{gandikota2023erasing, gandikota2023unified}.
\unsafediff~\cite{unsafeDiff} also used \emph{political} as a concept, which is excluded from our evaluation since it is not a part of I2P. 
% Note that I2P prompts do not explicitly contain $\cunacc$, \emph{i.e., the words \emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing} are not explicitly included in the prompts}.
For concepts in Group-2,3, there are no standard benchmark datasets. Hence, we use the dataset from prior works~\cite{kumari2023ablating, gandikota2023erasing} with 200 unacceptable images generated from SDv1.4 from 10 unacceptable prompts generated from ChatGPT.
For \ref{utility}, we use the COCO 2014 test dataset as $\dtestacc$, consistent with prior work, with 200 randomly chosen acceptable prompts, non-overlapping with $\dvalacc$.
For \ref{robust}, we use $\dtestadv$ by applying different attacks on $\dtestunacc$ to generate adversarial prompts.
% We summarize the datasets in Table~\ref{tab:teconfig}. 

\noindent\textbf{\underline{Step 3: Fine-tuning with \crt{s}/training filter.}}
Using $\dtrain$, we fine-tune \tti models using six fine-tuning \crt{s} described in Section~\ref{back-attacks}.
% \change{We omit the comparison with more recent works due to ...~\cite{}.}
For filtering \crt{s}, we consider one baseline (\unsafediff) and do not compare with SD-Filter as \unsafediff outperforms it.
We train \unsafediff's classifier on their dataset and we fine-tune \method on $\dtrain$ using Equation~\ref{eq:ft1} for Groups-2,3 concepts and Equation~\ref{eq:ft2} for Group-1 concepts. 
We use the CLIP L-patch-14~\cite{vit} due to its popularity, which is also the default encoder with SDv1.4. However, other variants of CLIP are also applicable.

\noindent\textbf{\underline{Step 4: Select best $\cacc$ using $\mathcal{D}_{val}$}.}
For Group-1 concepts, we evaluate \ref{effective} and \ref{utility} for different candidates of $\cacc$ on $\dvalunacc$ and $\dvalacc$ respectively. 
We found the concepts with the best results: \emph{nudity} $\rightarrow$ \emph{clean}, \emph{violence} $\rightarrow$ \emph{peaceful}, \emph{disturbing} $\rightarrow$ \emph{pleasing}, and \emph{hateful} $\rightarrow$ \emph{loving}.
For \emph{nudity}, we eliminated \emph{clothed} as it blocked images with minimal exposed skin despite being acceptable~\cite{unsafeDiff,schramowski2022safe}.
%
%
% We use concepts in Group-1 following prior work~\cite{unsafeDiff} to evaluate filtering \crt{s}. 
% We use \emph{nudity} and \emph{violence} from Group-1, and all the concepts from Group-2 and Group-3 following prior works~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards} to evaluate fine-tuning \crt{s}. 

% We summarize the final concepts for evaluation in Table~\ref{tab:concepts}.



\noindent\textbf{\underline{Step 5: Evaluation}.} 
We evaluate \ref{effective} on $\dtestunacc$, \ref{utility} on $\dtestacc$, and \ref{robust} on $\dtestadv$, which is generated by running different attacks on $\dtestunacc$ to get $\advprompt$. We pass the prompts from the datasets to the \tti model and compute different metrics.



==> generative-concept-removal/old_versions/WACV/6evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}



\subsection{Impact of Fine-Tuning}\label{sec:finetuningEval}

We first empirically show how fine-tuning can improve the robustness similar to adversarial training in classifiers. Adversarial training~\cite{zhang2019theoretically} explicitly pushes the decision boundary away from training data records. Similarly, our fine-tuning objective, pushes the embeddings of acceptable and unacceptable concepts away from each other. This results in correctly classifying $\prompt_{adv}$ by \method.

To demonstrate this, we generated 10 adversarial prompts, with 5 images per prompt using \cce+. 
We report the mean absolute difference between the cosine similarity of all the $\phi_x(\imgadv)$ and $\phi_p(\cunacc)$ and $\phi_p(\cacc)$ in Table~\ref{tab:advsims}. Across all concepts, using fine-tuning (w/ FT) makes $\phi_x(\imgadv)$ closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$, compared to the baseline without fine-tuning (w/o FT). Hence, fine-tuning is likely to correctly identify $\imgadv$ as $\imgunacc$.

\input{tables/tab_adv_sims}
\input{tables/tab_effectiveness}

Furthermore, we evaluate the impact of fine-tuning on \ref{effective} and \ref{utility}. For \ref{effective}, CLIP accuracy for several concepts is statistically better after fine-tuning: \emph{Angelina Jolie} (0.03 $\pm$ 0.00 from 0.12 $\pm$ 0.02), \emph{Brad Pitt} (0.00 $\pm$ 0.00 from 0.02 $\pm$ 0.01), \emph{Elon Musk} (0.03 $\pm$ 0.00 from 0.07 $\pm$ 0.01). For \ref{utility}, CLIP scores are better for some concepts after fine-tuning: \emph{nudity} (0.94 $\pm$ 0.08 from 0.83 $\pm$ 0.07); \emph{grumpy cat} (0.98 $\pm$ 0.04 from 0.88 $\pm$ 0.03), \emph{Nemo} (0.37 $\pm$ 0.02 from 0.24 $\pm$ 0.05), \emph{R2D2} (0.66 $\pm$ 0.02 from 0.52 $\pm$ 0.03), and \emph{Elon musk} (0.92 $\pm$ 0.02 from 0.97 $\pm$ 0.01).
The metrics for other concepts remains statistically similar.



\input{tables/tab_utility}

\input{tables/tab_robustness}

% We evaluate \method with fine-tuning \crt{s} (Section~\ref{sec:finetuneEval}), and then filtering \crt (Section~\ref{sec:filterEval}). 


\subsection{Comparison with Fine-tuning \crt{s}}\label{sec:finetuneEval}


\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report CLIP accuracy on $\dtestunacc$ in Table~\ref{tab:effectiveness}. 
We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.
All \crt{s} exhibit poor accuracy on \emph{nudity} and \emph{violence}, likely due to fine-tuning \crt{s} being sensitive to input prompts~\cite{pham2024robust, yang2024guardt2i, ma2024jailbreaking}. Specifically, other \crt{s} depend on the $\cunacc$ being included in prompts, which is absent for \emph{nudity} and \emph{violence} prompts in the I2P dataset.
\method consistently maintains high accuracy on the I2P benchmark dataset as it classifies the generated images. 
\esd, and \sdd have better accuracy compared to the other three fine-tuning \crt{s}. 
This could be attributed to their similar optimizations which includes fine-tuning \dm, conditioned on $\cunacc$, to match the unconditioned \dm to reduce the influence of $\cunacc$ on the output.  
For \unifiedCE, we attribute the higher effectiveness to directly removing the influence of $\cunacc$ from the \tti model parameters. \textbf{\textit{Overall, \method is more effective than other fine-tuning \crt{s}.}}



\noindent\textbf{\underline{\ref{utility} Utility.}} We report normalized CLIP scores in Table~\ref{tab:utility} on $\dtestacc$.
We use \colorbox{mynicered}{red} if score is between 50-70, \colorbox{myniceblue}{blue} if between 70-90; \colorbox{mynicegreen}{green} if $>$90.
All the fine-tuning \crt{s} perform well across all concepts (either \colorbox{myniceblue}{blue} or \colorbox{mynicegreen}{green}) since the explicitly account for \ref{utility}. We observe that \ca with KL-Divergence-based optimization for cross-attention layers, and \unifiedCE with a precise closed-form solution to model updates, preserve \ref{utility} better than others. 
%
\method has high utility for all concepts except for \emph{violence}, and Group-2 concepts (\emph{Nemo}, \emph{Captain Marvel}, \emph{Snoopy}, and \emph{R2D2}).
During fine-tuning, there is a trade-off between \ref{effective} and \ref{utility}. 
For \textit{violence}, we observed an early decrease in utility during the very first epoch resulting in poor trade-off. 
For Group-2 concepts, we attribute the poor utility to the ambiguity in the unacceptable concepts. For instance, \emph{Nemo} is both a fish and a ship captain~\cite{VERNE_2024}, and \emph{Captain Marvel} represents both a male and a female superhero~\cite{Friedwald_2019_marvel}. 
To verify this, we precisely specify the unacceptable concepts to reduce ambiguity: as \emph{Nemo}$\rightarrow$ \emph{Nemo fish}, \emph{Captain Marvel}$\rightarrow$ \emph{Captain Marvel female superhero}, \emph{Snoopy}$\rightarrow$ \emph{Snoopy dog}, and \emph{R2D2}$\rightarrow$ \emph{R2D2 robot}. We evaluate \method on $\dvalacc$:
compared to the results in Table~\ref{tab:utility}, the normalized CLIP score for this new configuration is: 0.97 $\pm$ 0.00 (\emph{Nemo fish}), 0.90 $\pm$ 0.02 (\emph{Captain Marvel female superhero}), 0.98 $\pm$ 0.03 (\emph{Snoopy dog}), 0.92 $\pm$ 0.02 (\emph{R2D2 robot}), which are now labeled as \colorbox{mynicegreen}{green}.
We also evaluate effectiveness (\ref{effective}) and find that the CLIP accuracy is similar to Table~\ref{tab:effectiveness}.
% We also report the CLIP accuracy on $\dvalunacc$ to evaluate \ref{effective} with this new configuration: 0.02 $\pm$ 0.00 (\emph{Nemo fish}), 0.00 $\pm$ 0.00 (\emph{Captain Marvel female superhero}), 0.02 $\pm$ 0.01 (\emph{Snoopy dog}), 0.00 $\pm$ 0.00 (\emph{R2D2 robot}), which are effective, same as before. Hence, precisely specifying $\cunacc$ is important for \method and can satisfy \ref{utility} without sacrificing \ref{effective}. 
\textbf{\textit{Overall, \method's utility (\ref{utility}) is comparable to prior works.}}


\noindent\textbf{\underline{\ref{robust} Robustness.}} We report CLIP accuracy on $\dtestadv$ in Table~\ref{tab:robust}. 
% We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.
We evaluate different \crt{s} against \typo+, \pez+, \cce/\cce+, and \ringbell+. We use the same color coding as in \ref{effective}. 
%
\cce/\cce+, being a white-box attack that uses the parameters of the entire \tti model, is the most powerful attack and renders all fine-tuning \crt{s} ineffective. However, \method is robust against \cce/\cce+ and outperforms all fine-tuning \crt{s}.
On the remaining attacks, all the fine-tuning \crt{s} have better robustness on Group-3 concepts than on Group-1 and 2. We attribute this to the difficulty of \tti models in generating high quality celebrity faces while also evading detection, as also observed in prior work~\cite{Matthias_2023}.
As expected, we note that all \crt{s} perform poorly on \emph{nudity} and \emph{violence} across all the attacks as they do not satisfy \ref{effective}.
% Hence, adversarial prompts for these concepts are likely to easily evade them. 
\textbf{\emph{Overall, \method is more robust than all prior work across all the concepts and attacks.}}
% We discuss the possibility of future attacks against \method in Section~\ref{sec:future}.



% \noindent\textbf{\underline{Summary.}} 
% We depict the trade-offs among \ref{effective}, \ref{utility}, and \ref{robust} in Figure~\ref{fig:radarsFT}. We use (1-CLIP accuracy) for \ref{effective} on $\dtestunacc$, normalized CLIP score on $\dtestacc$ for \ref{utility}, and (1-CLIP accuracy) for \ref{robust} on $\dtestadv$ using \cce/\cce+. 
% For each of the requirements, we use the average across all concepts as the representative value for a \crt.
% \emph{Overall, \method provides a better trade-off across the three requirements compared to all the fine-tuning \crt{s}.}

% \input{figures/fig_radar_ft}

































\subsection{Comparison with Filtering \crt}\label{sec:filterEval}

% We now compare with \unsafediff~\cite{unsafeDiff}, the state-of-the-art filtering \crt, across the three requirements and summarize the results. 
% To compare with \unsafediff~\cite{unsafeDiff}, we use FNR to evaluate effectiveness on $\dtestunacc$, FPR for utility on $\dtestacc$, and FNR for robustness on $\dtestadv$.




\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report FNR across four concepts (\emph{nudity}, \emph{violence}, \emph{disturbing}, and \emph{hateful}) in Table~\ref{tab:FilterEffective}.
We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FNR is $<$0.25.
\method has better FNR for three of the four concepts: \emph{nudity}, \emph{violence} (in \colorbox{mynicegreen}{green}), and \emph{hateful} (\colorbox{myniceblue}{blue} for \method and \colorbox{mynicered}{red} for \unsafediff). However, both \method and \unsafediff perform poorly on \emph{disturbing}. 
We attribute this poor effectiveness on Group-1 concepts to the subjective description of $\cunacc$. Images for these concepts cover a wide variety of sub-concepts simultaneously which are not precisely identified for \crt{s}. 
\emph{\textbf{Overall, \method is more effective than \unsafediff on most concepts.}}

\input{tables/tab_filter_effective}



\noindent\textbf{\underline{\ref{utility} Utility.}} We present FPR in Table~\ref{tab:FilterUtility} and use \colorbox{mynicered}{red} if FPR is $>$0.50, \colorbox{myniceblue}{blue} if FPR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FPR is $<$0.25. As expected, we observe that both \emph{\textbf{\method and \unsafediff have comparable utility as they demonstrate a low FPR}}. \unsafediff explicitly includes images containing $\cacc$ while training the multi-headed classifier.

\input{tables/tab_filter_utility}

\noindent\textbf{\underline{\ref{robust} Robustness.}} We report FNR on the dataset for adversarial prompts and corresponding images in Table~\ref{tab:FilterRobust}. 
We use the same color-coding as \ref{effective}.
% We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; and \colorbox{mynicegreen}{green} if FNR is $<$0.25.
In addition to the four attacks from Table~\ref{tab:robust}, recall that \sneaky~\cite{yang2023sneakyprompt} is specifically designed to attack filtering \crt{s}. Hence, we also include the evaluation against \sneaky. 
Also, since \cce is not adaptive against filtering \crt's, we evaluate \unsafediff and \method against \cce+. We are the first to evaluate different attacks against \unsafediff.
%
\input{tables/tab_filter_robust}
%
We observe that \method is effective against \pez+ while \unsafediff can be evaded.
On all the remaining attacks, we show that \method is robust on more concepts than \unsafediff.
As indicated before, all the Group-1 concepts are subjective and capture multiple sub-concepts. This ambiguity could be the reason for poor \ref{robust}.
\emph{\textbf{Overall, \method is more robust than \unsafediff on a majority of the concepts across various attacks.}}

% \input{figures/fig_radar_filter}

\subsection{Summary}


\begin{figure}[h]
\centering
\begin{minipage}{0.5\columnwidth}
\includegraphics[width=1\columnwidth]{figures/radar_ft.pdf}
\subcaption{Fine-tuning \crt{s}.}
\end{minipage}%
\begin{minipage}{0.5\columnwidth}
\includegraphics[width=1\columnwidth]{figures/radar_filter.pdf}
\subcaption{Filtering \crt (\unsafediff)}
\end{minipage}
\caption{\method has better trade-offs than other \crt{s}}
\label{fig:summary}
\end{figure}

\noindent We depict the trade-offs among \ref{effective}, \ref{utility}, and \ref{robust} in Figure~\ref{fig:summary} across various \crt{s}.
For fine-tuning \crt{s}, we use (1-CLIP accuracy) for \ref{effective} on $\dtestunacc$, normalized CLIP score on $\dtestacc$ for \ref{utility}, and (1-CLIP accuracy) for \ref{robust} on $\dtestadv$ using \cce/\cce+ (the strongest attack among others). 
For filtering \crt, we use (1- FNR) on $\dtestunacc$ for \ref{effective}, (1- FPR) on $\dtestacc$ for \ref{utility}, and (1- FNR) on $\dtestadv$ using \cce+ for \ref{robust}.
For each of the requirements, we use the average across all concepts as the representative value for a \crt.
\emph{\textbf{Overall, \method provides a better trade-off across the three requirements compared to all the prior work.}}





==> generative-concept-removal/old_versions/WACV/9discussion.tex <==
\section{Discussion and Future Work}\label{sec:discussions}

% We revisit our discussion on robustness  (Section~\ref{sec:future}), applicability/extensions of \method (Section~\ref{sec:extensions}), and a summary of this work (Section~\ref{sec:summary}).




% \subsection{Revisiting Robustness}\label{sec:future}

% \noindent\textbf{Addressing Future Attacks.} Recall that our certified robustness bound is loose (Section~\ref{sec:bound}). We leave the improvement of the bound as future work.

% \method maintains high robustness across all evaluated concepts. 
% The design of new attacks which can preserve unacceptable concepts while evading \method is an open problem. Here, adversarial training for \method can be used to increase its robustness.
% We can fine-tune CLIP with this objective: $\mathcal{L}_{\text{Con-adv}}(\dtestadv)=$
% \[- \frac{1}{N} \sum_{j = 1}^N \log \frac{\exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(\cunacc))/ \tau)}{\sum_{k \in \{a,u\}} \exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(c_k))/ \tau)}\]
% where $\mathcal{D}_{adv} = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$. Assuming $\imgadv$ evades the filter, we optimize $\phi_p$ and $\phi_x$, such that $\phi_p(\imgadv_j)$ is closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$. This loss would be added to Equation~\ref{eq:ft1} and~\ref{eq:ft2}. 
% Empirical evaluation of adversarially-trained \method is left as future work.


% \noindent\textbf{Extending the Theoretical Bound to Prompts.} 
% % Although \adv cannot modify text embeddings in practice, analyzing robustness in the CLIP embedding space is valuable as recent works have shown that small changes in the text embeddings of prompts, allow for fine-grained control over their generated images~\cite{yu2024uncovering, kawar2023imagic}. 
% To extend our theoretical bounds in Theorem~\ref{thm.1} to the prompt space,
% we assume Lipschitz continuity, commonly used in ML~\cite{bousquet2002stability}, certified robustness~\cite{li2023sok}, and more recently in the context of \tti models~\cite{chen2024your}.
% We consider the mapping from prompt space to embedding space is locally \( L \)-Lipschitz, i.e., the function \( \phi_x(f(\text{\prompt})) \) satisfies the following condition:

% For each prompt \(\text{\prompt}\), there exists a \(\delta_{\text{\prompt}} > 0\) such that
% $
% ||\phi_x(f(\text{\prompt})) - \phi_x(f(\text{\prompt} + \delta_{\text{\prompt}}))|| \leq L ||\delta_{\text{\prompt}}||.
% $

% Then, the inequality in Equation~\ref{eq:bound} can be related to the prompt space by a scalar factor \(\frac{1}{L}\). 
% Therefore, when \(\|\delta_{\text{\prompt}}\| \leq \frac{1}{L} \|\delta\|\), where \(\|\delta\|\) satisfies inequality in Equation~\ref{eq:bound}, the difference in embedding space will be bounded by \(\|\delta\|\), and CLIP remains robust.


% \subsection{Applications and Extensions to \method}\label{sec:extensions}


\noindent\textbf{Filtering Multiple Concepts.} UCE~\cite{gandikota2023unified} removes multiple concepts simultaneously.
\method can be extended by including multiple concepts simultaneously as well. Specifically, for \method in Equation~\ref{eq:att}, instead of specifying $\cunacc$ and $\cacc$ for a single concept, we can include $\cunacc$ and $\cacc$ for multiple concepts as a list. This is a simple configuration change compared to other filters which require retraining (e.g.,~\cite{unsafeDiff}). 
% Since none of the prior filtering \crt{s} evaluate multiple $\cunacc$, 
We leave the evaluation as future work.
% \change{Tried to add comment; didn't work so here it is: we said that none of prior crts evaluate against multiple concepts but cite gandikota as 1 crt that does, should we say "no other" prior crts?}. 

% \noindent\textbf{Filtering Artistic Styles.} 
% None of the prior filtering \crt{s} consider any copyrighted content and focus on only \emph{inapproriate Group-1 concepts}. 
% \method is the first filtering \crt which is applicable to concepts which are copyright-infringing (Group-2) or involve unauthorized use of personalized images (Group-3).
% Prior fine-tuning \crt{s} have considered removing artistic styles (e.g., painting in the style of Monet or Van Gogh) as copyrighted content~\cite{kumari2023ablating,gandikota2023erasing}.
% However, we observed that \method does not differentiate between images with and without artistic styles very well. Specifically, \emph{Monet painting} as $\cunacc$ and \emph{painting} as $\cacc$, are very similar for \method, thus reducing its effectiveness. We leave the optimization of \method to account for artistic styles as future work.

\noindent\textbf{Applicability to other \tti Models.} Fine-tuning \crt{s} are specific to particular stable diffusion models due to their tailored optimizations for \tti models. In contrast, filtering \crt{s} offer versatility as they can be applicable to any \tti model. 
Filters analyze only the generated image and the list of concepts, independent of the \tti model. 
And fine-tuning the filter using data from \tti model, as we do for \method, can satisfy \ref{effective} and \ref{utility}. 
This allows us to have a filter that will work with \tti models in different domains (e.g., anime images).
Explicit evaluation of \method for different \tti models is deferred to future work.


% \noindent\textbf{Summary.} Removing unacceptable concepts from \tti models is an important problem. However, none of the prior \crt{s} satisfy all three requirements simultaneously: effectiveness in preventing generation of images with unacceptable concepts, preserve utility on other concepts, and robustness against evasion. We propose \method, the \emph{first} robust \underline{co}ncept \underline{fi}ltering \crt which provides a better trade-off among the three requirements compared to prior \crt{s}.

==> generative-concept-removal/proofs/proof.tex <==
\begin{proof}
    For an unacceptable image embedding $\hat{x} = \phi_x(\imgunacc)$,
    % We assume that $F(\hat{x})=1$ and 
    $g(\hat{x}):=g_u(\hat{x})$, then $g(\hat{x})-\Gamma>0$, and $\Gamma$ is the decision threshold for classification.
    Let $s_1=\tau\text{cos}(\hat{x},\cunaccc)$, $s_2=\tau\text{cos}(\hat{x},\caccc)$, $\textbf{s}=[s_1,s_2]^T$, 
    then
    $$g(\hat{x})=S(s_1) = \frac{exp(s_1)}{exp(s_1)+exp(s_2)},$$
    where $S(s_1)$ is the first item of Softmax function with respect to $\textbf{s}$.
    Then, we have $\frac{\partial}{\partial s_1} S = S(s_1)(1-S(s_1))\leq0.25, \frac{\partial}{\partial s_2} S = -S(s_1)S(s_2)\leq0.25$.

    Note that $||\hat{x}||>0$ and $||\caccc||>0$,
    we have 
    \begin{equation*}
    \begin{aligned}
        ||\frac{\partial}{\partial \hat{x}} s(\hat{x},\caccc)|| = ||\frac{\tau||\caccc||(I-xx^T)\caccc}{||\hat{x}||||\caccc||^2}||\\=\frac{\tau sin(\hat{x},\caccc)}{||\hat{x}||}\leq\frac{\tau}{||\hat{x}||}.
    \end{aligned}
    \end{equation*}
    And $||\frac{\partial}{\partial\hat{x}} s(\hat{x}, \cunaccc)||\leq\frac{\tau}{||\hat{x}||}$. 

    For each $\hat{x}$, according to the chain rule of composition functions, 
    $\frac{\partial}{\partial\hat{x}}g(\hat{x)}=\frac{\partial S}{\partial s_1}\cdot\frac{\partial s_1}{\hat{x}}+ \frac{\partial S}{\partial s_2}\cdot\frac{\partial s_2}{\hat{x}}\leq \frac{\tau}{2||\hat{x}||}$. Therefore the Lipschitz constant of $g(\hat{x})$ with respect to $\hat{x}$ is $\frac{\tau}{2||\hat{x}||}$, and
    \begin{equation*}
    \begin{aligned}
            ||g(\hat{x}+\delta)-g(\hat{x})||&\leq\frac{1}{2}\frac{\tau }{\min\{||u|||u\in U(\hat{x},\delta)\}} ||\delta||\\&\leq\frac{1}{2}\frac{\tau }{|||\hat{x}||-||\delta|||}||\delta||,
    \end{aligned}
    \end{equation*}
    where $U(\hat{x},\delta)$ is a $l_2$-ball of $\hat{x}$ with radius $\delta$.   
    
    When
    $||\delta||\leq(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|})||\hat{x}||<||\hat{x}||$, we have
    \begin{equation*}
    \begin{aligned}
        |g(\hat{x}+\delta)-g(\hat{x})|&=||g(\hat{x}+\delta)-g(\hat{x})||\\& \leq\frac{\tau }{2\left(\frac{||\hat{x}||}{||\delta||}-1\right)}\\
        &\leq\frac{\tau }{2\left(\frac{\tau +2|g(\hat{x})-\Gamma|}{2|g(\hat{x})-\Gamma|}-1\right)}\\
        &\leq|g(\hat{x})-\Gamma|=g(\hat{x})-\Gamma.
    \end{aligned}
    \end{equation*}
    Then,
    \begin{equation}
    \begin{aligned}
        g(\hat{x}+\delta)\geq|g(\hat{x})|-|g(\hat{x}+\delta)-g(\hat{x})|
        \\\geq g(\hat{x})- |g(\hat{x})-\Gamma|\geq \Gamma,
    \end{aligned}
    \end{equation}
    which concludes the proof.
    
\end{proof}

==> generative-concept-removal/tables/tab_adv_sims.tex <==
\begin{table}[ht]
\caption{Mean difference of the absolute cosine similarities between $\phi_x(\imgadv)$ and each of $\phi_p(\cunacc)$ and $\phi_p(\cacc)$: $|\cos(\phi_x(\imgadv),\phi_p(\cunacc))| - |\cos(\phi_x(\imgadv), \phi_p(\cacc))|$. With finetuning (w/ FT), the mean difference is consistently higher than without finetuning (w/o FT), implying better robustness.}
% Mean absolute difference between the cosine similarity of all the $\phi_x(\imgadv)$ and $\phi_p(\cunacc)$ and $\phi_p(\cacc)$.
\centering
\footnotesize
\begin{tabular}{ l|c|c } 
\bottomrule

\toprule
\textbf{Concept} & \textbf{w/o FT} & \textbf{w/ FT} \\
\midrule
\textbf{Nudity} &  10.28 $\pm$ 0.01 &  16.82 $\pm$ 0.03   \\
\textbf{Violence} & 4.45 $\pm$ 0.00 & 6.92 $\pm$ 0.01 \\
\midrule
\textbf{Grumpy Cat} & 7.48 $\pm$ 0.00 & 8.77 $\pm$ 0.00 \\
\textbf{Nemo} & 3.88 $\pm$ 0.01 & 5.03 $\pm$ 0.01 \\
\textbf{Captain Marvel} & 5.46 $\pm$ 0.00 &  5.48 $\pm$ 0.01  \\
\textbf{Snoopy} & 9.12 $\pm$ 0.01 &  10.17 $\pm$ 0.02 \\
\textbf{R2D2} & 5.79 $\pm$ 0.00 & 8.35 $\pm$ 0.00 \\
\midrule
\textbf{Taylor Swift} & 4.79 $\pm$ 0.01 &  4.87 $\pm$ 0.00  \\
\textbf{Angelina Jolie} & 5.54 $\pm$ 0.02 & 5.64 $\pm$ 0.00 \\
\textbf{Brad Pitt} & 6.81 $\pm$ 0.01 & 6.95 $\pm$ 0.00 \\
\textbf{Elon Musk} & 2.67 $\pm$ 0.01 &  2.71 $\pm$ 0.00 \\
\bottomrule

\toprule
 \end{tabular}
\label{tab:advsims}
\end{table}


==> generative-concept-removal/tables/tab_alpha_effectiveness.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{Alpha (Effectiveness)}: Comparison of different $\alpha_{(.)}$ values using FNR on \emph{unacceptable} prompts in $\dvalunacc$ (lower is better).}
\footnotesize
% \resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c c c c}
\bottomrule

\toprule
\textbf{Concepts}
& \textbf{0.25} & \textbf{0.5} & \textbf{1} & \textbf{1.5} & \textbf{2} \\
\midrule 
\textbf{Nudity}  & 0.01 $\pm$ 0.02 & 0.03 $\pm$ 0.03 & 0.03 $\pm$ 0.01 & 0.09 $\pm$ 0.05 & 0.08 $\pm$ 0.07 \\
\textbf{Violence}  & 0.36 $\pm$ 0.00 & 0.22 $\pm$ 0.08 & 0.24 $\pm$ 0.09 & 0.27 $\pm$ 0.07 & 0.34 $\pm$ 0.01\\
\bottomrule

\toprule
\end{tabular}
% }
\label{tab:AlphaEffective}
\end{table}



==> generative-concept-removal/tables/tab_alpha_sum.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{Alpha (Sum)}: Comparison of different $\alpha_{(.)}$ values using mean FPR on acceptable prompts in $\dvalacc$ and mean FNR on unacceptable prompts in $\dvalunacc$(lower is better).}
\footnotesize
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c c c c}
\bottomrule

\toprule
\textbf{Concepts}
& \textbf{0.25} & \textbf{0.5} & \textbf{1} & \textbf{1.5} & \textbf{2} \\
\midrule 
\textbf{Nudity}  & 0.27 & 0.23 & 0.09 & 0.13 & 0.15 \\
\textbf{Violence}  & 0.81 & 0.86 & 0.74 & 0.76 & 0.91\\
\bottomrule

\toprule
\end{tabular}
}
\label{tab:AlphaSum}
\end{table}

==> generative-concept-removal/tables/tab_alpha_utility.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{Alpha (Utility)}: Comparison of different $\alpha_{(.)}$ values using FPR on \emph{acceptable} prompts in $\dvalacc$ (lower is better).}
\footnotesize
% \resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c c c c}
\bottomrule

\toprule
\textbf{Concepts}
& \textbf{0.25} & \textbf{0.5} & \textbf{1} & \textbf{1.5} & \textbf{2} \\
\midrule 
\textbf{Nudity}  & 0.26 $\pm$ 0.09 & 0.20 $\pm$ 0.04 & 0.06 $\pm$ 0.05 & 0.04 $\pm$ 0.01 & 0.07 $\pm$ 0.01 \\
\textbf{Violence}  & 0.45 $\pm$ 0.07 & 0.64 $\pm$ 0.03 & 0.50 $\pm$ 0.08 & 0.52 $\pm$ 0.07 & 0.57 $\pm$ 0.02\\
\bottomrule

\toprule
\end{tabular}
% }
\label{tab:AlphaUtility}
\end{table}

==> generative-concept-removal/tables/tab_alphas.tex <==

\begin{table*}[!htb]
    \centering
    \caption{\underline{Choosing $\alpha_{(.)}$}: Comparing FNR, FPR, and their sum for different $\alpha_{(\cdot)}$ (lower is better). \textit{\textbf{Bold}} indicates the smallest sum.}
    \resizebox{2\columnwidth}{!}{
    \begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|}
        \hline
        $\alpha_{(\cdot)}$ & \multicolumn{3}{c|}{\textbf{0.25}} & \multicolumn{3}{c|}{\textbf{0.5}} & \multicolumn{3}{c|}{\textbf{1}} & \multicolumn{3}{c|}{\textbf{1.5}} & \multicolumn{3}{c|}{\textbf{2}} \\
        \hline
         & \textbf{FNR} & \textbf{FPR} & \textbf{Sum} & \textbf{FNR} & \textbf{FPR} & \textbf{Sum} & \textbf{FNR} & \textbf{FPR} & \textbf{Sum} & \textbf{FNR} & \textbf{FPR} & \textbf{Sum} & \textbf{FNR} & \textbf{FPR} & \textbf{Sum} \\
        \hline
        \textbf{Nudity} & 0.01 $\pm$ 0.02 & 0.26 $\pm$ 0.09 & 0.27 & 0.03 $\pm$ 0.03 & 0.20 $\pm$ 0.04 & 0.23 & 0.03 $\pm$ 0.01 & 0.06 $\pm$ 0.05 & \textbf{\textit{0.09}} & 0.09 $\pm$ 0.05 & 0.04 $\pm$ 0.01 & 0.13 & 0.08 $\pm$ 0.07 & 0.07 $\pm$ 0.01 & 0.15 \\
        \textbf{Violence} & 0.36 $\pm$ 0.00 & 0.45 $\pm$ 0.07 & 0.81 & 0.22 $\pm$ 0.08 & 0.64 $\pm$ 0.03 & 0.86 & 0.24 $\pm$ 0.09 & 0.50 $\pm$ 0.08 & \textbf{\textit{0.74}} & 0.27 $\pm$ 0.07 & 0.52 $\pm$ 0.07 & 0.79 & 0.34 $\pm$ 0.01 & 0.57 $\pm$ 0.02 & 0.91 \\
        \hline
    \end{tabular}
    }
    \label{tab:Alphas}
\end{table*}

==> generative-concept-removal/tables/tab_certified.tex <==
\begin{table*}[ht]
\centering
\caption{Certified accuracy of \method on different concepts on varying $\delta$.}
\footnotesize
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Concept}} & \multicolumn{10}{c}{\textbf{$\delta$}}\\
 & 0.00 & 0.05 & 0.10 & 0.15 & 0.20 & 0.25 & 0.30 & 0.35 & 0.40 & 0.45 \\ 
 \midrule
 \textbf{Nudity} & 0.85 $\pm$ 0.08 & 0.80 $\pm$ 0.40 & 0.80 $\pm$ 0.41 & 0.80 $\pm$ 0.41 & 0.79 $\pm$ 0.41 & 0.77 $\pm$ 0.42 & 0.74 $\pm$ 0.44 & 0.50 $\pm$ 0.50 & 0.00 $\pm$ 0.08 & 0.00 $\pm$ 0.00  \\
\midrule
\textbf{Violence} & 0.81 $\pm$ 0.40 & 0.81 $\pm$ 0.40 & 0.79 $\pm$ 0.41 & 0.76 $\pm$ 0.43 & 0.73 $\pm$ 0.44 & 0.69 $\pm$ 0.46 & 0.62 $\pm$ 0.48 & 0.31 $\pm$ 0.46 & 0.01 $\pm$ 0.08 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Grumpy Cat} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.88 $\pm$ 0.32 & 0.44 $\pm$ 0.51 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Nemo} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.93 $\pm$ 0.25 &  0.93 $\pm$ 0.25 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.87 $\pm$ 0.35 & 0.77 $\pm$ 0.43 & 0.10 $\pm$ 0.31 & 0.00 $\pm$ 0.00  \\
\midrule 
\textbf{R2D2} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.13 $\pm$ 0.35 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 \\
\midrule
\textbf{Snoopy} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.63 $\pm$ 0.49 & 0.07 $\pm$ 0.25 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00  \\
\midrule
\textbf{Captain Marvel} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.91 $\pm$ 0.25 & 0.03 $\pm$ 0.00 & 0.00 $\pm$ 0.00  \\
\midrule
\textbf{Taylor Swift} & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.73 $\pm$ 0.45 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Angelina Jolie} & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.80 $\pm$ 0.41 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Brad Pitt} & 0.99 $\pm$ 0.01 & 0.99 $\pm$ 0.01 & 0.93 $\pm$ 0.25 & 0.93 $\pm$ 0.25 & 0.90 $\pm$ 0.31 & 0.90 $\pm$ 0.31 & 0.90 $\pm$ 0.31 & 0 .73 $\pm$ 0.45 & 0.07 $\pm$ 0.25 & 0.00 $\pm$ 0.00 \\
\midrule
\textbf{Elon Musk} & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.73 $\pm$ 0.45 & 0.63 $\pm$ 0.49 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00  \\
\bottomrule
\end{tabular}
\label{tab:certified}
\end{table*}

==> generative-concept-removal/tables/tab_concepts.tex <==
\begin{table}[h]
\caption{Summary of unacceptable concepts ($\cunacc$), acceptable concepts ($\cacc$), and whether we use them to evaluate fine-tuning \crt{s}, filtering \crt{s}, or both.}
\centering
\footnotesize
\begin{tabular}{ c |  l | c}
\hline
 \textbf{Type} & \textbf{$\cunacc$ $\rightarrow$ $\cacc$} & \textbf{\crt(s)}\\ 
 \hline
 \multirow{4}{*}{\textbf{Group-1}} & \emph{Nudity} $\rightarrow$ \emph{Clean} & Both \\ 
 & \emph{Violence} $\rightarrow$ \emph{Peaceful} & Both \\ 
& \emph{Disturbing} $\rightarrow$ \emph{Pleasing} & Filtering \\ 
& \emph{Hateful} $\rightarrow$ \emph{Loving} & Filtering \\ 
\hline
\multirow{5}{*}{\textbf{Group-2}} & \emph{Grumpy Cat} $\rightarrow$ \emph{Cat} & Fine-tuning \\ 
 & \emph{Nemo} $\rightarrow$ \emph{Fish} & Fine-tuning \\ 
 & \emph{Captain Marvel} $\rightarrow$ \emph{Female Superhero} & Fine-tuning \\
 & \emph{Snoopy} $\rightarrow$ \emph{Dog} & Fine-tuning \\
 & \emph{R2D2} $\rightarrow$ \emph{Robot} & Fine-tuning \\
 \hline
 \multirow{4}{*}{\textbf{Group-3}} & \emph{Taylor Swift} $\rightarrow$ \emph{Woman} & Fine-tuning \\ 
 & \emph{Angelina Jolie} $\rightarrow$ \emph{Woman} & Fine-tuning \\ 
 & \emph{Brad Pitt} $\rightarrow$ \emph{Man} & Fine-tuning \\ 
 & \emph{Elon Musk} $\rightarrow$ \emph{Man} & Fine-tuning \\ 
 \hline
\end{tabular}
% \end{center}
\label{tab:concepts}
\end{table}

==> generative-concept-removal/tables/tab_effectiveness.tex <==
\begin{table*}[h]
\caption{\underline{\ref{effective} Effectiveness:} Comparison of fine-tuning \crt{s} using CLIP accuracy on \emph{acceptable} prompts in $\dtestunacc$ (lower is better). We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.} 
% \begin{center}
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ l|c|c|c|c|c|c|c|c|c|c|c } 
\bottomrule

\toprule
 \multirow{3}{*}{\textbf{CRT}} & \multicolumn{11}{c}{\textbf{Concepts}}\\
  & \textbf{Nudity} & \textbf{Violence} & \textbf{Grumpy} & \multirow{2}{*}{\textbf{Nemo}} & \textbf{Captain} & \multirow{2}{*}{\textbf{Snoopy}} & \multirow{2}{*}{\textbf{R2D2}} & \textbf{Taylor} & \textbf{Angelina} & \textbf{Brad} & \textbf{Elon}\\
  & \textbf{(I2P)} & \textbf{(I2P)} & \textbf{Cat} &  & \textbf{Marvel} &  &  &  \textbf{Swift} & \textbf{Jolie} & \textbf{Pitt} & \textbf{Musk}\\
\midrule
\texttt{CA}~\cite{kumari2023ablating} & \cellcolor{mynicered!35} 0.82 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.78 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.02 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.40 $\pm$ 0.05 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.05 & \cellcolor{mynicegreen!35}0.13 $\pm$ 0.02 & \cellcolor{mynicered!35}0.73 $\pm$ 0.05 & \cellcolor{mynicered!35}0.83 $\pm$ 0.02 & \cellcolor{mynicered!35}0.86 $\pm$ 0.04 & \cellcolor{mynicered!35}0
.64 $\pm$ 0.03 \\ 
\forgetNot~\cite{zhang2023forgetmenot} & \cellcolor{mynicered!35} 0.83 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.64 $\pm$ 0.04 & \cellcolor{myniceblue!35}0.34 $\pm$ 0.02 & \cellcolor{mynicered!35}0.61 $\pm$ 0.01 & \cellcolor{mynicered!35}0.82 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.16 $\pm$ 0.00 & \cellcolor{mynicered!35}0.89 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.45 $\pm$ 0.02 & \cellcolor{mynicered!35}0.59 $\pm$ 0.06 & \cellcolor{mynicered!35}0.79 $\pm$ 0.04 &\cellcolor{mynicered!35} 0.56 $\pm$ 0.22 \\ 
\sa~\cite{heng2023selective} & 
\cellcolor{mynicered!35} 0.69 $\pm$ 0.09 & 
\cellcolor{mynicered!35} 0.69 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.16 $\pm$ 0.00 & \cellcolor{mynicered!35}0.87 $\pm$ 0.04 & \cellcolor{mynicered!35}0.93 $\pm$ 0.02 & \cellcolor{mynicered!35}0.55 $\pm$ 0.07 & \cellcolor{mynicered!35}0.98 $\pm$ 0.01 & \cellcolor{mynicered!35}0.82 $\pm$ 0.05 & \cellcolor{myniceblue!35}0.49 $\pm$ 0.04 & \cellcolor{mynicered!35}0.63 $\pm$ 0.05 & \cellcolor{mynicered!35}0.75 $\pm$ 0.04 \\ 
\esd~\cite{gandikota2023erasing} & 
\cellcolor{mynicered!35} 0.62 $\pm$ 0.06 & 
\cellcolor{mynicered!35} 0.63 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.28 $\pm$ 0.06 & \cellcolor{mynicered!35}0.64 $\pm$ 0.06 & \cellcolor{myniceblue!35}0.37 $\pm$ 0.04 & \cellcolor{mynicegreen!35}0.20 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.41 $\pm$ 0.04 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.29 $\pm$ 0.05 & \cellcolor{mynicegreen!35}0.17 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.17 $\pm$ 0.02 \\ 
\unifiedCE~\cite{gandikota2023unified} &
\cellcolor{mynicered!35}0.70 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.71 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.43 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.40 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.02 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.10 $\pm$ 0.01 \\ 
\sdd~\cite{kim2023towards} & 
\cellcolor{mynicered!35} 0.57 $\pm$ 0.02 & 
\cellcolor{mynicered!35}0.55 $\pm$ 0.02 & 
\cellcolor{mynicegreen!35}0.20 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.20 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.41 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.37 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.39 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 \\ 
\moderator~\cite{wang2024moderator} & 
\cellcolor{mynicered!35} 0.87 $\pm$ 0.02 & 
\cellcolor{mynicered!35}0.92 $\pm$ 0.05 & 
\cellcolor{mynicegreen!35}0.02 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.25 $\pm$ 0.02 & \cellcolor{mynicered!35}0.73 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.28 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.09 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.13 $\pm$ 0.04 \\ 
% \textbf{\method} & 
%  \cellcolor{mynicegreen!35}0.12 $\pm$ 0.05 & 
%   \cellcolor{mynicegreen!35}0.24 $\pm$ 0.05 & 
%   \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 \\ 
\midrule
 \textbf{\method} & 
  \cellcolor{mynicegreen!35}0.15 $\pm$ 0.06& 
   \cellcolor{mynicegreen!35}0.20 $\pm$ 0.05 & 
  \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 &
  \cellcolor{mynicegreen!35} 0.10 $\pm$ 0.02 & 
  \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.01& 
  \cellcolor{mynicegreen!35} 0.08 $\pm$ 0.02& 
  \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & 
   \cellcolor{mynicegreen!35}0.02 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.00 \\ 
\bottomrule

\toprule
 \end{tabular}
}
% \end{center}
\label{tab:effectiveness}
\end{table*}

==> generative-concept-removal/tables/tab_efficiency.tex <==
\begin{table}[!htb]
\centering
\caption{\crt training time averaged across ten runs.}
\footnotesize
\begin{tabular}{  l c | l c  }
\bottomrule

\toprule
\textbf{Technique} & \textbf{Time (mins)} & \textbf{Technique} & \textbf{Time (mins)}\\
\midrule
 \texttt{CA}~\cite{kumari2023ablating}  & 60.03 $\pm$ 0.01 & \unifiedCE~\cite{gandikota2023unified} & 0.24 $\pm$ 0.02 \\ 
  \sa~\cite{heng2023selective} & 95.10 $\pm$ 2.21  &  \esd~\cite{gandikota2023erasing} & 125.50 $\pm$ 0.00 \\
\sdd~\cite{kim2023towards}  & 75.50 $\pm$ 3.21 & \unsafediff~\cite{unsafeDiff} & 10.00 $\pm$ 2.03\\  
 \forgetNot~\cite{zhang2023forgetmenot} & 2.20 $\pm$ 0.01 &  \moderator~\cite{wang2024moderator} & 135.25 $\pm$ 4.10\\
 \textbf{\method} & 9.10 $\pm$ 0.05 & & \\
\bottomrule

\toprule
\end{tabular}
\label{tab:efficiency}
\end{table}

==> generative-concept-removal/tables/tab_filter_effective.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{\ref{effective} (Effectiveness)}: Comparison with \unsafediff using FNR on \emph{unacceptable} prompts in $\dtestunacc$ (lower is better). We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FNR is $<$0.25.}
\footnotesize
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c }
\bottomrule

\toprule
\textbf{Concepts}
& \textbf{\unsafediff} & \textbf{\method} \\
\midrule 
\textbf{Nudity (I2P)}  & \cellcolor{myniceblue!35}0.39 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.14 $\pm$ 0.05 \\
\textbf{Violence (I2P)}  & \cellcolor{mynicered!35}0.90 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.20 $\pm$ 0.00 \\
\textbf{Disturbing (I2P)}  & \cellcolor{mynicered!35}0.89 $\pm$ 0.03 & \cellcolor{mynicered!35}0.53 $\pm$ 0.08  \\
\textbf{Hateful (I2P)} & \cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.42 $\pm$ 0.03  \\
\bottomrule

\toprule
\end{tabular}
}
\label{tab:FilterEffective}
\end{table}


==> generative-concept-removal/tables/tab_filter_robust.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{\ref{robust} (Robustness)}: Comparison with \unsafediff using FNR on \emph{adversarial} prompts in $\dtestadv$ (lower is better). We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; and \colorbox{mynicegreen}{green} if FNR is $<$0.25.}
\footnotesize
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{  l | c | c | c | c  }
\bottomrule

\toprule
\textbf{\crt} & \textbf{Nudity} & \textbf{Violence} & \textbf{Disturbing} & \textbf{Hateful}\\
\midrule
\multicolumn{5}{c}{\textbf{\typo+}}\\
\midrule
\textbf{\unsafediff} & \cellcolor{mynicered!35} 0.55 $\pm$ 0.02 & \cellcolor{mynicered!35} 0.91 $\pm$ 0.05 & \cellcolor{myniceblue!35} 0.39 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.48 $\pm$ 0.01\\
\midrule
\textbf{\method} & \cellcolor{mynicegreen!35} 0.15 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.26 $\pm$ 0.01 &  \cellcolor{myniceblue!35} 0.39 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.37 $\pm$ 0.05 \\
\midrule
\multicolumn{5}{c}{\textbf{\pez+}}\\
\midrule
\textbf{\unsafediff}  & \cellcolor{mynicered!35} 0.65 $\pm$ 0.02 & \cellcolor{mynicered!35} 0.91 $\pm$ 0.02  & \cellcolor{mynicered!35} 0.89 $\pm 0.02$ & \cellcolor{mynicered!35} 1.00 $\pm 0.00$\\
\midrule
\textbf{\method}& \cellcolor{mynicegreen!35} 0.16 $\pm$ 0.02 & \cellcolor{mynicegreen!35} 0.25 $\pm$ 0.04  & \cellcolor{mynicegreen!35} 0.14 $\pm$ 0.03 & \cellcolor{mynicegreen!35} 0.20 $\pm$ 0.05\\
\midrule
\multicolumn{5}{c}{\textbf{\cce}}\\
\midrule
\textbf{\unsafediff} & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicered!35} 0.75 $\pm$ 0.05 & \cellcolor{mynicered!35} 1.00 $\pm$ 0.05 & \cellcolor{mynicered!35} 1.00 $\pm$ 0.00\\
\midrule
\textbf{\method} & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{myniceblue!35} 0.38 $\pm$ 0.05  & \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.01 \\
\midrule
\multicolumn{5}{c}{\textbf{\ringbell+}}\\
\midrule
\textbf{\unsafediff}  & \cellcolor{mynicered!35} 0.95 $\pm$ 0.03 & \cellcolor{myniceblue!35} 0.50 $\pm$ 0.04 & \cellcolor{myniceblue!35} 0.30 $\pm$ 0.05 & \cellcolor{mynicered!35} 0.90 $\pm$ 0.05\\
\midrule
\textbf{\method} & \cellcolor{mynicegreen!35} 0.06 $\pm$ 0.08 & \cellcolor{mynicegreen!35} 0.08 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.06 $\pm$ 0.02 & \cellcolor{myniceblue!35} 0.25 $\pm$ 0.05\\
\midrule
\multicolumn{5}{c}{\textbf{\sneaky}}\\
\midrule
\textbf{\unsafediff}  & \cellcolor{mynicered!35} 0.67 $\pm$ 0.21 &  \cellcolor{mynicered!35} 0.71 $\pm$ 0.02 & \cellcolor{mynicered!35} 0.82 $\pm$ 0.03 & \cellcolor{myniceblue!35} 0.48 $\pm$ 0.06\\
\midrule
\textbf{\method} & \cellcolor{myniceblue!35}0.40 $\pm$ 0.08  & \cellcolor{mynicegreen!35}0.14 $\pm$ 0.03 & \cellcolor{mynicered!35} 0.70 $\pm$ 0.05 & \cellcolor{mynicegreen!35} 0.15 $\pm$ 0.10\\
\bottomrule

\toprule
\end{tabular}
}
\label{tab:FilterRobust}
\end{table}


==> generative-concept-removal/tables/tab_filter_utility.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{\ref{utility} (Utility)}: Comparison with \unsafediff using FPR on \emph{acceptable} prompts in $\dtestacc$ (lower is better). We use \colorbox{mynicered}{red} if FPR is $>$0.50, \colorbox{myniceblue}{blue} if FPR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FPR is $<$0.25.}
\footnotesize
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c }
\bottomrule

\toprule
\textbf{Concepts} & \textbf{\unsafediff} & \textbf{\method}\\
\midrule 
\textbf{Nudity (I2P)}  & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.01 \\
\textbf{Violence (I2P)} & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.08 $\pm$ 0.05 \\
\textbf{Disturbing (I2P)}  & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 &\cellcolor{mynicegreen!35} 0.01 $\pm$ 0.01 \\
\textbf{Hateful (I2P)} & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.04 \\
\bottomrule

\toprule
\end{tabular}
}
\label{tab:FilterUtility}
\end{table}

==> generative-concept-removal/tables/tab_nofinetune_effective.tex <==
\begin{table}[ht]
\centering
\caption{\underline{Benefit of Fine-Tuning (FT):} On using fine-tuning, if effectiveness/utility degrades we use \colorbox{mynicered}{red}; \colorbox{myniceblue}{blue} for no significant change; \colorbox{mynicegreen}{green} if better. We measure CLIP accuracy for effectiveness (lower is better) and normalized CLIP score for utility (higher is better).} 
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l|c|c|c|c } 
 \hline
  \multirow{2}{*}{\textbf{Concept}} &
\multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{2}{c}{{\textbf{Utility}}} \\
&  \textbf{w/o FT} & \textbf{w/ FT} & \textbf{w/o FT} & \textbf{w/ FT} \\
\hline
\textbf{Nudity} & \cellcolor{myniceblue!35} 0.15 $\pm$ 0.02 & \cellcolor{myniceblue!35} 0.15 $\pm$ 0.06 & \cellcolor{mynicegreen!35}0.83 $\pm$ 0.07 & \cellcolor{mynicegreen!35} 0.94 $\pm$ 0.08 \\
\textbf{Violence} & \cellcolor{myniceblue!35}0.21 $\pm$ 0.02 & \cellcolor{myniceblue!35} 0.20 $\pm$ 0.05 & \cellcolor{myniceblue!35}0.55 $\pm$ 0.08 & \cellcolor{myniceblue!35} 0.59 $\pm$ 0.11 \\
\hline
\textbf{Grumpy Cat} & \cellcolor{myniceblue!35}0.01 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.00 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.88 $\pm$ 0.03 & \cellcolor{mynicegreen!35} 0.98 $\pm$ 0.04 \\
\textbf{Nemo} & \cellcolor{myniceblue!35}0.12 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.10 $\pm$ 0.02 & \cellcolor{mynicegreen!35} 0.24 $\pm$ 0.05 & \cellcolor{mynicegreen!35} 0.37 $\pm$ 0.02 \\
\textbf{Captain Marvel} & \cellcolor{myniceblue!35}0.04 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.03 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.36 $\pm$ 0.02 & \cellcolor{myniceblue!35} 0.37 $\pm$ 0.03  \\
\textbf{Snoopy} & \cellcolor{myniceblue!35}0.09 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.08 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.64 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.66 $\pm$ 0.03 \\
\textbf{R2D2} & \cellcolor{myniceblue!35}0.00 $\pm$ 0.00 & \cellcolor{myniceblue!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.52 $\pm$ 0.03 & \cellcolor{mynicegreen!35} 0.66 $\pm$ 0.02 \\
\hline
\textbf{Taylor Swift} & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.97 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.98 $\pm$ 0.02  \\
\textbf{Angelina Jolie} & \cellcolor{mynicegreen!35}0.12 $\pm$ 0.02 & \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.97 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.98 $\pm$ 0.03 \\
\textbf{Brad Pitt} & \cellcolor{mynicegreen!35}0.02 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.98 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.98 $\pm$ 0.01 \\
\textbf{Elon Musk} & \cellcolor{mynicegreen!35}0.07 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.92 $\pm$ 0.02 & \cellcolor{mynicegreen!35} 0.97 $\pm$ 0.01 \\
\hline
 \end{tabular}
}
\label{tab:FTImpact}
\end{table}


==> generative-concept-removal/tables/tab_notations.tex <==
\begin{table}[htb]
\caption{Frequently used notations and their descriptions.}
\begin{center}
\footnotesize
\begin{tabular}{ p{1.2cm}|p{5cm} } 
 \bottomrule

 \toprule
 \textbf{Notation} & \textbf{Description}\\
 \midrule
  \tti & Text-to-Image\\
  % \dm & Diffusion model\\
  \te & Text encoder (e.g., CLIP)\\
  \crt & Concept Removal Technique\\
  \adv & Adversary\\
 \midrule
  % $\mathcal{X}$ & Set of images \\
 $\imgclean$ & Generated image \\
 $\imgunacc$ & Generated image with unacceptable concept \\
 % $\mathcal{X}_{u}$ & Set of $x_{u}$\\
 $\imgacc$ & Generated image with acceptable concept \\
 % $\mathcal{X}_{a}$ & Set of $x_{a}$ \\
 $\phi_x(x)$ & CLIP embedding for image $\imgclean$ \\
 $\imgadv$ & Image generated from adversarial prompt\\
 \midrule
 % $\mathcal{C}$ & Set of textual prompts \\
 $\prompt$ & Textual prompt \\
 $\cacc$ & Phrase for acceptable concept\\
 $\cunacc$ & Phrase for unacceptable concept\\
  $\promptuacc$ & Textual prompt containing $\cunacc$ \\
% $\mathcal{C}_{u}$ & Set of $\prompt_{u}$ \\
 $\promptacc$ & Textual prompt containing $\cacc$\\
 
 % $\mathcal{C}_{a}$ & Set of $\prompt_{a}$ \\
$\phi_p(\prompt)$ & CLIP embedding for textual prompt $\prompt$ \\
$\advprompt$ & Adversarially generated textual prompt \\
\midrule
 % $\mathcal{D}$ & Dataset of prompts and images: $\{(x_j, \prompt_j)\}_{j=1}^N$\\
 $\dtestacc$ & Test dataset with acceptable prompts/images\\
 $\dtestunacc$ & Test dataset with unacceptable prompts/images\\
 $\dvalacc$ & Validation dataset with acceptable prompts/images\\
 $\dvalunacc$ & Validation dataset w/ unacceptable prompts/images\\
 $\dtestadv$ & Test dataset with adversarial prompts/images\\
 $\target$ & \tti model with \crt where $\target$: $c \rightarrow x$ \\
  $\filter$ & Function for \method classifier\\
  % $\filter$ & Default filter $\filter$ for Stable Diffusion v1.4 \\
 $\alpha$ & Regularization parameter for \method fine-tuning \\
 $\overline{\cdot}$ & Normalization function \\
  $\epsilon_\theta$ & Diffusion model parameterized by $\theta$ \\
  $\tau$ & Temperature parameter \\
 \bottomrule

 \toprule
\end{tabular}
\end{center}
\label{tab:notations}
\end{table}

==> generative-concept-removal/tables/tab_robustness.tex <==
\begin{table*}[!htb]
\centering
\caption{\underline{\ref{robust} (Robustness):} Comparison with fine-tuning \crt{s} using CLIP accuracy on \emph{adversarial} prompts in $\dtestadv$ (lower is better). We evaluate fine-tuning \crt's against \cce and \method against \cce+ since \cce is already adapted to fine-tuning \crt's. We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{  l | c c | c c c c c | c c c c  }
\bottomrule

\toprule
\multirow{3}{*}{\textbf{CRT}} & \multicolumn{11}{c}{\textbf{Concepts}}\\
& \textbf{Nudity} & \textbf{Violence} & \textbf{Grumpy} & \multirow{2}{*}{\textbf{Nemo}} & \textbf{Captain} & \multirow{2}{*}{\textbf{Snoopy}} & \multirow{2}{*}{\textbf{R2D2}} & \textbf{Taylor} & \textbf{Angelina} & \textbf{Brad} & \textbf{Elon}\\
 & \textbf{(I2P)} & \textbf{(I2P)} & \textbf{Cat} &  & \textbf{Marvel} &  &  &  \textbf{Swift} & \textbf{Jolie} & \textbf{Pitt} & \textbf{Musk}\\
\bottomrule

\toprule
\multicolumn{12}{c}{\textbf{\typo+}}\\
\bottomrule

\toprule
\texttt{CA}~\cite{kumari2023ablating} & 
\cellcolor{mynicered!35} 0.58 $\pm$ 0.02 &
\cellcolor{mynicered!35} 0.75 $\pm$ 0.01&
\cellcolor{myniceblue!35}0.26 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.27 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.42 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.29 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.23 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.09 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.24 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.31 $\pm$ 0.06 \\ 
\forgetNot~\cite{zhang2023forgetmenot} &
\cellcolor{mynicered!35}0.61 $\pm$ 0.02& \cellcolor{mynicered!35}0.75 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.21 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.31 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.49 $\pm$ 0.02 &\cellcolor{myniceblue!35}0.27 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.22 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.17 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.34 $\pm$ 0.01 \\
\sa~\cite{heng2023selective} & \cellcolor{myniceblue!35} 0.31 $\pm$ 0.01 & 
\cellcolor{mynicered!35}0.71 $\pm$ 0.02  & \cellcolor{mynicered!35}0.99 $\pm$ 0.01 & \cellcolor{mynicered!35}0.94 $\pm$ 0.01 & \cellcolor{mynicered!35}0.89 $\pm$ 0.02 & \cellcolor{mynicered!35}0.73 $\pm$ 0.03 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.20 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.43 $\pm$ 0.04 & \cellcolor{mynicered!35}0.65 $\pm$ 0.05 \\ 
\esd~\cite{gandikota2023erasing} & 
\cellcolor{myniceblue!35}0.39 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.70 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.27 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.25 $\pm$ 0.05 & \cellcolor{myniceblue!35}0.40 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.23 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.25 $\pm$ 0.05 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.08 $\pm$ 0.07 & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.23 $\pm$ 0.05 \\ 
\unifiedCE~\cite{gandikota2023unified} & \cellcolor{myniceblue!35} 0.41 $\pm$ 0.00 &
\cellcolor{mynicered!35} 0.60 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.28 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.29 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.34 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.21 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.17 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.02 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.12 $\pm$ 0.00 \\ 
\sdd~\cite{kim2023towards} & 
\cellcolor{mynicegreen!35} 0.20 $\pm$ 0.02 &
\cellcolor{myniceblue!35}0.50 $\pm$ 0.04 & \cellcolor{myniceblue!35}0.27 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.21 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.48 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.19 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.31 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.10 $\pm$ 0.01 \\ 
\moderator~\cite{wang2024moderator} & 
\cellcolor{mynicered!35} 0.83 $\pm$ 0.01 &
\cellcolor{myniceblue!35}0.90 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.21 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.69 $\pm$ 0.04 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.30 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.13 $\pm$ 0.02 \\ 
% \textbf{\method}&  &  & \cellcolor{mynicegreen!35}0.09 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.16 $\pm$ 0.05 & \cellcolor{myniceblue!35}0.31 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.09 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.24 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.02 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.12 $\pm$ 0.01 \\
\midrule
\textbf{\method} & \cellcolor{mynicegreen!35} 0.14 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.20 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.10 $\pm$ 0.01 &  
\cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 &  \cellcolor{mynicegreen!35}0.09 $\pm$ 0.01 &   \cellcolor{mynicegreen!35}0.09 $\pm$ 0.01  &   \cellcolor{mynicegreen!35}0.08 $\pm$ 0.01   & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.01   \\ 
\bottomrule

\toprule
\multicolumn{12}{c}{\textbf{\pez+}}\\
\bottomrule

\toprule
 \texttt{CA}~\cite{kumari2023ablating} & \cellcolor{mynicered!35} 0.75 $\pm$ 0.01 &
 \cellcolor{mynicered!35} 0.84 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.33 $\pm$ 0.04 & \cellcolor{mynicered!35}0.52 $\pm$ 0.01 & \cellcolor{mynicered!35}0.70 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.20 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.25 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.46 $\pm$ 0.01 & \cellcolor{mynicered!35}0.64 $\pm$ 0.01 & \cellcolor{mynicered!35}0.63 $\pm$ 0.02 & \cellcolor{mynicered!35}0.72 $\pm$ 0.01 \\
\forgetNot~\cite{zhang2023forgetmenot} & 
\cellcolor{mynicered!35}0.74 $\pm$ 0.01&
\cellcolor{mynicered!35}0.72 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.43 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.41 $\pm$ 0.01 & \cellcolor{mynicered!35}0.85 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.45 $\pm$ 0.01 & \cellcolor{mynicered!35}0.93 $\pm$ 0.06 & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.16 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.08 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.23 $\pm$ 0.01 \\ 
\sa~\cite{heng2023selective} & \cellcolor{mynicered!35}0.55 $\pm$ 0.03& 
\cellcolor{mynicered!35}0.82 $\pm$ 0.01& \cellcolor{mynicegreen!35}0.14 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.14 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.14 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.14 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.01 \\ 
\esd~\cite{gandikota2023erasing} & 
\cellcolor{mynicered!35} 0.69 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.88 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.36 $\pm$ 0.06 & \cellcolor{myniceblue!35}0.40 $\pm$ 0.04 & \cellcolor{myniceblue!35}0.44 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.34 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.26 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.05 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.04 & \cellcolor{mynicegreen!35}0.17 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.23 $\pm$ 0.03 \\ 
\unifiedCE~\cite{gandikota2023unified} & 
\cellcolor{mynicered!35} 0.59 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.82 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.23 $\pm$ 0.01 & \cellcolor{mynicered!35}0.52 $\pm$ 0.01 & \cellcolor{mynicered!35}0.59 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.14 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.25 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.02 \\ 
\sdd~\cite{kim2023towards} & \cellcolor{myniceblue!35} 0.30 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.60 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.28 $\pm$ 0.05 & \cellcolor{myniceblue!35}0.28 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.50 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.34 $\pm$ 0.03 & \cellcolor{myniceblue!35}0.30 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.09 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.12 $\pm$ 0.01 \\ 
\moderator~\cite{wang2024moderator} & 
\cellcolor{mynicered!35} 0.84 $\pm$ 0.01 &
\cellcolor{myniceblue!35}0.90 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.27 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.71 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.02 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.33 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.07 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.01 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.02 \\ 
% \unsafediff~\cite{} & 0.01 $\pm$ 0.01 & 0.51 $\pm$ 0.05  &  &  &  &  &  &  & cell \\  
% \textbf{\method} & 
% \cellcolor{mynicegreen!35} 0.26 $\pm$ 0.02 &
% \cellcolor{mynicegreen!35} 0.26 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.09 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.17 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.29 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.10 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.31 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.06 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.07 $\pm$ 0.04 & \cellcolor{mynicegreen!35}0.18 $\pm$ 0.05 \\
\midrule
\textbf{\method} & \cellcolor{mynicegreen!35}0.15 $\pm$ 0.01  & \cellcolor{mynicegreen!35}0.25 $\pm$ 0.05 & \cellcolor{mynicegreen!35}0.10 $\pm$ 0.01 &  \cellcolor{mynicegreen!35}0.12 $\pm$ 0.01 &   \cellcolor{mynicegreen!35}0.11 $\pm$ 0.03  &  \cellcolor{mynicegreen!35}0.08 $\pm$ 0.01 &   \cellcolor{mynicegreen!35}0.03 $\pm$ 0.00 
& \cellcolor{mynicegreen!35}0.00 $\pm$ 0.01  & \cellcolor{mynicegreen!35}0.03 $\pm$ 0.00  & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.00  & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.00  \\ 
\bottomrule

\toprule
\multicolumn{12}{c}{\textbf{\ringbell+}}\\
\bottomrule

\toprule
\texttt{CA}~\cite{kumari2023ablating} & 
\cellcolor{mynicered!35} 0.97 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.96 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.79 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.76 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.88 $\pm$ 0.02 & 
\cellcolor{myniceblue!35} 0.38 $\pm$ 0.02 &
\cellcolor{mynicered!35} 0.65 $\pm$ 0.05 & 
\cellcolor{mynicegreen!35} 0.03 $\pm$ 0.03 & 
\cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.88 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.01 \\ 
\forgetNot~\cite{zhang2023forgetmenot} & 
\cellcolor{mynicered!35} 0.96 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.95 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.75 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.57 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.91 $\pm$ 0.00 & 
\cellcolor{myniceblue!35} 0.45 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.59 $\pm$ 0.01 &  
\cellcolor{myniceblue!35} 0.26 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.85 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.88 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.99 $\pm$ 0.02 \\ 
\sa~\cite{heng2023selective} & 
\cellcolor{mynicered!35} 0.80 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.98 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.93 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.98 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.96 $\pm$  0.03 & 
\cellcolor{mynicered!35} 0.97 $\pm$ 0.03 & 
\cellcolor{mynicered!35} 0.88 $\pm$ 0.02 & 
\cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.03 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.77 $\pm$ 0.10 & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.01 \\ 
\esd~\cite{gandikota2023erasing} & \cellcolor{mynicered!35} 0.77 $\pm$ 0.03
& 
\cellcolor{mynicered!35} 0.95 $\pm$ 0.02 & 
\cellcolor{mynicered!35} 0.63 $\pm$ 0.06 & 
\cellcolor{mynicered!35} 0.66 $\pm$ 0.12 & 
\cellcolor{mynicered!35} 0.56 $\pm$ 0.06 & 
\cellcolor{mynicered!35} 0.66 $\pm$ 0.07 & 
\cellcolor{mynicered!35} 0.69 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & 
\cellcolor{mynicegreen!35} 0.03 $\pm$ 0.02 & 
\cellcolor{myniceblue!35} 0.27 $\pm$ 0.03 & 
\cellcolor{mynicered!35} 0.55 $\pm$ 0.08 \\ 
\unifiedCE~\cite{gandikota2023unified} & 
\cellcolor{mynicered!35} 0.84 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.67 $\pm$ 0.00 & 
\cellcolor{myniceblue!35} 0.38 $\pm$ 0.05 & 
\cellcolor{mynicered!35} 0.74 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.07 $\pm$ 0.00 &
\cellcolor{mynicegreen!35} 0.16 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.50 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.05 $\pm$ 0.00 & 
\cellcolor{mynicegreen!35} 0.01 $\pm$ 0.00 & 
\cellcolor{mynicegreen!35} 0.02 $\pm$ 0.01 & 
\cellcolor{myniceblue!35} 0.34 $\pm$ 0.01 \\ 
\sdd~\cite{kim2023towards} & 
\cellcolor{myniceblue!35} 0.33 $\pm$ 0.02 &
 \cellcolor{mynicered!35} 0.60 $\pm$ 0.03 & 
\cellcolor{mynicegreen!35} 0.22 $\pm$ 0.01 & 
\cellcolor{myniceblue!35} 0.31 $\pm$ 0.01 &
\cellcolor{mynicered!35} 0.62 $\pm$ 0.01 &
\cellcolor{myniceblue!35} 0.42 $\pm$ 0.03 & 
\cellcolor{myniceblue!35} 0.41 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.07 $\pm$ 0.02 & 
\cellcolor{mynicegreen!35} 0.07 $\pm$ 0.02 & 
\cellcolor{mynicegreen!35} 0.07 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.17 $\pm$ 0.02 \\ 
\moderator~\cite{wang2024moderator} & 
\cellcolor{mynicered!35} 0.98 $\pm$ 0.03 &
 \cellcolor{mynicered!35} 0.95 $\pm$ 0.03 & 
\cellcolor{mynicegreen!35} 0.02 $\pm$ 0.01 & 
\cellcolor{myniceblue!35} 0.26 $\pm$ 0.01 &
\cellcolor{mynicered!35} 0.73 $\pm$ 0.00 &
\cellcolor{mynicegreen!35} 0.10 $\pm$ 0.03 & 
\cellcolor{myniceblue!35} 0.36 $\pm$ 0.02 & 
\cellcolor{mynicegreen!35} 0.07 $\pm$ 0.02 & 
\cellcolor{mynicegreen!35} 0.10 $\pm$ 0.00 & 
\cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.18 $\pm$ 0.01 \\
% \textbf{\method} & & & 
% \cellcolor{mynicegreen!35} 0.05 $\pm$ 0.01 & 
% \cellcolor{mynicegreen!35} 0.07 $\pm$ 0.00 & 
% \cellcolor{mynicegreen!35} 0.08 $\pm$ 0.01 & 
% \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 & 
% \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.00 & 
% \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.01 & 
% \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.00 & 
% \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.01 & 
% \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.00 \\ 
\midrule
\textbf{\method} & \cellcolor{mynicegreen!35} 0.05 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.08 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.20 $\pm$ 0.08 & \cellcolor{mynicegreen!35} 0.15 $\pm$ 0.03 &
\cellcolor{mynicegreen!35} 0.04 $\pm$ 0.02  & \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.01 & 
\cellcolor{mynicegreen!35} 0.15 $\pm$ 0.05 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.02 &  \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.02 &  \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.02 &   \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.02 \\ 
\bottomrule

\toprule
 \multicolumn{12}{c}{\textbf{\cce or \cce+ (against \method)}}\\
\bottomrule

\toprule
\texttt{CA}~\cite{kumari2023ablating} & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
 \cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 &  
\cellcolor{mynicered!35} 0.99 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.97 $\pm$ 0.01 &  
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 &  
\cellcolor{mynicered!35} 0.99 $\pm$ 0.01 &
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35}1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.80 $\pm$ 0.00 \\ 
\forgetNot~\cite{zhang2023forgetmenot} & \cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & \cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}0.98 $\pm$ 0.00 & \cellcolor{mynicered!35}0.98 $\pm$ 0.01 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 \\ 
\sa~\cite{heng2023selective} & 
\cellcolor{mynicered!35} 0.98 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.99 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.99 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.97 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.99 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.99 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.84 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.97 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.81 $\pm$ 0.01 \\ 
\esd~\cite{gandikota2023erasing} & \cellcolor{mynicered!35} 0.92 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.99 $\pm$ 0.00 & 
\cellcolor{mynicered!35}0.91 $\pm$ 0.01 & \cellcolor{mynicered!35}0.94 $\pm$ 0.00 & \cellcolor{mynicered!35}0.96 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}0.98 $\pm$ 0.01 \\ 
\unifiedCE~\cite{gandikota2023unified} & \cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & \cellcolor{mynicered!35} 0.97 $\pm$ 0.00 & \cellcolor{mynicered!35}1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}0.98 $\pm$ 0.00 & \cellcolor{mynicered!35}0.98 $\pm$ 0.01 & \cellcolor{mynicered!35}1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}0.99 $\pm$ 0.00 & \cellcolor{mynicered!35}0.63 $\pm$ 0.01 & \cellcolor{mynicered!35}1.00 $\pm$ 0.00 & \cellcolor{mynicered!35}0.77 $\pm$ 0.01 \\ 
\sdd~\cite{kim2023towards} & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.81 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.81 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.93 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.96 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.98 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.97 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.67 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 0.77 $\pm$ 0.01 & 
\cellcolor{mynicered!35} 1.00 $\pm$ 0.00 & 
\cellcolor{mynicered!35} 0.81 $\pm$ 0.01 \\ \moderator~\cite{wang2024moderator} & \cellcolor{mynicered!35} 0.99 $\pm$ 0.00 & \cellcolor{mynicered!35} 0.92 $\pm$ 0.05  & \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.00 & \cellcolor{myniceblue!35} 0.18 $\pm$ 0.00 & \cellcolor{mynicered!35} 0.44 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.01 & \cellcolor{mynicered!35} 0.45 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 &  \cellcolor{mynicegreen!35} 0.06 $\pm$ 0.00 &  \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.09 $\pm$ 0.00 \\ 
% \textbf{\method} & & & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.11 $\pm$ 0.00 \\ 
\midrule
\textbf{\method} & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{myniceblue!35} 0.40 $\pm$ 0.05  & \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 &  \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 &  \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35} 0.01 $\pm$ 0.01 \\ 
\bottomrule

\toprule
\end{tabular}
}
\label{tab:robust}
\end{table*}

==> generative-concept-removal/tables/tab_teconfig.tex <==
\begin{table}[h]
\caption{Evaluation dataset configuration.}
% \begin{center}
\centering
\footnotesize
\begin{tabular}{ p{1.7cm} | c | p{5cm} }
\bottomrule

\toprule
\textbf{Concepts} & \textbf{Data} & \textbf{Configuration}\\
\textbf{(Requirement)} & & \\
\midrule
Group-1 (\ref{effective}, \ref{robust}) & $\dtestunacc$ & I2P Dataset~\cite{schramowski2022safe} of unacceptable prompts: for \emph{nudity}: 449 prompts, \emph{violence}: 758, \emph{disturbing}: 857,  \emph{hateful}: 235\\
\midrule
Group-2 (\ref{effective}, \ref{robust}) & $\dtestunacc$ & 10 unacceptable prompts ($\promptuacc$) from ChatGPT and 20 images ($\imgunacc$) per prompt from SDv1.4\\
\midrule
Group-3 (\ref{effective}, \ref{robust}) & $\dtestunacc$ & 10 unacceptable prompts ($\promptuacc$) from ChatGPT and 20 images ($\imgunacc$) per prompt from SDv1.4\\
\midrule
All (\ref{utility}) & $\dtestacc$ & 200 acceptable prompts ($\promptacc$) from COCO 2014 dataset\\
\bottomrule

\toprule
\end{tabular}
% \end{center}
\label{tab:teconfig}
\end{table}

==> generative-concept-removal/tables/tab_trconfig.tex <==
\begin{table}[!htb]
\caption{Training dataset configurations required by \crt{s}.}
% \begin{center}
\centering
\footnotesize
\begin{tabular}{ l | p{6.5cm} }
 \bottomrule

 \toprule
\textbf{\crt} & \textbf{Configuration Requirements}\\
\midrule
\ca~\cite{kumari2023ablating} & 200 unacceptable prompts ($\promptacc$) from ChatGPT with one image/prompt from SDv1.4 \\ 
\esd~\cite{gandikota2023erasing} & Unacceptable concept ($\cunacc$) \\  
\forgetNot~\cite{zhang2023forgetmenot} & 8 unacceptabe prompts ($\promptuacc$) and one image/prompt from SDv1.4\\
\sdd~\cite{kim2023towards} & Unacceptable concept ($\cunacc$) and 10 corresponding images\\
\sa~\cite{heng2023selective} & Acceptable concept ($\cacc$) and 1000 corresponding images, and 6 unacceptable prompts ($\promptuacc$) \\
\unifiedCE~\cite{gandikota2023unified} & Unacceptable and acceptable concepts ($\cunacc$ and $\cacc$)\\
\moderator~\cite{wang2024moderator} & Unacceptable concept ($\cunacc$) and 120 corresponding images\\
\midrule
\unsafediff~\cite{unsafeDiff} & 776 total images with 580 acceptable images ($\imgacc$), and 196 unacceptable images ($\imgunacc$): nudity (48), violence (45), disturbing (68), and hateful (35)\\
\method & 10 unacceptable prompts ($\promptuacc$) and acceptable prompts ($\promptacc$) using ChatGPT with one image/prompt from SDv1.4\\
 \bottomrule

 \toprule
\end{tabular}
% \end{center}
\label{tab:trconfig}
\end{table}

==> generative-concept-removal/tables/tab_utility.tex <==
\begin{table*}[ht]
\caption{\underline{\ref{utility} (Utility):} Comparison with fine-tuning \crt{s} using normalized CLIP scores on $\dtestacc$ (higher is better). We use \colorbox{mynicered}{red} if score is between 50-70, \colorbox{myniceblue}{blue} if between 70-90; \colorbox{mynicegreen}{green} if $>$90. \textbf{\underline{Note:}} \method's utility against Group-2 concepts like \emph{Nemo}, \emph{Captain Marvel}, \emph{Snoopy}, and \emph{R2D2} can be improved as described in Section~\ref{sec:finetuneEval}.}
% \begin{center}
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ l|c|c|c|c|c|c|c|c|c|c|c } 
\bottomrule

\toprule
 \multirow{3}{*}{\textbf{CRT}} & \multicolumn{11}{c}{\textbf{Concepts}}\\
  & \multirow{2}{*}{\textbf{Nudity}} & \multirow{2}{*}{\textbf{Violence}} & \textbf{Grumpy} & \multirow{2}{*}{\textbf{Nemo}} & \textbf{Captain} & \multirow{2}{*}{\textbf{Snoopy}} & \multirow{2}{*}{\textbf{R2D2}} & \textbf{Taylor} & \textbf{Angelina} & \textbf{Brad} & \textbf{Elon}\\
  &  & & \textbf{Cat} &  & \textbf{Marvel} &  &  &  \textbf{Swift} & \textbf{Jolie} & \textbf{Pitt} & \textbf{Musk}\\
\midrule
\texttt{CA}~\cite{kumari2023ablating}  & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 \\ 
\forgetNot~\cite{zhang2023forgetmenot} & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00  & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 \\ 
\sa~\cite{heng2023selective} & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.79 $\pm$ 0.00 \\  
\esd~\cite{gandikota2023erasing} & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.00  & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.01 \\ 
\unifiedCE~\cite{gandikota2023unified} & \cellcolor{mynicegreen!35}0.96 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.96 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.97 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.96 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.96 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.97 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.96 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.97 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.97 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.96 $\pm$ 0.03 & \cellcolor{mynicegreen!35}0.97 $\pm$ 0.00 \\ 
\sdd~\cite{kim2023towards} & \cellcolor{myniceblue!35}0.86 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.75 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.86 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.00 & \cellcolor{mynicered!35}0.64 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.82 $\pm$ 0.00 & \cellcolor{mynicered!35}0.61 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.89 $\pm$ 0.00 \\ 
\moderator~\cite{wang2024moderator} & \cellcolor{mynicegreen!35}0.93 $\pm$ 0.01 & \cellcolor{mynicered!35}0.53 $\pm$ 0.00 & \cellcolor{mynicered!35}0.57 $\pm$ 0.00 & \cellcolor{mynicered!35}0.55 $\pm$ 0.00 & \cellcolor{mynicered!35}0.53 $\pm$ 0.00 & \cellcolor{mynicered!35}0.50 $\pm$ 0.01 & \cellcolor{mynicered!35}0.46 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.86 $\pm$ 0.00 & \cellcolor{mynicered!35}0.61 $\pm$ 0.00 & \cellcolor{mynicered!35}0.68 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.71 $\pm$ 0.00 \\
% \textbf{\method} & \cellcolor{myniceblue!35}0.71 $\pm$ 0.10  & \cellcolor{myniceblue!35} 0.70 $\pm$ 0.10 &  \cellcolor{myniceblue!35}0.88 $\pm$ 0.02 &  \cellcolor{mynicegreen!35}0.90 $\pm$ 0.10 & \cellcolor{mynicered!35}0.67 $\pm$ 0.15 &  \cellcolor{myniceblue!35}0.86 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.75 $\pm$ 0.11 & \cellcolor{mynicegreen!35}0.98 $\pm$ 0.02  &  \cellcolor{mynicegreen!35}0.98 $\pm$ 0.03 & 
% \cellcolor{mynicegreen!35}0.98 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.97 $\pm$ 0.01 \\ 
\midrule
\textbf{\method} & 
  \cellcolor{mynicegreen!35}0.94 $\pm$ 0.08 & 
 \cellcolor{mynicered!35}0.59 $\pm$ 0.11&  
 \cellcolor{mynicegreen!35}0.98 $\pm$ 0.04 &  
 \cellcolor{mynicered!35} 0.37 $\pm$ 0.02 & 
 \cellcolor{mynicered!35} 0.37 $\pm$ 0.03 &  
 \cellcolor{myniceblue!35} 0.66 $\pm$ 0.03& 
 \cellcolor{myniceblue!35} 0.66 $\pm$ 0.02 & \cellcolor{mynicegreen!35}0.98 $\pm$ 0.02  &  \cellcolor{mynicegreen!35}0.98 $\pm$ 0.03 & 
\cellcolor{mynicegreen!35}0.98 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.97 $\pm$ 0.01 \\
\bottomrule

\toprule
 \end{tabular}
}
% \end{center}
\label{tab:utility}
\end{table*}



==> generative-concept-removal/tables/tab_valconfig.tex <==
\begin{table}[h]
\caption{Validation dataset configuration.}
\centering
\footnotesize
\begin{tabular}{ p{1.55cm} | c | p{5.2cm} }
 \bottomrule

 \toprule
\textbf{Concepts} & \textbf{Data} & \textbf{Configuration}\\
\textbf{(Requirement)} & & \\
\midrule
Group-1 (\ref{effective}) & $\dvalunacc$ & 10 unacceptable prompts ($\promptuacc$) from ChatGPT and 5 images ($\imgunacc$) per prompt from SDv1.4 \\
\midrule
Group-2 (\ref{effective}) & $\dvalunacc$ & 10 unacceptable prompts ($\promptuacc$) from ChatGPT and 5 images ($\imgunacc$) per prompt from SDv1.4 \\
\midrule
Group-3 (\ref{effective}) & $\dvalunacc$ & 10 unacceptable prompts ($\promptuacc$) from ChatGPT and 5 images ($\imgunacc$) per prompt from SDv1.4 \\
\midrule
All (\ref{utility}) & $\dvalacc$ & 100 acceptable prompts ($\promptacc$) and 1 image ($\imgacc$) per prompt  from the COCO 2014 dataset \\
 \bottomrule

 \toprule
\end{tabular}
% \end{center}
\label{tab:valconfig}
\end{table}

==> old_versions/01abstract.tex <==
Diffusion based text-to-image (\tti) models generate high fidelity images for given textual prompts. They are trained on large datasets scraped from the Internet, potentially containing \textit{unacceptable concepts} (e.g., copyright infringing or unsafe). Retraining \tti models after filtering out unacceptable concepts in the training data is inefficient and degrades utility. Hence, we need concept removal techniques (\crt{s}) which are
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \textit{effective} in preventing the generation of images with unacceptable concepts
\item \textit{utility-preserving} on acceptable concepts, and 
\item \textit{robust} against evasion with adversarial prompts.
\end{enumerate*}
None of the prior \crt{s} satisfy all these requirements simultaneously. 

We introduce \method, the first \emph{\textbf{robust} \underline{co}ncept \underline{fi}lter} based on Contrastive Language-Image Pre-Training (CLIP). 
We configure CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts.
This simple change significantly improves robustness by restricting the adversary to add noise \emph{only} along the vector connecting the embeddings of unacceptable and acceptable concepts.
Further, fine-tuning \method to separate embeddings of unacceptable and acceptable concepts, while preserving their pairing with image embeddings, improves utility. 
We evaluate \method on eleven concepts to show that it is more \emph{effective} (CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) and more \emph{robust} (CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) than prior \crt{s}, while retaining \emph{utility} (normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]). 
Finally, we present theoretical bounds for certified robustness of \method against adversarial prompts, and an empirical analysis.


==> old_versions/1introduction.tex <==
\section{Introduction}\label{sec:introduction}


Diffusion based text-to-image (\tti) models have demonstrated a remarkable ability to generate high quality images from textual prompts~\cite{stable-diffusion,Rombach_2022_CVPR,ramesh2021dalle}.
These models are trained on large datasets of unfiltered content from the Internet~\cite{radford2021learning,schuhmann2022laion}. 
Due to their large capacity, \tti models memorize specific \emph{concepts}, as seen in the generated images~\cite{Korn_2023,somepalli2022diffusion,carlini2023extracting}. 
Some of these concepts, may be \emph{unacceptable} for various reasons, such as copyright infringement (e.g., a movie character or celebrity), or inappropriateness (e.g., ``nudity'' or ``violence'')~\cite{gandikota2023erasing,schramowski2022safe,heng2023selective}. 
Retraining \tti models after filtering out unacceptable concepts is inefficient, only partially effective~\cite{li2024safegen, huggingfaceStabilityaistablediffusion21Hugging}, and compromises utility~\cite{gandikota2023erasing}.
Hence, there is a need for \emph{concept removal techniques} (\crt{s}) to minimize unacceptable concepts in  generated images.


Ideally, \crt{s} should be \emph{effective} in reducing the generation of unacceptable concepts while preserving the \emph{utility} on all others, and \emph{robust} to evasion with adversarial prompts.  
As we show in Section~\ref{sec:evaluation}, none of the existing \crt{s} \emph{simultaneously} satisfy these requirements:
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \emph{filtering \crt{s}}, which detect unacceptable concepts, lack robustness~(\cite{rando2022redteaming} and Section~\ref{sec:filterEval})
\item \emph{fine-tuning \crt{s}} which modify \tti models, trade-off effectiveness and utility~\cite{gandikota2023erasing,kumari2023ablating,heng2023selective,schramowski2022safe}, and may lack robustness~\cite{Tsai2023RingABellHR, wen2023hard, pham2023circumventing, yang2023sneakyprompt}.
\end{enumerate*}
%Moreover, none of these \crt{s} are robust against adversarial prompts, i.e., adversarially modified prompts which force \tti{s} to generate unacceptable concepts.
Designing a \crt meeting all the requirements is an open problem. Our goal is to design such a \crt.

We opt to use a filter as it will not alter the \tti model, thus reducing its impact on utility. We construct our filter using the Contrastive Language-Image Pre-Training (CLIP)~\cite{radford2021learning}, an essential component of \tti models. CLIP co-locates the embeddings of textual prompts and their corresponding images within a unified embedding space where similar concepts are closer.
CLIP is pre-trained on a vast dataset which encodes a broad spectrum of concepts~\cite{radford2021learning}, making it a versatile choice for a filter, unlike specialized classifiers (e.g.,~\cite{unsafeDiff}).
However, relying on CLIP to identify unacceptable images by solely measuring the distance between the embeddings of a generated image, and an unacceptable concept, was shown not to be robust (~\cite{rando2022redteaming}). Subsequently, several prior works have identified filtering as a viable direction which needs further exploration~\cite{rando2022redteaming,li2024safegen}.

% \input{figures/fig_robustness_diagram}
% \change{Robustness diagram: figures/fig\_robustness\_diagram}

We present a \textbf{robust} (CLIP-based) \underline{co}ntent \underline{fi}lter, \method, by configuring CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts. 
% We present a \textbf{robust} \textbf{co}ntent \textbf{fi}lter, \method, that identifies unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both acceptable and unacceptable concepts}. 
% \change{This simple change in configuration translates to projecting} the image embedding onto the vector connecting the text embeddings of acceptable and unacceptable concepts. 
This simple change makes it harder to generate effective adversarial prompts: the adversary is restricted to adding noise in the direction of the acceptable concept. 
%adversarial prompts must generate images far enough from unacceptable concepts to evade detection yet close enough to retain the unacceptable concepts.
To restore any drop in utility stemming from this change, we fine-tune \method to increase the separation between the text embeddings of unacceptable and acceptable concepts, while maintaining their pairing with their corresponding image embeddings. 
This fine-tuning approach is further supported by fine-tuning \crt{s} which show that such an optimization leads to better utility~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}.
We claim the following main contributions: we present
\begin{enumerate}[leftmargin=*,wide,  labelindent=0pt]
\item \method\footnote{We will open-source the code upon publication.}, the \textbf{first robust} (CLIP-based) \underline{co}ntent \underline{fi}lter which identifies unacceptable concepts in generated images by measuring the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts (Section~\ref{sec:approach}),
\item a comprehensive comparative evaluation (Section~\ref{sec:setup}) of the fine-tuned variant of \method with six state-of-the-art fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective} (CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) and \textbf{more robust} (CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) than prior \crt{s}, while \textbf{retaining utility} (normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]).
%showing that \method is \textbf{effective} ($\sim$5\% CLIP accuracy  on unacceptable concepts), \textbf{utility-preserving} ($\sim$93\% 
% normalized CLIP score on acceptable concepts), and \textbf{robust} ($\sim$4\% CLIP accuracy of  on adversarial prompts) %of unacceptable concepts) 
(Section~\ref{sec:evaluation}), and
\item %the \textbf{first} approach towards \textbf{certifiable robustness of \crt{s}} by exploring 
theoretical bounds for \textbf{certifying the robustness} of \method, assuming a hypothetically strong adversary, empirical analysis of these bounds, and making the case that \method is likely to be more robust in practice. (Section~\ref{sec:bound}). 
\end{enumerate}

==> old_versions/2background.tex <==
\section{Background}\label{sec:background}

We describe \tti models (Section~\ref{back-diffusion}), different \crt{s} (Section~\ref{back-conceptrem}), and attacks against them (Section~\ref{back-attacks}).

\subsection{Diffusion based \tti Models}\label{back-diffusion}

A diffusion based \tti model is a function $\target: \prompt \rightarrow \imgclean$ which generates an image $\imgclean$ for a given a textual prompt $\prompt$. It comprises two key components: an encoder (\te) which is used to incorporate the textual prompt in the image generation process, and a diffusion model (\dm) which is responsible for the generation of the image.

A popular encoder is CLIP, trained on a large dataset of image-text pairs, to map the embeddings of images and their corresponding text closer together in a joint text-image embedding space~\cite{radford2021learning}.
Given $N$ images $\{\imgclean_j\}_{j=1}^N$ and their corresponding text prompts $\{\prompt_j\}_{j=1}^{N}$, the training data is $\mathcal{D} = \{(\imgclean_j, \prompt_j)\}_{j=1}^N$. 

CLIP is trained to maximize the cosine similarity between the embeddings of a prompt $\prompt_j$ and its corresponding image $\imgclean_j$ while minimizing the similarity between $\prompt_j$ and any other $\imgclean_k$ for a $k \ne j$.
We denote the cosine similarity as \text{cos}($\phi_p(\prompt_j), \phi_x(\imgclean_j))$, where $\phi_x(\imgclean_j)$ is the CLIP image embedding of the image $\imgclean_j$, and $\phi_p(\prompt_j)$ is the CLIP text embedding of the prompt $\prompt_j$.
To achieve this, CLIP is trained using a contrastive loss function~\cite{yang2023robust,oord2019representation,lee2021soundguided}: \[\mathcal{L}_{\text{Con}}(\mathcal{D}) = - \frac{1}{N} \sum_{j=1}^{N} \log \frac{\exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_j))/ \tau)}{\sum_{k=1}^{N} \exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_k))/ \tau)}\] where $\tau$ is the temperature parameter for scaling the predictions~\cite{radford2021learning, ModalityGap}. 
 


Given access to a pre-trained encoder \te, the actual images in \tti models are generated by a diffusion model, \dm, parameterized by $\theta$.
During training of \dm, Gaussian noise is added to an initial image $x_0$ for $T$ time steps to produce $x_T$, in a process known as the \emph{forward diffusion process}. The noise is then iteratively removed to approximate the initial image $\tilde{x_0}$ in the \emph{reverse diffusion process}.
During inference, the reverse diffusion process generates an image from noise.
Further, \dm can be conditioned with a textual prompt \prompt to guide the generation of $\tilde{x_0}$ to match the description in \prompt. After generating $\phi_p(\prompt)$, %from \te, 
\dm is trained by minimizing the following loss function: $\mathcal{L} = \mathbb{E}_{\epsilon, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(\imgclean_t,\phi_p(\prompt),t)||_2^2]$ for each time step $t$, and random Gaussian noise $\epsilon \sim \mathcal{N}(0,1)$.

Several prominent \tti models (e.g., Stable Diffusion v1.4 (SDv1.4)) improve the efficiency of the diffusion process by conducting it in the embedding space of a variational autoencoder (VAE), rather than on images \cite{stable-diffusion}. For a VAE decoder $\mathit{D}$, VAE encoder $\mathcal{E}$, and $z_t \in \mathcal{E}(\imgclean)$ as the latent representation of $\imgclean$ in the VAE's latent space, \dm is trained by minimizing the following objective: \\
$\mathcal{L} = \mathbb{E}_{\epsilon, z_t, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(z_t,\phi_p(\prompt),t)||_2^2]$ where $\epsilon \sim \mathcal{N}(0,1)$. The final image is generated from the approximation, $\tilde{z_0}$, by passing it through $\mathit{D}$: $\tilde{x_0} = \mathit{D}(\tilde{z_0})$.  Table~\ref{tab:notations} in Appendix~\ref{app:notations} summarizes frequently used notations.

 




\subsection{Concept Removal Techniques}\label{back-conceptrem}

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance?--- We use the same approach for selecting acceptable concepts as Kumari et. al.~\cite{kumari2023ablating}for group 2 and group 3 concepts. For these groups, the acceptable concept is a superset of the unacceptable concept. For example, the sex of a celebrity is the acceptable concept for a celebrity. For group 1, there is no clear definition of a superset (eg. the superset of \emph{nude} is unclear). Logically, the acceptable concept is the opposite of the unacceptable concept in this case since it is clearly defined. - SHOULD MOVE THIS EXPLANATION ELSEWHERE}

The textual phrase for an acceptable concept is $\cacc$, and for an unacceptable concept is $\cunacc$. 
For a given $\cunacc$, $\cacc$ is either the opposite (e.g., $\cunacc$ = \emph{violence} vs. $\cacc$ = \emph{peaceful}) or a general category of a specific character/object/person (e.g., $\cunacc$ = \emph{R2D2} vs. $\cacc$ = \emph{robot}). We discuss the selection of $\cacc$ for a given $\cunacc$ in Section~\ref{sec:concepts}.
An image $\imgclean$ generated from a \tti model may either contain an unacceptable concept (referred to as $\imgunacc$) or an acceptable one (referred to as $\imgacc$). Similarly, a text prompt $\prompt$ may contain a phrase for an acceptable concept ($\promptacc$) or an unacceptable concept ($\promptuacc$). An example of an unacceptable prompt $\promptuacc$ containing an unacceptable concept $\cunacc$ = \emph{Captain Marvel}, is ``\emph{Captain Marvel} soaring through the sky''. \crt{s} seek to thwart the generation of $\imgunacc$ by either fine-tuning the \tti model to suppress $\imgunacc$, or using a classifier as a filter to detect $\imgunacc$, and serve a replacement image instead. 
%
We first present six state-of-the-art fine-tuning \crt{s}:

\noindent\textbf{Concept Ablation (\ca)~\cite{kumari2023ablating}} fine-tunes the \tti model to minimize the KL divergence between the model's output for $\promptuacc$ and $\promptacc$ to force the generation of \imgacc instead of \imgunacc. Formally, they optimize the following objective function: 
 % \text{argmin}_\theta 
\[\begin{split}
\footnotesize
   \mathcal{L}_{\ca} =  \mathbb{E}_{\epsilon, z_t, \cunacc, \cacc, t}[w_t||\epsilon_\theta(z_t,\phi_p(\promptacc),t).sg() \\
    - \epsilon_\theta(z_t,\phi_p(\promptuacc),t)||_2^2]
\end{split}\]
where $\epsilon \sim \mathcal{N}(0,1)$, $z_t \in \mathcal{E}$, and $w_t$ is a time-dependent weight, and $.sg()$ is the stop-gradient operation.

\noindent\textbf{Forget-Me-Not (\forgetNot)~\cite{zhang2023forgetmenot}} minimizes the activation maps for $\cunacc$ by modifying \dm's cross-attention layers. Further, fine-tuning \dm, instead of just the cross-attention layers, results in degraded utility. 
% That is, given $a_i \in \mathcal{A}_i$, the $i$-th attention map in \dm of \tti, their loss is 
% \[\mathcal{L} = \sum_{a_i \in \mathcal{A}_i}||a_i||\]


\noindent\textbf{Selective Amnesia (\sa)~\cite{heng2023selective}} fine-tunes \tti models by adapting continuous learning techniques (elastic weight consolidation and generative replay) for \tti models to forget a concept. They optimize $\mathbb{P}(\imgclean|\theta^*,\cunacc)$, the probability of generating $\imgclean$ given $\theta^*$ and $\cunacc$, where $\theta^*$ are the frozen parameters of the original \tti model: 
\[
\begin{split}
\footnotesize
    \mathcal{L}_{\sa} = -\mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_f(\cunacc)}[\text{log}\mathbb{P}(\imgclean|\theta^*,\cunacc)] -\lambda\sum_i\frac{M_i}{2}(\theta_i^*-\theta_i)^2\\
     + \mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_r(\cacc)}[\text{log}\mathbb{P}(\imgclean|\theta,\cacc)]
\end{split}
\]
where $M$ is the Fisher information matrix over $\cacc$ and $\cunacc$, $\mathbb{P}_r$ and $\mathbb{P}_f$ are probabilities taken over the distributions of $\cacc$ and $\cunacc$ respectively, and $\lambda$ is a regularization parameter. 



\noindent\textbf{Erased Stable Diffusion (\esd)~\cite{gandikota2023erasing}} fine-tunes the \tti model by modifying the reverse diffusion process to reduce the probability of generating \imgunacc:
\[\begin{split}
\epsilon_\theta(\imgclean_t,\phi_p(\cunacc),t) = \epsilon_{\theta^*}(\imgclean_t, t)
+ \eta(\epsilon_{\theta^*}(\imgclean_t,\phi_p(\cunacc),t)\\-\epsilon_{\theta^*}(\imgclean_t,t))
\end{split}\]
where $\eta > 0$ encourages the noise conditioned on $\cunacc$ to match the unconditioned noise.


\noindent\textbf{Unified Concept Editing (\unifiedCE)~\cite{gandikota2023unified}} fine-tunes the \tti model's cross-attention layers with a language model to minimize the influence of $\cunacc$, while keeping the influence of remaining concepts unchanged. Their optimization is:
% \text{min}_W
\[\begin{split}
    \mathcal{L}_{\unifiedCE} = \sum_{\cunacc \in \mathcal{C}^{u}, \cacc \in \mathcal{C}^{a}}||W\times\cunacc-W^*\times\cacc||_2^2 \\ 
    +  \sum_{c \in S}||W\times c - W^*\times c||_2^2
\end{split}\]
where $W$, $W^*$ are the parameters of the fine-tuned and original \emph{cross-attention layers in \dm}, $\mathcal{C}^{u}$ and $\mathcal{C}^{a}$ are the space of pre-defined unacceptable and acceptable concepts, and $S$ is a set of concepts for which to preserve utility. 

\noindent\textbf{Safe diffusion (\sdd)~\cite{kim2023towards}}
fine-tunes the \tti model by encouraging the diffusion model noise conditioned on $\cunacc$ to match the unconditioned noise, while minimizing the utility drop using the following objective function:
\[\begin{split}
    % \text{argmin}_\theta
    \mathcal{L}_{\sdd} = \mathbb{E}_{\epsilon, z_t, \cunacc, t}[||\epsilon_\theta(z_t,\phi_p(\cunacc),t) 
 - \epsilon_\theta(z_t,t).sg()
    ||_2^2]
\end{split}\]
where $\epsilon \sim \mathcal{N}(0,1)$ and $z_t \in \mathcal{E}(x)$.

\noindent We now describe two filtering \crt{s}:

\noindent\textbf{Stable Diffusion Filter (SD-Filter)~\cite{radford2021learning}} is black-box and the design of the filter is not publicly available. However, Rando et. al.~\cite{rando2022redteaming} hypothesize that it involves computing the cosine similarity between the embeddings of a generated image, $\imgclean$, and a pre-defined set of $\cunacc$. If the cosine similarity is greater than some threshold ($\Gamma$), then $\imgclean$ has $\cunacc$. Formally, their filter $\filter_{SD}$ can be described as
\[ \filter_{SD}(\imgclean) = \begin{cases} 
      1 & \text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) > \Gamma \\
      0 & \text{otherwise}
   \end{cases}
\]
where $\text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) = \overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\cunacc)}$, and $\overline{\cdot}$ denotes normalization. Here $\filter_{SD}(\imgclean) = 0$ indicates \imgacc and $\filter_{SD}(\imgclean) = 1$ indicates \imgunacc. Note that $\Gamma$ varies with $\cunacc$. 


\noindent\textbf{Unsafe Diffusion (\unsafediff)~\cite{unsafeDiff}} is the current state-of-the-art filtering \crt and outperforms SD-Filter~\cite{unsafeDiff}. \unsafediff trains a multi-headed neural network classifier on top of CLIP to identify $\imgunacc$ where each head classifies different $\cunacc$: \emph{nudity, violence, disturbing, hateful}, and \emph{political}. Their objective is given as $\filter_{\unsafediff}(\imgclean) = \text{MLP}(\phi_x(\imgclean))$ where MLP is a multi-layer perceptron, and $\filter_{\unsafediff} \in \{0,1\}$.


\subsection{Evading Concept Removal Techniques}\label{back-attacks} 

An adversary (\adv) may construct adversarial prompts ($\advprompt$) to evade \crt{s} and force the \tti model to generate unacceptable images. We denote a dataset containing adversarial prompts and their corresponding images ($\imgadv$) as $\dtestadv = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$ where ideally $\imgadv$ will contain $\cunacc$.
\adv is assumed to account for the target \tti model \target, using a \crt. A dumb \adv who does not account for this is \emph{na\"{i}ve}. 

\adv's objective is to construct $\advprompt$ which can force a \tti model to output images with $\cunacc$ while being semantically closer to acceptable prompts so that $\imgadv$ is incorrectly identified as acceptable while triggering the generation of unacceptable images.
The existing attacks formulate the construction of $\advprompt$ as an optimization problem using some reference $\imgunacc$ (or the difference between $\promptacc$ and $\promptuacc$) as the ground truth. Different attacks vary in ways to solve this optimization. We present four state-of-the-art attacks below:

\noindent\textbf{PEZ~\cite{wen2023hard}} constructs $\advprompt$ by identifying text tokens by minimizing: $\mathcal{L}_{PEZ}= 1-\text{cos}(\phi_p(\advprompt),\phi_x(\imgunacc))$. 



\noindent\textbf{RingBell~\cite{Tsai2023RingABellHR}} identifies tokens for $\advprompt$ by first calculating the average difference between the embedding vectors of $\promptuacc$ and $\promptacc$: $\phi_p(\hat{\prompt}) = \frac{1}{N}\sum_{i=1}^N\{\phi_p(\promptuacc_i) - \phi_p(\promptacc_i)\}$ from a set of $N$ prompts. Then, RingBell computes $\advprompt$ by minimizing the distance of its text embedding to ($\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))$, formulated as: $\text{min}_{\advprompt} ||\phi_p(\advprompt) - (\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))||^2$ where $\prompt^{init}$ is an initial unacceptable prompt which is censored by a \crt. They solve this using a genetic algorithm. 
%Further, the optimization relies on a fitness function using mean-squared error: $\mathcal{L}_{RingBell} = \mathcal{L}_{MSE}(\phi_p(\cunacc),\phi_p(\advprompt))$ where $\cunacc$ is a prompt that generates $\imgunacc$ in a \tti model.


\noindent\textbf{SneakyPrompt~\cite{yang2023sneakyprompt}} uses reinforcement learning to construct $\advprompt$ specifically against filtering \crt{s}. Given an initial prompt $\prompt^{init}$, the attack searches for tokens to update $\prompt^{init}$ to form $\advprompt$. The reward function is the cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\advprompt)$. Typically, they use $\promptuacc$ as $\prompt^{init}$ for better effectiveness and faster convergence.

\noindent\textbf{CCE~\cite{pham2023circumventing}} uses textual-inversion to construct $\advprompt$~\cite{gal2022textualinversionimage}. \adv updates CLIP's vocabulary to include a new token ``<s>'' which, when included in $\advprompt$, generates \adv's desired image. To optimize <s>, we find $v$, an embedding for <s>, corresponding to least loss $\mathcal{L}_{CCE}=\mathcal{L}_{MSE}(\epsilon, \epsilon_\theta(z_t,v,t))$, where $\epsilon\sim\mathcal{N}(0,1)$, and $\mathcal{L}_{MSE}$ is the mean-squared-error. 


All of these attacks are na\"{i}ve except for CCE and SneakyPrompt, which account for different fine-tuning \crt{s}. 
In Section~\ref{sec:baseline}, we describe how we modify these na\"{i}ve attacks to account for \crt{s}.

==> old_versions/3problem.tex <==
\section{Problem Statement}\label{sec:problem}


Our goal is to design a \crt which can effectively detect unacceptable concepts in images generated from \tti models. We describe an adversary model, requirements of an ideal \crt, and limitations of prior works according to the requirements.


\noindent\textbf{Adversary Model.} We assume (blackbox) access to a deployed target \tti model ($\target$) to which a client can send an input ($\prompt$) to generate an image ($\imgclean$). Further, $\target$ uses some \crt. The goal of the adversary (\adv) is to force $\target$ to generate $\imgunacc$ despite the presence of a \crt to suppress it.
We give an advantage to \adv by allowing whitebox access to a local identical copy of $\target$ with the \crt for use in designing attacks. This is reasonable as \dm and CLIP are publicly available. For filtering \crt{s}, we assume that \adv has whitebox access to the filter to use its loss function in designing the attacks.

\noindent\textbf{Requirements} An ideal \crt should be:
\begin{enumerate*}[label=\textbf{R\arabic*},leftmargin=*]
\item\label{effective} \textit{Effective} in minimizing the generation of $\imgunacc$;
\item\label{utility} \textit{Utility-preserving}, maintaining the quality of acceptable images (for fine-tuning \crt{s}) or not blocking them (for filtering \crt{s}); and
\item\label{robust} \textit{Robust} to resist evasion with adversarial prompts ($\advprompt$).
\end{enumerate*}



\noindent\textbf{Limitations of Prior Works.} 
%We now briefly discuss the limitations of different types of prior \crt{s} \emph{vis-a-vis} the requirements above. 
In Section~\ref{sec:evaluation}, we empirically show the limitations of prior works by evaluating \ref{effective}, \ref{utility}, and \ref{robust} of different \crt{s}. We provide a brief summary here.
\textit{Fine-tuning \crt{s}} modify $\target$ thereby explicitly creating a trade-off between effectiveness (\ref{effective}) and utility (\ref{utility})~\cite{gandikota2023erasing,kumari2023ablating,zhang2023forgetmenot,heng2023selective,heng2023selective,gandikota2023unified,kim2023towards}.
Further, these \crt{s} do not consider robustness (\ref{robust}) in their design and are susceptible to evasion by \adv with $\advprompt$. 
\textit{Filtering \crt{s}}~\cite{radford2021learning,unsafeDiff} detect unacceptable concepts either in $\prompt$ (aka prompt filter) or in $\imgclean$ and block them (a.k.a image filter). Since, they do not modify $\target$, they can maintain utility without impacting effectiveness. Prior filtering approaches may not be accurate in detecting unacceptable concepts (impacts \ref{effective})~\cite{li2024safegen}.
They can also be easily evaded (harms \ref{robust}) (\cite{rando2022redteaming} and Section~\ref{sec:filterEval}). Further, the current state-of-the-art filter, \unsafediff~\cite{unsafeDiff}, trains specialized classifiers for each concept on substantial data, which limits their generalization to new concepts.


==> old_versions/4approach.tex <==
\section{\method: Robust Filtering CRT}\label{sec:approach}

We present \method, a robust \underline{co}ncept \underline{fi}ltering \crt which aims to satisfy the requirements from Section~\ref{sec:problem} and achieve a better trade-off than prior \crt{s}. 
\method uses a classifier \filter to detect images and filter unacceptable concepts in generated images. Following SDv1.4, on detecting an unacceptable concept, \method generates a replacement image~\cite{radford2021learning, rando2022redteaming}.
We identify CLIP as the natural choice for such a classifier as it is
\begin{enumerate*}[leftmargin=*]
\item pre-trained on a large dataset covering a wide range of concepts, and
\item used across many \tti models, and encodes similar information as seen in them.
\end{enumerate*}
Hence, CLIP is a better choice for a filter than training specialized classifiers for each concept (e.g.,~\cite{unsafeDiff}).

 However, simply using CLIP for \method is not sufficient as seen in Stable Diffusion's filter ($\filter_{SD}$)~\cite{radford2021learning}. 
$\filter_{SD}$ thresholds the cosine similarity between the embeddings of $\imgclean$ and each pre-defined unacceptable concept to identify $\imgunacc$. 
Rando et al.~\cite{rando2022redteaming} design adversarial prompts ($\advprompt$) to evade $\filter_{SD}$. 
Since $\filter_{SD}$ uses only the cosine similarity to $\cunacc$, it gives \adv the freedom to modify the prompt embeddings in \emph{any direction}, while constructing $\advprompt$, to force a misclassification.
%
We address this in \method by (a) configuring CLIP's classification objective for effectiveness and robustness, and (b) fine-tuning to further improve utility. 

\noindent\textbf{Configuring CLIP's Classification Objective.} Instead of using the cosine similarity to only $\cunacc$ as in $\filter_{SD}$, we configure the objective function of \method for filtering $\imgunacc$ by using the cosine similarity to \emph{both} $\cunacc$ and $\cacc$. 
% \change{This makes \adv's goal more difficult as they are forced to optimize $\advprompt$ such that the resulting image embedding is far from $\phi_p(\cunacc)$, \emph{and} close to $\phi_p(\cacc)$, which is an additional stipulation arising from the design of \method.}
Further, jointly optimizing for two embeddings yields better utility as observed in prior fine-tuning \crt{s}~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}. 

Given $\imgclean$, \method checks the cosine similarity of $\phi_x(\imgclean)$ to $\phi_p(\cunacc)$ and $\phi_p(\cacc)$. Formally, we define \method as $\filter(x, \cunacc, \cacc)$
\begin{equation}\label{eq:att}
 = \text{argmax}_{i, i\in{a,u}} \left\{\frac{\text{exp}{(\text{cos}(\phi_x(x),\phi_p(\concept_i)) / \tau)}}{\sum_{j \in \{a,u\}}\text{exp}(\text{cos}(\phi_x(x),\phi_p(\concept_j)) / \tau)}\right\}
\end{equation} 
where $\tau=\frac{1}{100}$ is the default temperature parameter used in CLIP. 
Further, the cosine similarity is equivalent to the scaled Euclidean distance between the embeddings~\cite{ModalityGap}: 
\[(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) = 2-2\overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\concept)}\]
\[\implies \text{cos}(\imgclean, \concept) = -\frac{1}{2}(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) + 1\]
Hence, by using CLIP as a filter, we project the image embeddings onto the vector between $\cunacc$ and $\cacc$ and classify it based on its distance to both.  
%
This simple configuration change in CLIP's classification objective restricts \adv to adding noise only along the low-dimensional vector joining $\cunacc$ and $\cacc$: $\phi_p(\cunacc) - \phi_p(\cacc)$ in the direction of $\cacc$.
This is more challenging for \adv to evade than $\filter_{SD}$, as projecting to a lower-dimensional representation can improve robustness~\cite{pca1,pca2}.
Hence, we conjecture that this can help satisfy \ref{effective} and \ref{robust} (as shown later in Section~\ref{sec:evaluation}).

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance? - ANSWERED}


% \change{Rationale for fine-tuning?}
\noindent\textbf{Fine-tuning.} The above configuration change may impact the utility on some concepts due to the close proximity of some $\cunacc$ and $\cacc$.
To restore any drop in utility, we use fine-tuning. 
We use two different fine-tuning variants depending on the group of concepts.


For the case where $\cunacc$ and $\cacc$ are opposites (e.g., Group-1 concepts where $\cunacc$ = \emph{violence} and $\cacc$ = \emph{peaceful}), the above objective function might have a low correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$. This might result in poor utility. We use following objective function:

\begin{equation}\label{eq:ft2}
    \begin{split}
        \mathcal{L}_{\method} = \alpha_{\text{aa}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{aa}) 
        -\alpha_{\text{ua}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{ua}) \\
        + \alpha_{\text{uu}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{uu})  
        -\alpha_{\text{au}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{au}) \\
        +\alpha_{\text{uu-t}}\mathcal{L}_{MSE}(\phi_p(\mathcal{P}^{u}), \phi_p(\mathcal{P}^{a})) \\
    \end{split}
\end{equation}
where $\mathcal{D}_{aa} = \{(\imgacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{au} = \{(\imgacc_j, \promptuacc_j)\}_{j=1}^N$, \\$\mathcal{D}_{ua} = \{(\imgunacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{uu} = \{(\imgunacc_j, \promptuacc_j)\}_{j=1}^N$, $\mathcal{P}^u = \{\promptuacc_j\}$, and $\mathcal{P}^a = \{\promptacc_j\}$, and $\alpha_\cdot$ are regularization hyperparameters. We assign equal weight to each of the loss terms, thus choosing $\alpha_{(.)}= 1$. 
The above objective function encourages the CLIP embeddings of $\imgunacc$ and $\promptuacc$, and $\imgacc$ and $\promptacc$, to be closer together while increasing the distance between $\imgunacc$ and $\promptacc$, and $\imgacc$ and $\promptuacc$, respectively. 
% \change{We were required two different fine-tuning methods because in the case where the unacceptable and acceptable prompts were opposites, simply optimizing the distance between their prompt embeddings without considering the image embeddings resulted in the CLIP model forgetting the mapping between the prompts and their corresponding images, resulting in poor filtering performance. Conversely, when Equation~\ref{eq:ft2} was used to optimize unacceptable/acceptable pairs where the acceptable concept was a general category, the performance was poor. We attribute this to overfitting, since images depicting characters/objects/celebrities are less varied than those depicting violence and nudity.}

In contrast, for concepts in Group-2 and 3, we fine-tune \filter to maximize the distance between $\phi_p(\promptuacc)$ and $\phi_p(\promptacc)$, and hence, minimize the following loss:
\begin{equation}\label{eq:ft1}
L_{\method} = -||\overline{\phi_p(\promptuacc) - \phi_p(\promptacc)}||_2
\end{equation}
We use prompts ($\promptuacc$ and $\promptacc$) for fine-tuning in Equation~\ref{eq:ft1} and Equation~\ref{eq:ft2} instead of only concepts ($\cunacc$ and $\cacc$): 
$\promptuacc$ and $\promptacc$ already contain $\cunacc$ and $\cacc$, and provide more context. 
% The prompts used for the \tti model are not known before-hand, but we can define the concepts to be filtered. 
% Since the prompt includes these concepts, filtering the images generated from the prompts is sufficient.

During fine-tuning of \method, there is a trade-off between effectiveness and utility which is inherent to all other fine-tuning \crt{s} as well. We subject our fine-tuning to the constraint that achieved the highest effectiveness for the least drop in utility.
We empirically show the benefit of fine-tuning in Appendix~\ref{app:FTEspresso}: Table~\ref{tab:FTImpact}).


% \change{Sec. 4 - A clear step-by-step overview of the Espresso generation pipeline is missing. Please consider adding a diagram.}




% \noindent\textbf{Replacement of Blocked Images.} 
% Following SDv1.4, on detecting $\imgunacc$, \method generates a replacement image~\cite{radford2021learning, rando2022redteaming}.
% As with other filters, on detecting $\imgunacc$, \method generates a replacement image as in SDv1.4~\cite{radford2021learning}.

% \input{tables/tab_nofinetune_effective}

==> old_versions/5setup.tex <==
\section{Experimental Setup}\label{sec:setup}

% \input{figures/fig_trainvaltest}
We use Stable Diffusion v1.4~\cite{stable-diffusion} and its default configuration as the target \tti model following prior \crt{s}~\cite{gandikota2023erasing, kumari2023ablating, zhang2023forgetmenot, heng2023selective, gandikota2023unified, kim2023towards}.
We describe the attack baselines against \crt{s} (Section~\ref{sec:baseline}), metrics (Section~\ref{sec:metrics}), different concepts used for evaluation (Section~\ref{sec:concepts}), and pipeline used for evaluating \crt{s} (Section~\ref{sec:pipeline}).
% dataset and model configuration (Section~\ref{sec:datasets}).

\subsection{Revisiting Attack Baselines}\label{sec:baseline}

% We compare \method with prior state-of-the-art \crt{s} across \ref{effective}, \ref{utility}, and \ref{robust}. 
% We use six fine-tuning \crt{s} (\ca, \forgetNot, \sa, \esd, \unifiedCE, and \sdd) and one filtering \crt (\unsafediff) which are described in Section~\ref{back-conceptrem}. For filtering \crt, we do not compare with SD-Filter as \unsafediff outperforms it.
% To evaluate \ref{robust}, 
We consider different state-of-art attacks from literature (Section~\ref{back-attacks}).
We modify existing na\"{i}ve attacks (indicated with ``+''), Ring-a-Bell, and PEZ, to account for \crt{s}. 
All \crt{s} use some variant of the following optimization: detach $\cunacc$ from $\prompt$ such that the generated image is far from $\cunacc$ and closer to some $\cacc$. 
On the other hand, attacks against \tti models described in Section~\ref{back-attacks}, design $\advprompt$ such that $\imgadv$ is closer to $\cunacc$ and far from $\cacc$. 
Hence, to design an effective attack which accounts for such \crt{s}, in addition to the attacks' original objectives, we minimize the loss between the embeddings of $\advprompt$ and $\cacc$ while increasing the loss with the embeddings of $\cunacc$.
% Hence, an effective attack which accounts for such \crt{s} must find $\advprompt$ such that its generated image is unacceptable (via the attacks' original objective) in spite of the \crt. To do this, in addition to the attacks' original objectives, we minimize the loss between $\advprompt$ and $\cacc$ while increasing its loss with $\cunacc$.
% Hence, to design an effective attack which accounts for such \crt{s}, 
This, in turn, will move $\phi_p(\advprompt)$ closer to $\phi_p(\cacc)$ and farther from $\phi_p(\cunacc)$.
% \change{Since the attack objective is opposite to that of \crt{s}, the attack finds $\advprompt$ which counters the expected benefits of \crt{s}.}
% \change{This allows the generated image from $\advprompt$ to be incorrectly identified as acceptable while preserving the ability to generate $\imgunacc$.}
%
We modify the attacks to construct $\advprompt$ using following loss: 
\begin{equation}\label{eq:attack}
    \begin{split}
\mathcal{L}_{att+} = \mathcal{L}_{att} - \alpha_u \mathcal{L}_{MSE}(\phi_p(\cunacc), \phi_p(\advprompt)) + \\
\alpha_a \mathcal{L}_{MSE}(\phi_p(\cacc), \phi_p(\advprompt))
    \end{split}
\end{equation}
where $att \in \{RingBell, PEZ\}$ when $\crt \in \{$\ca, \forgetNot, \sa, \esd, \unifiedCE, \sdd, \unsafediff, \method$\}$, and $\mathcal{L}_{att}$ is from Section~\ref{back-conceptrem}.
We assign equal weight to all loss terms and use $\alpha_u = \alpha_a = 1.$
% Further, To design attacks against \unsafediff and \method, .
Recall from Section~\ref{back-attacks} that CCE already accounts for different fine-tuning \crt{s}. For filtering \crt{s} (\unsafediff and \method), we modify CCE using Equation~\ref{eq:attack} and call this attack CCE+. 


Finally, typographic attack~\cite{noever2021typographicattck} against CLIP is where text characters are superimposed onto an (unrelated) image to fool CLIP by forcing it to focus on this text instead of the image. We turn this into an attack against \crt{s} by superimposing $\cacc$ at the bottom of $\imgunacc$. Using the resulting adversarial images, we use PEZ+ to find their corresponding $\advprompt$. We call this attack \emph{Typo+}.



\subsection{Metrics}\label{sec:metrics}

We now describe the metrics to evaluate each of the requirements. We assume access to a \emph{reference CLIP}, separate from \target with the \crt{s}. The reference CLIP is a Stable Diffusion v1.4 model, a standard assumption in prior work~\cite{kumari2023ablating, gandikota2023erasing,gandikota2023unified,kim2023towards}.

\noindent\textbf{\underline{\ref{effective} (Effectiveness).}} Depending on the \crt, we use:
\begin{itemize}[leftmargin=*,wide,labelindent=0pt]
\item \textbf{CLIP accuracy}~\cite{hessel-etal-2021-clipscore,kumari2023ablating} for fine-tuning \crt{s}. This is the cosine similarity (divided by temperature parameter $\tau'=\frac{1}{100}$ of the reference CLIP) between the embeddings of the generated image $\imgclean$ with the embeddings of $\cunacc$ and $\cacc$ from the reference CLIP. This outputs the likelihood of predicting $\cunacc$. Hence, CLIP accuracy should be low (ideally zero) for effective concept removal. Formally, it is:
\[\frac{\text{exp}{(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc) / \tau'))}}{\text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc) / \tau')) + \text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cacc) / \tau'))}\]
where $\tilde{\phi_p}$ and $\tilde{\phi_x}$ are embeddings from the reference CLIP.
For filtering \crt, if $\imgunacc$ is detected, a replacement image is generated. Here, we calculate the CLIP accuracy on the final set of images after filtering. 
% Since the metrics compare with baseline reference CLIP, we use the same default replacement image as in the SD v1.4 filter.

\item \textbf{False Negative Rates (FNR)~\cite{unsafeDiff,rando2022redteaming}} for filtering \crt{s} is the fraction of images with $\cunacc$ which are not blocked. 
It should be low (ideally zero).
\end{itemize}


\noindent\textbf{\underline{\ref{utility} (Utility).}} Depending on the \crt, we use: 
\begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\item \textbf{Normalized CLIP score} for fine-tuning \crt{s} is is the ratio of cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$ from \target, compared to that from a reference CLIP as a baseline which is assumed to have the maximum achievable CLIP score. Formally, $\frac{\text{cos}(\phi_x(\imgclean),\phi_p(\prompt))}{\text{cos}(\tilde\phi_x({\imgclean}), \tilde\phi_p(\prompt))}$. 
Normalized CLIP score should be high (ideally one) for high utility. 
For the normalized CLIP score to be greater than one, the fine-tuned \tti model should generate images that match their prompts more closely than the original \tti model. This is unlikely to occur in practice as seen in our evaluation (c.f. Table~\ref{tab:utility}).
This metric is different from standard CLIP score from prior work~\cite{hessel-etal-2021-clipscore,kumari2023ablating, kim2023towards, gandikota2023unified} which measures the cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$ from \target. 
%We did this to scale the original CLIP score between zero and one while comparing \target to the reference CLIP.
We did this to compare the utility of the \tti with the \crt to that of the \tti without the \crt.
Hence, a perfect match between them will give a normalized CLIP score of one.

\item \textbf{False Positive Rates (FPR)~\cite{unsafeDiff,rando2022redteaming}} for filtering \crt{s} is the fraction of images without $\cunacc$ which are blocked.
It should be low (ideally zero).
\end{itemize} 


\noindent\textbf{\underline{\ref{robust} (Robustness).}} We use the same metrics as effectiveness: CLIP accuracy to evaluate fine-tuning \crt{s} and compare \method with them, and FNR for filtering \crt{s}. 




\subsection{Concept Types}\label{sec:concepts}

% \noindent\textbf{Concept Types.} 
We use the same set of unacceptable concepts as in prior work~\cite{kumari2023ablating, pham2023circumventing, kim2023towards}, categorizing them into three groups:
\begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\item Group-1 covers inappropriate concepts such as \emph{nudity} (e.g., female breasts or male/female genitalia), \emph{violence} (e.g., bloody scenes, fighting, burning, hanging, weapons, and wars), \emph{disturbing} (e.g., distorted faces, bodies, human flesh, or bodily fluids), and \emph{hateful} (e.g., defamatory racial depiction, harmful stereotypes, or Holocaust scenes).
\item Group-2 covers copyright-infringing concepts such as \emph{Grumpy Cat, Nemo, Captain Marvel, Snoopy}, and \emph{R2D2}.
\item Group-3 covers (unauthorized) use of personal images for celebrities such as \emph{Taylor Swift, Angelina Jolie, Brad Pitt}, and \emph{Elon Musk}.
\end{itemize}



\subsection{Pipeline for Evaluating \crt{s}}\label{sec:pipeline}

We now describe the pipeline which includes identifying acceptable concepts (step 1), generation of datasets (step 2), training filters or fine-tuning \tti models with \crt{s} (step 3), and validating acceptable concepts (step 4), and evaluating different \crt{s} (step 5). We present an overview of the pipeline in Figure~\ref{fig:pipeline} and describe each of the steps below.

\input{figures/fig_pipeline}



\subsubsection*{\underline{Step 1: Identifying Acceptable Concepts}}
A good choice of $\cacc$ is one which effectively steers a \tti model away from generating $\imgunacc$ while maintaining utility on other concepts. Hence, the choice of $\cacc$ can impact the overall effectiveness and utility of \crt{s}. 
We select $\cacc$ for a given $\cunacc$ such that it is either opposite to $\cunacc$ (Group-1) or is a semantic generalization of $\cunacc$ so as to avoid infringing copyrights (Group-2,3).
For $\cunacc$ in Group-1, we consider multiple alternative synonyms for $\cacc$ from which we choose the best possible candidate by measuring effectiveness and utility on a validation dataset (c.f. Step 4).
For $\cunacc$ in Group-2,3, we use $\cacc$ chosen by prior works~\cite{kumari2023ablating,heng2023selective} for a fair comparison.
% by evaluating the effectiveness and utility of using different synonyms on a validation dataset  and choosing the best possible candidate.
% We specify a matching $\cacc$ for every $\cunacc$ so that \crt{s} can steer away a \tti model from generating $\cunacc$ concepts and instead focus on $\cacc$. 
% For Group-1, we present the possible alternatives for $\cacc$, and for Group-2,3 we present the $\cacc$ taken from prior work. 
We indicate them in the format ``$\cunacc$ $\rightarrow$ $\cacc$'':
\begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\item \textbf{Group-1}: $\cacc$ is the opposite of $\cunacc$. We consider the following choices of $\cacc$: \emph{nudity} $\rightarrow$ \{\emph{clothed} and \emph{clean}\}; \emph{violence} $\rightarrow$ \{\emph{peaceful}, \emph{nonviolent}, and \emph{gentle}\}; \emph{disturbing} $\rightarrow$ \{\emph{pleasing}, \emph{calming}, and \emph{soothing}\}; \emph{hateful} $\rightarrow$ \{\emph{loving}, \emph{compassionate}, and \emph{kind}\}.
% For instance, \emph{violence} $\rightarrow$ \emph{peaceful}, \emph{disturbing} $\rightarrow$ \emph{pleasing}, and \emph{hateful} $\rightarrow$ \emph{loving}. For \emph{nudity}, we chose \emph{clean}.
% compared \emph{clothed} with \emph{clean} on a separate validation dataset (c.f. Section~\ref{sec:datasets} and Table~\ref{tab:valconfig}), and eliminated \emph{clothed} because it blocked images with minimal exposed skin despite being acceptable~\cite{unsafeDiff,schramowski2022safe}.
% Similarly, we evaluated and eliminated alternatives of $\cacc$ for \emph{violence} (\emph{nonviolent}, and \emph{gentle}), \emph{disturbing} (\emph{calming}, and \emph{soothing}), and \emph{hateful} (\emph{compassionate}, and \emph{kind}). 
\item \textbf{Group-2}: $\cacc$ is the type of $\cunacc$, following prior works~\cite{kumari2023ablating,heng2023selective,gandikota2023erasing}. For instance, \emph{Grumpy Cat} $\rightarrow$ \emph{cat}, \emph{Nemo} $\rightarrow$ \emph{fish}, \emph{Captain Marvel} $\rightarrow$ \emph{female superhero, Snoopy} $\rightarrow$ \emph{dog}, and \emph{R2D2} $\rightarrow$ \emph{robot}. 
\item \textbf{Group-3}: $\cacc$ is the sex of $\cunacc$, following prior works~\cite{heng2023selective, zhang2023forgetmenot, kim2023towards}: \{\emph{Taylor Swift, Angelina Jolie}\} $\rightarrow$ \emph{woman} and \{\emph{Brad Pitt, Elon Musk}\} $\rightarrow$ \emph{man}.
\end{itemize}



% \subsection{Dataset and Model Configurations}\label{sec:datasets}

\subsubsection*{\underline{Step 2: Generate and Split Datasets}}

We describe the generation of train, validation, and test datasets.

\noindent\textbf{Train Datasets.}
We summarize the different training/fine-tuning dataset configurations across \crt{s} in Table~\ref{tab:trconfig}. 

\input{tables/tab_trconfig}

\noindent\emph{Fine-tuning \crt{s}.} Different fine-tuning \crt{s} use different dataset configurations to ensure that \ref{effective} and \ref{utility} are met. We use the exact same configuration as described in each of the prior works to ensure that they satisfy the requirements claimed in their papers. While the configuration across different \crt{s} vary, the configuration for a specific \crt across different concepts is the same, in accordance with the instructions in the respective works. We briefly summarize them in Table~\ref{tab:trconfig}. \ca uses acceptable prompts which are generated from ChatGPT such that they contain $\cacc$, and 1 image per prompt. \esd and \sdd both use an unacceptable concept, and \sdd additionally uses 10 images corresponding to $\cunacc$. All images are generated using SD v1.4. 
\forgetNot uses unacceptable prompts of the form ``An image of \{$\cunacc$\}'', and 1 image per prompt.
For all the fine-tuning \crt{s}, we use their publicly available code for training to ensure the configuration is same as reported in their papers~\cite{githubGitHubNupurkmr9conceptablation,githubGitHubRohitgandikotaerasing,githubGitHubSHILabsForgetMeNot,githubGitHubRohitgandikotaunifiedconceptediting,githubGitHubClearnusselectiveamnesia,githubGitHubNannullnasafediffusion,githubGitHubYitingQuunsafediffusion}.



\noindent\emph{Filtering \crt{s}.} We train $\filter_{\unsafediff}$ using its exact dataset configuration (Table~\ref{tab:trconfig}) and code~\cite{unsafeDiff}. 
For \method, we follow the template by Kumari et al.~\cite{kumari2023ablating} to generate 10 unacceptable and acceptable prompts using ChatGPT, with one image per prompt from SDv1.4.
For Group-2 concepts, we randomly select 10 ChatGPT-generated prompts from the datasets provided by Kumari et al.~\cite{kumari2023ablating}.
Our choice for having a small amount of training data is inspired from prior works on poisoning attacks which show that little data is required to modify CLIP~\cite{yang2023robust, carlini2022poisoning}. Our results also show that using such little data is indeed sufficient to meet \ref{effective}, \ref{utility}, and \ref{robust} (c.f. Section~\ref{sec:evaluation}).



\noindent\textbf{Validation Datasets.}
We consider the following validation datasets ($\mathcal{D}_{val}$): we denote dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalunacc$; and dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalacc$.
For \ref{effective}, we use $\dvalunacc$ by generating 10 unacceptable prompts using ChatGPT, and generate 5 images per prompt using SD v1.4. 
For \ref{utility}, we use $\dvalacc$ by randomly choosing 100 non-overlapping acceptable prompts from the COCO 2014 dataset~\cite{coco}, and 1 image per prompt, generated from SD v1.4.
We summarize them in Table~\ref{tab:valconfig}. 

\input{tables/tab_valconfig}

\noindent\textbf{Test Datasets.} %We now present datasets for evaluating different \crt{s}. 
We consider test datasets ($\mathcal{D}_{te}$): we denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dtestacc$; and with unacceptable prompts ($\promptuacc$) and corresponding images ($\imgunacc$) as $\dtestunacc$.

\input{tables/tab_teconfig}

For evaluating effectiveness (\ref{effective}) and robustness (\ref{robust}), we use $\dtestunacc$ which is generated as follows:
For Group-1, we use an independent benchmark dataset, Inappropriate Image Prompts (I2P), containing prompts  likely to generate unsafe images~\cite{schramowski2022safe}. It covers all four Group-1 concepts. 
For \emph{nudity}, I2P includes a ``nudity percentage'' attribute. We choose all unacceptable prompts with a nudity percentage $>10$, resulting in a total of 300 unacceptable prompts, in accordance with prior works~\cite{gandikota2023erasing, gandikota2023unified}.
\unsafediff~\cite{unsafeDiff} also used \emph{political} as a concept, which is excluded from our evaluation since it is not a part of I2P. Note that I2P prompts do not explicitly contain $\cunacc$, \emph{i.e., the words \emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing} are not explicitly included in the prompts}.
For Group-2 and Group-3 concepts, there are no standard benchmark datasets. Hence, we generate the dataset by following prior works~\cite{kumari2023ablating, gandikota2023erasing} to obtain 200 unacceptable images generated from SDv1.4 from 10 unacceptable prompts generated from ChatGPT. 
For \ref{utility}, we use $\dtestacc$ which includes the COCO 2014 test dataset with 200 randomly chosen acceptable prompts.
We summarize the datasets in Table~\ref{tab:teconfig}. 


\subsubsection*{\underline{Step 3: Fine-tune \tti model with \crt{s} or train filter}}

Using $\dtrain$, we fine-tune \tti models using different fine-tuning \crt{s} whose optimizations are described in Section~\ref{back-attacks}.
We use six fine-tuning \crt{s} (\ca, \forgetNot, \sa, \esd, \unifiedCE, and \sdd). 
For filtering \crt, we consider one baseline (\unsafediff) and do not compare with SD-Filter as \unsafediff outperforms it.
For \unsafediff, we train the filtering classifier on their dataset. 
We fine-tune \method on $\dtrain$ and use the CLIP L-patch-14~\cite{vit} due to its popularity, which is also the default text encoder with Stable Diffusion v1.4. However, other variants of CLIP are also applicable.


\subsubsection*{\underline{Step 4: Select best $\cacc$ using $\mathcal{D}_{val}$}}

\input{tables/tab_concepts}
 \input{tables/tab_effectiveness}
 \input{tables/tab_utility}

 
For concepts in Group-1, we evaluate the effectiveness (\ref{effective}) and utility (\ref{utility}) for different candidates of $\cacc$ on $\dvalunacc$ and $\dvalacc$ respectively. 
We found that the following concepts gave the best results: \emph{nudity} $\rightarrow$ \emph{clean}, \emph{violence} $\rightarrow$ \emph{peaceful}, \emph{disturbing} $\rightarrow$ \emph{pleasing}, and \emph{hateful} $\rightarrow$ \emph{loving}.
For \emph{nudity}, we eliminated \emph{clothed} as it blocked images with minimal exposed skin despite being acceptable~\cite{unsafeDiff,schramowski2022safe}.



We use concepts in Group-1 following prior work~\cite{unsafeDiff} to evaluate filtering \crt{s}. 
We use \emph{nudity} and \emph{violence} from Group-1, and all the concepts from Group-2 and Group-3 following prior works~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards} to evaluate fine-tuning \crt{s}. 
Hence, we compare \method with each \crt category separately using concepts they were evaluated on.
We summarize the final concepts for evaluation in Table~\ref{tab:concepts}.



\subsubsection*{\underline{Step 5: Evaluating \ref{effective}, \ref{utility}, and \ref{robust} on $\mathcal{D}_{te}$}}

We evaluate effectiveness (\ref{effective}) on $\dtestunacc$, utility (\ref{utility} on $\dtestacc$, and robustness (\ref{robust}) $\dtestadv$ which is generated by running different attacks $\dtestunacc$ to get $\advprompt$. In all cases, we only pass the prompts from the dataset to \tti models and compute different metrics described in Section~\ref{sec:metrics}.

==> old_versions/6evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}


\input{tables/tab_robustness}

We evaluate \method with fine-tuning \crt{s} (Section~\ref{sec:finetuneEval}), and then filtering \crt (Section~\ref{sec:filterEval}). 


\subsection{Comparison with Fine-tuning \crt{s}}\label{sec:finetuneEval}


\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report CLIP accuracy in Table~\ref{tab:effectiveness} for all eleven concepts on $\dtestunacc$. 
%
All \crt{s} show poor accuracy on \emph{nudity} and \emph{violence}. We attribute this to fine-tuning \crt{s} being sensitive to the input prompts~\cite{pham2024robust, yang2024guardt2i, ma2024jailbreaking}. Hence, they perform poorly for \emph{nudity} and \emph{violence} which do not explicitly include $\cunacc$.
In comparison to other \crt{s}, \method consistently maintains high accuracy on the I2P benchmark dataset as it classifies the generated images and does not depend on the prompts. 
Further, \method satisfies \ref{effective} using only 20 prompts and corresponding images for training. This is consistent with results on CLIP poisoning where changing the performance of CLIP only required a small number of poison samples~\cite{carlini2022poisoning, yang2023robust}.

\esd, \unifiedCE, and \sdd have better accuracy compared to the other three fine-tuning \crt{s}. 
This could be attributed to the similar optimizations used by \esd and \sdd for fine-tuning the \tti model: both fine-tune \dm, conditioned on $\cunacc$, to match original \dm without any prompt to reduce the influence of $\cunacc$ on the output.  
For \unifiedCE, higher effectiveness can be attributed to directly removing the influence of $\cunacc$ from the \tti model parameters. \textit{Overall, \method is more effective than other fine-tuning \crt{s}.}



\noindent\textbf{\underline{\ref{utility} Utility.}} We report normalized CLIP scores in Table~\ref{tab:utility} on $\dtestacc$.
%
All the fine-tuning \crt{s} perform well across all concepts (either \colorbox{myniceblue}{blue} or \colorbox{mynicegreen}{green}). This could be attributed to explicitly fine-tuning for utility. We observe that \ca with KL-Divergence-based optimization targeted for cross-attention layers, and \unifiedCE with a precise closed-form solution to model updates, preserve utility better than others. 

\method has high utility for all concepts except for \emph{violence}, and some Group-2 concepts (\emph{Nemo}, \emph{Captain Marvel}, \emph{Snoopy}, and \emph{R2D2}).
During fine-tuning, effectiveness improves but at the cost of utility, which is inherent to all fine-tuning \crt{s}.
For \textit{violence}, in our experiments, we observed an early decrease in utility during the very first epoch resulting in poor trade-off between effectiveness and utility. 
We attribute the poor utility on Group-2 concepts to the ambiguity in the unacceptable concepts. For instance, \emph{Nemo} is both a fish and a ship captain~\cite{VERNE_2024}, and \emph{Captain Marvel} represents both a male and a female superhero~\cite{Friedwald_2019_marvel}. 
To verify this, we precisely specify the unacceptable concepts to reduce ambiguity: as \emph{Nemo}$\rightarrow$ \emph{Nemo fish}, \emph{Captain Marvel}$\rightarrow$ \emph{Captain Marvel female superhero}, \emph{Snoopy}$\rightarrow$ \emph{Snoopy dog}, and \emph{R2D2}$\rightarrow$ \emph{R2D2 robot}. We evaluate \method on $\dvalacc$ and then report the numbers for the evaluation dataset below:
compared to the results in Table~\ref{tab:utility}, the normalized CLIP score for this new configuration is: 0.97 $\pm$ 0.00 (\emph{Nemo fish}), 0.90 $\pm$ 0.02 (\emph{Captain Marvel female superhero}), 0.98 $\pm$ 0.03 (\emph{Snoopy dog}), 0.92 $\pm$ 0.02 (\emph{R2D2 robot}), which are now indicated in \colorbox{mynicegreen}{green}.
We also report the CLIP accuracy on $\dvalunacc$ to evaluate effectiveness with this new configuration: 0.02 $\pm$ 0.00 (\emph{Nemo fish}), 0.00 $\pm$ 0.00 (\emph{Captain Marvel female superhero}), 0.02 $\pm$ 0.01 (\emph{Snoopy dog}), 0.00 $\pm$ 0.00 (\emph{R2D2 robot}), which are effective, same as before. Hence, precisely specifying $\cunacc$ is important for \method and can improve utility without sacrificing effectiveness. 
\textit{Overall, \method preserves utility on most concepts, and poor utility on some concepts can be improved by removing ambiguity in $\cunacc$.}


\noindent\textbf{\underline{\ref{robust} Robustness.}} We report CLIP accuracy in Table~\ref{tab:robust} on $\dtestadv$. We evaluate different \crt{s} against four attacks: Typo+, PEZ+, CCE/CCE+, and RingBell+. We evaluate fine-tuning \crt's against CCE, and evaluate \method against CCE+ as CCE already accounts for fine-tuning \crt{s}. We use the same color coding as in Table~\ref{tab:effectiveness}. 

CCE/CCE+, being a white-box attack which uses the parameters of the entire \tti model, is the strongest attack and it makes all fine-tuning \crt{s} ineffective. However, \method is more robust against CCE/CCE+ and outperforms all fine-tuning \crt{s}.
On the remaining attacks, all the fine-tuning \crt{s} have better robustness on Group-3 concepts than on Group-1 and 2. We attribute this to the difficulty of \tti models in generating precise faces while also evading detection, as shown in prior works~\cite{Matthias_2023}.
Similar to results in Table~\ref{tab:effectiveness}, we note that all \crt{s} perform poorly on \emph{nudity} and \emph{violence} across all the attacks. This is expected as the \crt{s} have poor effectiveness on these concepts as seen in Table~\ref{tab:effectiveness}. Hence, adversarial prompts for these concepts are likely to easily evade them. 
\emph{Overall, \method is more robust than all prior fine-tuning \crt{s} on all the concepts across all the attacks.} 
We discuss the possibility of future attacks against \method in Section~\ref{sec:future}.



\noindent\textbf{\underline{Summary.}} 
We depict the trade-offs among \ref{effective}, \ref{utility}, and \ref{robust} in Figure~\ref{fig:radarsFT}. We use (1-CLIP accuracy) for \ref{effective} on $\dtestunacc$, normalized CLIP score on $\dtestacc$ for \ref{utility}, and (1-CLIP accuracy) for \ref{robust} on $\dtestadv$ using CCE/CCE+. 
For each of the requirements, we use the average across all concepts as the representative value for a \crt.
\emph{Overall, \method provides a better trade-off across the three requirements compared to all the fine-tuning \crt{s}.}

\input{figures/fig_radar_ft}

































\subsection{Comparison with Filtering \crt}\label{sec:filterEval}

We now compare with \unsafediff~\cite{unsafeDiff}, the state-of-the-art filtering \crt, across the three requirements and summarize the results. We use FNR to evaluate effectiveness on $\dtestunacc$, FPR for utility on $\dtestacc$, and FNR for robustness on $\dtestadv$.




\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report FNR across four concepts (\emph{nudity}, \emph{violence}, \emph{disturbing}, and \emph{hateful}).
\method has better FNR for three of the four concepts: \emph{nudity}, \emph{violence} (in \colorbox{mynicegreen}{green}), and \emph{hateful} (\colorbox{myniceblue}{blue} for \method and \colorbox{mynicered}{red} for \unsafediff). However, both \method and \unsafediff perform poorly on \emph{disturbing}. 
We attribute this poor effectiveness on Group-1 concepts to the subjective description of $\cunacc$. Images for these concepts cover a wide variety of sub-concepts simultaneously which are not precisely identified for \crt{s}. 
\emph{Overall, \method is more effective than \unsafediff on most concepts.}

\input{tables/tab_filter_effective}



\noindent\textbf{\underline{\ref{utility} Utility.}} We present FPR in Table~\ref{tab:FilterUtility} across the four  Group-1 concepts. As expected, we observe that both \method and \unsafediff have comparable utility they demonstrate a low FPR. This is expected since \unsafediff explicitly includes images containing $\cacc$ while training the multi-headed classifier.

\input{tables/tab_filter_utility}

\noindent\textbf{\underline{\ref{robust} Robustness.}} We report FNR on the dataset for adversarial prompts and corresponding images in Table~\ref{tab:FilterRobust}. In addition to the four attacks from Table~\ref{tab:robust}, recall that SneakyPrompt~\cite{yang2023sneakyprompt} is specifically designed to attack filtering \crt{s}. Hence, we also include the evaluation against SneakyPrompt. 
Also, since CCE is not adaptive against filtering \crt's, we evaluate \unsafediff and \method against CCE+. We are the first to evaluate different attacks against \unsafediff.
\input{tables/tab_filter_robust}

We observe that \method is effective in thwarting $\advprompt${s} from PEZ+ while \unsafediff can be evaded.
On all the remaining attacks, we show that \method is robust on more concepts than \unsafediff.
As indicated before, all the Group-1 concepts are subjective and capture multiple sub-concepts. This ambiguity could be the reason for poor robustness on some of these concepts.
\emph{Overall, \method is more robust than \unsafediff on majority of the concepts across different attacks.}

\input{figures/fig_radar_filter}

\noindent\textbf{\underline{Summary.}} 
We present the trade-offs in the form of radar plots in Figure~\ref{fig:radarsFilt}. 
We use (1- FNR) on $\dtestunacc$ for \ref{effective}, (1- FPR) on $\dtestacc$ for \ref{utility}, and (1- FNR) on $\dtestadv$ using CCE+ for \ref{robust}. Hence, a higher value indicates better performance.
\method has comparable utility to \unsafediff but outperforms in effectiveness and robustness.
\emph{Overall, \method covers a larger area, and hence provides a better trade-off than \unsafediff.}






==> old_versions/7robustness.tex <==
\section{Certifying Robustness of \method}\label{sec:bound}

We empirically showed that \method is robust against several state-of-the-art attacks (Section~\ref{sec:evaluation}).
Inspired by the literature on certified robustness against adversarial examples~\cite{cohen2019certified}, it is natural to ask whether a similar notion of certified robustness is possible for \crt{s}.
None of the existing \crt{s} have considered certified robustness.
To this end, we are the first to explore its feasibility for \method.


We first present a theoretical bound on the worst-case modification by \adv under which we can guarantee \method's accuracy (Section~\ref{sec:theoretical}). We then empirically evaluate this bound on different concepts (Section~\ref{sec:empirical}) and finally discuss some implications of our results (Section~\ref{sec:implications}).


\subsection{Theoretical Bound}\label{sec:theoretical} 

Certified robustness aims to find provable guarantees that an ML model's predictions (generally a classifier) are robust, i.e., the predictions do not change on adding noise to the input~\cite{carlini2023certified}. 
Our goal is to have a similar provable robustness bound for a \tti model with \method. 
We want to find the maximum noise to an input which \method can tolerate.

We give advantage to \adv by assuming they can directly add adversarial noise to \method's embeddings. This is a strong assumption as in practice, \adv can only send prompts to the \tti model. We revisit this assumption later in Section~\ref{sec:implications}.
Formally, given an unacceptable image $\imgunacc$, \adv adds noise $\delta$ to its embeddings, $\phi_x(\imgunacc)$, such that $\filter(\phi_x(\imgunacc) + \delta)$ is misclassified as acceptable.
Using this assumption, we specify the maximum noise $\delta$ added to the embeddings, $\phi_x(\imgunacc)$, that \method can tolerate in Theorem~\ref{thm.1}.


\input{figures/fig_certified}


\begin{theorem}~\label{thm.1}
    Let $\hat{x} = \phi_x(x), \hat{c}^i = \phi_p(c^i), i\in\{a,u\}$. 
    % For $F(x)$ defined in equation~\ref{eq:att}, 
    Define 
    \[g_i(\hat{x}):=\frac{exp(s(\hat{x},\hat{c}^i))}{exp(s(\hat{x},\caccc))+exp(s(\hat{x},\cunaccc))},\] 
    where $s(\hat{x},\hat{c}^i) = \tau \text{cos}(\hat{x},\hat{c}^i))$, then $g_i$ is the confidence of $\hat{x}$ being classified as $\concept^i$. $F(x)$ in equation~\ref{eq:att} can be defined as $F(\hat{x})=argmax_i g_i(\hat{x})$, and $F(\hat{x})$ classifies $\hat{x}$ as unacceptable if $g_u(\hat{x})>\Gamma$, where $\Gamma$ is the decision threshold.
     For a given image embedding $\hat{x}$, if $g(\hat{x}):=g_u(\hat{x})>\Gamma$, then $g$ is robust against noise $\delta$ where 
     \[||\delta||\leq\left(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|}\right)||\hat{x}||,\]
     % on the image embedding, 
     and $\Gamma$ is the decision threshold i.e. 
    \begin{equation}\label{eq:bound}
            F(\hat{x}) = F(\hat{x}+\delta), \forall ||\delta||\leq \left(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|}\right)||\hat{x}||.
    \end{equation}
\end{theorem}

\noindent\textit{Proof Sketch.} We prove the above theorem by applying Lipschitz continuity over $g(\hat{x})$. \filter($\cdot$) is the composition of the softmax function and the scaled cosine similarity over the embeddings, where both functions are Lipschitz continuous when $||\hat{x}||>0$. In the detailed proof, we compute the Lipschitz constant for the softmax function and scaled cosine similarity function respectively, which is 0.25 and $\frac{\tau}{||\hat{x}||}$. Then the Lipschitz constant for $g(\hat{x})$ will be $\frac{\tau}{2||x||}$ according to the chain rule. Finally, using the triangle inequality on $|g(\hat{x})-g(\hat{x}+\delta)|$, and plugging the bound in to the inequality, we get $g(\hat{x}+\delta)\geq \Gamma$.
We present the full proof in Appendix~\ref{app:proof}.
We discuss extending the bound to prompt space in Section~\ref{sec:future}.




\subsection{Empirical Validation}\label{sec:empirical}

We now compute the maximum noise that \method can tolerate for each unacceptable image's embedding using Equation~\ref{eq:bound}. 
Following prior literature on certified robustness~\cite{cohen2019certified}, we compute the certified accuracy described in~\cite{cohen2019certified} to evaluate the robustness of \method.
Certified accuracy at radius $r$ is the fraction of unacceptable images which are correctly classified and are robust against adversarial noise $\delta > r$.
This shows the robustness of \method against attacks under some noise $r$. A robust model will have a larger certified radius and higher certified accuracy. 
Since we add noise directly to $\phi_x(\imgunacc)$, we compare our certified accuracy with the accuracy of clean unacceptable images (without adversarial noise) which we refer as ``clean accuracy''. 
Ideally, certified accuracy should be close to the accuracy of clean unacceptable images.

We present the results in Figure~\ref{fig:certified} for the three groups of concepts. 
Clean accuracy in Figure~\ref{fig:certified} is the certified accuracy at radius zero. 
\method is robust against $\delta<0.07$, incurring less than a $5\%$ drop in certified accuracy. 
When $\delta<0.15$, the certified accuracy remains higher than $50\%$ for all concepts. 
\method is particularly robust for some concepts in Group-2 (\emph{Grumpy Cat}, \emph{R2D2}, \emph{Captain Marvel}), and Group-3 (\emph{Taylor Swift}, \emph{Angelina Jolie}, and \emph{Elon Musk}). For these concepts, the certified accuracy remains the same for the clean unacceptable images until $\delta>0.15$.
Further, \method is more robust for concepts where the clean accuracy is $1.00$ (CLIP accuracy from Table~\ref{tab:effectiveness}). We find that the robustness is higher for concepts on which \method is more accurate. We attribute this to the increased separation between acceptable and unacceptable concepts.



\subsection{Practical Implications}\label{sec:implications} 

Having discussed the theoretical bound and empirically validated it on different concepts, we now revisit the practicality of this bound.
We discuss the usefulness of the certification and revisit our assumption about \adv's capability.


\noindent\textbf{Usefulness of Certified Bound.} 
In Figure~\ref{fig:certified}, we find that the certified bound is less than \(0.15\) across all the concepts. We found this to be smaller than the $l_2$-norms of realistic image embeddings, which had a mean of \(17\).
This suggests that our certified bound can only be robust against 
adversarial noise when it is only 0.8\% (=0.15/17) of the embeddings.

A certified bound is practical if there are adversarial image embeddings with less noise than the bound. Then, the bound is effective against these embeddings.
We use \method without fine-tuning with Equation~\ref{eq:ft1} to check the existence of such adversarial image embeddings. We can find embeddings that  \emph{potentially} evade \method (without fine-tuning) when the noise is as small as $0.028$.
Our certified bound is useful against such embeddings\footnote{Note that to find an actual attack against \method, \adv will have to (a) find a prompt that generates this perturbed embedding, and (b) ensure that the resulting image retains the unacceptable content.}.


However, the distance between acceptable and unacceptable images, which is at least \(7\), is much larger than the certified bound. This suggests that our certified bound is loose. We leave a tighter certified bound and the possibility of using adversarial training for improving robustness as future work (c.f. Section~\ref{sec:future}). 


\noindent\textbf{\adv's Capability.} To compute the certified bound, we assumed a strong \adv who can directly add adversarial noise to the \emph{embeddings}.
In practice, \adv can only modify the \emph{prompts} sent to the \tti model, and can only obtain the corresponding filtered outputs. Hence, in practice, \adv is much weaker and the robustness of \method is much higher than indicated in Figure~\ref{fig:certified}.

To illustrate this, we consider a concrete attack that \adv could adopt given its inability to directly add adversarial noise to embeddings:
\adv begins with unacceptable images and incorporate adversarial noise using standard evasion techniques (e.g., PGD~\cite{MadryPgd}) to find an adversarial example that evades the \method classifier. 
\adv then finds the corresponding adversarial prompt using one of the attacks (PEZ+) in Section~\ref{back-attacks}. 
We want to see if \target still generates an adversarial image which evades \method. 
We use PGD to generate unacceptable images with adversarial noise, and PEZ+ to find their corresponding adversarial prompts.
We find that \target fails to generate an adversarial image which evades \method using the adversarial prompt.
This is due to the adversarial-prompt-generation process being an approximation, which fails to fully capture all aspects of the adversarial image. 
Moreover, using the \tti model to generate the image from the adversarial prompt is unlikely to capture the adversarial noise due to the de-noising used in the diffusion model (Section~\ref{back-diffusion}). This claim is further supported by prior literature on the robustness of diffusion models~\cite{Kim_2022_CVPR,chen2024diffusion,zhang2023diffsmooth,xiao2022densepure}. 

 
We compare the original adversarial images with the images generated from their adversarial prompts. We present one concept from each group in Appendix~\ref{app:adv}: Table~\ref{fig:adversarial}. We find that the generated images are significantly different from the original adversarial images. This confirms our conjecture that the adversarial noise is not retained in the generated images.
A more thorough exploration of such an attack is left as future work. Based on the above preliminary exploration, we conjecture that \method is likely to be robust against such attacks by \adv with realistic capabilities.

==> old_versions/8related.tex <==
\section{Related Work}\label{sec:related}


\noindent\textbf{Prompt Filters.} We focus on image filters to detect $\imgunacc$. Prior works have explored using prompt filters to identify unacceptable concepts before passing them to \tti models~\cite{yang2024guardt2i}.
Such filters are being used for DALLE-2 \cite{ramesh2021dalle}, and MidJourney~\cite{midjourney}. However, these prompt filters are not robust and easy to evade~\cite{ba2023surrogateprompt,ma2024jailbreaking}. Hence, prior works have identified image filters are a better alternative, with the possibility of making it effective and robust~\cite{li2024safegen}.

% \change{https://arxiv.org/abs/2404.03631 
% https://arxiv.org/pdf/2405.16341v1
% Water down the claim that none of the prior fine-tuning CRTs are robust in intro and abstract...}

\noindent\textbf{Additional \crt{s}.} We use state-of-the-art \crt{s} for evaluation. Hence, we omit the discussion about prior \crt{s} which have been outperformed by those considered in this work~\cite{schramowski2022safe, automatic1111_negative_prompt,radford2021learning}. We discuss recent fine-tuning \crt{s}.

Hong et al.~\cite{hong2023one} propose an approach to make minimal changes for concept removal. Instead of matching the entire distribution of features for $\cunacc$ to the distribution of $\cacc$, they selectively modify the features with highest density in $\cunacc$. 
Wu et al.~\cite{wu2024erasediff} propose concept removal as an unlearning problem which is solved as constraint optimization while preserving utility. 
Basu et al.~\cite{basu2023ldiffquickfix} present a closed-form solution to remove concepts from \te by identifying causal features for one concept and overriding it with another concept. 
Since these approaches are similar to other fine-tuning \crt{s} considered in this work, and do not optimize for robustness, making them susceptible to evasion.

Huang et al.~\cite{huang2024receler} modify the cross entropy layers of \dm to erase $\cunacc$ with adversarial training for better robustness against only two na\"{i}ve attacks: Prompting4Debugging~\cite{chin2023prompting4debugging} and RingBell~\cite{Tsai2023RingABellHR}. 
Li et al.~\cite{li2024safegen} modify the self-attention layers of \dm using triplets of $\imgunacc$, censored $\imgunacc$, and $\imgacc$. They evaluate robustness against SneakyPrompt. However, the robustness for both these works against recent attacks which account for their \crt{s} is not clear.

Pham et al.~\cite{pham2024robust} fine-tune \tti model to generate a specific concept and subtract the task vector for this concept from the model parameters of the original model, thereby erasing $\cunacc$.
They demonstrate robustness against CCE and RingBell but suffer from a trade-off between \ref{utility} and \ref{robust}.
Wu et al.~\cite{wu2023backdooring} insert backdoors to textual inversion embeddings such that a $\cunacc$ results in a pre-defined image instead of $\imgunacc$.
Despite accounting for robustness, these \crt{s} incur trade-offs between \ref{effective}, \ref{utility}, and \ref{robust}.

\noindent\textbf{Additional Attacks against \crt{s}.} Prompting4Debugging uses PEZ while matching the noise between a \tti model with a \crt, and one without a \crt, during the reverse diffusion process. In our setting, \tti model with and without \method are identical, hence Prompting4Debugging reduces to PEZ.
Rando et al.~\cite{rando2022redteaming} propose PromptDilution against filters. However, as SneakyPrompt outperformed PromptDilution~\cite{yang2023sneakyprompt}, we do not consider it for evaluation.

Ba et al.~\cite{ba2023surrogateprompt} generate  substitutes for $\cunacc$ in their input prompts to evade a black-box filter. They show effectiveness against the Q16 filter which is outperformed by \unsafediff. 
Ma et al.~\cite{ma2024jailbreaking} optimize for $\advprompt$ to match $\cunacc$ using TextGrad, a gradient based search over text, to identify the tokens. Their attack outperforms Prompting4Debugging, Prompt Dilution, and RingBell. 
Shahgir~\cite{shahgir2024asymmetric} replace an object in $\imgclean$ with a target object to create $\imgadv$, which can be inverted to get $\advprompt$.
Kou et al.~\cite{ijcai2023p109} use a character-level gradient attack that replaces specific characters to design $\advprompt$.




==> old_versions/9discussion.tex <==
\section{Discussion and Future Work}\label{sec:discussions}

We revisit our discussion on robustness  (Section~\ref{sec:future}), applicability/extensions of \method (Section~\ref{sec:extensions}), and a summary of this work (Section~\ref{sec:summary}).




\subsection{Revisiting Robustness}\label{sec:future}

\noindent\textbf{Addressing Future Attacks.} Recall that our certified robustness bound is loose (Section~\ref{sec:bound}). We leave the improvement of the bound as future work.

\method maintains high robustness across all evaluated concepts. 
The design of new attacks which can preserve unacceptable concepts while evading \method is an open problem. Here, adversarial training for \method can be used to increase its robustness.
We can fine-tune CLIP with this objective: $\mathcal{L}_{\text{Con-adv}}(\dtestadv)=$
\[- \frac{1}{N} \sum_{j = 1}^N \log \frac{\exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(\cunacc))/ \tau)}{\sum_{k \in \{a,u\}} \exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(c_k))/ \tau)}\]
where $\mathcal{D}_{adv} = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$. Assuming $\imgadv$ evades the filter, we optimize $\phi_p$ and $\phi_x$, such that $\phi_p(\imgadv_j)$ is closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$. This loss would be added to Equation~\ref{eq:ft1} and~\ref{eq:ft2}. 
Empirical evaluation of adversarially-trained \method is left as future work.


\noindent\textbf{Extending the Theoretical Bound to Prompts.} 
% Although \adv cannot modify text embeddings in practice, analyzing robustness in the CLIP embedding space is valuable as recent works have shown that small changes in the text embeddings of prompts, allow for fine-grained control over their generated images~\cite{yu2024uncovering, kawar2023imagic}. 
To extend our theoretical bounds in Theorem~\ref{thm.1} to the prompt space,
we assume Lipschitz continuity, commonly used in ML~\cite{bousquet2002stability}, certified robustness~\cite{li2023sok}, and more recently in the context of \tti models~\cite{chen2024your}.
We consider the mapping from prompt space to embedding space is locally \( L \)-Lipschitz, i.e., the function \( \phi_x(f(\text{\prompt})) \) satisfies the following condition:

For each prompt \(\text{\prompt}\), there exists a \(\delta_{\text{\prompt}} > 0\) such that
$
||\phi_x(f(\text{\prompt})) - \phi_x(f(\text{\prompt} + \delta_{\text{\prompt}}))|| \leq L ||\delta_{\text{\prompt}}||.
$

Then, the inequality in Equation~\ref{eq:bound} can be related to the prompt space by a scalar factor \(\frac{1}{L}\). 
Therefore, when \(\|\delta_{\text{\prompt}}\| \leq \frac{1}{L} \|\delta\|\), where \(\|\delta\|\) satisfies inequality in Equation~\ref{eq:bound}, the difference in embedding space will be bounded by \(\|\delta\|\), and CLIP remains robust.


\subsection{Applications and Extensions to \method}\label{sec:extensions}


\noindent\textbf{Filtering Multiple Concepts.} Gandikota et. al.~\cite{gandikota2023unified} have considered removing multiple concepts simultaneously.
While we focus on filtering one concept at a time for comparison with other \crt{s}, \method can be extended by including multiple concepts simultaneously as well. Specifically, for $\filter(x, \cunacc, \cacc)$ in Equation~\ref{eq:att}, instead of only specifying $\cunacc$ and $\cacc$ for a single concept, we can include $\cunacc$ and $\cacc$ for multiple concepts as a list. This is a simple configuration change with minimal fine-tuning or retraining in contrast to other filters (e.g.,~\cite{unsafeDiff}) which require training with extensive datasets. Since none of the prior \crt{s} evaluate multiple $\cunacc$, we leave its evaluation as future work. 

\noindent\textbf{Filtering Artistic Styles.} 
None of the prior filtering \crt{s} consider any copyrighted content and focus on only \emph{inapproriate Group-1 concepts}. 
\method is the first filtering \crt which is applicable to concepts which are copyright-infringing (Group-2) or involve unauthorized use of personalized images (Group-3).
Prior fine-tuning \crt{s} have considered removing artistic styles (e.g., painting in the style of Monet or Van Gogh) as copyrighted content~\cite{kumari2023ablating,gandikota2023erasing}.
However, we observed that \method does not differentiate between images with and without artistic styles very well. Specifically, \emph{Monet painting} as $\cunacc$ and \emph{painting} as $\cacc$, are very similar for \method, thus reducing its effectiveness. We leave the optimization of \method to account for artistic styles as future work.

\noindent\textbf{Applicability to other \tti Models.} Fine-tuning \crt{s} are specific to particular stable diffusion models due to their tailored optimizations for \tti models. In contrast, filtering \crt{s} offer versatility, as they can be applicable to any \tti model. 
Filters analyze only the generated image and the list of concepts, independently of the \tti model. 
However, fine-tuning the filter using data from \tti model, as we do it for \method, can improve effectiveness and utility. 
This allows to use the filter we will have a filter that will work with \tti model in different domains (e.g., anime images).
Explicit evaluation of \method for different \tti models is deferred to future work.


\subsection{Summary}\label{sec:summary}

Removing unacceptable concepts from \tti models is an important problem. However, none of the prior \crt{s} satisfy all three requirements simultaneously: effectiveness in preventing generation of images with unacceptable concepts, preserve utility on other concepts, and robustness against evasion. We propose \method, the \emph{first} robust \underline{co}ncept \underline{fi}ltering \crt which provides a better trade-off among the three requirements compared to prior \crt{s}.

==> old_versions/WACV/01abstract.tex <==
Diffusion based text-to-image models are trained on large datasets scraped from the Internet, potentially containing \textit{unacceptable concepts} (e.g., copyright infringing or unsafe). 
We need concept removal techniques (\crt{s}) which are
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \textit{effective} in preventing the generation of images with unacceptable concepts
\item \textit{utility-preserving} on acceptable concepts, and 
\item \textit{robust} against evasion with adversarial prompts.
\end{enumerate*}
None of the prior \crt{s} satisfy all these requirements simultaneously. 
We introduce \method, the first \emph{\textbf{robust \underline{co}ncept \underline{fi}lter} }based on Contrastive Language-Image Pre-Training (CLIP). 
We configure CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts.
This lets us fine-tune for robustness by separating the text embeddings of unacceptable and acceptable concepts while preserving their pairing with image embeddings for utility.
We present a pipeline to evaluate various \crt{s}, attacks against them, and show that \method, is \textbf{more effective and robust} than prior \crt{s}, while retaining \emph{utility}.
% Code will be publicly available upon publication.
%(CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) 

%(CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) 

%(normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]). 
% Finally, we present theoretical bounds for certified robustness of \method against adversarial prompts, and an empirical analysis.


==> old_versions/WACV/1introduction.tex <==
\section{Introduction}\label{sec:introduction}


Diffusion-based text-to-image (\tti) models have demonstrated a remarkable ability to generate high quality images from textual prompts~\cite{stable-diffusion,Rombach_2022_CVPR,ramesh2021dalle}.
They are trained on large datasets of unfiltered content from the Internet~\cite{radford2021learning,schuhmann2022laion}. 
Due to their large capacity, \tti models memorize specific \emph{concepts}, as seen in the generated images~\cite{Korn_2023,somepalli2022diffusion,carlini2023extracting}. 
Some of these concepts, may be \emph{unacceptable} for various reasons, such as copyright infringement (e.g., a movie character or celebrity), or inappropriateness (e.g., ``nudity'' or ``violence'')~\cite{gandikota2023erasing,schramowski2022safe,heng2023selective}. 
% Retraining \tti models after filtering out unacceptable concepts is inefficient, only partially effective~\cite{li2024safegen, huggingfaceStabilityaistablediffusion21Hugging}, and compromises utility~\cite{gandikota2023erasing}.
We need \emph{concept removal techniques} (\crt{s}) to minimize unacceptable concepts in  generated images.


Ideally, \crt{s} should be \emph{effective} in reducing the generation of unacceptable concepts while preserving the \emph{utility} on all others, and \emph{robust} to evasion with adversarial prompts.  
As we show in Section~\ref{sec:evaluation}, no existing \crt \emph{simultaneously} satisfies these requirements:
\begin{enumerate*}[label=\roman*),itemjoin={,\xspace}]
\item \emph{fine-tuning \crt{s}} which modify \tti models, trade-off effectiveness for utility~\cite{gandikota2023erasing,kumari2023ablating,heng2023selective,schramowski2022safe}, and  lack robustness~\cite{Tsai2023RingABellHR, wen2023hard, pham2023circumventing, yang2023sneakyprompt}
\item \emph{filtering \crt{s}}, which detect unacceptable concepts, lack robustness~(\cite{rando2022redteaming} and Section~\ref{sec:filterEval}).
\end{enumerate*}
%Moreover, none of these \crt{s} are robust against adversarial prompts, i.e., adversarially modified prompts which force \tti{s} to generate unacceptable concepts.
Our goal is to design a \crt that can simultaneously meet all the requirements.

We opt to use a filter as it will not alter the \tti model, thus minimizing impact on utility. We construct our filter using a Contrastive Language-Image Pre-Training (CLIP) model~\cite{radford2021learning}, an essential component of \tti models. 
% CLIP co-locates the embeddings of textual prompts and their corresponding images within a unified embedding space where similar concepts are closer.
CLIP is pre-trained on a vast dataset which encodes a broad spectrum of concepts~\cite{radford2021learning}, making it a versatile choice for a filter, unlike specialized classifiers (e.g.,~\cite{unsafeDiff}).
However, a naive CLIP-based filter is susceptible to evasion~\cite{rando2022redteaming}. 
%by solely measuring the distance between the embeddings of a generated image, and an unacceptable concept,
\begin{arxiv}
Subsequently, prior works have identified the design of a robust filtering-based \crt as an open problem~\cite{rando2022redteaming,li2024safegen}.
\end{arxiv}

% \input{figures/fig_robustness_diagram}
% \change{Robustness diagram: figures/fig\_robustness\_diagram}

We present a \textbf{robust \underline{co}ntent \underline{fi}lter}, \method, by configuring CLIP to identify unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts. 
% We present a \textbf{robust} \textbf{co}ntent \textbf{fi}lter, \method, that identifies unacceptable concepts in generated images using the distance of their embeddings to the text embeddings of \emph{both acceptable and unacceptable concepts}. 
% \change{This simple change in configuration translates to projecting} the image embedding onto the vector connecting the text embeddings of acceptable and unacceptable concepts. 
% This simple change makes it harder to generate effective adversarial prompts: the adversary is restricted to adding noise in the direction of the acceptable concept. 
%adversarial prompts must generate images far enough from unacceptable concepts to evade detection yet close enough to retain the unacceptable concepts.
This allows fine-tuning for better robustness by increasing the separation between the text embeddings of unacceptable and acceptable concepts, while preserving utility by maintaining their pairing with their corresponding image embeddings. 
% We liken this to adversarial training in classifiers, thus, improving the robustness of \method.
% This fine-tuning approach is further supported by fine-tuning \crt{s} which show that such an optimization leads to better utility~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}.
Our contributions are presenting 
\begin{enumerate*}[label=\roman*)]
\item \method, the \textbf{first robust \underline{co}ntent \underline{fi}lter} (Section~\ref{sec:approach}), 
\item \emph{a pipeline} to evaluate state-of-the-art \crt{s} and attacks (Section~\ref{sec:setup}),
\item and a comprehensive evaluation of \method against six fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective} and \textbf{robust} while \textbf{retaining utility} (Section~\ref{sec:evaluation}).
\end{enumerate*}\begin{arxiv} In Appendix~\cite{sec:bound} \end{arxiv}\begin{submission} In the supplementary material, \end{submission}
we present the \emph{first} approach for \emph{certifiable robustness of \crt{s}} by exploring 
theoretical robustness bounds of \method with a hypothetically strong adversary. 
We empirically analyze these bounds to show that \method is likely to be more robust in practice.
% \begin{enumerate}[leftmargin=*,wide,  labelindent=0pt]
% \item \method\footnote{We will open-source the code upon publication.}, the \textbf{first robust} (CLIP-based) \underline{co}ntent \underline{fi}lter (Section~\ref{sec:approach}) 
%which identifies unacceptable concepts in generated images by measuring the distance of their embeddings to the text embeddings of \emph{both} unacceptable and acceptable concepts ,
% \item a comprehensive comparative evaluation of \method with six state-of-the-art fine-tuning \crt{s}, and one filtering \crt, showing that it is \textbf{more effective} and \textbf{more robust} while \textbf{retaining utility}. (Section~\ref{sec:setup})
% (CLIP accuracy on unacceptable concepts in [0.00, 0.20] and FNR in [0.14, 0.53]) and \textbf{more robust} (CLIP accuracy on adversarial prompts for unacceptable concepts in [0.00, 0.40] and FNR in [0.00, 0.40]) than prior \crt{s}, while \textbf{retaining utility} (normalized CLIP score on acceptable concepts in [0.59, 0.98] and FPR in [0.01, 0.08]).
%showing that \method is \textbf{effective} ($\sim$5\% CLIP accuracy  on unacceptable concepts), \textbf{utility-preserving} ($\sim$93\% 
% normalized CLIP score on acceptable concepts), and \textbf{robust} ($\sim$4\% CLIP accuracy of  on adversarial prompts) %of unacceptable concepts) 
% (Section~\ref{sec:evaluation}), and
% \item %the \textbf{first} approach towards \textbf{certifiable robustness of \crt{s}} by exploring 
% theoretical bounds for \textbf{certifying the robustness} of \method, assuming a hypothetically strong adversary, empirical analysis of these bounds, and making the case that \method is likely to be more robust in practice. (Section~\ref{sec:bound}). 
% \end{enumerate}

==> old_versions/WACV/2background.tex <==
\section{Background and Related Work}\label{sec:background}

% We describe \tti models (Section~\ref{back-diffusion}), different \crt{s} (Section~\ref{back-conceptrem}), and attacks against them (Section~\ref{back-attacks}).

\subsection{Diffusion based \tti Models}\label{back-diffusion}

A diffusion based \tti model is a function $\target: \prompt \rightarrow \imgclean$ which generates an image $\imgclean$ for a given a textual prompt $\prompt$. It comprises two key components: a text and image encoder ($\phi$) which is used to incorporate the textual prompt in the image generation process, and a diffusion model (\dm) which is responsible for the generation of the image.

A popular encoder is CLIP, trained on a large dataset of image-text pairs, to map the embeddings of images and their corresponding text closer together in a joint text-image embedding space~\cite{radford2021learning}.
We denote the image embeddings as $\phi_x()$ and text embeddings as $\phi_p()$.
%Given $N$ images $\{\imgclean_j\}_{j=1}^N$ and their corresponding text prompts $\{\prompt_j\}_{j=1}^{N}$, the training data is $\mathcal{D} = \{(\imgclean_j, \prompt_j)\}_{j=1}^N$. 
CLIP is trained to maximize the cosine similarity (\text{cos}($\phi_p(\prompt_j), \phi_x(\imgclean_j))$) between the embedding of a prompt $\prompt_j$ ($\phi_p(\prompt_j)$) and the embedding of its corresponding image $\imgclean_j$ ($\phi_x(\imgclean_j)$) while minimizing the similarity between $\phi_p(\prompt_j)$ and any other $\phi_x(\imgclean_k)$ for $k \ne j$.
% We denote the cosine similarity as , where $\phi_x(\imgclean_j)$ is the CLIP image embedding of the image $\imgclean_j$, and $\phi_p(\prompt_j)$ is the CLIP text embedding of the prompt $\prompt_j$.
To achieve this, CLIP is trained using a contrastive loss function ($\mathcal{L}_{\text{Con}}$)~\cite{yang2023robust,oord2019representation,lee2021soundguided,radford2021learning}.
 % \[\mathcal{L}_{\text{Con}}(\mathcal{D}) = - \frac{1}{N} \sum_{j=1}^{N} \log \frac{\exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_j))/ \tau)}{\sum_{k=1}^{N} \exp(\text{cos}(\phi_x(x_j), \phi_p(\prompt_k))/ \tau)}\] where $\tau$ is the temperature parameter for scaling the predictions~\cite{radford2021learning, ModalityGap}. 
 


Given access to a pre-trained encoder, the actual images in \tti models are generated by a diffusion model, \dm, parameterized by $\theta$.
%During training of \dm, Gaussian noise is added to an initial image $x_0$ for $T$ time steps to produce $x_T$, in a process known as the \emph{forward diffusion process}. The noise is then iteratively removed to approximate the initial image $\tilde{x_0}$ in the \emph{reverse diffusion process}.
During inference, \dm generates an image from noise and can be conditioned with the embedding of a textual prompt $\phi_p(\prompt)$ to guide the generation of the image to match the description in \prompt. %After generating $\phi_p(\prompt)$, %from \te, 
%\dm is trained by minimizing the following loss function: $\mathcal{L} = \mathbb{E}_{\epsilon, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(\imgclean_t,\phi_p(\prompt),t)||_2^2]$ for each time step $t$, and random Gaussian noise $\epsilon \sim \mathcal{N}(0,1)$.

%Several prominent \tti models (e.g., Stable Diffusion v1.4 (SDv1.4)) improve the efficiency of the diffusion process by conducting it in the embedding space of a variational autoencoder (VAE), rather than on images \cite{stable-diffusion}. For a VAE decoder $\mathit{D}$, VAE encoder $\mathcal{E}$, and $z_t \in \mathcal{E}(\imgclean)$ as the latent representation of $\imgclean$ in the VAE's latent space, \dm is trained by minimizing the following objective: \\
%$\mathcal{L} = \mathbb{E}_{\epsilon, z_t, \phi_p(\prompt), t}[||\epsilon - \epsilon_\theta(z_t,\phi_p(\prompt),t)||_2^2]$ where $\epsilon \sim \mathcal{N}(0,1)$. The final image is generated from the approximation, $\tilde{z_0}$, by passing it through $\mathit{D}$: $\tilde{x_0} = \mathit{D}(\tilde{z_0})$.  
% Table~\ref{tab:notations} in Appendix~\ref{app:notations} summarizes frequently used notations.

 




\subsection{Concept Removal Techniques}\label{back-conceptrem}

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance?--- We use the same approach for selecting acceptable concepts as Kumari et. al.~\cite{kumari2023ablating}for group 2 and group 3 concepts. For these groups, the acceptable concept is a superset of the unacceptable concept. For example, the sex of a celebrity is the acceptable concept for a celebrity. For group 1, there is no clear definition of a superset (eg. the superset of \emph{nude} is unclear). Logically, the acceptable concept is the opposite of the unacceptable concept in this case since it is clearly defined. - SHOULD MOVE THIS EXPLANATION ELSEWHERE}

The textual phrase for an acceptable concept is $\cacc$, and for an unacceptable concept is $\cunacc$. 
For a given $\cunacc$, we define $\cacc$ as either the opposite, e.g., $\cunacc$ = \emph{violence} vs. $\cacc$ = \emph{peaceful}, or a generalization of a specific instance, e.g., $\cunacc$ = \emph{R2D2} vs. $\cacc$ = \emph{robot} (discussed later in Section~\ref{sec:pipeline}).
% We discuss the selection of $\cacc$ for a given $\cunacc$ in .
A \tti model may generate an image containing an unacceptable concept (referred to as $\imgunacc$) or an acceptable one (referred to as $\imgacc$). Similarly, a text prompt $\prompt$ may contain a phrase for an acceptable concept ($\promptacc$) or an unacceptable concept ($\promptuacc$). An example of $\promptuacc$ containing an unacceptable concept $\cunacc$ = \emph{Captain Marvel}, is ``\emph{Captain Marvel} soaring through the sky''. \crt{s} seek to thwart the generation of $\imgunacc$ by either fine-tuning the \tti model to suppress $\imgunacc$, or using a classifier as a filter to detect and replace $\imgunacc$. 
%
We discuss six state-of-the-art fine-tuning \crt{s}:
\noindent\textsc{Concept Ablation} (\ca)~\cite{kumari2023ablating} minimizes the KL divergence between the model's output for $\promptuacc$ and $\promptacc$ to force the generation of \imgacc instead of \imgunacc; 
% Formally, they optimize the following objective function: 
 % \text{argmin}_\theta 
% \[\begin{split}
% \footnotesize
%    \mathcal{L}_{\ca} =  \mathbb{E}_{\epsilon, z_t, \cunacc, \cacc, t}[w_t||\epsilon_\theta(z_t,\phi_p(\promptacc),t).sg() \\
%     - \epsilon_\theta(z_t,\phi_p(\promptuacc),t)||_2^2]
% \end{split}\]
% where $\epsilon \sim \mathcal{N}(0,1)$, $z_t \in \mathcal{E}$, and $w_t$ is a time-dependent weight, and $.sg()$ is the stop-gradient operation.
\textsc{Forget-Me-Not} (\forgetNot)~\cite{zhang2023forgetmenot} minimizes the activation maps for $\cunacc$ by modifying \dm's cross-attention layers; %Further, fine-tuning \dm, instead of just the cross-attention layers, results in degraded utility. 
% That is, given $a_i \in \mathcal{A}_i$, the $i$-th attention map in \dm of \tti, their loss is 
% \[\mathcal{L} = \sum_{a_i \in \mathcal{A}_i}||a_i||\]
\textsc{Selective Amnesia} (\sa)~\cite{heng2023selective} adapts continuous learning techniques (elastic weight consolidation and generative replay) for \tti models to forget a concept; %They optimize $\mathbb{P}(\imgclean|\theta^*,\cunacc)$, the probability of generating $\imgclean$ given $\theta^*$ and $\cunacc$, where $\theta^*$ are the frozen parameters of the original \tti model.
% \[
% \begin{split}
% \footnotesize
%     \mathcal{L}_{\sa} = -\mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_f(\cunacc)}[\text{log}\mathbb{P}(\imgclean|\theta^*,\cunacc)] -\lambda\sum_i\frac{M_i}{2}(\theta_i^*-\theta_i)^2\\
%      + \mathbb{E}_{\mathbb{P}(\imgclean|\prompt)\mathbb{P}_r(\cacc)}[\text{log}\mathbb{P}(\imgclean|\theta,\cacc)]
% \end{split}
% \]
% where $M$ is the Fisher information matrix over $\cacc$ and $\cunacc$, $\mathbb{P}_r$ and $\mathbb{P}_f$ are probabilities taken over the distributions of $\cacc$ and $\cunacc$ respectively, and $\lambda$ is a regularization parameter. 
\textsc{Erased Stable Diffusion} (\esd)~\cite{gandikota2023erasing} modifies the diffusion process to reduce the probability of generating \imgunacc;
% \[\begin{split}
% \epsilon_\theta(\imgclean_t,\phi_p(\cunacc),t) = \epsilon_{\theta^*}(\imgclean_t, t)
% + \eta(\epsilon_{\theta^*}(\imgclean_t,\phi_p(\cunacc),t)\\-\epsilon_{\theta^*}(\imgclean_t,t))
% \end{split}\]
% where $\eta > 0$ encourages the noise conditioned on $\cunacc$ to match the unconditioned noise.
\textsc{Unified Concept Editing} (\unifiedCE)~\cite{gandikota2023unified} fine-tunes the cross-attention layers to minimize the influence of $\cunacc$; 
% Their optimization is:
% % \text{min}_W
% \[\begin{split}
%     \mathcal{L}_{\unifiedCE} = \sum_{\cunacc \in \mathcal{C}^{u}, \cacc \in \mathcal{C}^{a}}||W\times\cunacc-W^*\times\cacc||_2^2 \\ 
%     +  \sum_{c \in S}||W\times c - W^*\times c||_2^2
% \end{split}\]
% where $W$, $W^*$ are the parameters of the fine-tuned and original \emph{cross-attention layers in \dm}, $\mathcal{C}^{u}$ and $\mathcal{C}^{a}$ are the space of pre-defined unacceptable and acceptable concepts, and $S$ is a set of concepts for which to preserve utility. 
\textsc{Safe diffusion} (\sdd)~\cite{kim2023towards}
encourages the diffusion model output conditioned on $\cunacc$ to match the unconditioned output.
% using the following objective function:
% \[\begin{split}
%     % \text{argmin}_\theta
%     \mathcal{L}_{\sdd} = \mathbb{E}_{\epsilon, z_t, \cunacc, t}[||\epsilon_\theta(z_t,\phi_p(\cunacc),t) 
%  - \epsilon_\theta(z_t,t).sg()
%     ||_2^2]
% \end{split}\]
% where $\epsilon \sim \mathcal{N}(0,1)$ and $z_t \in \mathcal{E}(x)$.
All current fine-tuning \crt{s} trade-off effectiveness for utility~\cite{gandikota2023erasing,kumari2023ablating,heng2023selective,schramowski2022safe} and are not robust (see Section~\ref{back-attacks}).


\noindent We also discuss two state-of-the-art filtering \crt{s}.
\textsc{Stable Diffusion Filter} (\texttt{SD-Filter})~\cite{radford2021learning} is black-box and the design of the filter is not publicly available, but Rando et. al.~\cite{rando2022redteaming} hypothesize that it involves computing the cosine similarity between the embeddings of a generated image, $\imgclean$, and a pre-defined set of $\cunacc$. If the cosine similarity is greater than some threshold, then $\imgclean$ has $\cunacc$. 
% Formally, their filter $\filter_{SD}$ can be described as
% \[ \filter_{SD}(\imgclean) = \begin{cases} 
%       1 & \text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) > \Gamma \\
%       0 & \text{otherwise}
%    \end{cases}
% \]
% where $\text{cos}(\phi_x(\imgclean), \phi_p(\cunacc)) = \overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\cunacc)}$, and $\overline{\cdot}$ denotes normalization. Here $\filter_{SD}(\imgclean) = 0$ indicates \imgacc and $\filter_{SD}(\imgclean) = 1$ indicates \imgunacc. Note that $\Gamma$ varies with $\cunacc$. 
\textsc{Unsafe Diffusion} (\unsafediff)~\cite{unsafeDiff} is the current state-of-the-art filtering \crt and outperforms the SD-Filter~\cite{unsafeDiff}. \unsafediff trains a multi-headed neural network classifier on top of CLIP to identify $\imgunacc$ where each head classifies different $\cunacc$: \emph{nudity, violence, disturbing, hateful}, and \emph{political}. %Their objective is given as $\filter_{\unsafediff}(\imgclean) = \text{MLP}(\phi_x(\imgclean))$ where MLP is a multi-layer perceptron, and $\filter_{\unsafediff} \in \{0,1\}$.
In Section~\ref{sec:filterEval}, we show that \unsafediff is not robust.

\subsection{Evading Concept Removal Techniques}\label{back-attacks} 

An adversary \adv may construct adversarial prompts ($\advprompt$) to evade \crt{s} and force the \tti model to generate $\imgunacc$. %while being semantically closer to acceptable prompts so that $\imgadv$ is incorrectly identified as acceptable while triggering the generation of unacceptable images. We denote a dataset containing adversarial prompts and their corresponding images ($\imgadv$) as $\dtestadv = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$ where ideally $\imgadv$ will contain $\cunacc$.
\adv is assumed to know and account for the target \tti model \target and its \crt. A dumb \adv who does not account for this is \emph{na\"{i}ve}. 
%
% \adv's objective is to construct $\advprompt$ which can force a \tti model to output images with $\cunacc$ 
Existing attacks formulate the construction of $\advprompt$ as an optimization problem using some reference $\imgunacc$ (or the difference between $\promptacc$ and $\promptuacc$) as the ground truth. 
% Different attacks vary in ways to solve this optimization. We present four state-of-the-art attacks:
%
\noindent\pez~\cite{wen2023hard} constructs $\advprompt$ by identifying text tokens which 
minimize the cosine similarity between $\phi_p(\advprompt)$ and $\phi_x(\imgunacc)$.
% : $\mathcal{L}_{\pez}= 1-\text{cos}(\phi_p(\advprompt),\phi_x(\imgunacc))$. 
%
\ringbell~\cite{Tsai2023RingABellHR} identifies tokens for $\advprompt$ by first calculating the average difference between the embedding vectors of $\promptuacc$ and $\promptacc$ and then minimizes the distance of $\advprompt$'s text embedding to $\promptuacc$'s embedding using a genetic algorithm.
%: $\phi_p(\hat{\prompt}) = \frac{1}{N}\sum_{i=1}^N\{\phi_p(\promptuacc_i) - \phi_p(\promptacc_i)\}$ from a set of $N$ prompts.
% Then, RingBell computes $\advprompt$ by minimizing the distance of its text embedding to an acceptable prompt embedding using a genetic algorithm.
% , formulated as: $\text{min}_{\advprompt} ||\phi_p(\advprompt) - (\phi_p(\prompt^{init})+\eta\cdot\phi_p(\hat{\prompt}))||^2$ where $\prompt^{init}$ is an initial unacceptable prompt which is censored by a \crt. They solve this using a genetic algorithm. 
%Further, the optimization relies on a fitness function using mean-squared error: $\mathcal{L}_{RingBell} = \mathcal{L}_{MSE}(\phi_p(\cunacc),\phi_p(\advprompt))$ where $\cunacc$ is a prompt that generates $\imgunacc$ in a \tti model.
%
\sneaky~\cite{yang2023sneakyprompt} uses reinforcement learning to construct $\advprompt$ (starting from some initial $\promptuacc$) specifically against filtering \crt{s} using cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\advprompt)$ as the reward function. 
% Given an initial prompt $\prompt^{init}$, the attack searches for tokens to update $\prompt^{init}$ to form $\advprompt$ using cosine similarity between $\phi_x(\imgadv)$ and $\phi_p(\advprompt)$ as the reward function. 
% Typically, they use $\promptuacc$ as $\prompt^{init}$ for better effectiveness and faster convergence.
%
\cce~\cite{pham2023circumventing} uses textual-inversion~\cite{gal2022textualinversionimage} to construct $\advprompt$ by updating CLIP's vocabulary to include a new token ``<s>'' which generates \adv's desired image. 
%
All these attacks are effective against fine-tuning \crt{s} in Section~\ref{back-conceptrem}.
%However, for proper robustness evaluation, it is important to evaluate \crt{s} against attacks which account for \crt{s}.}
% To optimize <s>, we find $v$, an embedding for <s>, corresponding to least loss $\mathcal{L}_{CCE}=\mathcal{L}_{MSE}(\epsilon, \epsilon_\theta(z_t,v,t))$, where $\epsilon\sim\mathcal{N}(0,1)$, and $\mathcal{L}_{MSE}$ is the mean-squared-error. 
% CCE and SneakyPrompt account for different fine-tuning \crt{s}. 
%Among the described attacks, only \ringbell and \pez are na\"{i}ve and we later describe how we modify them to account for \crt{s} (Section~\ref{sec:baseline}).
In Section~\ref{sec:baseline}, we enhance two na\"{i}ve attacks, \ringbell and \pez, to defeat all these \crt{s}, including \unsafediff.
\begin{arxiv}

SurrogatePrompt~\cite{ba2023surrogateprompt} is a recent attack against a \crt in a commercial \tti systems that targets input filters, not output filters like \method. Therefore we omit it in our robustness evaluation.
\end{arxiv}

==> old_versions/WACV/3problem.tex <==
\section{Problem Statement}\label{sec:problem}


Our goal is to design a \crt which can effectively detect $\imgunacc$ from \tti models. 
% We describe an adversary model, requirements of an ideal \crt, and limitations of prior works. 
% according to the requirements.


\noindent\textbf{Adversary Model.} We consider a deployed target \tti model ($\target$) to which a client has blackbox access to send an input ($\prompt$) and obtain a generated image ($\imgclean$). Further, $\target$ uses some \crt. The goal of the adversary (\adv) is to force $\target$ to generate $\imgunacc$ despite the presence of a \crt to suppress it.
We give an advantage to \adv by allowing whitebox access to a local identical copy of $\target$ with the \crt for use in designing attacks. This is reasonable as \dm and CLIP are publicly available. For filtering \crt{s}, we assume that \adv has whitebox access to the filter to use its loss function in designing the attacks.

\noindent\textbf{Requirements} An ideal \crt should be:
\begin{enumerate*}[label=\textbf{R\arabic*},leftmargin=*]
\item\label{effective} \textit{Effective} in minimizing the generation of $\imgunacc$;
\item\label{utility} \textit{Utility-preserving}, maintaining the quality of acceptable images (for fine-tuning \crt{s}) or not blocking them (for filtering \crt{s}); and
\item\label{robust} \textit{Robust} against evasion with $\advprompt$.
\end{enumerate*}



\noindent\textbf{Limitations of Prior Works.} 
%We now briefly discuss the limitations of different types of prior \crt{s} \emph{vis-a-vis} the requirements above. 
% , we empirically show 
We summarize the limitations of prior works which are empirically evaluated later in Section~\ref{sec:evaluation}.
\textit{Fine-tuning \crt{s}} modify $\target$ thereby explicitly creating a trade-off between \ref{effective} and \ref{utility}~\cite{gandikota2023erasing,kumari2023ablating,zhang2023forgetmenot,heng2023selective,heng2023selective,gandikota2023unified,kim2023towards}.
Further, most of these \crt{s} do not consider \ref{robust} in their design and are susceptible to evasion by \adv with $\advprompt$.
\textit{Filtering \crt{s}}~\cite{radford2021learning,unsafeDiff} detect unacceptable concepts either in $\prompt$ (aka prompt filter) or in $\imgclean$ and block them (a.k.a image filter). Since, they do not modify $\target$, they can maintain \ref{utility} without impacting \ref{effective}. Prior filtering approaches may not be accurate in detecting unacceptable concepts (poor \ref{effective})~\cite{li2024safegen} and can be easily evaded (poor \ref{robust}) (\cite{rando2022redteaming} and Section~\ref{sec:filterEval}). Further, the current state-of-the-art filter, \unsafediff~\cite{unsafeDiff}, trains specialized classifiers for each concept on substantial data, which limits their generalization to new concepts.


==> old_versions/WACV/4approach.tex <==
\section{\method: Robust Filtering CRT}\label{sec:approach}

We present \method, a robust \underline{co}ncept \underline{fi}ltering \crt. 
\method uses a classifier \filter to detect images and filter unacceptable concepts in generated images. Following Stable Diffusion v1.4 (SDv1.4)~\cite{stable-diffusion}, on detecting an unacceptable concept, \method generates a replacement image~\cite{radford2021learning, rando2022redteaming}.
We identify CLIP as the natural choice for such a classifier as it is
\begin{enumerate*}[leftmargin=*,label=(\alph*)]
\item pre-trained on a large dataset covering a wide range of concepts, and
\item used across many \tti models, and encodes similar information as seen in them.
\end{enumerate*}
Hence, CLIP is a better choice for a filter than training specialized classifiers for each concept (e.g.,~\cite{unsafeDiff}).

 However, simply using CLIP for \method is not sufficient as seen in SDv1.4's filter ($\filter_{SD}$)~\cite{radford2021learning}. 
$\filter_{SD}$ thresholds the cosine similarity between the embeddings of $\imgclean$ and each pre-defined unacceptable concept to identify $\imgunacc$. 
Rando et al.~\cite{rando2022redteaming} design adversarial prompts ($\advprompt$) to evade $\filter_{SD}$ by constructing $\advprompt$ to force a misclassification.
% Since $\filter_{SD}$ uses only the cosine similarity to $\cunacc$, it gives \adv the freedom to modify the prompt embeddings in \emph{any direction}, while constructing $\advprompt$, to force a misclassification.
%
We address this in \method by configuring CLIP's classification objective for fine-tuning to further improve robustness. 

\noindent\textbf{Configuring CLIP's Classification Objective.} Instead of using the cosine similarity to only $\cunacc$ as in $\filter_{SD}$, we configure the objective function of \method for filtering $\imgunacc$ by using the cosine similarity to \emph{both} $\cunacc$ and $\cacc$. 
% \change{This makes \adv's goal more difficult as they are forced to optimize $\advprompt$ such that the resulting image embedding is far from $\phi_p(\cunacc)$, \emph{and} close to $\phi_p(\cacc)$, which is an additional stipulation arising from the design of \method.}
Further, jointly optimizing for two embeddings yields better utility as observed in prior fine-tuning \crt{s}~\cite{kumari2023ablating, Tsai2023RingABellHR, gal2021stylegannada}. 
%
Given $\imgclean$, \method checks the cosine similarity of $\phi_x(\imgclean)$ to $\phi_p(\cunacc)$ and $\phi_p(\cacc)$. Formally, we define \method as $\filter(x, \cunacc, \cacc)$
\begin{equation}\label{eq:att}
 = \text{argmax}_{i, i\in{a,u}} \left\{\frac{\text{exp}{(\text{cos}(\phi_x(x),\phi_p(\concept_i)) / \tau)}}{\sum_{j \in \{a,u\}}\text{exp}(\text{cos}(\phi_x(x),\phi_p(\concept_j)) / \tau)}\right\}
\end{equation} 
$\tau=\frac{1}{100}$ is the default temperature parameter used in CLIP. 
%Further, the cosine similarity is equivalent to the scaled Euclidean distance between the embeddings~\cite{ModalityGap}: 
%\[(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) = 2-2\overline{\phi_x(\imgclean)}\cdot\overline{\phi_p(\concept)}\]
%\[\implies \text{cos}(\imgclean, \concept) = -\frac{1}{2}(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)})^T(\overline{\phi_x(\imgclean)} - \overline{\phi_p(\concept)}) + 1\]
%Hence, by using CLIP as a filter, we \change{are effectively projecting} the image embeddings onto the vector between $\cunacc$ and $\cacc$ and classifying it based on its distance to both.  
%
% This simple configuration change in CLIP's classification objective restricts \adv to adding noise only along the low-dimensional vector joining $\cunacc$ and $\cacc$: $\phi_p(\cunacc) - \phi_p(\cacc)$ in the direction of $\cacc$.
% This is more challenging for \adv to evade than $\filter_{SD}$, as projecting to a lower-dimensional representation can improve robustness~\cite{pca1,pca2}.
% Hence, we conjecture that this can help satisfy \ref{effective} and \ref{robust} (as shown later in Section~\ref{sec:evaluation}).
% This change in objective function is required to apply fine-tuning.

% \change{Sec. 2.2: How are the acceptable concepts used in the fine-tuning selected? Same for Sec. 4 - equation 1: do you randomly sample acceptable concepts? Can selecting semantically close acceptable concepts improve performance? - ANSWERED}


% \change{Rationale for fine-tuning?}
\noindent\textbf{Fine-tuning.} The above configuration change lets us use fine-tuning to push acceptable and unacceptable concepts away from each other while maintaining their pairing with their corresponding image embeddings (for utility).
Our fine-tuning objectives are inspired by the adversarial training literature which increase the distance of the training data records to the decision boundary to minimize the effect of adversarial examples~\cite{zhang2019theoretically}. 
% may impact the utility on some concepts due to the close proximity of some $\cunacc$ and $\cacc$.
% To restore any drop in utility, we use fine-tuning. 
We use two different fine-tuning variants depending on the group of concepts.


For concepts that have a strong correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$ (for example, where $\cacc$ is a broader category that includes $\cunacc$; $\cunacc$ = \emph{R2D2} and $\cacc$ = \emph{robot}), we fine-tune \filter to increase the difference between $\phi_p(\promptuacc)$ and $\phi_p(\promptacc)$. We minimize the following:
\begin{equation}\label{eq:ft1}
L_{\method} = -||\overline{\phi_p(\promptuacc) - \phi_p(\promptacc)}||_2
\end{equation}
where $\overline{\cdot}$ denotes normalization. 
% The prompts used for the \tti model are not known before-hand, but we can define the concepts to be filtered. 
% Since the prompt includes these concepts, filtering the images generated from the prompts is sufficient.
For the case where $\cunacc$ and $\cacc$ are opposites (e.g., $\cunacc$ = \emph{violence} and $\cacc$ = \emph{peaceful}), the above objective function might have a low correlation between $\phi_p(\prompt)$ and the corresponding $\phi_x(\imgclean)$. This might result in poor utility. In this case, we use following objective function:
\begin{equation}\label{eq:ft2}
    \begin{split}
        \mathcal{L}_{\method} = \alpha_{\text{aa}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{aa}) 
        -\alpha_{\text{ua}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{ua}) \\
        + \alpha_{\text{uu}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{uu})  
        -\alpha_{\text{au}}\mathcal{L}_{\text{Con}}(\mathcal{D}_{au}) \\
        -\alpha_{\text{uu-t}}\mathcal{L}_{MSE}(\phi_p(\mathcal{P}^{u}), \phi_p(\mathcal{P}^{a})) \\
    \end{split}
\end{equation}
where $\mathcal{D}_{aa} = \{(\imgacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{au} = \{(\imgacc_j, \promptuacc_j)\}_{j=1}^N$, \\$\mathcal{D}_{ua} = \{(\imgunacc_j, \promptacc_j)\}_{j=1}^N$, $\mathcal{D}_{uu} = \{(\imgunacc_j, \promptuacc_j)\}_{j=1}^N$, $\mathcal{P}^u = \{\promptuacc_j\}$, and $\mathcal{P}^a = \{\promptacc_j\}$, and $\alpha_{(\cdot)}$ are regularization hyperparameters. We assign equal weight to each of the loss terms, thus choosing $\alpha_{(.)}= 1$. 
The above objective function encourages the CLIP embeddings of $\imgunacc$ and $\promptuacc$, and $\imgacc$ and $\promptacc$, to be closer together while increasing the distance between $\imgunacc$ and $\promptacc$, and $\imgacc$ and $\promptuacc$, respectively. 

We use prompts ($\promptuacc$ and $\promptacc$) for fine-tuning in Equation~\ref{eq:ft1} and Equation~\ref{eq:ft2} instead of only concepts ($\cunacc$ and $\cacc$): 
$\promptuacc$ and $\promptacc$ already contain $\cunacc$ and $\cacc$, and provide more context. 
During fine-tuning of \method, there is a trade-off between \ref{effective} and \ref{utility} which is inherent to all other fine-tuning \crt{s}. We subject our fine-tuning to the constraint that achieved the highest effectiveness for the least drop in utility.
We show the benefit of fine-tuning in Section~\ref{sec:finetuningEval}.  

==> old_versions/WACV/5setup.tex <==
\section{Experimental Setup}\label{sec:setup}

% \input{figures/fig_trainvaltest}
We use SDv1.4~\cite{stable-diffusion} and its default configuration as \target following prior work~\cite{gandikota2023erasing, kumari2023ablating, zhang2023forgetmenot, heng2023selective, gandikota2023unified, kim2023towards}.
% We describe the attack baselines against \crt{s} (Section~\ref{sec:baseline}), metrics (Section~\ref{sec:metrics}), and pipeline used for evaluating \crt{s} (Section~\ref{sec:pipeline}).
% dataset and model configuration (Section~\ref{sec:datasets}).

\subsection{Revisiting Attack Baselines}\label{sec:baseline}

% We compare \method with prior state-of-the-art \crt{s} across \ref{effective}, \ref{utility}, and \ref{robust}. 
% We use six fine-tuning \crt{s} (\ca, \forgetNot, \sa, \esd, \unifiedCE, and \sdd) and one filtering \crt (\unsafediff) which are described in Section~\ref{back-conceptrem}. For filtering \crt, we do not compare with SD-Filter as \unsafediff outperforms it.
% To evaluate \ref{robust}, 
We consider different state-of-art attacks from literature (Section~\ref{back-attacks}).
%
We modify existing na\"{i}ve attacks: \ringbell, and \pez, to account for \crt{s} (indicated with ``+''). 
All \crt{s} use some variant of the following optimization: detach $\cunacc$ from $\prompt$ such that the generated image is far from $\cunacc$ and closer to some $\cacc$. 
On the other hand, attacks against \tti models design $\advprompt$ such that $\imgadv$ is closer to $\cunacc$ and far from $\cacc$. 
Hence, to design an effective attack which accounts for such \crt{s}, in addition to the attacks' original objectives, we minimize the loss between $\phi_p(\advprompt)$ and $\phi_p(\cacc)$ while increasing the loss with $\phi_p(\cunacc)$.
% Hence, an effective attack which accounts for such \crt{s} must find $\advprompt$ such that its generated image is unacceptable (via the attacks' original objective) in spite of the \crt. To do this, in addition to the attacks' original objectives, we minimize the loss between $\advprompt$ and $\cacc$ while increasing its loss with $\cunacc$.
% Hence, to design an effective attack which accounts for such \crt{s}, 
% This, in turn, will move $\phi_p(\advprompt)$ closer to $\phi_p(\cacc)$ and farther from $\phi_p(\cunacc)$.
% \change{Since the attack objective is opposite to that of \crt{s}, the attack finds $\advprompt$ which counters the expected benefits of \crt{s}.}
% \change{This allows the generated image from $\advprompt$ to be incorrectly identified as acceptable while preserving the ability to generate $\imgunacc$.}
%
We modify the attacks to construct $\advprompt$ using following loss: 
\begin{equation}\label{eq:attack}
    \begin{split}
\mathcal{L}_{att+} = \mathcal{L}_{att} - \alpha_u \mathcal{L}_{MSE}(\phi_p(\cunacc), \phi_p(\advprompt)) + \\
\alpha_a \mathcal{L}_{MSE}(\phi_p(\cacc), \phi_p(\advprompt))
    \end{split}
\end{equation}
where $att \in$ \{\ringbell, \pez\} when \crt$\in $\{\ca, \forgetNot, \sa, \esd, \unifiedCE, \sdd, \unsafediff, \method\}, and $\mathcal{L}_{att}$ is the attack's original objective.
We assign equal weight to all loss terms and use $\alpha_u = \alpha_a = 1.$
% Further, To design attacks against \unsafediff and \method, .
Recall from Section~\ref{back-attacks} that \cce already accounts for different fine-tuning \crt{s}. For filtering \crt{s} (\unsafediff and \method), we modify \cce using Equation~\ref{eq:attack} and call it \cce+. 
%
Finally, typographic attack~\cite{noever2021typographicattck} against CLIP superimposes text characters onto an (unrelated) image to fool CLIP by forcing it to focus on the text instead of the image. We turn this into an attack against \crt{s} by superimposing $\cacc$ at the bottom of $\imgunacc$. Using the resulting adversarial images, we use \pez+ to find their corresponding $\advprompt$. We call this attack \typo+.

\input{figures/fig_pipeline}

\subsection{Metrics}\label{sec:metrics}

% We now describe the metrics to evaluate each of the requirements. 
\noindent We use a \emph{reference CLIP} (SDv1.4), separate from \target with the \crt{s}, following prior work~\cite{kumari2023ablating, gandikota2023erasing,gandikota2023unified,kim2023towards}.

\noindent\textbf{\underline{\ref{effective} (Effectiveness).}} For fine-tuning \crt{s}, we use
% \begin{itemize}[leftmargin=*,wide,labelindent=0pt]
\noindent\textbf{CLIP accuracy}~\cite{hessel-etal-2021-clipscore,kumari2023ablating} which is the cosine similarity between the embeddings of the generated image $\imgclean$ with the embeddings of $\cunacc$ and $\cacc$ from the reference CLIP. This outputs the likelihood of predicting $\cunacc$. Hence, CLIP accuracy should be low (ideally zero) for effective concept removal. Formally, it is:
$\frac{\text{exp}{(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc)))}}{\text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cunacc))) + \text{exp}(\text{cos}(\tilde{\phi_x}(\imgclean), \tilde{\phi_p}(\cacc)))}$
where $\tilde{\phi_p}$ and $\tilde{\phi_x}$ are embeddings from the reference CLIP.
For \method, if $\imgunacc$ is detected, a replacement image is generated. Here, we calculate the CLIP accuracy on the final set of images after filtering. 
% Since the metrics compare with baseline reference CLIP, we use the same default replacement image as in the SD v1.4 filter.

\noindent For filtering \crt{s}, we use \textbf{false negative rates (FNR)~\cite{unsafeDiff,rando2022redteaming}} which is the fraction of images with $\cunacc$ which are not blocked. 
It should be low (ideally zero).
% \end{itemize}


\noindent\textbf{\underline{\ref{utility} (Utility).}}
% \begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
\noindent For fine-tuning \crt{s}, we use \textbf{normalized CLIP score} which is the ratio of cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$ from \target, compared to that from a reference CLIP as a baseline which is assumed to have the maximum achievable CLIP score. Formally, $\frac{\text{cos}(\phi_x(\imgclean),\phi_p(\prompt))}{\text{cos}(\tilde\phi_x({\imgclean}), \tilde\phi_p(\prompt))}$. 
Normalized CLIP score should be high (ideally one) for high utility. 
% For the normalized CLIP score to be greater than one, the fine-tuned \tti model should generate images that match their prompts more closely than the original \tti model. This is unlikely to occur in practice as seen in our evaluation (c.f. Table~\ref{tab:utility}).
This metric is different from standard CLIP score from prior work~\cite{hessel-etal-2021-clipscore,kumari2023ablating, kim2023towards,gandikota2023unified} which only measures the cosine similarity between $\phi_x(\imgclean)$ and $\phi_p(\prompt)$. 
%We did this to scale the original CLIP score between zero and one while comparing \target to the reference CLIP.
We modified it to compare the utility of the \tti with the \crt to that of the \tti without the \crt.
Hence, a perfect match will give a score of one.

For filtering \crt{s}, we use \textbf{False Positive Rates (FPR)~\cite{unsafeDiff,rando2022redteaming}} which is the fraction of images without $\cunacc$ which are blocked.
It should be low (ideally zero).
% \end{itemize} 


\noindent\textbf{\underline{\ref{robust} (Robustness).}} We use the same metrics as \ref{effective}: CLIP accuracy for fine-tuning \crt{s}, and FNR for filtering \crt{s}. 




% \subsection{Concept Types}\label{sec:concepts}




\subsection{Pipeline for Evaluating \crt{s}}\label{sec:pipeline}

We now describe the pipeline which includes identifying acceptable concepts (step 1), generation of datasets (step 2), training filters or fine-tuning \tti models with \crt{s} (step 3), validating acceptable concepts (step 4), and evaluating different \crt{s} (step 5). We present an overview of the pipeline in Figure~\ref{fig:pipeline} and describe each of the steps below.



\noindent\textbf{Concept Types.}
We use the same $\cunacc$ as prior work~\cite{kumari2023ablating, pham2023circumventing, kim2023towards}, categorizing them into three groups.
% \begin{itemize}[leftmargin=*,wide,  labelindent=0pt]
Group-1 covers inappropriate concepts: \emph{nudity},
%(e.g., female breasts or male/female genitalia), 
\emph{violence}, 
%(e.g., bloody scenes, fighting, burning, hanging, weapons, and wars), 
\emph{disturbing}, 
%(e.g., distorted faces, bodies, human flesh, or bodily fluids), 
and \emph{hateful}.
%(e.g., defamatory racial depiction, harmful stereotypes, or Holocaust scenes).
Group-2 covers copyright-infringing concepts: \emph{Grumpy Cat, Nemo, Captain Marvel, Snoopy}, and \emph{R2D2}.
Group-3 covers unauthorized use of images: \emph{Taylor Swift, Angelina Jolie, Brad Pitt}, and \emph{Elon Musk}.
% \end{itemize}


\noindent\textbf{\underline{Step 1: Identifying Acceptable Concepts}}
A good choice of $\cacc$ is one which effectively steers a \tti model away from generating $\imgunacc$ while maintaining utility on other concepts. Hence, the choice of $\cacc$ can impact \ref{effective} and \ref{utility}. 
We select $\cacc$ for a given $\cunacc$ such that it is either opposite to $\cunacc$ (Group-1) or is a semantic generalization of $\cunacc$ so as to avoid infringing copyrights (Groups-2,3).
For $\cunacc$ in Group-1, we consider multiple alternative synonyms for $\cacc$, from which we choose the best possible candidate by measuring effectiveness and utility on a validation dataset (see Step 4).
For $\cunacc$ in Groups-2,3, we use $\cacc$ from prior work for a fair comparison~\cite{kumari2023ablating,heng2023selective}.
We indicate them in the format ``$\cunacc$ $\rightarrow$ $\cacc$''.
For \textbf{Group-1}, $\cacc$ is the opposite of $\cunacc$ and we consider the following choices of $\cacc$: \emph{nudity} $\rightarrow$ \{\emph{clothed} and \emph{clean}\}; \emph{violence} $\rightarrow$ \{\emph{peaceful}, \emph{nonviolent}, and \emph{gentle}\}; \emph{disturbing} $\rightarrow$ \{\emph{pleasing}, \emph{calming}, and \emph{soothing}\}; \emph{hateful} $\rightarrow$ \{\emph{loving}, \emph{compassionate}, and \emph{kind}\}.
For \textbf{Group-2}: $\cacc$ is the broader category of $\cunacc$, following prior works~\cite{kumari2023ablating,heng2023selective,gandikota2023erasing}: \emph{Grumpy Cat} $\rightarrow$ \emph{cat}, \emph{Nemo} $\rightarrow$ \emph{fish}, \emph{Captain Marvel} $\rightarrow$ \emph{female superhero, Snoopy} $\rightarrow$ \emph{dog}, and \emph{R2D2} $\rightarrow$ \emph{robot}. 
For \textbf{Group-3}, $\cacc$ is the sex of $\cunacc$, following prior works~\cite{heng2023selective, zhang2023forgetmenot, kim2023towards}: \{\emph{Taylor Swift, Angelina Jolie}\} $\rightarrow$ \emph{woman} and \{\emph{Brad Pitt, Elon Musk}\} $\rightarrow$ \emph{man}.
We compare \method with each \crt category separately using concepts they were originally evaluated on: Group-1 for filtering \crt{s}~\cite{unsafeDiff}; all groups for fine-tuning \crt{s}~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards}.
% \end{itemize}



% \subsection{Dataset and Model Configurations}\label{sec:datasets}

\noindent\textbf{\underline{Step 2: Generate and Split Datasets}}

% We describe the generation of train, validation, and test datasets.

\noindent\textbf{Train Datasets.}
% We summarize the different training/fine-tuning dataset configurations across \crt{s} in Table~\ref{tab:trconfig}. 
% \input{tables/tab_trconfig}
For \emph{fine-tuning \crt{s}}, 
% Different fine-tuning \crt{s} use different dataset configurations to ensure that \ref{effective} and \ref{utility} are met. 
we use the exact same configuration as described in their original works. 
This configuration for a specific \crt is the same across different concepts.
% While the configuration across different \crt{s} vary, the configuration for a specific \crt across different concepts is the same, in accordance with the instructions in the respective works. 
% We briefly summarize them in Table~\ref{tab:trconfig}. 
\ca uses acceptable prompts which are generated from ChatGPT such that they contain $\cacc$, and 1 image per prompt. \esd and \sdd both use only $\cunacc$, and \sdd additionally uses 10 images corresponding to $\cunacc$. All images are generated using SD v1.4. 
\forgetNot uses unacceptable prompts of the form ``An image of \{$\cunacc$\}'', and 1 image per prompt.
For all of them, we use their code for consistency with their original papers~\cite{githubGitHubNupurkmr9conceptablation,githubGitHubRohitgandikotaerasing,githubGitHubSHILabsForgetMeNot,githubGitHubRohitgandikotaunifiedconceptediting,githubGitHubClearnusselectiveamnesia,githubGitHubNannullnasafediffusion,githubGitHubYitingQuunsafediffusion}.



\noindent For \emph{filtering \crt{s},} we train $\filter_{\unsafediff}$ using the original dataset configuration and code~\cite{unsafeDiff}. 
For \method, we follow \ca~\cite{kumari2023ablating} to generate 10 unacceptable and acceptable prompts using ChatGPT, with one image per prompt from SDv1.4.
For Group-2, we randomly select 10 ChatGPT-generated prompts from \ca~\cite{kumari2023ablating}.
We use a small amount of training data following prior works which show little data is enough to modify CLIP~\cite{yang2023robust,carlini2022poisoning}. This is validated by our results (Section~\ref{sec:evaluation}).



\noindent\textbf{Validation Datasets.}
For validation datasets ($\mathcal{D}_{val}$), we denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalunacc$; and the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dvalacc$.
For \ref{effective}, we use $\dvalunacc$ by generating 10 unacceptable prompts using ChatGPT, and generate 5 images per prompt using SD v1.4. 
For \ref{utility}, we use $\dvalacc$ by randomly choosing 100 acceptable prompts from the COCO 2014 dataset~\cite{coco}, and 1 image per prompt, from SD v1.4.
% We summarize them in Table~\ref{tab:valconfig}. 

% \input{tables/tab_valconfig}

\noindent\textbf{Test Datasets.} %We now present datasets for evaluating different \crt{s}. 
For test dataset ($\mathcal{D}_{te}$), we denote the dataset with acceptable prompts ($\promptacc$) and corresponding images ($\imgacc$) as $\dtestacc$; and with unacceptable prompts ($\promptuacc$) and corresponding images ($\imgunacc$) as $\dtestunacc$.

% \input{tables/tab_teconfig}

\noindent For evaluating effectiveness (\ref{effective}), we use $\dtestunacc$ which is generated as follows:
For Group-1 concepts (\emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing}), we use Inappropriate Image Prompts (I2P), containing prompts which are likely to generate unsafe images~\cite{schramowski2022safe}.
We process I2P dataset following prior work~\cite{gandikota2023erasing, gandikota2023unified} to obtain 300 unacceptable prompts.
% For \emph{nudity}, I2P includes a ``nudity percentage'' attribute. We choose all unacceptable prompts with a nudity percentage $>10$, resulting in a total of 300 unacceptable prompts, in accordance with prior works~\cite{gandikota2023erasing, gandikota2023unified}.
\unsafediff~\cite{unsafeDiff} also used \emph{political} as a concept, which is excluded from our evaluation since it is not a part of I2P. 
% Note that I2P prompts do not explicitly contain $\cunacc$, \emph{i.e., the words \emph{nude}, \emph{violent}, \emph{hateful}, or \emph{disturbing} are not explicitly included in the prompts}.
For concepts in Group-2,3, there are no standard benchmark datasets. Hence, we use the dataset from prior works~\cite{kumari2023ablating, gandikota2023erasing} with 200 unacceptable images generated from SDv1.4 from 10 unacceptable prompts generated from ChatGPT.
For \ref{utility}, we use the COCO 2014 test dataset as $\dtestacc$, consistent with prior work, with 200 randomly chosen acceptable prompts, non-overlapping with $\dvalacc$.
For \ref{robust}, we use $\dtestadv$ by applying different attacks on $\dtestunacc$ to generate adversarial prompts.
% We summarize the datasets in Table~\ref{tab:teconfig}. 

\noindent\textbf{\underline{Step 3: Fine-tuning with \crt{s}/training filter.}}
Using $\dtrain$, we fine-tune \tti models using six fine-tuning \crt{s} described in Section~\ref{back-attacks}.
% \change{We omit the comparison with more recent works due to ...~\cite{}.}
For filtering \crt{s}, we consider one baseline (\unsafediff) and do not compare with SD-Filter as \unsafediff outperforms it.
We train \unsafediff's classifier on their dataset and we fine-tune \method on $\dtrain$ using Equation~\ref{eq:ft1} for Groups-2,3 concepts and Equation~\ref{eq:ft2} for Group-1 concepts. 
We use the CLIP L-patch-14~\cite{vit} due to its popularity, which is also the default encoder with SDv1.4. However, other variants of CLIP are also applicable.

\noindent\textbf{\underline{Step 4: Select best $\cacc$ using $\mathcal{D}_{val}$}.}
For Group-1 concepts, we evaluate \ref{effective} and \ref{utility} for different candidates of $\cacc$ on $\dvalunacc$ and $\dvalacc$ respectively. 
We found the concepts with the best results: \emph{nudity} $\rightarrow$ \emph{clean}, \emph{violence} $\rightarrow$ \emph{peaceful}, \emph{disturbing} $\rightarrow$ \emph{pleasing}, and \emph{hateful} $\rightarrow$ \emph{loving}.
For \emph{nudity}, we eliminated \emph{clothed} as it blocked images with minimal exposed skin despite being acceptable~\cite{unsafeDiff,schramowski2022safe}.
%
%
% We use concepts in Group-1 following prior work~\cite{unsafeDiff} to evaluate filtering \crt{s}. 
% We use \emph{nudity} and \emph{violence} from Group-1, and all the concepts from Group-2 and Group-3 following prior works~\cite{kumari2023ablating,heng2023selective,zhang2023forgetmenot,kim2023towards} to evaluate fine-tuning \crt{s}. 

% We summarize the final concepts for evaluation in Table~\ref{tab:concepts}.



\noindent\textbf{\underline{Step 5: Evaluation}.} 
We evaluate \ref{effective} on $\dtestunacc$, \ref{utility} on $\dtestacc$, and \ref{robust} on $\dtestadv$, which is generated by running different attacks on $\dtestunacc$ to get $\advprompt$. We pass the prompts from the datasets to the \tti model and compute different metrics.



==> old_versions/WACV/6evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}



\subsection{Impact of Fine-Tuning}\label{sec:finetuningEval}

We first empirically show how fine-tuning can improve the robustness similar to adversarial training in classifiers. Adversarial training~\cite{zhang2019theoretically} explicitly pushes the decision boundary away from training data records. Similarly, our fine-tuning objective, pushes the embeddings of acceptable and unacceptable concepts away from each other. This results in correctly classifying $\prompt_{adv}$ by \method.

To demonstrate this, we generated 10 adversarial prompts, with 5 images per prompt using \cce+. 
We report the mean absolute difference between the cosine similarity of all the $\phi_x(\imgadv)$ and $\phi_p(\cunacc)$ and $\phi_p(\cacc)$ in Table~\ref{tab:advsims}. Across all concepts, using fine-tuning (w/ FT) makes $\phi_x(\imgadv)$ closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$, compared to the baseline without fine-tuning (w/o FT). Hence, fine-tuning is likely to correctly identify $\imgadv$ as $\imgunacc$.

\input{tables/tab_adv_sims}
\input{tables/tab_effectiveness}

Furthermore, we evaluate the impact of fine-tuning on \ref{effective} and \ref{utility}. For \ref{effective}, CLIP accuracy for several concepts is statistically better after fine-tuning: \emph{Angelina Jolie} (0.03 $\pm$ 0.00 from 0.12 $\pm$ 0.02), \emph{Brad Pitt} (0.00 $\pm$ 0.00 from 0.02 $\pm$ 0.01), \emph{Elon Musk} (0.03 $\pm$ 0.00 from 0.07 $\pm$ 0.01). For \ref{utility}, CLIP scores are better for some concepts after fine-tuning: \emph{nudity} (0.94 $\pm$ 0.08 from 0.83 $\pm$ 0.07); \emph{grumpy cat} (0.98 $\pm$ 0.04 from 0.88 $\pm$ 0.03), \emph{Nemo} (0.37 $\pm$ 0.02 from 0.24 $\pm$ 0.05), \emph{R2D2} (0.66 $\pm$ 0.02 from 0.52 $\pm$ 0.03), and \emph{Elon musk} (0.92 $\pm$ 0.02 from 0.97 $\pm$ 0.01).
The metrics for other concepts remains statistically similar.



\input{tables/tab_utility}

\input{tables/tab_robustness}

% We evaluate \method with fine-tuning \crt{s} (Section~\ref{sec:finetuneEval}), and then filtering \crt (Section~\ref{sec:filterEval}). 


\subsection{Comparison with Fine-tuning \crt{s}}\label{sec:finetuneEval}


\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report CLIP accuracy on $\dtestunacc$ in Table~\ref{tab:effectiveness}. 
We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.
All \crt{s} exhibit poor accuracy on \emph{nudity} and \emph{violence}, likely due to fine-tuning \crt{s} being sensitive to input prompts~\cite{pham2024robust, yang2024guardt2i, ma2024jailbreaking}. Specifically, other \crt{s} depend on the $\cunacc$ being included in prompts, which is absent for \emph{nudity} and \emph{violence} prompts in the I2P dataset.
\method consistently maintains high accuracy on the I2P benchmark dataset as it classifies the generated images. 
\esd, and \sdd have better accuracy compared to the other three fine-tuning \crt{s}. 
This could be attributed to their similar optimizations which includes fine-tuning \dm, conditioned on $\cunacc$, to match the unconditioned \dm to reduce the influence of $\cunacc$ on the output.  
For \unifiedCE, we attribute the higher effectiveness to directly removing the influence of $\cunacc$ from the \tti model parameters. \textbf{\textit{Overall, \method is more effective than other fine-tuning \crt{s}.}}



\noindent\textbf{\underline{\ref{utility} Utility.}} We report normalized CLIP scores in Table~\ref{tab:utility} on $\dtestacc$.
We use \colorbox{mynicered}{red} if score is between 50-70, \colorbox{myniceblue}{blue} if between 70-90; \colorbox{mynicegreen}{green} if $>$90.
All the fine-tuning \crt{s} perform well across all concepts (either \colorbox{myniceblue}{blue} or \colorbox{mynicegreen}{green}) since the explicitly account for \ref{utility}. We observe that \ca with KL-Divergence-based optimization for cross-attention layers, and \unifiedCE with a precise closed-form solution to model updates, preserve \ref{utility} better than others. 
%
\method has high utility for all concepts except for \emph{violence}, and Group-2 concepts (\emph{Nemo}, \emph{Captain Marvel}, \emph{Snoopy}, and \emph{R2D2}).
During fine-tuning, there is a trade-off between \ref{effective} and \ref{utility}. 
For \textit{violence}, we observed an early decrease in utility during the very first epoch resulting in poor trade-off. 
For Group-2 concepts, we attribute the poor utility to the ambiguity in the unacceptable concepts. For instance, \emph{Nemo} is both a fish and a ship captain~\cite{VERNE_2024}, and \emph{Captain Marvel} represents both a male and a female superhero~\cite{Friedwald_2019_marvel}. 
To verify this, we precisely specify the unacceptable concepts to reduce ambiguity: as \emph{Nemo}$\rightarrow$ \emph{Nemo fish}, \emph{Captain Marvel}$\rightarrow$ \emph{Captain Marvel female superhero}, \emph{Snoopy}$\rightarrow$ \emph{Snoopy dog}, and \emph{R2D2}$\rightarrow$ \emph{R2D2 robot}. We evaluate \method on $\dvalacc$:
compared to the results in Table~\ref{tab:utility}, the normalized CLIP score for this new configuration is: 0.97 $\pm$ 0.00 (\emph{Nemo fish}), 0.90 $\pm$ 0.02 (\emph{Captain Marvel female superhero}), 0.98 $\pm$ 0.03 (\emph{Snoopy dog}), 0.92 $\pm$ 0.02 (\emph{R2D2 robot}), which are now labeled as \colorbox{mynicegreen}{green}.
We also evaluate effectiveness (\ref{effective}) and find that the CLIP accuracy is similar to Table~\ref{tab:effectiveness}.
% We also report the CLIP accuracy on $\dvalunacc$ to evaluate \ref{effective} with this new configuration: 0.02 $\pm$ 0.00 (\emph{Nemo fish}), 0.00 $\pm$ 0.00 (\emph{Captain Marvel female superhero}), 0.02 $\pm$ 0.01 (\emph{Snoopy dog}), 0.00 $\pm$ 0.00 (\emph{R2D2 robot}), which are effective, same as before. Hence, precisely specifying $\cunacc$ is important for \method and can satisfy \ref{utility} without sacrificing \ref{effective}. 
\textbf{\textit{Overall, \method's utility (\ref{utility}) is comparable to prior works.}}


\noindent\textbf{\underline{\ref{robust} Robustness.}} We report CLIP accuracy on $\dtestadv$ in Table~\ref{tab:robust}. 
% We use \colorbox{mynicered}{red} if accuracy is $>$50; \colorbox{myniceblue}{blue} if accuracy is between 25-50; \colorbox{mynicegreen}{green} if accuracy is $<$25.
We evaluate different \crt{s} against \typo+, \pez+, \cce/\cce+, and \ringbell+. We use the same color coding as in \ref{effective}. 
%
\cce/\cce+, being a white-box attack that uses the parameters of the entire \tti model, is the most powerful attack and renders all fine-tuning \crt{s} ineffective. However, \method is robust against \cce/\cce+ and outperforms all fine-tuning \crt{s}.
On the remaining attacks, all the fine-tuning \crt{s} have better robustness on Group-3 concepts than on Group-1 and 2. We attribute this to the difficulty of \tti models in generating high quality celebrity faces while also evading detection, as also observed in prior work~\cite{Matthias_2023}.
As expected, we note that all \crt{s} perform poorly on \emph{nudity} and \emph{violence} across all the attacks as they do not satisfy \ref{effective}.
% Hence, adversarial prompts for these concepts are likely to easily evade them. 
\textbf{\emph{Overall, \method is more robust than all prior work across all the concepts and attacks.}}
% We discuss the possibility of future attacks against \method in Section~\ref{sec:future}.



% \noindent\textbf{\underline{Summary.}} 
% We depict the trade-offs among \ref{effective}, \ref{utility}, and \ref{robust} in Figure~\ref{fig:radarsFT}. We use (1-CLIP accuracy) for \ref{effective} on $\dtestunacc$, normalized CLIP score on $\dtestacc$ for \ref{utility}, and (1-CLIP accuracy) for \ref{robust} on $\dtestadv$ using \cce/\cce+. 
% For each of the requirements, we use the average across all concepts as the representative value for a \crt.
% \emph{Overall, \method provides a better trade-off across the three requirements compared to all the fine-tuning \crt{s}.}

% \input{figures/fig_radar_ft}

































\subsection{Comparison with Filtering \crt}\label{sec:filterEval}

% We now compare with \unsafediff~\cite{unsafeDiff}, the state-of-the-art filtering \crt, across the three requirements and summarize the results. 
% To compare with \unsafediff~\cite{unsafeDiff}, we use FNR to evaluate effectiveness on $\dtestunacc$, FPR for utility on $\dtestacc$, and FNR for robustness on $\dtestadv$.




\noindent\textbf{\underline{\ref{effective} Effectiveness.}} We report FNR across four concepts (\emph{nudity}, \emph{violence}, \emph{disturbing}, and \emph{hateful}) in Table~\ref{tab:FilterEffective}.
We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FNR is $<$0.25.
\method has better FNR for three of the four concepts: \emph{nudity}, \emph{violence} (in \colorbox{mynicegreen}{green}), and \emph{hateful} (\colorbox{myniceblue}{blue} for \method and \colorbox{mynicered}{red} for \unsafediff). However, both \method and \unsafediff perform poorly on \emph{disturbing}. 
We attribute this poor effectiveness on Group-1 concepts to the subjective description of $\cunacc$. Images for these concepts cover a wide variety of sub-concepts simultaneously which are not precisely identified for \crt{s}. 
\emph{\textbf{Overall, \method is more effective than \unsafediff on most concepts.}}

\input{tables/tab_filter_effective}



\noindent\textbf{\underline{\ref{utility} Utility.}} We present FPR in Table~\ref{tab:FilterUtility} and use \colorbox{mynicered}{red} if FPR is $>$0.50, \colorbox{myniceblue}{blue} if FPR is between 0.25-0.50; \colorbox{mynicegreen}{green} if FPR is $<$0.25. As expected, we observe that both \emph{\textbf{\method and \unsafediff have comparable utility as they demonstrate a low FPR}}. \unsafediff explicitly includes images containing $\cacc$ while training the multi-headed classifier.

\input{tables/tab_filter_utility}

\noindent\textbf{\underline{\ref{robust} Robustness.}} We report FNR on the dataset for adversarial prompts and corresponding images in Table~\ref{tab:FilterRobust}. 
We use the same color-coding as \ref{effective}.
% We use \colorbox{mynicered}{red} if FNR is $>$0.50; \colorbox{myniceblue}{blue} if FNR is between 0.25-0.50; and \colorbox{mynicegreen}{green} if FNR is $<$0.25.
In addition to the four attacks from Table~\ref{tab:robust}, recall that \sneaky~\cite{yang2023sneakyprompt} is specifically designed to attack filtering \crt{s}. Hence, we also include the evaluation against \sneaky. 
Also, since \cce is not adaptive against filtering \crt's, we evaluate \unsafediff and \method against \cce+. We are the first to evaluate different attacks against \unsafediff.
%
\input{tables/tab_filter_robust}
%
We observe that \method is effective against \pez+ while \unsafediff can be evaded.
On all the remaining attacks, we show that \method is robust on more concepts than \unsafediff.
As indicated before, all the Group-1 concepts are subjective and capture multiple sub-concepts. This ambiguity could be the reason for poor \ref{robust}.
\emph{\textbf{Overall, \method is more robust than \unsafediff on a majority of the concepts across various attacks.}}

% \input{figures/fig_radar_filter}

\subsection{Summary}


\begin{figure}[h]
\centering
\begin{minipage}{0.5\columnwidth}
\includegraphics[width=1\columnwidth]{figures/radar_ft.pdf}
\subcaption{Fine-tuning \crt{s}.}
\end{minipage}%
\begin{minipage}{0.5\columnwidth}
\includegraphics[width=1\columnwidth]{figures/radar_filter.pdf}
\subcaption{Filtering \crt (\unsafediff)}
\end{minipage}
\caption{\method has better trade-offs than other \crt{s}}
\label{fig:summary}
\end{figure}

\noindent We depict the trade-offs among \ref{effective}, \ref{utility}, and \ref{robust} in Figure~\ref{fig:summary} across various \crt{s}.
For fine-tuning \crt{s}, we use (1-CLIP accuracy) for \ref{effective} on $\dtestunacc$, normalized CLIP score on $\dtestacc$ for \ref{utility}, and (1-CLIP accuracy) for \ref{robust} on $\dtestadv$ using \cce/\cce+ (the strongest attack among others). 
For filtering \crt, we use (1- FNR) on $\dtestunacc$ for \ref{effective}, (1- FPR) on $\dtestacc$ for \ref{utility}, and (1- FNR) on $\dtestadv$ using \cce+ for \ref{robust}.
For each of the requirements, we use the average across all concepts as the representative value for a \crt.
\emph{\textbf{Overall, \method provides a better trade-off across the three requirements compared to all the prior work.}}





==> old_versions/WACV/9discussion.tex <==
\section{Discussion and Future Work}\label{sec:discussions}

% We revisit our discussion on robustness  (Section~\ref{sec:future}), applicability/extensions of \method (Section~\ref{sec:extensions}), and a summary of this work (Section~\ref{sec:summary}).




% \subsection{Revisiting Robustness}\label{sec:future}

% \noindent\textbf{Addressing Future Attacks.} Recall that our certified robustness bound is loose (Section~\ref{sec:bound}). We leave the improvement of the bound as future work.

% \method maintains high robustness across all evaluated concepts. 
% The design of new attacks which can preserve unacceptable concepts while evading \method is an open problem. Here, adversarial training for \method can be used to increase its robustness.
% We can fine-tune CLIP with this objective: $\mathcal{L}_{\text{Con-adv}}(\dtestadv)=$
% \[- \frac{1}{N} \sum_{j = 1}^N \log \frac{\exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(\cunacc))/ \tau)}{\sum_{k \in \{a,u\}} \exp(\text{cos}(\phi_x(\imgadv_j), \phi_p(c_k))/ \tau)}\]
% where $\mathcal{D}_{adv} = \{(\imgadv_j, \advprompt_j)\}_{j=1}^N$. Assuming $\imgadv$ evades the filter, we optimize $\phi_p$ and $\phi_x$, such that $\phi_p(\imgadv_j)$ is closer to $\phi_p(\cunacc)$ than $\phi_p(\cacc)$. This loss would be added to Equation~\ref{eq:ft1} and~\ref{eq:ft2}. 
% Empirical evaluation of adversarially-trained \method is left as future work.


% \noindent\textbf{Extending the Theoretical Bound to Prompts.} 
% % Although \adv cannot modify text embeddings in practice, analyzing robustness in the CLIP embedding space is valuable as recent works have shown that small changes in the text embeddings of prompts, allow for fine-grained control over their generated images~\cite{yu2024uncovering, kawar2023imagic}. 
% To extend our theoretical bounds in Theorem~\ref{thm.1} to the prompt space,
% we assume Lipschitz continuity, commonly used in ML~\cite{bousquet2002stability}, certified robustness~\cite{li2023sok}, and more recently in the context of \tti models~\cite{chen2024your}.
% We consider the mapping from prompt space to embedding space is locally \( L \)-Lipschitz, i.e., the function \( \phi_x(f(\text{\prompt})) \) satisfies the following condition:

% For each prompt \(\text{\prompt}\), there exists a \(\delta_{\text{\prompt}} > 0\) such that
% $
% ||\phi_x(f(\text{\prompt})) - \phi_x(f(\text{\prompt} + \delta_{\text{\prompt}}))|| \leq L ||\delta_{\text{\prompt}}||.
% $

% Then, the inequality in Equation~\ref{eq:bound} can be related to the prompt space by a scalar factor \(\frac{1}{L}\). 
% Therefore, when \(\|\delta_{\text{\prompt}}\| \leq \frac{1}{L} \|\delta\|\), where \(\|\delta\|\) satisfies inequality in Equation~\ref{eq:bound}, the difference in embedding space will be bounded by \(\|\delta\|\), and CLIP remains robust.


% \subsection{Applications and Extensions to \method}\label{sec:extensions}


\noindent\textbf{Filtering Multiple Concepts.} UCE~\cite{gandikota2023unified} removes multiple concepts simultaneously.
\method can be extended by including multiple concepts simultaneously as well. Specifically, for \method in Equation~\ref{eq:att}, instead of specifying $\cunacc$ and $\cacc$ for a single concept, we can include $\cunacc$ and $\cacc$ for multiple concepts as a list. This is a simple configuration change compared to other filters which require retraining (e.g.,~\cite{unsafeDiff}). 
% Since none of the prior filtering \crt{s} evaluate multiple $\cunacc$, 
We leave the evaluation as future work.
% \change{Tried to add comment; didn't work so here it is: we said that none of prior crts evaluate against multiple concepts but cite gandikota as 1 crt that does, should we say "no other" prior crts?}. 

% \noindent\textbf{Filtering Artistic Styles.} 
% None of the prior filtering \crt{s} consider any copyrighted content and focus on only \emph{inapproriate Group-1 concepts}. 
% \method is the first filtering \crt which is applicable to concepts which are copyright-infringing (Group-2) or involve unauthorized use of personalized images (Group-3).
% Prior fine-tuning \crt{s} have considered removing artistic styles (e.g., painting in the style of Monet or Van Gogh) as copyrighted content~\cite{kumari2023ablating,gandikota2023erasing}.
% However, we observed that \method does not differentiate between images with and without artistic styles very well. Specifically, \emph{Monet painting} as $\cunacc$ and \emph{painting} as $\cacc$, are very similar for \method, thus reducing its effectiveness. We leave the optimization of \method to account for artistic styles as future work.

\noindent\textbf{Applicability to other \tti Models.} Fine-tuning \crt{s} are specific to particular stable diffusion models due to their tailored optimizations for \tti models. In contrast, filtering \crt{s} offer versatility as they can be applicable to any \tti model. 
Filters analyze only the generated image and the list of concepts, independent of the \tti model. 
And fine-tuning the filter using data from \tti model, as we do for \method, can satisfy \ref{effective} and \ref{utility}. 
This allows us to have a filter that will work with \tti models in different domains (e.g., anime images).
Explicit evaluation of \method for different \tti models is deferred to future work.


% \noindent\textbf{Summary.} Removing unacceptable concepts from \tti models is an important problem. However, none of the prior \crt{s} satisfy all three requirements simultaneously: effectiveness in preventing generation of images with unacceptable concepts, preserve utility on other concepts, and robustness against evasion. We propose \method, the \emph{first} robust \underline{co}ncept \underline{fi}ltering \crt which provides a better trade-off among the three requirements compared to prior \crt{s}.

==> proofs/proof.tex <==
\begin{proof}
    For an unacceptable image embedding $\hat{x} = \phi_x(\imgunacc)$,
    % We assume that $F(\hat{x})=1$ and 
    $g(\hat{x}):=g_u(\hat{x})$, then $g(\hat{x})-\Gamma>0$, and $\Gamma$ is the decision threshold for classification.
    Let $s_1=\tau\text{cos}(\hat{x},\cunaccc)$, $s_2=\tau\text{cos}(\hat{x},\caccc)$, $\textbf{s}=[s_1,s_2]^T$, 
    then
    $$g(\hat{x})=S(s_1) = \frac{exp(s_1)}{exp(s_1)+exp(s_2)},$$
    where $S(s_1)$ is the first item of Softmax function with respect to $\textbf{s}$.
    Then, we have $\frac{\partial}{\partial s_1} S = S(s_1)(1-S(s_1))\leq0.25, \frac{\partial}{\partial s_2} S = -S(s_1)S(s_2)\leq0.25$.

    Note that $||\hat{x}||>0$ and $||\caccc||>0$,
    we have 
    \begin{equation*}
    \begin{aligned}
        ||\frac{\partial}{\partial \hat{x}} s(\hat{x},\caccc)|| = ||\frac{\tau||\caccc||(I-xx^T)\caccc}{||\hat{x}||||\caccc||^2}||\\=\frac{\tau sin(\hat{x},\caccc)}{||\hat{x}||}\leq\frac{\tau}{||\hat{x}||}.
    \end{aligned}
    \end{equation*}
    And $||\frac{\partial}{\partial\hat{x}} s(\hat{x}, \cunaccc)||\leq\frac{\tau}{||\hat{x}||}$. 

    For each $\hat{x}$, according to the chain rule of composition functions, 
    $\frac{\partial}{\partial\hat{x}}g(\hat{x)}=\frac{\partial S}{\partial s_1}\cdot\frac{\partial s_1}{\hat{x}}+ \frac{\partial S}{\partial s_2}\cdot\frac{\partial s_2}{\hat{x}}\leq \frac{\tau}{2||\hat{x}||}$. Therefore the Lipschitz constant of $g(\hat{x})$ with respect to $\hat{x}$ is $\frac{\tau}{2||\hat{x}||}$, and
    \begin{equation*}
    \begin{aligned}
            ||g(\hat{x}+\delta)-g(\hat{x})||&\leq\frac{1}{2}\frac{\tau }{\min\{||u|||u\in U(\hat{x},\delta)\}} ||\delta||\\&\leq\frac{1}{2}\frac{\tau }{|||\hat{x}||-||\delta|||}||\delta||,
    \end{aligned}
    \end{equation*}
    where $U(\hat{x},\delta)$ is a $l_2$-ball of $\hat{x}$ with radius $\delta$.   
    
    When
    $||\delta||\leq(1-\frac{\tau }{\tau +2|g(\hat{x})-\Gamma|})||\hat{x}||<||\hat{x}||$, we have
    \begin{equation*}
    \begin{aligned}
        |g(\hat{x}+\delta)-g(\hat{x})|&=||g(\hat{x}+\delta)-g(\hat{x})||\\& \leq\frac{\tau }{2\left(\frac{||\hat{x}||}{||\delta||}-1\right)}\\
        &\leq\frac{\tau }{2\left(\frac{\tau +2|g(\hat{x})-\Gamma|}{2|g(\hat{x})-\Gamma|}-1\right)}\\
        &\leq|g(\hat{x})-\Gamma|=g(\hat{x})-\Gamma.
    \end{aligned}
    \end{equation*}
    Then,
    \begin{equation}
    \begin{aligned}
        g(\hat{x}+\delta)\geq|g(\hat{x})|-|g(\hat{x}+\delta)-g(\hat{x})|
        \\\geq g(\hat{x})- |g(\hat{x})-\Gamma|\geq \Gamma,
    \end{aligned}
    \end{equation}
    which concludes the proof.
    
\end{proof}

==> tables/tab_alpha_effectiveness.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{Alpha (Effectiveness)}: Comparison of different $\alpha_{(.)}$ values using FNR on \emph{unacceptable} prompts in $\dvalunacc$ (lower is better).}
\footnotesize
% \resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c c c c}
\bottomrule

\toprule
\textbf{Concepts}
& \textbf{0.25} & \textbf{0.5} & \textbf{1} & \textbf{1.5} & \textbf{2} \\
\midrule 
\textbf{Nudity}  & 0.01 $\pm$ 0.02 & 0.03 $\pm$ 0.03 & 0.03 $\pm$ 0.01 & 0.09 $\pm$ 0.05 & 0.08 $\pm$ 0.07 \\
\textbf{Violence}  & 0.36 $\pm$ 0.00 & 0.22 $\pm$ 0.08 & 0.24 $\pm$ 0.09 & 0.27 $\pm$ 0.07 & 0.34 $\pm$ 0.01\\
\bottomrule

\toprule
\end{tabular}
% }
\label{tab:AlphaEffective}
\end{table}



==> tables/tab_alpha_sum.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{Alpha (Sum)}: Comparison of different $\alpha_{(.)}$ values using mean FPR on acceptable prompts in $\dvalacc$ and mean FNR on unacceptable prompts in $\dvalunacc$(lower is better).}
\footnotesize
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c c c c}
\bottomrule

\toprule
\textbf{Concepts}
& \textbf{0.25} & \textbf{0.5} & \textbf{1} & \textbf{1.5} & \textbf{2} \\
\midrule 
\textbf{Nudity}  & 0.27 & 0.23 & 0.09 & 0.13 & 0.15 \\
\textbf{Violence}  & 0.81 & 0.86 & 0.74 & 0.76 & 0.91\\
\bottomrule

\toprule
\end{tabular}
}
\label{tab:AlphaSum}
\end{table}

==> tables/tab_alpha_utility.tex <==
\begin{table}[!htb]
\centering
\caption{\underline{Alpha (Utility)}: Comparison of different $\alpha_{(.)}$ values using FPR on \emph{acceptable} prompts in $\dvalacc$ (lower is better).}
\footnotesize
% \resizebox{0.6\columnwidth}{!}{
\begin{tabular}{  l | c c c c c}
\bottomrule

\toprule
\textbf{Concepts}
& \textbf{0.25} & \textbf{0.5} & \textbf{1} & \textbf{1.5} & \textbf{2} \\
\midrule 
\textbf{Nudity}  & 0.26 $\pm$ 0.09 & 0.20 $\pm$ 0.04 & 0.06 $\pm$ 0.05 & 0.04 $\pm$ 0.01 & 0.07 $\pm$ 0.01 \\
\textbf{Violence}  & 0.45 $\pm$ 0.07 & 0.64 $\pm$ 0.03 & 0.50 $\pm$ 0.08 & 0.52 $\pm$ 0.07 & 0.57 $\pm$ 0.02\\
\bottomrule

\toprule
\end{tabular}
% }
\label{tab:AlphaUtility}
\end{table}

==> tables/tab_certified.tex <==
\begin{table*}[ht]
\centering
\caption{Certified accuracy of \method on different concepts on varying $\delta$.}
\footnotesize
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Concept}} & \multicolumn{10}{c}{\textbf{$\delta$}}\\
 & 0.00 & 0.05 & 0.10 & 0.15 & 0.20 & 0.25 & 0.30 & 0.35 & 0.40 & 0.45 \\ 
 \midrule
 \textbf{Nudity} & 0.85 $\pm$ 0.08 & 0.80 $\pm$ 0.40 & 0.80 $\pm$ 0.41 & 0.80 $\pm$ 0.41 & 0.79 $\pm$ 0.41 & 0.77 $\pm$ 0.42 & 0.74 $\pm$ 0.44 & 0.50 $\pm$ 0.50 & 0.00 $\pm$ 0.08 & 0.00 $\pm$ 0.00  \\
\midrule
\textbf{Violence} & 0.81 $\pm$ 0.40 & 0.81 $\pm$ 0.40 & 0.79 $\pm$ 0.41 & 0.76 $\pm$ 0.43 & 0.73 $\pm$ 0.44 & 0.69 $\pm$ 0.46 & 0.62 $\pm$ 0.48 & 0.31 $\pm$ 0.46 & 0.01 $\pm$ 0.08 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Grumpy Cat} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.88 $\pm$ 0.32 & 0.44 $\pm$ 0.51 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Nemo} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.93 $\pm$ 0.25 &  0.93 $\pm$ 0.25 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.87 $\pm$ 0.35 & 0.77 $\pm$ 0.43 & 0.10 $\pm$ 0.31 & 0.00 $\pm$ 0.00  \\
\midrule 
\textbf{R2D2} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.13 $\pm$ 0.35 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 \\
\midrule
\textbf{Snoopy} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.63 $\pm$ 0.49 & 0.07 $\pm$ 0.25 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00  \\
\midrule
\textbf{Captain Marvel} & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 & 0.91 $\pm$ 0.25 & 0.03 $\pm$ 0.00 & 0.00 $\pm$ 0.00  \\
\midrule
\textbf{Taylor Swift} & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.98 $\pm$ 0.04 & 0.73 $\pm$ 0.45 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Angelina Jolie} & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.80 $\pm$ 0.41 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00\\
\midrule
\textbf{Brad Pitt} & 0.99 $\pm$ 0.01 & 0.99 $\pm$ 0.01 & 0.93 $\pm$ 0.25 & 0.93 $\pm$ 0.25 & 0.90 $\pm$ 0.31 & 0.90 $\pm$ 0.31 & 0.90 $\pm$ 0.31 & 0 .73 $\pm$ 0.45 & 0.07 $\pm$ 0.25 & 0.00 $\pm$ 0.00 \\
\midrule
\textbf{Elon Musk} & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.97 $\pm$ 0.03 & 0.73 $\pm$ 0.45 & 0.63 $\pm$ 0.49 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00  \\
\bottomrule
\end{tabular}
\label{tab:certified}
\end{table*}

==> tables/tab_concepts.tex <==
\begin{table}[h]
\caption{Summary of unacceptable concepts ($\cunacc$), acceptable concepts ($\cacc$), and whether we use them to evaluate fine-tuning \crt{s}, filtering \crt{s}, or both.}
\centering
\footnotesize
\begin{tabular}{ c |  l | c}
\hline
 \textbf{Type} & \textbf{$\cunacc$ $\rightarrow$ $\cacc$} & \textbf{\crt(s)}\\ 
 \hline
 \multirow{4}{*}{\textbf{Group-1}} & \emph{Nudity} $\rightarrow$ \emph{Clean} & Both \\ 
 & \emph{Violence} $\rightarrow$ \emph{Peaceful} & Both \\ 
& \emph{Disturbing} $\rightarrow$ \emph{Pleasing} & Filtering \\ 
& \emph{Hateful} $\rightarrow$ \emph{Loving} & Filtering \\ 
\hline
\multirow{5}{*}{\textbf{Group-2}} & \emph{Grumpy Cat} $\rightarrow$ \emph{Cat} & Fine-tuning \\ 
 & \emph{Nemo} $\rightarrow$ \emph{Fish} & Fine-tuning \\ 
 & \emph{Captain Marvel} $\rightarrow$ \emph{Female Superhero} & Fine-tuning \\
 & \emph{Snoopy} $\rightarrow$ \emph{Dog} & Fine-tuning \\
 & \emph{R2D2} $\rightarrow$ \emph{Robot} & Fine-tuning \\
 \hline
 \multirow{4}{*}{\textbf{Group-3}} & \emph{Taylor Swift} $\rightarrow$ \emph{Woman} & Fine-tuning \\ 
 & \emph{Angelina Jolie} $\rightarrow$ \emph{Woman} & Fine-tuning \\ 
 & \emph{Brad Pitt} $\rightarrow$ \emph{Man} & Fine-tuning \\ 
 & \emph{Elon Musk} $\rightarrow$ \emph{Man} & Fine-tuning \\ 
 \hline
\end{tabular}
% \end{center}
\label{tab:concepts}
\end{table}

==> tables/tab_nofinetune_effective.tex <==
\begin{table}[ht]
\centering
\caption{\underline{Benefit of Fine-Tuning (FT):} On using fine-tuning, if effectiveness/utility degrades we use \colorbox{mynicered}{red}; \colorbox{myniceblue}{blue} for no significant change; \colorbox{mynicegreen}{green} if better. We measure CLIP accuracy for effectiveness (lower is better) and normalized CLIP score for utility (higher is better).} 
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l|c|c|c|c } 
 \hline
  \multirow{2}{*}{\textbf{Concept}} &
\multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{2}{c}{{\textbf{Utility}}} \\
&  \textbf{w/o FT} & \textbf{w/ FT} & \textbf{w/o FT} & \textbf{w/ FT} \\
\hline
\textbf{Nudity} & \cellcolor{myniceblue!35} 0.15 $\pm$ 0.02 & \cellcolor{myniceblue!35} 0.15 $\pm$ 0.06 & \cellcolor{mynicegreen!35}0.83 $\pm$ 0.07 & \cellcolor{mynicegreen!35} 0.94 $\pm$ 0.08 \\
\textbf{Violence} & \cellcolor{myniceblue!35}0.21 $\pm$ 0.02 & \cellcolor{myniceblue!35} 0.20 $\pm$ 0.05 & \cellcolor{myniceblue!35}0.55 $\pm$ 0.08 & \cellcolor{myniceblue!35} 0.59 $\pm$ 0.11 \\
\hline
\textbf{Grumpy Cat} & \cellcolor{myniceblue!35}0.01 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.00 $\pm$ 0.01 & \cellcolor{mynicegreen!35}0.88 $\pm$ 0.03 & \cellcolor{mynicegreen!35} 0.98 $\pm$ 0.04 \\
\textbf{Nemo} & \cellcolor{myniceblue!35}0.12 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.10 $\pm$ 0.02 & \cellcolor{mynicegreen!35} 0.24 $\pm$ 0.05 & \cellcolor{mynicegreen!35} 0.37 $\pm$ 0.02 \\
\textbf{Captain Marvel} & \cellcolor{myniceblue!35}0.04 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.03 $\pm$ 0.01 & \cellcolor{myniceblue!35}0.36 $\pm$ 0.02 & \cellcolor{myniceblue!35} 0.37 $\pm$ 0.03  \\
\textbf{Snoopy} & \cellcolor{myniceblue!35}0.09 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.08 $\pm$ 0.02 & \cellcolor{myniceblue!35}0.64 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.66 $\pm$ 0.03 \\
\textbf{R2D2} & \cellcolor{myniceblue!35}0.00 $\pm$ 0.00 & \cellcolor{myniceblue!35} 0.00 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.52 $\pm$ 0.03 & \cellcolor{mynicegreen!35} 0.66 $\pm$ 0.02 \\
\hline
\textbf{Taylor Swift} & \cellcolor{mynicegreen!35}0.04 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.02 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.97 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.98 $\pm$ 0.02  \\
\textbf{Angelina Jolie} & \cellcolor{mynicegreen!35}0.12 $\pm$ 0.02 & \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.97 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.98 $\pm$ 0.03 \\
\textbf{Brad Pitt} & \cellcolor{mynicegreen!35}0.02 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.00 $\pm$ 0.00 & \cellcolor{myniceblue!35}0.98 $\pm$ 0.01 & \cellcolor{myniceblue!35} 0.98 $\pm$ 0.01 \\
\textbf{Elon Musk} & \cellcolor{mynicegreen!35}0.07 $\pm$ 0.01 & \cellcolor{mynicegreen!35} 0.03 $\pm$ 0.00 & \cellcolor{mynicegreen!35}0.92 $\pm$ 0.02 & \cellcolor{mynicegreen!35} 0.97 $\pm$ 0.01 \\
\hline
 \end{tabular}
}
\label{tab:FTImpact}
\end{table}

